Physics-Informed Kernel Embeddings: Integrating Prior System Knowledge with Data-Driven Control

Data-driven control algorithms use observations of system dynamics to construct an implicit model for the purpose of control. However, in practice, data-driven techniques often require excessive sample sizes, which may be infeasible in real-world scenarios where only limited observations of the system are available. Furthermore, purely data-driven methods often neglect useful a priori knowledge, such as approximate models of the system dynamics. We present a method to incorporate such prior knowledge into data-driven control algorithms using kernel embeddings, a nonparametric machine learning technique based in the theory of reproducing kernel Hilbert spaces. Our proposed approach incorporates prior knowledge of the system dynamics as a bias term in the kernel learning problem. We formulate the biased learning problem as a least-squares problem with a regularization term that is informed by the dynamics, that has an efficiently computable, closed-form solution. Through numerical experiments, we empirically demonstrate the improved sample efficiency and out-of-sample generalization of our approach over a purely data-driven baseline. We demonstrate an application of our method to control through a target tracking problem with nonholonomic dynamics, and on spring-mass-damper and F-16 aircraft state prediction tasks.

==> figures/smd_phase_plots/phase_plot_100_full_space_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.0564323514699936 0.0191436633467674
-0.0648586601018906 0.0181306432932615
0.133227959275246 -0.00552427675575018
0.0285781156271696 0.0813358426094055
-0.0162621792405844 0.142968565225601
-0.0760493353009224 -0.0242771487683058
0.117157332599163 0.140991494059563
0.119702123105526 0.115484111011028
-0.0278323385864496 0.0890541821718216
0.0571985468268394 -0.140421941876411
-0.148211106657982 0.0649935454130173
-0.0782317891716957 -0.0764816328883171
-0.00708838691934943 0.0570777170360088
-0.127209782600403 0.0436292737722397
-0.0427417308092117 -0.0505176372826099
-0.00532725360244513 0.105660669505596
-0.0335741117596626 0.00274956808425486
0.0750314071774483 0.144773796200752
0.0861266255378723 -0.0235771462321281
-0.0975093245506287 0.0396153628826141
-0.0204700194299221 -0.0604487955570221
0.00150415685493499 0.147457897663116
0.0626757517457008 -0.102068223059177
-0.113669410347939 -0.0928089544177055
-0.107295744121075 0.0165606681257486
-0.0221126526594162 0.00721578625962138
0.102032221853733 -0.144445195794106
-0.0233929045498371 -0.000336387689458206
-0.0905305817723274 -0.0751754716038704
-0.0339684709906578 0.0603149421513081
-0.0614654570817947 -0.0345092453062534
0.0288694445043802 -0.0412826053798199
-0.103536941111088 -0.109410136938095
-0.0990852415561676 0.0734872370958328
-0.107443034648895 -0.0985833257436752
-0.123872444033623 -0.0423464216291904
0.126973927021027 -0.119279950857162
0.0648471042513847 0.0281054303050041
0.0806532576680183 0.0732622444629669
-0.0983110070228577 -0.122655138373375
0.0815353617072105 0.082908108830452
-0.058661624789238 0.127575755119324
0.0982014164328575 0.082085870206356
0.0810219049453735 -0.116040118038654
-0.146875157952309 0.070702038705349
0.0455750674009323 0.128386795520782
-0.139337420463562 -0.0155763104557991
0.00421418063342571 0.0798415988683701
0.12482613325119 -0.0699644386768341
0.0176787506788969 0.136209085583687
0.11806096881628 -0.0757949352264404
-0.106976255774498 -0.111786186695099
-0.0147676672786474 -0.00218048179522157
0.038668155670166 -0.00672357110306621
0.0457391291856766 0.0719281956553459
-0.0570533536374569 -0.121886752545834
-0.0446092896163464 -0.0185757149010897
0.115200527012348 -0.0917918011546135
-0.027430634945631 -0.0629935041069984
0.00154937407933176 -0.129307970404625
-0.00610308954492211 0.121613457798958
-0.0672652572393417 -0.0746083408594131
-0.0623658299446106 0.104670807719231
0.0831616520881653 0.101801835000515
0.140315845608711 0.143983751535416
-0.118541963398457 0.0972764641046524
0.112209938466549 0.0197082050144672
-0.128620132803917 -0.107769638299942
0.101860381662846 0.0831603556871414
-0.0578217916190624 0.0232317410409451
0.0833302885293961 0.101069591939449
-0.109393805265427 -0.00624653743579984
-0.0385861583054066 -0.141261234879494
-0.0814992561936378 -0.0875304192304611
-0.136515229940414 0.122600309550762
-0.108115166425705 0.0135378884151578
0.0864146575331688 0.00643907021731138
0.0742529258131981 0.00297301611863077
0.0508462749421597 -0.134100213646889
0.0547141768038273 -0.0226237121969461
0.114377349615097 -0.124202013015747
0.0377407483756542 0.131499499082565
0.105873264372349 -0.0788986906409264
0.0284953657537699 0.0632102489471436
-0.110552318394184 0.0378431417047977
0.12747286260128 0.044319361448288
0.115978196263313 0.00424777716398239
-0.0783208012580872 0.143538609147072
-0.0674099773168564 0.050542987883091
-0.0545390509068966 -0.104724168777466
0.0119496295228601 -0.00417771609500051
-0.0422165058553219 -0.131847277283669
-0.121815353631973 -0.0508831180632114
0.0500259920954704 0.139836370944977
-0.0760146975517273 -0.0734343901276588
0.0462333671748638 0.0875695198774338
0.0669484660029411 0.0571628659963608
0.121366657316685 0.137811914086342
-0.0252386853098869 -0.0881131365895271
-0.0148967783898115 -0.0480085089802742
};
\addplot [very thick, trueDynamics]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, approxDynamics, dashed]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, learnedWithSideInfo]
table {%
0.1 0.1
0.109245078114732 0.0848747884395325
0.116972311529696 0.0696694605911164
0.123181420003241 0.0545369280357259
0.127886800584227 0.0396184059510703
0.131116545711762 0.0250445317812143
0.13291122108325 0.0109362140720454
0.133322993610689 -0.00259497726576347
0.132414833899053 -0.0154469232666015
0.130259279227284 -0.0275275499866192
0.126937688377481 -0.0387556004261476
0.122538885617899 -0.0490613959406488
0.117158072977848 -0.0583874811732085
0.110895556287366 -0.0666889080819146
0.103855545724413 -0.073933301008609
0.0961448371241316 -0.0801006331769843
0.0878716348209046 -0.0851827329510968
0.0791444117088907 -0.0891827854302977
0.070070746930633 -0.0921146066648783
0.0607563460917949 -0.0940019572927474
0.0513040838296561 -0.0948778404962409
0.0418131246147382 -0.0947836651921779
0.0323780659127766 -0.0937684297623569
0.0230882899698507 -0.0918878448676399
0.0140272969724942 -0.0892034263747003
0.00527218675107144 -0.0857814996980235
-0.00310676871487954 -0.0816923017064224
-0.0110464787649725 -0.0770089217545489
-0.0184912613344253 -0.0718063774905492
-0.0253930027119219 -0.0661608178800252
-0.0317112162538929 -0.0601486825068359
-0.0374130577867061 -0.0538459528066854
-0.0424732194642488 -0.047327558233974
-0.0468738143051817 -0.0406667585184861
-0.0506041824917614 -0.0339345839432564
-0.0536606194275029 -0.0271993834259413
-0.0560461261435043 -0.0205263309700519
-0.0577700106894793 -0.0139769770154392
-0.0588475528540692 -0.00760884904341869
-0.0592995757539209 -0.00147507186222423
-0.059151976447718 0.00437597861812911
-0.0584352416515809 0.00990095205258329
-0.0571839150285716 0.0150617513193365
-0.0554361054581478 0.0198256954582239
-0.0532328984492423 0.0241656151049409
-0.0506178308813379 0.0280598413454645
-0.047636313591572 0.0314921913079636
-0.0443351433643543 0.0344518205416894
-0.0407618882599478 0.0369330849421291
-0.0369644815532901 0.0389352716201424
-0.0329906666617868 0.0404623985592648
-0.0288875519635013 0.0415228961780892
-0.0247012159057132 0.0421292555593926
-0.0204762897621452 0.0422977510903958
-0.0162556018545747 0.042048044466887
-0.0120798599606739 0.0414028702504951
-0.00798736165995707 0.0403876137086651
-0.00401374659119203 0.0390299814024768
-0.000191786254229212 0.0373596232572935
0.00344879510607343 0.0354077361725381
0.00688145659747326 0.0332067154679798
0.0100829427862149 0.0307898085005655
0.0130333488397148 0.0281907438040517
0.0157161503951629 0.0254433769437474
0.0181182065936089 0.0225813920923328
0.0202297181773896 0.0196379811820025
0.0220441688232428 0.0166455471667803
0.0235582348100794 0.0136354342156523
0.0247716695399439 0.0106376791033694
0.0256871396301783 0.00768078261856367
0.0263100870816895 0.00479150639694176
0.0266485281169884 0.00199469437555153
0.0267128687815102 -0.00068688193408456
0.0265156795661737 -0.00323264743564175
0.0260714756175317 -0.00562432439646271
0.025396483908854 -0.0078460046342394
0.0245083917843272 -0.00988419355730935
0.0234261271677948 -0.0117278374083855
0.022169597792628 -0.0133683071608664
0.0207594471949399 -0.0147993771508315
0.0192168311954741 -0.0160171693329955
0.01756317761693 -0.0170200781294614
0.0158199609019994 -0.0178086795350788
0.0140084972202484 -0.0183856216463675
0.0121497386427134 -0.0187554930315681
0.0102640868745289 -0.0189246947751253
0.00837122095585479 -0.0189012625393178
0.006489935208786 -0.0186947404946239
0.00463800977871179 -0.0183159922892457
0.00283207465723611 -0.0177770416587361
0.00108750665010273 -0.0170908870659565
-0.000581658404489641 -0.0162713386971839
-0.00216279793435674 -0.0153328284551488
-0.00364475688691353 -0.014290254309532
-0.00501788766404045 -0.0131588051630739
-0.00627406852002308 -0.0119537987376183
-0.00740670810519426 -0.0106905295295979
-0.00841073685548851 -0.00938411507107223
-0.00928258743753703 -0.00804936425809213
-0.0100201453922563 -0.00670064211613761
-0.0106227090905902 -0.00535175623667514
-0.0110909264064071 -0.00401584651638234
-0.0114267239381572 -0.00270529292484356
-0.0116332157415422 -0.00143162806616623
-0.0117146325506598 -0.000205467456967229
-0.0116762146774111 0.000963548760932464
-0.0115241151551296 0.00206680291001177
-0.011265297294009 0.00309673446354822
-0.0109074275795961 0.00404686306765076
-0.0104587648456598 0.00491179643797812
-0.00992805130951922 0.00568723279293129
-0.00932440826367032 0.00636994949611253
-0.0086572233852639 0.00695778080482226
-0.00793605108379514 0.00744958962552761
-0.00717050958900407 0.00784522486571282
-0.00637018409219281 0.00814547835582685
-0.00554453547534529 0.00835203481269209
-0.00470281555904236 0.00846740280302199
-0.00385398514466315 0.00849485635337158
-0.00300664206778899 0.00843836548689669
-0.00216895623685106 0.0083025248325215
-0.00134860956079017 0.00809247952618217
-0.000552745714049131 0.00781384827041898
0.000212074569090402 0.00747264181382928
0.000939908129684899 0.00707519109719176
0.00162545744232498 0.00662806897711307
0.00226409128065145 0.00613801468217345
0.00285185682637157 0.0056118601368986
0.00338548811113959 0.00505645813770905
0.00386240054657178 0.00447862026077861
0.00428068778268982 0.00388504757649577
0.00463910401434793 0.00328226809575161
0.00493704489028629 0.00267658903943319
0.00517452469700891 0.00207404377578876
0.0053521467904648 0.00148034350917225
0.00547106541272418 0.000900840206889547
0.00553295309660458 0.000340489616250383
0.00553995363455821 -0.000196176700210354
0.0054946434293705 -0.000705075389782067
0.00539998399717369 -0.00118258969797569
0.00525927540162989 -0.00162558244506184
0.00507610596271661 -0.00203140353800274
0.00485430615631489 -0.00239789163306067
0.00459789506313443 -0.0027233740250773
0.00431103706201794 -0.00300665574379905
0.00399799386659648 -0.00324701238277861
0.00366307400065876 -0.00344417224784516
0.00331059321645964 -0.00359829643021148
0.00294482955784794 -0.00370995726501966
0.00256998447701988 -0.00378011492143587
0.00219014511519616 -0.00381008682087952
0.00180925065785742 -0.00380151798219283
0.00143106020336712 -0.00375634997215482
0.00105912610301613 -0.00367678708171174
0.000696767417516353 -0.00356526249549113
0.000347050591175443 -0.00342440354371015
1.27709255226505e-05 -0.00325699509040656
-0.000303561255823628 -0.00306594849597369
-0.000599731589294689 -0.00285426338017947
-0.000873828560704289 -0.00262499658692331
-0.00112424823999413 -0.00238122695915852
-0.00134969374262557 -0.00212602847497803
-0.00154917464828279 -0.00186243617746629
-0.00172200077335417 -0.001593420819925
-0.00186777460452371 -0.00132186337189766
-0.00198638140412942 -0.00105052930702254
-0.00207797617212038 -0.000782049547187358
-0.00214296967673081 -0.000518899551944257
-0.00218201099258467 -0.000263383886536239
-0.00219597155214495 -1.76215393813961e-05
-0.00218592465692334 0.000216465734846655
-0.0021531254542697 0.000437162647346223
-0.00209898905144996 0.000642966579264936
-0.0020250718893287 0.000832592979348151
-0.00193304589819081 0.00100497606174985
-0.00182467963847435 0.00115926973459138
-0.00170181583255661 0.00129484446836378
-0.00156634901288624 0.00141128301403654
-0.00142020468352528 0.00150837536229501
-0.00126531964571786 0.00158610878041124
-0.00110362232349989 0.00164465993637147
-0.000937015301124706 0.00168438377842189
-0.000767356114228299 0.00170580090727959
-0.000596443163271629 0.00170958541340685
-0.000425999909800171 0.00169655063014645
-0.000257662594244532 0.00166763326149511
-9.2967953792862e-05 0.00162388052230961
6.66567825043753e-05 0.00156643311599941
0.000219902545186767 0.00149651005190832
0.000365585366065791 0.00141539231441645
0.000502651893746994 0.00132440954443838
0.000630183490414419 0.00122492196266691
0.000747398364006059 0.00111830774424562
0.000853652994695135 0.00100594784702604
0.000948441524014689 0.000889212568344983
0.00103139412538467 0.00076944857474856
0.00110227368654255 0.000647967604888527
0.00116097237559112 0.00052603453860664
0.0012075056458479 0.000404857898492178
0.00124200688095998 0.0002855805805001
0.00126472017735974 0.000169272080593447
0.00127599266101804 5.69213134388458e-05
0.0012762657564431 -5.05689096563511e-05
0.00126606738696536 -0.00015238659156358
0.00124600091537139 -0.000247814053098483
0.00121673769338339 -0.000336230340346105
0.00117900530374997 -0.000417112752337967
0.00113357976042699 -0.000490037054282993
0.00108127340136789 -0.000554676782417218
0.00102292743791587 -0.000610802143579031
0.000959400662446599 -0.000658277206431829
0.000891561241013948 -0.000697056511203553
0.000820277225413188 -0.000727181885954109
0.000746408753230645 -0.000748777058080158
0.000670799025533934 -0.000762042847604949
0.000594268194931046 -0.000767251781220835
0.000517605623793615 -0.000764741197192109
0.000441563714098405 -0.000754907919588543
0.000366852726764922 -0.000738200436393971
0.000294135833847965 -0.000715112760780873
0.000224024607263378 -0.000686177191285692
0.000157075991813646 -0.000651957129276848
9.37892127426225e-05 -0.000613040475956311
3.46037783106193e-05 -0.000570032449522945
-2.01019119055511e-05 -0.000523548925901368
-7.00112965817252e-05 -0.000474209833944111
-0.000114869772859021 -0.000422633017272023
-0.000154484165339649 -0.000369428383428488
-0.000188721549342049 -0.000315192285967714
-0.000217507914070693 -0.000260502398454571
-0.000240825812600787 -0.000205912877895204
-0.000258711815399172 -0.00015195020951303
-0.000271253585479911 -9.91094413259619e-05
-0.000278586778931957 -4.78508360960139e-05
-0.000280891014107906 1.40297664466549e-06
-0.000278386190046434 4.82692404077112e-05
-0.000271328557500158 9.24068796292477e-05
-0.00026000617877102 0.000133517826792023
-0.000244734824091055 0.000171347801201011
-0.00022585340233069 0.000205686784979897
-0.000203719755493797 0.000236368823310962
-0.000178706002092616 0.000263271590367847
-0.000151194433479132 0.00028631526000919
-0.000121573213736657 0.00030546162164849
-9.02323269203552e-05 0.000320712271516171
-5.75596916485298e-05 0.000332106453929448
-2.39374776005511e-05 0.000339719150175971
1.0261306064004e-05 0.00034365853065188
4.46760185537008e-05 0.000344063231233593
7.89612960804772e-05 0.000341099806397654
0.000112789671281218 0.000334959281247021
0.000145853926152341 0.000325854575646101
0.000177869055723444 0.000314017201310524
0.000208574079852404 0.000299694105828863
0.000237733265667158 0.000283144400113566
0.000265137248132575 0.000264636549209579
0.000290603976005762 0.000244444983311887
0.000313978959291111 0.000222847420150024
0.000335135414829777 0.000200121735833864
0.000353974353676112 0.000176543605872076
0.000370424202815617 0.000152383550119095
0.00038443996121189 0.000127904776131477
0.00039600258867869 0.000103360875900599
0.000405117667157074 7.89938865444206e-05
0.0004118144112262 5.5032428580154e-05
0.00041614418384948 3.16901971675609e-05
0.000418179099423627 9.16454849880788e-06
0.000418009782812498 -1.23646345213946e-05
0.000415744234320322 -3.27358381666254e-05
0.000411505443194039 -5.18065794666012e-05
0.000405429845133216 -6.94539397838312e-05
0.000397665081300048 -8.55747161884468e-05
0.000388368135677429 -0.000100085590908183
0.000377703297796488 -0.000112922917570701
0.000365840329187949 -0.000124042446202344
0.000352952455203427 -0.000133418649458317
0.000339214473253674 -0.000141044361400222
0.000324801122970982 -0.000146929690729936
0.00030988522354396 -0.000151101239021761
0.00029463610208189 -0.000153600985991598
0.000279218371228328 -0.000154485188668285
0.000263790124690863 -0.000153823107388595
0.000248502093199575 -0.000151695702220372
0.000233496349351381 -0.000148194286684278
0.000218905288945156 -0.000143419253353899
0.000204850917896696 -0.000137478350419079
0.000191444226479144 -0.000130485668498048
0.000178784461686797 -0.000122559931601957
0.000166958836163896 -0.000113823252249123
0.000156042280790615 -0.000104399762598933
0.000146097197266026 -9.4414297122758e-05
0.000137173559940981 -8.39911181340913e-05
0.000129309017652617 -7.32527719658205e-05
0.000122529053767618 -6.23189667514901e-05
0.000116847415438666 -5.13055551564778e-05
0.00011226645555088 -4.03235713841155e-05
0.000108777700224442 -2.94783733799098e-05
0.000106362474529826 -1.88689404809761e-05
0.000104992571858839 -8.58717196014491e-06
0.000104630901470856 1.28265150167728e-06
0.00010523239797657 1.06643195311729e-05
0.000106744792580574 1.94900466940484e-05
0.000109109471637963 2.77007287259323e-05
0.000112262313385642 3.52460890583606e-05
0.000116134699298747 4.20847492628718e-05
0.000120654227134552 4.81842217916473e-05
0.000125745736846246 5.352075248935e-05
0.000131332060010101 5.80791739658582e-05
0.0001373349802587 6.18526341224501e-05
0.000143676004541594 6.48422196391218e-05
0.000150277148936695 6.70566301565201e-05
0.000157061608050796 6.85116750865356e-05
0.000163954511730984 6.92297848557122e-05
0.000170883507155071 6.92394788905093e-05
0.000177779457336135 6.85748224483196e-05
0.000184576834040719 6.72747823569908e-05
0.000191214241672664 6.53826042620043e-05
0.000197634737428515 6.29452914155115e-05
0.000203786355186172 6.00127973476583e-05
0.000209622134620778 5.66375553420206e-05
0.000215100470468064 5.28737470403551e-05
0.000220185287162229 4.877673425982e-05
0.000224846126161667 4.44024542959887e-05
0.000229057956788926 3.98068408155872e-05
0.000232801525489663 3.50452880342189e-05
0.000236062875632186 3.017214576162e-05
0.000238833565797935 2.52402324444623e-05
0.000241110247787939 2.03003628051479e-05
0.000242894564767666 1.5401010248578e-05
0.00024419288934242 1.05879122936081e-05
0.000245015974319136 5.90375379849739e-06
0.000245378748985954 1.38791579121222e-06
0.000245299897112435 -2.92376092844715e-06
0.000244801391292724 -6.99915009866325e-06
0.000243908391085439 -1.08099733726885e-05
0.00024264858817981 -1.4331895188735e-05
0.000241051900806594 -1.75445593215418e-05
0.000239150080836317 -2.04315934455579e-05
0.000236976379085043 -2.29806028058943e-05
0.000234565065098917 -2.51830606266268e-05
0.00023195106335397 -2.70342339963037e-05
0.000229169560351151 -2.85330444620979e-05
0.000226255684469724 -2.96818761135742e-05
0.000223244200373024 -3.04864181362441e-05
0.000220169130652768 -3.09554422591729e-05
0.000217063522992863 -3.11005437502454e-05
0.000213958999053577 -3.09359098797368e-05
0.000210885681706479 -3.04780881885403e-05
0.000207872064059332 -2.9745664280878e-05
0.000204944558340422 -2.87589975156155e-05
0.000202127524994963 -2.7539946004268e-05
0.000199443098055321 -2.61115769328024e-05
0.0001969109523035 -2.44978787154737e-05
0.000194548434231133 -2.27234914162155e-05
0.0001923703292025 -2.08134315286268e-05
0.000190388963311047 -1.87928241421609e-05
0.000188614174269911 -1.66866657841103e-05
0.00018705322409406 -1.45195837660816e-05
0.000185711031925637 -1.23156025927662e-05
0.000184590115821187 -1.00979521707178e-05
0.000183690723714407 -7.88888043923297e-06
0.000183010920723087 -5.7094732894003e-06
0.000182546763768657 -3.57951473201057e-06
0.000182292359780526 -1.5173511368205e-06
0.000182240069420227 4.60210554664719e-07
0.000182380652598204 2.33800228718883e-06
0.000182703457647101 4.10255744170973e-06
0.000183196537735884 5.74215834603375e-06
0.000183846912803452 7.24687111913758e-06
0.000184640700525734 8.60855053308462e-06
0.000185563218179278 9.82083334402639e-06
0.000186599259127832 1.08791244617656e-05
0.000187733325654465 1.17805460902176e-05
0.000188949614410767 1.25238820146145e-05
0.000190232394768311 1.31095170030626e-05
0.00019156589240542 1.35393490020286e-05
0.000192934769522415 1.381670587558e-05
0.000194323862909774 1.39462395186418e-05
0.000195718780579411 1.39338127271016e-05
0.000197105639832997 1.37863878860445e-05
0.000198471387407031 1.35119075053425e-05
0.000199803653957003 1.31191593678026e-05
0.000201091176065572 1.26176697389235e-05
0.000202323490655885 1.2017560371641e-05
0.000203491298792538 1.13294263428265e-05
0.000204586363821164 1.0564209322661e-05
0.000205601525923644 9.73307272378321e-06
0.000206530716672763 8.84728082906072e-06
0.000207369090002445 7.91808889272216e-06
0.000208112847587247 6.95663358055154e-06
0.000208759253396971 5.97382983008599e-06
0.000209306779218227 4.98027128631451e-06
0.000209754857273974 3.98614682203813e-06
0.000210103880225532 3.00115851339933e-06
0.000210355230278107 2.03445476915087e-06
0.000210511191870911 1.09456346322756e-06
0.000210574820711234 1.89341375189667e-07
0.000210549987431324 -6.74072874268239e-07
0.000210441188414348 -1.48929185136981e-06
0.000210253502139264 -2.2507050828624e-06
0.000209992574629287 -2.95349364676234e-06
0.000209664473933054 -3.59364295648978e-06
0.000209275631916951 -4.16794162663714e-06
0.000208832742401531 -4.6739737786794e-06
0.000208342732057302 -5.11010502121656e-06
0.000207812673092691 -5.47545845600017e-06
0.000207249564974624 -5.7698866262057e-06
0.000206660610914262 -5.99394481207161e-06
0.000206052664893002 -6.14884262470361e-06
0.000205432566355478 -6.2364028282913e-06
0.000204807023793293 -6.2590174216004e-06
0.000204182352809282 -6.21960059773996e-06
0.0002035645343234 -6.12151815895801e-06
0.000202959330987355 -5.96855672890806e-06
0.000202372039800271 -5.7648513520081e-06
0.000201807463003443 -5.51483257016372e-06
0.000201270039046219 -5.22316575740644e-06
0.000200763638857804 -4.89470046499685e-06
0.000200291740468628 -4.53440207706657e-06
0.000199857225282593 -4.14731380082856e-06
0.000199462581802312 -3.73849604337617e-06
0.000199109701901103 -3.31297481148685e-06
0.000198799939029474 -2.87569510568075e-06
0.000198534326492769 -2.43148020842576e-06
0.000198313286411883 -1.98498686296289e-06
0.00019813684800101 -1.54067113330991e-06
0.000198004516599641 -1.1027537692998e-06
0.000197915506502374 -6.75188541160443e-07
0.000197868580887271 -2.61638251647378e-07
0.000197862139126673 1.34551274538763e-07
0.000197894347754332 5.10357313882048e-07
0.000197963038601365 8.63103417736433e-07
0.000198065694244136 1.19046983187987e-06
0.000198199797250249 1.49049077802221e-06
0.000198362393620817 1.76156604617117e-06
0.000198550674867261 2.00245245521313e-06
0.000198761410486727 2.21226070273861e-06
0.000198991588246483 2.39044790315002e-06
0.000199238035834639 2.53679910292015e-06
0.000199497464515891 2.65142531871709e-06
0.000199766774722201 2.73474574052912e-06
0.000200042910534379 2.78745765033839e-06
0.000200322830578699 2.8105185772842e-06
0.000200603624442497 2.80513515668601e-06
0.000200882483571121 2.77273099705266e-06
0.000201156817683773 2.71492586767508e-06
0.000201424152910798 2.63350764362347e-06
0.000201682291865377 2.53040696282514e-06
0.000201929197229044 2.40766314921204e-06
0.000202162904440373 2.26741804776331e-06
0.000202381754526399 2.11188231952208e-06
0.000202584350447493 1.94331280628512e-06
0.000202769615305914 1.76397437559594e-06
0.000202936443100144 1.57613035517423e-06
0.00020308412073083 1.38202389074471e-06
0.000203212269794021 1.18384248590231e-06
0.000203320439127799 9.83709024238166e-07
0.000203408526818059 7.83670477150222e-07
0.000203476809303117 5.85666114522043e-07
0.000203525388401084 3.91524290044298e-07
0.000203554773386592 2.02954681866041e-07
0.000203565779128134 2.15187700713937e-08
0.000203558987667075 -1.51362690992141e-07
0.000203535359398194 -3.14416923608007e-07
0.00020349600023931 -4.6652805413272e-07
0.000203442030664285 -6.06747186326917e-07
0.000203374658462368 -7.3428312269419e-07
0.000203295149634371 -8.48501911121513e-07
0.000203204886600402 -9.48931147937149e-07
0.000203105368199912 -1.03526065142745e-06
0.000202997947757092 -1.10733703417853e-06
0.000202884036807214 -1.16514492140563e-06
0.00020276501778514 -1.20880763515574e-06
0.000202642316784766 -1.23858039929869e-06
0.00020251731624726 -1.25484084356753e-06
0.000202391354960933 -1.25808266343563e-06
0.000202265684405163 -1.24890272643063e-06
0.000202141526957763 -1.22798907856159e-06
0.00020202003223898 -1.19611053805979e-06
0.000201902262559343 -1.15410787332459e-06
0.000201789134711658 -1.10287795848651e-06
0.000201681609145649 -1.04336563450103e-06
0.000201580384377439 -9.76550359993444e-07
0.000201486071612142 -9.03430369236791e-07
0.000201399340262751 -8.25012947430759e-07
0.000201320699671585 -7.42320991425904e-07
0.000201250513661572 -6.56366306694967e-07
0.00020118907329564 -5.68144639334633e-07
0.00020113653866889 -4.78626162342399e-07
0.000201093011667881 -3.8874620963969e-07
0.000201058361347483 -2.99396442554611e-07
0.000201032587728409 -2.11413321793419e-07
0.000201015516207323 -1.25588957455847e-07
0.000201006913971764 -4.26566348632473e-08
0.000201006460896219 3.67137116819016e-08
0.000201013749542052 1.11918896428254e-07
0.000201028328813069 1.82428244038801e-07
0.000201049674851799 2.47780542611542e-07
0.000201077220142958 3.075980666567e-07
0.000201110440825468 3.61564970990935e-07
0.000201148783932615 4.09438604104251e-07
0.000201191609184512 4.51044302740566e-07
0.000201238305403371 4.86277431238635e-07
0.000201288217753994 5.15100436027094e-07
0.000201340676847637 5.37541831713284e-07
0.000201395100605548 5.53690313737087e-07
0.000201450819636119 5.63689898314124e-07
0.000201507237305922 5.6774071149901e-07
0.000201563786084224 5.66088808939824e-07
0.000201619869335285 5.59027532737177e-07
0.000201675006837805 5.46885519647766e-07
0.000201728689265839 5.300245539408e-07
0.000201780465500314 5.08837753987468e-07
0.00020182989897353 4.83740184409331e-07
0.000201876611324963 4.5516659627487e-07
0.000201920340609062 4.23564858409442e-07
0.000201960766672536 3.89386575816442e-07
0.000201997656673432 3.53089121524208e-07
0.000202030821425561 3.1512896339625e-07
0.000202060115398607 2.75957250939207e-07
0.000202085436718269 2.36014275040164e-07
0.000202106814477852 1.95724598611724e-07
0.000202124219563655 1.55487108521868e-07
0.000202137608310283 1.15691185326172e-07
0.000202147038916296 7.67040377602779e-08
0.000202152627788572 3.88662906025683e-08
0.000202154505886545 2.49220716286302e-09
0.000202152804170417 -3.21347181087006e-08
0.00020214771180874 -6.47588196400761e-08
0.000202139476178567 -9.51588243758295e-08
0.000202128301001972 -1.23144228786343e-07
0.000202114448209541 -1.48559146928573e-07
0.000202098179732641 -1.71278914412598e-07
0.000202079786607266 -1.91211449451778e-07
0.000202059545318351 -2.08299286486024e-07
0.000202037746903448 -2.22512787778628e-07
0.000202014653296987 -2.33851277064989e-07
0.000201990570089865 -2.42343037665238e-07
0.000201965773769781 -2.48042375111668e-07
0.000201940540825053 -2.51027799741399e-07
0.00020191510408882 -2.5140112816513e-07
0.000201889798258054 -2.49281372072252e-07
0.000201864812511194 -2.44812431327013e-07
0.000201840379682734 -2.38150194009634e-07
0.000201816732607526 -2.29465939610707e-07
0.000201794045913085 -2.18942704605096e-07
0.000201772494227083 -2.0677077189335e-07
0.000201752223073574 -1.9314833926698e-07
0.000201733377976675 -1.78277002771399e-07
0.000201716089908706 -1.62361291439206e-07
0.000201700446186272 -1.45608910734341e-07
0.000201686505022064 -1.28222808704059e-07
0.000201674339180642 -1.10404351411075e-07
0.000201663963218718 -9.23474390568391e-08
0.000201655420796688 -7.42396344677321e-08
0.000201648682815183 -5.62612627874604e-08
0.000201643720174549 -3.85804280189639e-08
0.000201640518326784 -2.13555099437546e-08
0.000201639019067854 -4.73221267727197e-09
0.000201639149641498 1.11555203963221e-08
0.000201640822739206 2.61877766416507e-08
0.000201643951052081 4.02602542415309e-08
0.000201648447270908 5.3281320883114e-08
0.000201654194982263 6.51747303626049e-08
0.000201661077772363 7.58789428512152e-08
0.000201668964675175 8.53457677307823e-08
0.000201677739276163 9.35437556026653e-08
0.000201687270608586 1.00453677570611e-07
0.000201697427705331 1.06070782573964e-07
0.000201708094150946 1.10400841413227e-07
0.000201719138977705 1.1346410450086e-07
0.000201730416665696 1.15291683283614e-07
0.000201741767142792 1.15926905908115e-07
0.000201753117648044 1.15425658531176e-07
0.00020176442452432 1.1384393860947e-07
0.000201775527698979 1.11245890610512e-07
0.000201786296202921 1.07707197383178e-07
0.000201796686378424 1.03307839893763e-07
0.000201806596360011 9.81317592185782e-08
0.000201815938834027 9.22662880264991e-08
0.000201824670142467 8.58032878081616e-08
0.000201832746627338 7.88334862111828e-08
0.000201840095526815 7.14478368413207e-08
0.000201846673182836 6.37400088265849e-08
0.000201852465041227 5.58014100759952e-08
0.000201857456547874 4.77205036042427e-08
0.00020186163314875 3.95830419275267e-08
0.00020186499484181 3.14711528781597e-08
0.000201867541625128 2.34626681139272e-08
0.000201869302600728 1.56306680931806e-08
0.000201870277766931 8.04280250732425e-09
0.000201870496225965 7.63552582272453e-10
0.000201870030736019 -6.15119732927383e-09
0.000201868881295925 -1.26543860945461e-08
0.000201867106112211 -1.8700765436197e-08
0.000201864748839752 -2.42548115203522e-08
0.000201861867685394 -2.92843989613267e-08
0.000201858506304319 -3.37664486371736e-08
0.000201854722903771 -3.76846714944534e-08
0.000201850575691121 -4.10273023054852e-08
0.00020184612287387 -4.37884604131966e-08
0.000201841408107813 -4.59699545096726e-08
0.000201836518704589 -4.757834801139e-08
0.000201831483768342 -4.86263110333063e-08
0.000201826390610914 -4.91280968684116e-08
0.000201821297440581 -4.91090482168666e-08
0.000201816204258001 -4.85958636109451e-08
0.000201811169271432 -4.76122973547266e-08
0.000201806265241266 -4.61920639238667e-08
0.000201801521272205 -4.43702321273332e-08
0.000201796966468998 -4.21839075337438e-08
0.00020179265904023 -3.96706482108655e-08
0.000201788628090745 -3.68718612864249e-08
0.000201784888173514 -3.38296269608573e-08
0.000201781453841447 -3.05846730996873e-08
0.000201778368751325 -2.71786294581133e-08
0.000201775618352258 -2.36529007213715e-08
0.000201773217197106 -2.00454966792218e-08
0.000201771179838754 -1.63962404486906e-08
0.000201769506278143 -1.27422341289485e-08
0.000201768196516135 -9.11900266409305e-09
0.000201767250553578 -5.56048243560703e-09
0.000201766668391281 -2.09948114449077e-09
0.000201766420926159 1.2343639999024e-09
0.00020176650815884 4.41548547724935e-09
0.000201766900986107 7.41899441880634e-09
0.000201767584856538 1.0225434804445e-08
0.000201768530666744 1.28169327373584e-08
0.00020176975296903 1.51774222356682e-08
0.000201771164452202 1.72958206645646e-08
0.000201772808772214 1.91630750989713e-08
0.000201774613169668 2.07723994116726e-08
0.000201776563092716 2.21213055651148e-08
0.00020177862943754 2.32091137974955e-08
0.00020178081220412 2.40367299675359e-08
0.000201783024080817 2.4610489313126e-08
0.000201785352379004 2.49349169922919e-08
0.000201787680683202 2.50165744786202e-08
0.000201790008993123 2.48674547065342e-08
0.000201792337308476 2.44988681008529e-08
0.000201794520109698 2.3928011932961e-08
0.000201796702915502 2.31725345301026e-08
0.000201798769310246 2.22451041476113e-08
0.000201800748397295 2.11649542058989e-08
0.000201802625624279 1.99501841158245e-08
0.000201804371886948 1.86179895667049e-08
0.000201805972632898 1.71880550070558e-08
0.000201807413309788 1.56778023618909e-08
0.000201808708469035 1.41069136927463e-08
0.0002018098435583 1.24930392142453e-08
0.000201810818577141 1.08538262821867e-08
0.000201811618973212 9.20646861524155e-09
0.000201812259297991 7.56906889942677e-09
0.000201812739551108 5.95587776319739e-09
0.000201813059732202 4.38205710606709e-09
0.000201813219840926 2.86140716676542e-09
0.000201813234428908 1.4054670482988e-09
0.000201813103495873 2.50959808489881e-11
0.000201812841593497 -1.26952276469083e-09
0.000201812448721571 -2.47047243773224e-09
0.000201811939431817 -3.5696059164092e-09
0.00020181135737982 -4.56104362611676e-09
0.000201810629805927 -5.44116288136998e-09
0.000201809858573461 -6.20679704854687e-09
0.000201808985474664 -6.85410031509015e-09
0.000201808112372972 -7.38465719130055e-09
0.000201807108301187 -7.7993710656532e-09
0.000201806089674542 -8.09530228962352e-09
0.000201805071045087 -8.27765400668312e-09
0.000201804052412955 -8.35185606784528e-09
0.000201803033778273 -8.32334007272451e-09
0.000201802015141172 -8.19685497255307e-09
0.000201800996501761 -7.97738089475253e-09
0.000201799977860147 -7.66898930470994e-09
0.000201799017424126 -7.27710963710493e-09
0.000201798144297867 -6.81577116967702e-09
0.000201797271170068 -6.29266727614208e-09
0.0002017964708004 -5.71096234192048e-09
0.000201795743189188 -5.08468725457512e-09
0.000201795044680827 -4.4190449632886e-09
0.000201794462587045 -3.72353670119452e-09
0.000201793895044609 -3.00517732920724e-09
0.000201793458469059 -2.27324439827647e-09
0.00020179303644524 -1.53384493994935e-09
0.000201792745388693 -7.96256116597505e-10
0.000201792483436151 -6.59083343457212e-11
0.000201792337899324 6.47921438723387e-10
0.000201792206914936 1.34071009849634e-09
0.000201792206898445 2.00657437887664e-09
0.000201792206882751 2.6400836239393e-09
0.000201792337835181 3.23716436989585e-09
0.000201792483340586 3.79171077868889e-09
0.000201792672502756 4.3048519193789e-09
0.000201792963529561 4.76776262914314e-09
0.000201793254557627 5.17999368399025e-09
0.000201793545586885 5.54426005106023e-09
0.000201793953032681 5.85874798675334e-09
0.000201794389583758 6.11463688016123e-09
0.000201794826136191 6.31577201648525e-09
0.000201795262689922 6.46464368148081e-09
0.000201795699244877 6.56396462184183e-09
0.000201796135801005 6.61599969253857e-09
0.000201796572358251 6.62278298868557e-09
0.000201797008916562 6.58680557319435e-09
0.000201797445475883 6.50987522221591e-09
0.000201797882036163 6.39425584703091e-09
0.000201798318597357 6.24175752750311e-09
0.000201798755159427 6.05396355268795e-09
0.000201799191722316 5.83313716773226e-09
0.000201799599182149 5.58108756432141e-09
0.000201799890227202 5.30754457050975e-09
0.000201800181272635 5.01861605051168e-09
0.000201800472318424 4.71543440405675e-09
0.000201800763364555 4.39845090904889e-09
0.000201801010755241 4.06970418476149e-09
0.000201801156282559 3.73937211750608e-09
0.000201801301809837 3.41085137911534e-09
0.000201801447337076 3.08391431835808e-09
0.000201801592864282 2.75810746463989e-09
0.000201801607424088 2.43954279000036e-09
0.000201801607431595 2.1365899605108e-09
0.000201801607438734 1.8483428398941e-09
0.000201801607445533 1.57389754007475e-09
0.000201801607452002 1.3128014508812e-09
0.000201801491042744 1.06844888492219e-09
0.000201801345529029 8.49436632144318e-10
0.000201801200014695 6.5553912298455e-10
0.000201801054499787 4.84718876148094e-10
0.000201800908984321 3.36524447197561e-10
0.000201800763468309 2.10276074330551e-10
0.000201800617951799 1.04164704639587e-10
0.000201800472434805 1.75106595889929e-11
0.000201800326917365 -5.10428643796246e-11
0.000201800181399489 -1.0194803334862e-10
0.000201800035881202 -1.3633766338117e-10
0.000201799890362523 -1.54889018277871e-10
0.000201799744843471 -1.58508317582573e-10
0.000201799599324062 -1.47419687568373e-10
0.000201799453804313 -1.22984317174613e-10
0.000201799308284245 -8.5424500806397e-11
0.000201799162763872 -3.56479568086598e-11
0.000201799017243207 2.61214661012588e-11
0.00020179887172227 9.85228010286221e-11
0.00020179872620106 1.82238363288789e-10
0.000201798580679604 2.75681699690722e-10
0.000201798435157908 3.79081627199795e-10
0.000201798289635978 4.9152970582611e-10
0.000201798144113859 6.11897976732223e-10
0.000201797998591521 7.4109021697133e-10
0.000201797853068989 8.7797433212522e-10
0.000201797707546272 1.02232486365317e-09
0.000201797562023372 1.17436926849734e-09
0.000201797474707978 1.33229496879217e-09
0.000201797474704191 1.48501533292489e-09
0.000201797474700577 1.6309488759525e-09
0.000201797474697142 1.76964223830289e-09
0.000201797474693873 1.90154783585861e-09
0.000201797474690761 2.02711825103563e-09
0.000201797474687804 2.14658066322038e-09
0.000201797474684982 2.26038551764951e-09
0.0002017974746823 2.36876135373265e-09
0.000201797474679757 2.47125325758546e-09
0.000201797474677342 2.56876850346366e-09
0.000201797474675039 2.66175884111597e-09
0.000201797532880526 2.74931827304314e-09
0.000201797678397883 2.82126555450901e-09
0.00020179782391568 2.87556592426519e-09
0.000201797969433884 2.91312191036397e-09
0.00020179811495249 2.93461457911981e-09
0.000201798260471476 2.94094909536469e-09
0.000201798405990817 2.93280297269938e-09
0.0002017985515105 2.91085511250344e-09
0.0002017986970305 2.8760105130754e-09
0.000201798842550818 2.82849652033512e-09
0.000201798988071426 2.76898967643824e-09
0.000201799089936563 2.69885083725718e-09
0.000201799089938315 2.62803304118542e-09
0.000201799089939976 2.56106250096089e-09
0.00020179908994156 2.4970323586615e-09
0.000201799089943072 2.43617098716342e-09
0.000201799089944505 2.37824973603473e-09
0.000201799089945872 2.32304375735737e-09
0.000201799089947166 2.27100646621459e-09
0.000201799089948381 2.22190935095234e-09
0.000201799089949547 2.17484852349514e-09
0.000201799089950663 2.12982428915431e-09
0.000201799089951722 2.08706246729307e-09
0.000201799089952726 2.04633593403614e-09
0.00020179908995368 2.00787292348181e-09
0.000201799089954589 1.97122018708029e-09
0.000201799089955459 1.93615110055667e-09
0.000201799089956296 1.90243967801429e-09
0.000201799089957077 1.87076351632065e-09
0.000201799089957824 1.84067208697236e-09
0.000201799089958549 1.81148590572278e-09
0.000201799089959218 1.7843347910329e-09
0.000201799089959866 1.7583161593393e-09
0.000201799089960479 1.73342759590689e-09
0.000201799089961064 1.70989783443432e-09
0.000201799089961622 1.68727201654839e-09
0.000201799089962151 1.66600469531097e-09
0.000201799089962654 1.64564134541578e-09
0.000201799089963144 1.6259580903899e-09
0.00020179908996359 1.60785726399659e-09
0.000201799089964037 1.58975654862559e-09
0.000201799089964444 1.57346702334138e-09
0.000201799089964834 1.55762902576129e-09
0.000201799089965225 1.54179086164774e-09
0.000201799089965571 1.52799017882899e-09
0.000201799089965905 1.51441459372847e-09
0.00020179908996624 1.50083906413911e-09
0.000201799089966546 1.48862225324287e-09
0.000201799089966825 1.47730930266654e-09
0.000201799089967104 1.46599632433464e-09
0.000201799089967383 1.45468331824716e-09
0.00020179908996764 1.44450282291153e-09
0.000201799089967862 1.43545256237054e-09
0.000201799089968086 1.42640210754053e-09
0.000201799089968309 1.41735176373281e-09
0.000201799089968532 1.4083014199251e-09
0.000201799089968732 1.40038353135807e-09
0.0002017990899689 1.39359571105224e-09
0.000201799089969067 1.38680800176871e-09
0.000201799089969234 1.38002018146288e-09
0.000201799089969402 1.3732324166682e-09
0.00020179908996957 1.36644465187352e-09
0.000201799089969737 1.35965688707884e-09
0.00020179908996987 1.35445402116297e-09
0.000201799089969982 1.34992889089247e-09
0.000201799089970094 1.34540370511083e-09
0.000201799089970205 1.34087851932918e-09
0.000201799089970316 1.33635336130311e-09
0.000201799089970428 1.33182812001031e-09
0.000201799089970539 1.3273030174954e-09
0.000201799089970651 1.32277783171375e-09
0.000201799089970763 1.31825264593211e-09
0.000201799089970874 1.31372734912816e-09
0.000201799089970958 1.31056088203962e-09
0.000201799089971013 1.30829841404889e-09
0.000201799089971069 1.30603572401355e-09
0.000201799089971125 1.30377325602282e-09
0.000201799089971182 1.30151070476536e-09
0.000201799089971236 1.29924795921887e-09
0.000201799089971292 1.29698532469469e-09
0.000201799089971348 1.29472285670396e-09
0.000201799089971404 1.29246036095765e-09
0.00020179908997146 1.29019767092231e-09
0.000201799089971516 1.28793511966485e-09
0.000201799089971572 1.28567251289624e-09
0.000201799089971627 1.28340996163878e-09
0.000201799089971683 1.28114727160344e-09
0.000201799089971739 1.27888458156811e-09
0.000201799089971795 1.27662216908853e-09
0.000201799089971851 1.27435953456434e-09
0.000201799089971906 1.27209690004015e-09
0.000201799089971962 1.26983434878269e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
};
\addplot [very thick, learnedWithSideInfo, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131116545711762 0.0250445317812143
0.126937688377481 -0.0387556004261476
0.0961448371241316 -0.0801006331769843
0.0513040838296561 -0.0948778404962409
0.00527218675107144 -0.0857814996980235
-0.0317112162538929 -0.0601486825068359
-0.0536606194275029 -0.0271993834259413
-0.059151976447718 0.00437597861812911
-0.0506178308813379 0.0280598413454645
-0.0329906666617868 0.0404623985592648
-0.0120798599606739 0.0414028702504951
0.00688145659747326 0.0332067154679798
0.0202297181773896 0.0196379811820025
0.0263100870816895 0.00479150639694176
0.025396483908854 -0.0078460046342394
0.0192168311954741 -0.0160171693329955
0.0102640868745289 -0.0189246947751253
0.00108750665010273 -0.0170908870659565
-0.00627406852002308 -0.0119537987376183
-0.0106227090905902 -0.00535175623667514
-0.0116762146774111 0.000963548760932464
-0.00992805130951922 0.00568723279293129
-0.00637018409219281 0.00814547835582685
-0.00216895623685106 0.0083025248325215
0.00162545744232498 0.00662806897711307
0.00428068778268982 0.00388504757649577
0.00547106541272418 0.000900840206889547
0.00525927540162989 -0.00162558244506184
0.00399799386659648 -0.00324701238277861
0.00219014511519616 -0.00381008682087952
0.000347050591175443 -0.00342440354371015
-0.00112424823999413 -0.00238122695915852
-0.00198638140412942 -0.00105052930702254
-0.00218592465692334 0.000216465734846655
-0.00182467963847435 0.00115926973459138
-0.00110362232349989 0.00164465993637147
-0.000257662594244532 0.00166763326149511
0.000502651893746994 0.00132440954443838
0.00103139412538467 0.00076944857474856
0.00126472017735974 0.000169272080593447
0.00121673769338339 -0.000336230340346105
0.000959400662446599 -0.000658277206431829
0.000594268194931046 -0.000767251781220835
0.000224024607263378 -0.000686177191285692
-7.00112965817252e-05 -0.000474209833944111
-0.000240825812600787 -0.000205912877895204
-0.000278386190046434 4.82692404077112e-05
-0.000203719755493797 0.000236368823310962
-5.75596916485298e-05 0.000332106453929448
0.000112789671281218 0.000334959281247021
0.000265137248132575 0.000264636549209579
0.000370424202815617 0.000152383550119095
0.00041614418384948 3.16901971675609e-05
0.000405429845133216 -6.94539397838312e-05
0.000352952455203427 -0.000133418649458317
0.000279218371228328 -0.000154485188668285
0.000204850917896696 -0.000137478350419079
0.000146097197266026 -9.4414297122758e-05
0.00011226645555088 -4.03235713841155e-05
0.00010523239797657 1.06643195311729e-05
0.000120654227134552 4.81842217916473e-05
0.000150277148936695 6.70566301565201e-05
0.000184576834040719 6.72747823569908e-05
0.000215100470468064 5.28737470403551e-05
0.000236062875632186 3.017214576162e-05
0.000245015974319136 5.90375379849739e-06
0.00024264858817981 -1.4331895188735e-05
0.00023195106335397 -2.70342339963037e-05
0.000217063522992863 -3.11005437502454e-05
0.000202127524994963 -2.7539946004268e-05
0.000190388963311047 -1.87928241421609e-05
0.000183690723714407 -7.88888043923297e-06
0.000182380652598204 2.33800228718883e-06
0.000185563218179278 9.82083334402639e-06
0.00019156589240542 1.35393490020286e-05
0.000198471387407031 1.35119075053425e-05
0.000204586363821164 1.0564209322661e-05
0.000208759253396971 5.97382983008599e-06
0.000210511191870911 1.09456346322756e-06
0.000209992574629287 -2.95349364676234e-06
0.000207812673092691 -5.47545845600017e-06
0.000204807023793293 -6.2590174216004e-06
0.000201807463003443 -5.51483257016372e-06
0.000199462581802312 -3.73849604337617e-06
0.00019813684800101 -1.54067113330991e-06
0.000197894347754332 5.10357313882048e-07
0.000198550674867261 2.00245245521313e-06
0.000199766774722201 2.73474574052912e-06
0.000201156817683773 2.71492586767508e-06
0.000202381754526399 2.11188231952208e-06
0.000203212269794021 1.18384248590231e-06
0.000203554773386592 2.02954681866041e-07
0.000203442030664285 -6.06747186326917e-07
0.000202997947757092 -1.10733703417853e-06
0.000202391354960933 -1.25808266343563e-06
0.000201789134711658 -1.10287795848651e-06
0.000201320699671585 -7.42320991425904e-07
0.000201058361347483 -2.99396442554611e-07
0.000201013749542052 1.11918896428254e-07
0.000201148783932615 4.09438604104251e-07
0.000201395100605548 5.53690313737087e-07
0.000201675006837805 5.46885519647766e-07
0.000201920340609062 4.23564858409442e-07
0.000202085436718269 2.36014275040164e-07
0.000202152627788572 3.88662906025683e-08
0.000202128301001972 -1.23144228786343e-07
0.000202037746903448 -2.22512787778628e-07
0.00020191510408882 -2.5140112816513e-07
0.000201794045913085 -2.18942704605096e-07
0.000201700446186272 -1.45608910734341e-07
0.000201648682815183 -5.62612627874604e-08
0.000201640822739206 2.61877766416507e-08
0.000201668964675175 8.53457677307823e-08
0.000201719138977705 1.1346410450086e-07
0.000201775527698979 1.11245890610512e-07
0.000201824670142467 8.58032878081616e-08
0.000201857456547874 4.77205036042427e-08
0.000201870277766931 8.04280250732425e-09
0.000201864748839752 -2.42548115203522e-08
0.00020184612287387 -4.37884604131966e-08
0.000201821297440581 -4.91090482168666e-08
0.000201796966468998 -4.21839075337438e-08
0.000201778368751325 -2.71786294581133e-08
0.000201768196516135 -9.11900266409305e-09
0.000201766900986107 7.41899441880634e-09
0.000201772808772214 1.91630750989713e-08
0.000201783024080817 2.4610489313126e-08
0.000201794520109698 2.3928011932961e-08
0.000201804371886948 1.86179895667049e-08
0.000201810818577141 1.08538262821867e-08
0.000201813219840926 2.86140716676542e-09
0.000201811939431817 -3.5696059164092e-09
0.000201808112372972 -7.38465719130055e-09
0.000201803033778273 -8.32334007272451e-09
0.000201798144297867 -6.81577116967702e-09
0.000201794462587045 -3.72353670119452e-09
0.000201792483436151 -6.59083343457212e-11
0.000201792337835181 3.23716436989585e-09
0.000201793545586885 5.54426005106023e-09
0.000201795699244877 6.56396462184183e-09
0.000201797882036163 6.39425584703091e-09
0.000201799890227202 5.30754457050975e-09
0.000201801156282559 3.73937211750608e-09
0.000201801607431595 2.1365899605108e-09
0.000201801345529029 8.49436632144318e-10
0.000201800617951799 1.04164704639587e-10
0.000201799890362523 -1.54889018277871e-10
0.000201799162763872 -3.56479568086598e-11
0.000201798435157908 3.79081627199795e-10
0.000201797707546272 1.02232486365317e-09
0.000201797474697142 1.76964223830289e-09
0.0002017974746823 2.36876135373265e-09
0.000201797678397883 2.82126555450901e-09
0.000201798405990817 2.93280297269938e-09
0.000201799089936563 2.69885083725718e-09
0.000201799089944505 2.37824973603473e-09
0.000201799089950663 2.12982428915431e-09
0.000201799089955459 1.93615110055667e-09
0.000201799089959218 1.7843347910329e-09
0.000201799089962151 1.66600469531097e-09
0.000201799089964444 1.57346702334138e-09
0.00020179908996624 1.50083906413911e-09
0.00020179908996764 1.44450282291153e-09
0.000201799089968732 1.40038353135807e-09
0.00020179908996957 1.36644465187352e-09
0.000201799089970205 1.34087851932918e-09
0.000201799089970763 1.31825264593211e-09
0.000201799089971125 1.30377325602282e-09
0.000201799089971404 1.29246036095765e-09
0.000201799089971683 1.28114727160344e-09
0.000201799089971962 1.26983434878269e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
0.000201799089971967 1.26983548676129e-09
};
\addplot [very thick, learnedWithoutSideInfo]
table {%
0.1 0.1
0.111796811918241 0.0870725912737864
0.12163252693286 0.0728793495815427
0.128659019621105 0.0576611527329911
0.132625197050847 0.0420048181572819
0.133959639595182 0.0266316873450343
0.133410585095159 0.0121353508583164
0.131673414724467 -0.00116223691997952
0.129237287470303 -0.0131990280305292
0.126391518263561 -0.0240812099492285
0.123282238877946 -0.0339909429701191
0.119964486894895 -0.0431255132967685
0.11643679885916 -0.0516659228361043
0.112660856148374 -0.0597630578965163
0.108571392545421 -0.06753126683682
0.10408066177837 -0.0750430483631197
0.0990806932772159 -0.0823217154725073
0.0934461220144343 -0.0893315400874553
0.0870404474351378 -0.0959678693796651
0.0797286245095563 -0.102053264758347
0.0713980725189813 -0.107348268915611
0.0619876710918197 -0.111583337205351
0.0515199170601113 -0.114509141655369
0.0401260734294686 -0.1159497203439
0.0280503669322352 -0.11583701478101
0.0156222077059951 -0.114212593952418
0.00319971916300332 -0.111198019631662
-0.00889289201008925 -0.10694923750393
-0.020405833054955 -0.101615173503216
-0.0311692293457391 -0.0953149410309937
-0.0410720834032938 -0.088137219305267
-0.0500328992001622 -0.0801569153495709
-0.0579772585284042 -0.0714605487720199
-0.0648299389551967 -0.0621706225354597
-0.0705216894914455 -0.0524590958220852
-0.0750045866657825 -0.0425426949195744
-0.0782662915290082 -0.0326600505152674
-0.0803348360271636 -0.0230398205417144
-0.0812716367616462 -0.0138733405537685
-0.0811570401804307 -0.00530134272159621
-0.0800754007401476 0.00258423390393148
-0.0781050303260633 0.00972871136430964
-0.075315045913567 0.0161002531965302
-0.071768584884726 0.0216775579405164
-0.0675305799092882 0.0264421611578722
-0.0626776863349496 0.0303760027209918
-0.0573074777174991 0.0334637916245875
-0.0515437312021465 0.0356988883731741
-0.0455351125464674 0.0370907123527875
-0.0394463608544537 0.0376712472134724
-0.0334438114696258 0.0374984310441171
-0.0276793893815022 0.0366552128978856
-0.0222776122807549 0.0352444674269226
-0.0173284769476378 0.0333811350340047
-0.0128865821402551 0.0311834463814336
-0.00897493341871947 0.0287648978083155
-0.00559121441476229 0.0262280664947854
-0.00271462653085219 0.0236607073669539
-0.00031210438698448 0.0211340497450383
0.00165662832823354 0.0187028820585589
0.00323525665152857 0.0164068747317092
0.00446818923266434 0.0142726019347279
0.00539876818266993 0.0123158232515248
0.00606814698971458 0.0105437202126328
0.00651464141025038 0.00895690964289564
0.00677340108890245 0.00755115493675351
0.00687629079842367 0.00631876261575037
0.00685190437562166 0.00524968910435497
0.00672566042178779 0.004332399392454
0.0065199473139339 0.00355452287367886
0.00625429745432271 0.00290334821348015
0.00594557851753841 0.00236619268429017
0.00560819411834768 0.00193067441058403
0.00525428892852542 0.00158490961058
0.00489395463699616 0.00131765167694198
0.00453543384157307 0.00111838486479243
0.00418531934255562 0.0009773823129402
0.00384874658768997 0.000885735906469343
0.00352957729813141 0.000835363888463725
0.00323057262311277 0.000819000968839134
0.00295355452696278 0.00083017482144232
0.00269955448762715 0.000863172207303364
0.00246894895769501 0.000912997444233454
0.0022615813871063 0.000975325515288006
0.00207687091502962 0.00104645174499751
0.00191390809852621 0.00112323965423577
0.00177153825328347 0.00120306832436956
0.00164843313847385 0.00128378035252119
0.00154315182691445 0.00136363125982175
0.00145419166886285 0.00144124102057042
0.00138003028973177 0.00151554821167199
0.00131915956478146 0.0015857671355537
0.0012701124939225 0.00165134814582313
0.00123148386223448 0.00171194129982588
0.0012019455225456 0.00176736337564076
0.00118025707754033 0.00181756822026102
0.00116527267629429 0.00186262033918716
0.00115594457388468 0.00190267159374446
0.00115132403684814 0.00193794083969046
0.00115056011284764 0.00196869631704821
0.00115289672002739 0.00199524058612699
0.00115766845334342 0.00201789779598993
0.00116429544977414 0.00203700306906551
0.00117227760371996 0.00205289378736673
0.00118118837799397 0.0020659025716423
0.00119066841373261 0.00207635175303267
0.00120041910566382 0.00208454914790313
0.00121019627590702 0.0020907849583347
0.00121980405083022 0.00209532963454784
0.00122908902021823 0.00209843254904563
0.00123793473653677 0.00210032134640414
0.00124625659366284 0.00210120184665641
0.00125399710926555 0.00210125839351161
0.00126112162189429 0.0021006545519171
0.00126761440394407 0.00209953407150199
0.00127347518290666 0.00209802204393128
0.0012787160571035 0.00209622619293448
0.00128335878699026 0.00209423824525867
0.00128743243986307 0.00209213533958152
0.00129097136298562 0.00208998143831707
0.00129401345902558 0.00208782871421054
0.00129659873699506 0.00208571888967324
0.00129876811168739 0.00208368451216856
0.00130056242551291 0.00208175015356726
0.0013020216671471 0.00207993352526881
0.00130318436304666 0.00207824650417354
0.00130408711897623 0.00207669606732974
0.00130476429055637 0.00207528513524657
0.00130524776358865 0.00207401332578439
0.00130556682627514 0.0020728776216572
0.00130574811764816 0.00207187295593858
0.00130581563785803 0.00207099272045674
0.00130579080790305 0.00207022920265221
0.00130569256759472 0.0020695739565868
0.00130553750235318 0.00206901811413651
0.00130533999046456 0.00206855264221772
0.00130511236400288 0.00206816855179159
0.00130486507740191 0.00206785706423851
0.00130460687898193 0.00206760974041664
0.00130434498138587 0.00206741857728154
0.00130408522791825 0.00206727607668533
0.0013038322523462 0.00206717529061784
0.00130358963031441 0.00206710984665026
0.0013033600210921 0.00206707395713845
0.00130314529887876 0.00206706241507781
0.00130294667321973 0.00206707057960376
0.00130276479823088 0.00206709435325969
0.00130259987084091 0.00206713015325999
0.00130245171833998 0.00206717487846042
0.00130231987560858 0.00206722587353525
0.00130220365262801 0.00206728089162311
0.00130210219285054 0.00206733805649684
0.00130201452321188 0.00206739582504589
0.00130193959635339 0.00206745295078736
0.00130187632587297 0.00206750844889481
0.00130182361532594 0.00206756156304433
0.00130178038158668 0.00206761173453263
0.00130174557330953 0.00206765857368474
0.00130171818505787 0.00206770183360128
0.00130169726768337 0.00206774138651333
0.00130168193565439 0.00206777720243423
0.00130167137156079 0.00206780933017647
0.00130166482841076 0.00206783788069664
0.00130166163014245 0.00206786301247597
0.00130166117061492 0.00206788491895971
0.00130166291145173 0.00206790381777999
0.0013016663789811 0.00206791994169997
0.00130167116054736 0.00206793353106605
0.00130167690035332 0.00206794482754624
0.00130168329504787 0.00206795406922033
0.00130169008910741 0.00206796148662125
0.0013016970703239 0.00206796729978365
0.00130170406523078 0.00206797171601814
0.00130171093477216 0.00206797492842803
0.00130171757011421 0.00206797711500073
0.00130172388875938 0.002067978438129
0.00130172983084975 0.00206797904457812
0.00130173535585154 0.00206797906577005
0.00130174043943221 0.00206797861824182
0.00130174507072578 0.00206797780439061
0.00130174924986903 0.00206797671329717
0.00130175298578372 0.00206797542161841
0.00130175629423235 0.00206797399462921
0.00130175919617415 0.00206797248716661
0.00130176171628893 0.00206797094470179
0.00130176388176917 0.002067969404286
0.00130176572129947 0.00206796789553287
0.00130176726414977 0.00206796644151463
0.00130176853955088 0.00206796505963158
0.00130176957610306 0.0020679637623946
0.00130177040132207 0.00206796255818187
0.00130177104137275 0.00206796145186416
0.00130177152078481 0.00206796044543456
0.00130177186231339 0.00206795953854755
0.00130177208686 0.00206795872898091
0.00130177221343342 0.00206795801307091
0.00130177225914707 0.00206795738604448
0.00130177223926431 0.00206795684235939
0.00130177216728011 0.00206795637595825
0.00130177205501347 0.00206795598047904
0.00130177191270242 0.00206795564947182
0.00130177174911772 0.00206795537648841
0.00130177157172273 0.00206795515526004
0.0013017713867054 0.0020679549797471
0.00130177119920649 0.00206795484424127
0.00130177101338447 0.00206795474338506
0.00130177083251759 0.00206795467222154
0.00130177065913628 0.0020679546261988
0.00130177049512703 0.00206795460120013
0.00130177034181855 0.00206795459349696
0.00130177020005551 0.00206795459978881
0.00130177007030863 0.00206795461715181
0.00130176995268627 0.00206795464304843
0.00130176984706232 0.00206795467525112
0.00130176975308594 0.00206795471188492
0.00130176967026951 0.00206795475134758
0.00130176959800377 0.0020679547923006
0.00130176953558347 0.00206795483365418
0.0013017694822528 0.00206795487451483
0.00130176943724081 0.0020679549141942
0.00130176939976501 0.00206795495214163
0.00130176936903759 0.00206795498797696
0.00130176934432136 0.00206795502142221
0.00130176932489512 0.00206795505229262
0.00130176931006698 0.00206795508051361
0.00130176929922854 0.00206795510605584
0.00130176929177228 0.0020679551289664
0.00130176928718395 0.00206795514931724
0.00130176928497683 0.00206795516722291
0.00130176928470238 0.00206795518282643
0.00130176928599823 0.00206795519628589
0.00130176928852066 0.00206795520776204
0.00130176929197923 0.00206795521742809
0.00130176929611459 0.00206795522546344
0.00130176930071269 0.00206795523202974
0.00130176930560033 0.00206795523728331
0.001301769310599 0.00206795524139913
0.00130176931560477 0.00206795524452641
0.00130176932051729 0.00206795524679837
0.00130176932525217 0.00206795524834114
0.00130176932976234 0.00206795524926129
0.00130176933400961 0.00206795524968317
0.00130176933795845 0.0020679552496885
0.00130176934158666 0.00206795524936165
0.0013017693448889 0.00206795524876568
0.00130176934786785 0.00206795524797254
0.00130176935054482 0.00206795524703729
0.00130176935289317 0.00206795524601588
0.00130176935496262 0.00206795524493408
0.00130176935676118 0.00206795524382297
0.00130176935830395 0.00206795524272252
0.00130176935961046 0.00206795524164427
0.00130176936071624 0.002067955240598
0.00130176936162574 0.00206795523961123
0.00130176936235493 0.00206795523868575
0.00130176936293669 0.00206795523782333
0.00130176936338255 0.00206795523703729
0.00130176936372184 0.00206795523632497
0.00130176936395632 0.00206795523568104
0.0013017693641082 0.00206795523510639
0.00130176936419168 0.00206795523459569
0.00130176936422632 0.00206795523414627
0.00130176936421122 0.00206795523375547
0.00130176936416326 0.00206795523342773
0.001301769364078 0.00206795523314618
0.00130176936397763 0.00206795523290815
0.00130176936386484 0.00206795523271541
0.00130176936373871 0.00206795523255998
0.00130176936360549 0.0020679552324383
0.00130176936345539 0.00206795523233616
0.00130176936331772 0.00206795523227843
0.00130176936318538 0.00206795523222425
0.00130176936306103 0.00206795523219228
0.00130176936294646 0.00206795523218073
0.00130176936283188 0.0020679552321754
0.00130176936274218 0.00206795523218428
0.00130176936264714 0.0020679552321976
0.00130176936256099 0.0020679552322207
0.00130176936248905 0.00206795523224557
0.00130176936242066 0.00206795523227221
0.00130176936236914 0.00206795523230507
0.00130176936232029 0.0020679552323255
0.00130176936227944 0.00206795523234682
0.00130176936223858 0.00206795523237435
0.00130176936221282 0.00206795523239833
0.00130176936218085 0.00206795523242231
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
};
\addplot [very thick, learnedWithoutSideInfo, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.133959639595182 0.0266316873450343
0.123282238877946 -0.0339909429701191
0.10408066177837 -0.0750430483631197
0.0713980725189813 -0.107348268915611
0.0156222077059951 -0.114212593952418
-0.0410720834032938 -0.088137219305267
-0.0750045866657825 -0.0425426949195744
-0.0800754007401476 0.00258423390393148
-0.0626776863349496 0.0303760027209918
-0.0334438114696258 0.0374984310441171
-0.00897493341871947 0.0287648978083155
0.00323525665152857 0.0164068747317092
0.00677340108890245 0.00755115493675351
0.00625429745432271 0.00290334821348015
0.00453543384157307 0.00111838486479243
0.00295355452696278 0.00083017482144232
0.00191390809852621 0.00112323965423577
0.00138003028973177 0.00151554821167199
0.00118025707754033 0.00181756822026102
0.00115289672002739 0.00199524058612699
0.00119066841373261 0.00207635175303267
0.00123793473653677 0.00210032134640414
0.00127347518290666 0.00209802204393128
0.00129401345902558 0.00208782871421054
0.00130318436304666 0.00207824650417354
0.00130574811764816 0.00207187295593858
0.00130533999046456 0.00206855264221772
0.00130408522791825 0.00206727607668533
0.00130294667321973 0.00206707057960376
0.00130220365262801 0.00206728089162311
0.00130182361532594 0.00206756156304433
0.00130168193565439 0.00206777720243423
0.00130166291145173 0.00206790381777999
0.00130169008910741 0.00206796148662125
0.00130172388875938 0.002067978438129
0.00130174924986903 0.00206797671329717
0.00130176388176917 0.002067969404286
0.00130177040132207 0.00206796255818187
0.00130177221343342 0.00206795801307091
0.00130177191270242 0.00206795564947182
0.00130177101338447 0.00206795474338506
0.00130177020005551 0.00206795459978881
0.00130176967026951 0.00206795475134758
0.00130176939976501 0.00206795495214163
0.00130176929922854 0.00206795510605584
0.00130176928599823 0.00206795519628589
0.00130176930560033 0.00206795523728331
0.00130176932976234 0.00206795524926129
0.00130176934786785 0.00206795524797254
0.00130176935830395 0.00206795524272252
0.00130176936293669 0.00206795523782333
0.00130176936419168 0.00206795523459569
0.00130176936397763 0.00206795523290815
0.00130176936331772 0.00206795523227843
0.00130176936274218 0.00206795523218428
0.00130176936236914 0.00206795523230507
0.00130176936218085 0.00206795523242231
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
0.0013017693621622 0.00206795523243564
};

==> figures/smd_phase_plots/phase_plot_100_quarter_space_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.0483499839901924 0.141897454857826
0.11503766477108 0.122913159430027
0.0785158202052116 0.0972380340099335
0.112731285393238 0.130300760269165
0.0280732959508896 0.116635769605637
0.00600947020575404 0.0179075319319963
0.139512360095978 0.0480624325573444
0.12991289794445 0.106046535074711
0.121770523488522 0.0501096919178963
0.00745475199073553 0.0356143489480019
0.131836712360382 0.12271448969841
0.139614269137383 0.0951960161328316
0.114962287247181 0.0961377397179604
0.0701436102390289 0.0344149433076382
0.0358739644289017 0.0248856134712696
0.0851626172661781 0.0784569531679153
0.0433087944984436 0.0945643708109856
0.0775911137461662 0.124814674258232
0.107141308486462 0.0339269489049911
0.0933225080370903 0.137005507946014
0.105258874595165 0.147549405694008
0.0534050911664963 0.140254870057106
0.0569222532212734 0.0897052511572838
0.0404710881412029 0.0848271697759628
0.0911833494901657 0.045405887067318
0.11817778646946 0.086422510445118
0.126068741083145 0.0484955348074436
0.134626403450966 0.0376733131706715
0.0509465076029301 0.137888863682747
0.000294292985927314 0.142952337861061
0.142132714390755 0.0831343308091164
0.0566836707293987 0.138762265443802
0.14408116042614 0.137433126568794
0.0025108577683568 0.0047277333214879
0.0690243616700172 0.139255657792091
0.115116275846958 0.0676542595028877
0.0258397720754147 0.0546195916831493
0.0520978271961212 0.0848119333386421
0.118037104606628 0.134559750556946
0.104880228638649 0.112051486968994
0.00836778711527586 0.100203417241573
0.0283552277833223 0.0458506383001804
0.137104973196983 0.0361109040677547
0.130142718553543 0.110110342502594
0.0599146485328674 0.0432487241923809
0.0585291087627411 0.0990993157029152
0.0986373871564865 0.00711761880666018
0.104536898434162 0.0813784524798393
0.0457173250615597 0.00577366957440972
0.0643585473299026 0.1263737231493
0.0476247519254684 0.0466810427606106
0.0930472388863564 0.143961831927299
0.00906130112707615 0.129335030913353
0.148844838142395 0.00707785878330469
0.145483240485191 0.0465302132070065
0.0361443273723125 0.0992181450128555
0.00576944183558226 0.0188985075801611
0.0933742895722389 0.0826461017131805
0.122434213757515 0.0126915276050568
0.0275251343846321 0.0732061192393303
0.143171295523643 0.139956280589104
0.0670974552631378 0.128255262970924
0.138785630464554 0.0143069149926305
0.106468468904495 0.137433335185051
0.090683251619339 0.0384356528520584
0.102514356374741 0.036594595760107
0.106262728571892 0.124472513794899
0.0405312888324261 0.114618994295597
0.0231780838221312 0.0584027953445911
0.117823578417301 0.0170953702181578
0.0693604052066803 0.0101192016154528
0.135613843798637 0.0104174325242639
0.0457076989114285 0.0745806843042374
0.135606825351715 0.127570018172264
0.114220604300499 0.0638028904795647
0.139378041028976 0.129244670271873
0.0186410415917635 0.115355148911476
0.0669341906905174 0.0251625068485737
0.121327266097069 0.128826573491096
0.0579857043921947 0.0776307433843613
0.107227861881256 0.0920865088701248
0.127498283982277 0.0598821416497231
0.0117002865299582 0.00982911884784698
0.0273569636046886 0.0253059286624193
0.0559093281626701 0.10799103975296
0.111371673643589 0.0679899677634239
0.144354343414307 0.0108326058834791
0.0900163501501083 0.132489919662476
0.0817112252116203 0.0796327367424965
0.119032450020313 0.11580566316843
0.101587131619453 0.103340692818165
0.0993812307715416 0.0983299314975739
0.00442994246259332 0.00850098114460707
0.000598621729295701 0.0816336125135422
0.0984762385487556 0.0955890715122223
0.00807077810168266 0.0638101845979691
0.0622699148952961 0.118677109479904
0.014829465188086 0.0653865039348602
0.116885535418987 0.0440747886896133
0.121060855686665 0.0383744426071644
};
\addplot [very thick, trueDynamics]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, approxDynamics, dashed]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, learnedWithSideInfo]
table {%
0.1 0.1
0.109247062579702 0.0849136685935313
0.116979715175546 0.0697373650169222
0.123196582683375 0.054622666331561
0.127911049236702 0.0397117093206761
0.131150103691391 0.0251356025722856
0.132953311736207 0.0110134003390415
0.13337149744594 -0.00254822887526807
0.132465543973492 -0.0154547451374139
0.130305216478445 -0.0276230225493118
0.126968029637955 -0.0389804261332939
0.122538278968927 -0.0494638854601279
0.117106176391065 -0.0590191414939067
0.110766888901617 -0.0676003119107607
0.103619778412813 -0.0751696517219756
0.0957675894598062 -0.0816976800135551
0.0873155698896051 -0.0871635011473345
0.0783705990473089 -0.0915552066414659
0.0690403160102689 -0.0948704282604026
0.0594320206260521 -0.0971167482312771
0.0496518577121472 -0.0983119976459421
0.0398035915047672 -0.0984843775957062
0.0299876707014768 -0.0976722558562022
0.0203002301826857 -0.0959237383270715
0.0108321216025952 -0.0932959724778207
0.00166806992534072 -0.0898541185842259
-0.0071140624915404 -0.0856701683559529
-0.0154438975243614 -0.0808215533542129
-0.0232590120673933 -0.0753897072233798
-0.0305052758979861 -0.0694586555136293
-0.0371370056327868 -0.0631135958967026
-0.0431170858700346 -0.056439686208219
-0.048416838885867 -0.049520816049883
-0.0530158738389843 -0.0424387169076976
-0.0569018279358737 -0.0352721307420708
-0.0600700498393938 -0.0280962719098358
-0.0625231973824819 -0.0209822418539371
-0.0642708389899526 -0.0139966798076459
-0.0653289321501649 -0.00720147380527832
-0.0657194173596185 -0.000653510227636683
-0.0654696369696904 0.00559551711088195
-0.0646118657872419 0.0114992724685751
-0.0631827001120248 0.0170169140972242
-0.0612225473579604 0.0221131998953602
-0.0587751082265791 0.0267585759077914
-0.0558866875201988 0.0309292179767128
-0.0526057098498749 0.0346070037545409
-0.0489821422150653 0.0377794848867172
-0.0450668979577607 0.0404397547238691
-0.0409113226753687 0.0425862894919421
-0.0365666577808287 0.0442227151578759
-0.0320835115111532 0.045357498343687
-0.027511447281483 0.0460036523464774
-0.0228984975303707 0.0461783654974339
-0.0182907911818317 0.0459025857104089
-0.0137321839008316 0.0452006162944087
-0.00926395912526997 0.0440996902043337
-0.00492454819014396 0.0426295368220914
-0.000749293814892219 0.0408219676698792
0.00322972156525653 0.0387104545445669
0.00698383215913619 0.0363297262510094
0.0104878876693235 0.0337153614197099
0.0137203284498807 0.0309034164407077
0.0166632014058949 0.027930116174397
0.0193021818904458 0.0248314407665749
0.0216265057250144 0.0216428457900281
0.0236289189159375 0.0183989378658249
0.0253055724205083 0.0151332205985254
0.0266559066689585 0.0118778210375273
0.02768249697004 0.00866325694340173
0.0283908765637439 0.00551823968443439
0.0287893503603265 0.00246948518887156
0.0288887956401881 -0.000458441002753926
0.0287024254997433 -0.00324324817135897
0.0282455709232268 -0.00586502795744892
0.027535429326037 -0.00830632854027768
0.026590809372124 -0.0105522119523867
0.0254319018680117 -0.0125902779451056
0.0240799985020682 -0.014410670996429
0.0225572478366065 -0.0160060638184944
0.020886424338161 -0.017371618583699
0.0190906489788756 -0.0185049295503987
0.0171931694418448 -0.0194059276454828
0.0152171207698711 -0.020076796918857
0.0131853204712944 -0.0205218373564641
0.0111200524515847 -0.0207473553077486
0.0090428807455338 -0.0207614890665888
0.00697446045641862 -0.0205740677921079
0.00493439386338661 -0.0201964277726574
0.00294107954351965 -0.0196412324946441
0.00101159339167783 -0.0189222740868918
-0.000838420231232325 -0.01805431382036
-0.00259483034346625 -0.0170528521918245
-0.0042450866340158 -0.0159339675794919
-0.00577826743079864 -0.0147141151619272
-0.00718510845982325 -0.0134099406372933
-0.00845801018379415 -0.0120381153337564
-0.0095910345468108 -0.0106151712967675
-0.0105798891465213 -0.00915733178122636
-0.0114218699613208 -0.00768038250128846
-0.0121158366743519 -0.00619952482223503
-0.0126621316514661 -0.00472926879438117
-0.0130625054384305 -0.00328331710444797
-0.0133200348072071 -0.0018744731725546
-0.0134390333509589 -0.000514563138760395
-0.0134249406584718 0.000785631880188264
-0.0132842226639545 0.00201642797453561
-0.0130242561640078 0.0031692775977005
-0.0126532133343478 0.0042368006806635
-0.0121799443832408 0.00521279078721276
-0.0116138695183155 0.00609222525533532
-0.0109648466982847 0.00687125341831554
-0.0102430552170126 0.00754717367772005
-0.00945889698266962 0.00811840802313765
-0.0086228773071594 0.00858446224285499
-0.00774549174928579 0.00894587306707921
-0.00683713717192089 0.00920416004483338
-0.00590801255464 0.00936175925693643
-0.00496802818780531 0.00942195758540515
-0.00402672790551244 0.0093888213254963
-0.00309321318041546 0.00926711191239
-0.00217607560122709 0.00906221732604397
-0.00128334203877909 0.00878006408006383
-0.000422422373383035 0.00842703662858418
0.000399931223277063 0.00800989764219476
0.00117765796366853 0.00753569814801625
0.00190541376661651 0.00701170200171836
0.00257858715007984 0.00644530201974351
0.00319331096171092 0.0058439509391034
0.00374646217715412 0.00521507800347591
0.00423565619726028 0.0045660254807805
0.00465923579030777 0.00390397961512792
0.00501625246689399 0.00323591198940864
0.00530644063716661 0.00256852067299405
0.00553019176774472 0.00190818178479207
0.00568851247326772 0.00126090185956265
0.00578299378369779 0.000632277583221028
0.0058157613192645 2.74629731598017e-05
0.00578943570992008 -0.000548859927285192
0.00570707764776946 -0.00109250357028334
0.00557214551225802 -0.00159979243846421
0.00538843483439114 -0.00206757274304901
0.00516003405902962 -0.00249321966198587
0.00489126494017392 -0.00287463712171991
0.00458663131811956 -0.00321025362730655
0.00425077301871133 -0.003499012772493
0.0038884064811634 -0.00374035841230411
0.00350428145107728 -0.0039342165993122
0.00310313092137454 -0.00408097472528882
0.00268962666095497 -0.00418145465127049
0.00226833893441109 -0.0042368867479724
0.00184369447529557 -0.00424887862457982
0.00141994330690283 -0.00421937711542043
0.00100112463171479 -0.00415063632289344
0.000591037261258447 -0.00404518748010194
0.000193216390004797 -0.00390578797742794
-0.000189089513708945 -0.00373539587880151
-0.000552935763552627 -0.00353712775255348
-0.00089569571699382 -0.00331421997167755
-0.00121507096253034 -0.00306999280361551
-0.00150909778165114 -0.0028078138052163
-0.00177614965258594 -0.00253106352787182
-0.00201493800781692 -0.00224310238515401
-0.00222450734550629 -0.00194723660083356
-0.00240423022418405 -0.00164669422012924
-0.00255379527281427 -0.00134459233289906
-0.00267319683035301 -0.00104391505885066
-0.00276272097649422 -0.000747490264780555
-0.00282292597436624 -0.000457969955130422
-0.00285462760263542 -0.000177813100047254
-0.00285887633844492 9.07287829478298e-05
-0.00283693733427475 0.000345623626384614
-0.00279026736791549 0.000585067604643878
-0.00272049155957066 0.00080749207120686
-0.00262938032168993 0.0010115667105753
-0.00251882537744825 0.00119620137224664
-0.00239081531349087 0.00136054505977693
-0.00224741276244281 0.00150398274709086
-0.00209072809289421 0.00162612970473477
-0.0019229008991781 0.00172682443593009
-0.00174607567033335 0.0018061198761635
-0.0015623809514696 0.00186427146109331
-0.00137391083343464 0.00190172635934835
-0.00118270457979225 0.00191910933820217
-0.000990731376052707 0.00191720886632875
-0.000799873914693128 0.00189696031755512
-0.00061191483239815 0.00185943137751311
-0.000428523787548074 0.00180580501291919
-0.000251247186139375 0.00173736314256373
-8.14991591536113e-05 0.00165546809967097
7.94459684350497e-05 0.00156154768965615
0.000230458996858307 0.00145707642559068
0.000370559984633795 0.00134356115997617
0.000498920591867769 0.00122252312927094
0.000614864684508952 0.00109548440319003
0.000717867687156066 0.000963951718335833
0.000807554356950024 0.000829403273896155
0.000883695495130918 0.000693276740613903
0.000946203057903445 0.000556956225836756
0.000995123986673531 0.000421761729422876
0.00103063403826324 0.000288940254225559
0.00105302969425376 0.000159656374318112
0.00106271896434225 3.4985418064043e-05
0.00106021288816768 -8.40926912713189e-05
0.00104611575653444 -0.000196698324743685
0.00102111428487492 -0.000302055964745571
0.000985967485165989 -0.000399496548962923
0.000941496654246641 -0.000488459009544202
0.00088857274274775 -0.000568490449400612
0.0008281069836371 -0.000639245360804515
0.000761040007346363 -0.000700484120182525
0.000688331306099536 -0.000752069803785907
0.000610948581822125 -0.000793964771321147
0.000529858723860401 -0.000826226901207913
0.000446018728433965 -0.000849003567546892
0.000360365890520573 -0.000862526717435627
0.000273810760558743 -0.000867105978421476
0.000187229300824064 -0.000863122924309123
0.000101456009443975 -0.00085102285080571
1.72778157052435e-05 -0.000831308172736064
-6.45709769197744e-05 -0.000804531010161653
-0.000143413456725214 -0.000771284730088355
-0.000218633909278552 -0.000732197172420034
-0.000289680720722435 -0.000687922248833538
-0.000356068568022077 -0.000639132587265577
-0.000417380216292881 -0.000586512929480414
-0.000473267071969257 -0.000530751730180107
-0.00052344937214179 -0.000472534903036788
-0.000567715457106005 -0.000412539766892789
-0.00060592063547673 -0.000351428210000074
-0.000637985670917476 -0.000289841593445535
-0.00066389407561793 -0.000228395117176552
-0.000683689316430927 -0.000167673533546533
-0.000697471729976535 -0.000108226629111231
-0.000705394622807569 -5.05658570324266e-05
-0.00070766037157574 4.83889397479009e-06
-0.000704516464969025 5.75618073138315e-05
-0.000696250323277376 0.000107223151766159
-0.000683184932850091 0.000153490683048756
-0.000665674829790731 0.000196080674146414
-0.000644099406082603 0.000234758316079317
-0.000618859824578823 0.000269337613213926
-0.000590373198217868 0.000299680717597776
-0.000559068049805673 0.000325697307345461
-0.000525379538945839 0.00034734281966517
-0.000489745271047211 0.000364616974774697
-0.000452600669757884 0.000377561575443316
-0.000414374785951832 0.000386257958252416
-0.000375486950726763 0.000390824677648061
-0.000336342642580004 0.000391414116874024
-0.000297330722469933 0.000388209796275872
-0.000258820261423457 0.000381423070495088
-0.000221157862890619 0.000371289596429215
-0.000184665508981885 0.000358066002162739
-0.000149638683186602 0.000342026586047879
-0.000116344653157536 0.000323459609324804
-8.50212700917967e-05 0.000302663820889039
-5.58761901245661e-05 0.000279945242538188
-2.90862030412498e-05 0.000255613954607756
-4.79702801940138e-06 0.000229980837096973
1.68765986880176e-05 0.000203354253879393
3.58505572854344e-05 0.000176037648915439
5.20707014882486e-05 0.000148326692789816
6.55119622805301e-05 0.000120506690858682
7.61771815404205e-05 9.28504982361938e-05
8.40958024133673e-05 6.56164116021041e-05
8.93222577354832e-05 3.90463597933557e-05
9.19343220627874e-05 1.33643889340049e-05
9.20312126779074e-05 -1.12246418346104e-05
8.97316178305859e-05 -3.45361358472379e-05
8.51716376600468e-05 -5.64065610709832e-05
7.85026669050289e-05 -7.66940485604009e-05
6.98891684662498e-05 -9.52786578614015e-05
5.95065415538009e-05 -0.000112062574706022
4.75388006526857e-05 -0.000126969955397474
3.41764836758652e-05 -0.000139946626705877
1.96145037224658e-05 -0.000150959477771329
4.05003357961393e-06 -0.000159995989883317
-1.23194860951245e-05 -0.000167063222701075
-2.92982603776696e-05 -0.000172186830155893
-4.66939409032135e-05 -0.000175409916124109
-6.431932301412e-05 -0.000176791920103871
-8.1993864652713e-05 -0.000176407038400175
-9.95451852391381e-05 -0.00017434308065712
-0.000116810257152574 -0.000170699688616549
-0.000133636573553106 -0.000165587119903783
-0.000149883108852133 -0.000159124437850329
-0.000165421097277026 -0.000151438020094402
-0.000180134745953405 -0.000142660023771071
-0.00019392166422328 -0.000132926835792198
-0.000206693314794136 -0.000122377531015773
-0.000218375057427449 -0.000111152459988544
-0.00022890639635909 -9.93917503972139e-05
-0.000238240616530934 -8.72340614974446e-05
-0.000246344870934968 -7.4815273692283e-05
-0.00025319974408545 -6.22672684521403e-05
-0.000258798669965924 -4.9716932590739e-05
-0.000263147553704294 -3.72851409657232e-05
-0.000266263825719454 -2.50858784819064e-05
-0.000268176179805132 -1.32254770502244e-05
-0.000268923583615845 -1.80194051907501e-06
-0.000268554376461081 9.09560664589387e-06
-0.000267124988746106 1.93873294771219e-05
-0.000264699709149548 2.90030146732762e-05
-0.000261349287644186 3.78823052288313e-05
-0.000257149829553526 4.59747966077562e-05
-0.000252182242578867 5.32400413285269e-05
-0.000246530810709095 5.96474894516141e-05
-0.000240282422964501 6.51762857969487e-05
-0.000233525569307645 6.98150457961455e-05
-0.000226349467519108 7.35614571892376e-05
-0.000218843088209783 7.642191811396e-05
-0.000211094427212076 7.84110449561712e-05
-0.00020318951603771 7.95511654345035e-05
-0.000195211839784087 7.98716671746164e-05
-0.00018724160952521 7.94084546856255e-05
-0.000179355165666392 7.82032687769788e-05
-0.00017162439584994 7.63029843392909e-05
-0.000164116327485576 7.37589659790261e-05
-0.000156892560207034 7.0626285962376e-05
-0.000150009076680395 6.69631091142486e-05
-0.000143515922444367 6.2829881433718e-05
-0.000137457016718168 5.82887369083365e-05
-0.000131869977763301 5.34027875243315e-05
-0.00012678613741716 4.82354211583449e-05
-0.00012223046832028 4.2849758518218e-05
-0.0001182217003162 3.73079977591187e-05
-0.000114772364093683 3.16708787689857e-05
-0.000111889074936599 2.59971636076411e-05
-0.000109572627300858 2.03432020530817e-05
-0.000107818344048852 1.47624482328898e-05
-0.000106616374755135 9.30510672621232e-06
-0.000105952015841077 4.01782118992361e-06
-0.000105806067089757 -1.0566240868301e-06
-0.000106155304577881 -5.87953055135315e-06
-0.000106972793537941 -1.0416456823488e-05
-0.000108228404948212 -1.46373528194521e-05
-0.000109889222984602 -1.85166380153728e-05
-0.000111920003405488 -2.20332348330188e-05
-0.000114283610109753 -2.51705537538394e-05
-0.000116941437143246 -2.79164571271445e-05
-0.00011985394712327 -3.02631352985874e-05
-0.000122980998659245 -3.22069943503381e-05
-0.000126282312018291 -3.37484950756264e-05
-0.000129717789272925 -3.48919449090698e-05
-0.000133248038175071 -3.56452715723626e-05
-0.000136834554061357 -3.60197878766719e-05
-0.000140440200074033 -3.60298949584545e-05
-0.000144029323581586 -3.56928359553435e-05
-0.000147568192745145 -3.50283703826754e-05
-0.000151025156596855 -3.40584590927673e-05
-0.000154370863326292 -3.28069638620074e-05
-0.000157578362151462 -3.12993233106892e-05
-0.000160623394366094 -2.9562212735354e-05
-0.000163484437001952 -2.76232671159726e-05
-0.000166142630077174 -2.55107461858903e-05
-0.000168582111298341 -2.32532249928724e-05
-0.000170789754132176 -2.08793277378522e-05
-0.000172755400643834 -1.84174255376188e-05
-0.000174471614119987 -1.58953992627844e-05
-0.000175933751834973 -1.33403689139625e-05
-0.000177139819536539 -1.07784899642457e-05
-0.000178090413243514 -8.23473842002237e-06
-0.00017878853007525 -5.73272569582423e-06
-0.000179239451840105 -3.29454157690229e-06
-0.000179450599519718 -9.4060938343743e-07
-0.000179431358648849 1.31043010692666e-06
-0.000179192861038737 3.44181078831135e-06
-0.000178747839259736 5.43871908367105e-06
-0.00017811037925976 7.28833376507226e-06
-0.00017729580394971 8.97986741542345e-06
-0.000176320323957455 1.05045630308734e-05
-0.000175201008523507 1.18556832056776e-05
-0.000173955465358345 1.30284870524938e-05
-0.000172601695121582 1.40201659654532e-05
-0.000171157844038109 1.48297993158852e-05
-0.000169642102032229 1.54582539921636e-05
-0.000168072498998945 1.59081038364831e-05
-0.000166466628313934 1.61835030452265e-05
-0.000164841792351488 1.62901191075593e-05
-0.00016321443495499 1.62349446021018e-05
-0.000161600286953577 1.60262067433123e-05
-0.000160014351606765 1.56732134612217e-05
-0.000158470482595369 1.5186228600951e-05
-0.000156981573192916 1.45763089107465e-05
-0.000155559308879333 1.3855170188197e-05
-0.000154214181889322 1.30350370143029e-05
-0.000152955520313011 1.2128512419475e-05
-0.000151791269813431 1.11484249419036e-05
-0.000150728182798454 1.01077037067895e-05
-0.000149771643794407 9.01924632216305e-06
-0.000148925829514247 7.8957948566466e-06
-0.000148193577887544 6.74982361813237e-06
-0.000147576548128991 5.59343325348682e-06
-0.000147075191631962 4.43824304078438e-06
-0.000146688824726192 3.29531032408625e-06
-0.000146415715987182 2.1750481646321e-06
-0.00014625308623467 1.0871574351104e-06
-0.000146197239498446 4.05680999140956e-08
-0.000146243650328475 -9.56616958348866e-07
-0.000146386992898027 -1.89715397129475e-06
-0.000146621330178003 -2.77468517440038e-06
-0.000146940070280568 -3.5837614177428e-06
-0.00014733608287431 -4.31985276602015e-06
-0.000147801873807275 -4.97935066923888e-06
-0.000148329686970693 -5.55955489804638e-06
-0.00014891141698796 -6.0586535135243e-06
-0.000149538987565155 -6.47570232550909e-06
-0.000150204191420627 -6.8105913698796e-06
-0.000150898733941773 -7.06400714405725e-06
-0.000151614640639987 -7.23738558202486e-06
-0.00015234400976914 -7.33286360170282e-06
-0.000153079172398097 -7.35322391715726e-06
-0.000153812736067756 -7.30184300160724e-06
-0.000154537715759871 -7.18262728693214e-06
-0.000155247533898543 -6.99995616382926e-06
-0.000155936093111502 -6.75860638012227e-06
-0.000156597834439581 -6.46368828560728e-06
-0.000157227620922528 -6.12058921369701e-06
-0.000157820897672072 -5.73489975919106e-06
-0.000158373750080902 -5.31235674408603e-06
-0.000158882700097355 -4.85878326200728e-06
-0.00015934501181742 -4.38001536918337e-06
-0.000159758400447457 -3.88185976717831e-06
-0.000160121265136461 -3.37003000980274e-06
-0.000160432499802102 -2.85010212466852e-06
-0.000160691522235839 -2.32746626742386e-06
-0.000160898390519392 -1.80728022901311e-06
-0.000161053570194957 -1.29443007042263e-06
-0.000161158021577369 -7.93502943928492e-07
-0.000161213156099341 -3.0874846624479e-07
-0.000161220792656034 1.55937533156958e-07
-0.000161183128501893 5.97040362662615e-07
-0.00016110266649126 1.01143453121871e-06
-0.000160982156871163 1.39640372556066e-06
-0.000160824757352509 1.7496435105388e-06
-0.000160633683863943 2.06926148369618e-06
-0.000160412414279018 2.35378538380321e-06
-0.000160164426480988 2.602142780396e-06
-0.00015989356216122 2.81366937344985e-06
-0.000159603313774134 2.98808059601835e-06
-0.00015929746482164 3.12545929520569e-06
-0.00015897975515854 3.22624493243745e-06
-0.00015865380823257 3.29121592396869e-06
-0.000158323101979553 3.32145119169569e-06
-0.000157991056134501 3.31831068611788e-06
-0.000157660915815682 3.28341277148342e-06
-0.00015733582428349 3.21860526403261e-06
-0.000157018502797326 3.12593061520955e-06
-0.000156711745380223 3.00759735678141e-06
-0.000156418055020617 2.8659692593927e-06
-0.000156139643671168 2.70352100489174e-06
-0.000155878359488469 2.5228083141704e-06
-0.000155635934214777 2.32643127839882e-06
-0.000155413866762573 2.11702778785128e-06
-0.000155213234038445 1.89723239755329e-06
-0.000155034996532954 1.66965206403746e-06
-0.000154879852801003 1.43685032780172e-06
-0.000154748064837856 1.20131136249063e-06
-0.000154639938292475 9.65433802221916e-07
-0.000154555269493829 7.31505238625585e-07
-0.000154493811111766 5.01677515321597e-07
-0.000154455112086096 2.77972835624474e-07
-0.000154438270242984 6.22486225412833e-08
-0.000154442587131523 -1.4380063619035e-07
-0.000154467029602515 -3.38648198740243e-07
-0.000154510258911808 -5.2095372884281e-07
-0.000154571081830025 -6.89560018210522e-07
-0.000154648086844504 -8.43491754033698e-07
-0.000154739658710967 -9.81966268992496e-07
-0.000154844240388078 -1.10439415795111e-06
-0.000154960303934174 -1.21035784649004e-06
-0.000155086117676323 -1.29961832162628e-06
-0.000155220037248856 -1.37211094530798e-06
-0.000155360403730227 -1.42793273017611e-06
-0.000155505543643123 -1.46733837110002e-06
-0.00015565382716246 -1.4907280094234e-06
-0.000155803653563667 -1.4986375598755e-06
-0.000155953538534467 -1.49172904925776e-06
-0.000156101997759924 -1.47077416450675e-06
-0.000156247677889957 -1.43664439538477e-06
-0.000156389356539751 -1.3902942962718e-06
-0.000156525811322754 -1.33275049182813e-06
-0.000156655979922057 -1.26510013911951e-06
-0.000156778916434992 -1.18847760176982e-06
-0.000156893762269683 -1.10404784173929e-06
-0.000156999804352982 -1.0129959746169e-06
-0.000157096489682674 -9.16515076519742e-07
-0.000157183381672325 -8.15783736229925e-07
-0.000157259985527982 -7.11972101274938e-07
-0.000157326082942725 -6.06229758712273e-07
-0.00015738152837017 -4.99668460496316e-07
-0.000157426307232359 -3.93354665714774e-07
-0.00015746056502384 -2.88298337175474e-07
-0.000157484432688869 -1.85443708736188e-07
-0.000157498128484554 -8.56801503079652e-08
-0.000157502030741016 1.01792030568482e-08
-0.000157496546894049 1.01395539658933e-07
-0.000157482171692889 1.8730866898492e-07
-0.000157459574511975 2.67345834935317e-07
-0.000157429322864563 3.41025923049354e-07
-0.000157392027921424 4.07941134615564e-07
-0.000157348402718879 4.67768733476703e-07
-0.000157299116639529 5.20269706774656e-07
-0.000157244940931333 5.65283321561638e-07
-0.000157186617740454 6.02731884201402e-07
-0.000157124932870671 6.32613952160355e-07
-0.000157060643023707 6.55001851104786e-07
-0.000156994504903057 6.70038493327807e-07
-0.000156927173350186 6.7792768082553e-07
-0.000156859390519541 6.78931122849447e-07
-0.000156791854911146 6.73365972078677e-07
-0.000156725206818593 6.61600294937781e-07
-0.00015666002832875 6.44042443070925e-07
-0.000156596886977485 6.21138101841723e-07
-0.000156536262989841 5.93362610643022e-07
-0.000156478665695263 5.61213476496514e-07
-0.000156424473456389 5.25208812433842e-07
-0.000156374079188103 4.85879625887475e-07
-0.000156327759390079 4.43764178945094e-07
-0.000156285776010069 3.99400962226848e-07
-0.000156248361891898 3.53324848496872e-07
-0.000156215618911903 3.06063485146224e-07
-0.000156187648946043 2.58127884199266e-07
-0.00015616437924665 2.10007245725341e-07
-0.000156145882584633 1.62164964172262e-07
-0.000156132158970971 1.15049838232684e-07
-0.000156123106552451 6.90818357240719e-08
-0.000156118594371252 2.46489063118749e-08
-0.000156118447813097 -1.7889392800452e-08
-0.000156122448606871 -5.82160321685454e-08
-0.000156130363928755 -9.60473616820612e-08
-0.00015614194640208 -1.31136947599531e-07
-0.000156156890441548 -1.6327658731996e-07
-0.000156174934116735 -1.92295876312587e-07
-0.000156195699080866 -2.180628568757e-07
-0.000156218879745838 -2.40484725785861e-07
-0.000156244126866896 -2.59504764996143e-07
-0.000156271105750337 -2.75101667557287e-07
-0.000156299496253555 -2.87288182951317e-07
-0.000156328920025493 -2.96108393346706e-07
-0.000156359056922006 -3.01637836180868e-07
-0.000156389586798281 -3.03979996424397e-07
-0.000156420233164645 -3.03262794508485e-07
-0.000156450646771252 -2.99638472978092e-07
-0.000156480536575415 -2.93280662040651e-07
-0.000156509669741668 -2.84381662545019e-07
-0.000156537798882282 -2.73148029659998e-07
-0.000156564691161161 -2.59798655144472e-07
-0.000156590157397762 -2.44560577102038e-07
-0.000156614008411233 -2.27673277911067e-07
-0.000156636084124568 -2.09377380148978e-07
-0.000156656268116405 -1.89917124186756e-07
-0.000156674443965437 -1.69535510942398e-07
-0.000156690553458104 -1.48473172194297e-07
-0.00015670452382907 -1.26963831496851e-07
-0.000156716311416935 -1.05238278903796e-07
-0.000156725916216317 -8.35170132842955e-08
-0.000156733367325932 -6.2009559903542e-08
-0.00015673867929297 -4.09107425644595e-08
-0.00015674191032058 -2.04055370933709e-08
-0.000156743118612309 -6.64106311609736e-10
-0.000156742391475961 1.81610369381913e-08
-0.000156739830771576 3.59301617069985e-08
-0.000156735552911629 5.25236694137732e-08
-0.000156729659756974 6.78357726935364e-08
-0.000156722311376702 8.1781372784917e-08
-0.000156713638736373 9.42899767639171e-08
-0.000156703787353973 1.0531008950293e-07
-0.000156692902747848 1.14806172700488e-07
-0.00015668114498868 1.22759202920986e-07
-0.000156668659595592 1.29164523660075e-07
-0.000156655621191959 1.34035128419863e-07
-0.00015664217529765 1.37397134288009e-07
-0.000156628438329006 1.39289558345745e-07
-0.000156614614014173 1.39763631834544e-07
-0.000156600789666283 1.38883713779459e-07
-0.000156587125358184 1.36720273803681e-07
-0.0001565737375073 1.33356449494304e-07
-0.000156560742531197 1.28882058351987e-07
-0.000156548256847601 1.23393025047713e-07
-0.000156536353218591 1.16990029275232e-07
-0.000156525148062109 1.09778388414361e-07
-0.000156514699588491 1.01866478863233e-07
-0.000156505066008139 9.33648234141549e-08
-0.000156496320083298 8.43820273585538e-08
-0.000156488490920541 7.50287269812855e-08
-0.000156481607626305 6.5411948940719e-08
-0.000156475684755087 5.56365639392542e-08
-0.00015647076596512 4.58037102690767e-08
-0.000156466836706922 3.60136277743894e-08
-0.000156463882430818 2.63577277018201e-08
-0.00015646187403509 1.69233535241009e-08
-0.000156460796969747 7.78958775260463e-09
-0.000156460607580822 -9.69573650533295e-10
-0.000156461291318011 -9.28817317502606e-09
-0.000156462789975093 -1.71057904022054e-08
-0.00015646504534567 -2.43699258342667e-08
-0.000156467984671188 -3.10371281453392e-08
-0.000156471564296726 -3.70725460330235e-08
-0.000156475711463355 -4.24481138155963e-08
-0.000156480382515838 -4.71424462245018e-08
-0.000156485475591021 -5.11427461560854e-08
-0.000156490932481312 -5.44449339431874e-08
-0.000156496680427111 -5.70493455948062e-08
-0.000156502661220482 -5.89649062632258e-08
-0.000156508787549576 -6.02050727535608e-08
-0.000156515044861984 -6.07899822910318e-08
-0.000156521302189785 -6.07443944589114e-08
-0.000156527559532248 -6.00984030596496e-08
-0.0001565336713693 -5.88869522727409e-08
-0.000156539666803818 -5.71495283180345e-08
-0.000156545443971326 -5.49278670741726e-08
-0.000156550988318841 -5.22652962992032e-08
-0.000156556241637494 -4.92100046128874e-08
-0.000156561174822281 -4.58096189315249e-08
-0.000156565758768183 -4.21123323157691e-08
-0.000156569949818184 -3.81685941255872e-08
-0.000156573733419155 -3.40286387540134e-08
-0.000156577095017968 -2.97415629971209e-08
-0.000156580020061514 -2.53557864288156e-08
-0.000156582508548643 -2.09184862556833e-08
-0.000156584545926333 -1.64744609065792e-08
-0.000156586132193529 -1.20672687328738e-08
-0.000156587281901141 -7.73820457017349e-09
-0.000156588009600173 -3.52483014304239e-09
-0.000156588315289766 5.37669297973054e-10
-0.000156588228072995 4.4174992136492e-09
-0.000156587762501054 8.08547213904109e-09
-0.00015658693312526 1.15160146627047e-08
-0.000156585783600859 1.4688421305642e-08
-0.000156584313927395 1.75835704122052e-08
-0.000156582582312199 2.01869756119577e-08
-0.000156580603306893 2.24864169090511e-08
-0.000156578406015181 2.44757804718221e-08
-0.00015657601954076 2.61492946601605e-08
-0.000156573487539384 2.75065026034138e-08
-0.000156570853666879 2.85493206020337e-08
-0.000156568088819504 2.92827331480061e-08
-0.000156565323964758 2.97139629082399e-08
-0.000156562559102992 2.98579456159409e-08
-0.000156559794234555 2.9728709154131e-08
-0.000156557029359777 2.93399437731323e-08
-0.00015655426447898 2.87044310751106e-08
-0.000156551601455934 2.78356265606683e-08
-0.000156549011187356 2.6756044761711e-08
-0.000156546551881393 2.54846868608105e-08
-0.000156544223538608 2.40439504139989e-08
-0.00015654205526334 2.24551069544221e-08
-0.000156540061608077 2.07404374855114e-08
-0.000156538242573386 1.89234758904422e-08
-0.000156536598159819 1.702673500803e-08
-0.000156535157471723 1.50712573462886e-08
-0.000156533905957738 1.3079441703312e-08
-0.000156532843618349 1.10713137546625e-08
-0.00015653201410982 9.06757435109595e-09
-0.000156531359224958 7.08779793190395e-09
-0.00015653089351608 5.14861603351235e-09
-0.000156530646087441 3.26722395666001e-09
-0.000156530573283679 1.45946142671161e-09
-0.000156530675105129 -2.60414044495061e-10
-0.000156530937000168 -1.88052361876911e-09
-0.000156531358969047 -3.39034484514444e-09
-0.000156531926460073 -4.78048570867751e-09
-0.000156532639473455 -6.04246137153597e-09
-0.000156533468905463 -7.17140360290136e-09
-0.000156534400204313 -8.16188113622607e-09
-0.000156535418818185 -9.00982048690491e-09
-0.000156536524747024 -9.71691576506784e-09
-0.0001565376888871 -1.0279094186938e-08
-0.000156538853030577 -1.07018903530709e-08
-0.000156540148144705 -1.0987355185399e-08
-0.000156541457814171 -1.11332151830901e-08
-0.000156542767486889 -1.11459163912309e-08
-0.000156544077162702 -1.10317936521942e-08
-0.000156545386841462 -1.07970703766558e-08
-0.000156546580107555 -1.04514637569442e-08
-0.00015654774427213 -1.00103678471464e-08
-0.000156548908438929 -9.47808506679415e-09
-0.000156549970744316 -8.86241325465109e-09
-0.000156550989395615 -8.17761009602735e-09
-0.000156551935288863 -7.42921913571282e-09
-0.000156552808423725 -6.6302477258473e-09
-0.00015655357969617 -5.7888405388673e-09
-0.000156554307313601 -4.91642915267931e-09
-0.000156554889412327 -4.02296015250547e-09
-0.000156555413303668 -3.11704044519967e-09
-0.000156555849883495 -2.20975078513153e-09
-0.000156556170047826 -1.30776864337712e-09
-0.000156556432004092 -4.20939297307577e-10
-0.000156556577544409 4.42938470623933e-10
-0.000156556650324396 1.27684067485756e-09
-0.00015655665034384 2.07319306166909e-09
-0.000156556548498828 2.82826023018101e-09
-0.000156556402996838 3.53412089870719e-09
-0.000156556170182103 4.19009688751304e-09
-0.000156555879158241 4.78747717164163e-09
-0.00015655555902916 5.32829189103801e-09
-0.00015655512248314 5.80576663133936e-09
-0.000156554685935535 6.21807515893691e-09
-0.000156554249386414 6.5684997996307e-09
-0.000156553725524284 6.85817920509368e-09
-0.000156553143452775 7.07896750246073e-09
-0.000156552561379647 7.23357278936687e-09
-0.000156551979304971 7.32470943620722e-09
-0.000156551397228825 7.35565887366452e-09
-0.000156550815151277 7.32913574968963e-09
-0.000156550233072382 7.24751662156686e-09
-0.000156549650992211 7.11362944938454e-09
-0.000156549068910831 6.93018920028265e-09
-0.000156548486828296 6.6994588418523e-09
-0.00015654805026404 6.43024856972207e-09
-0.000156547613699072 6.13162197404815e-09
-0.00015654717713343 5.80550419543302e-09
-0.000156546740567156 5.45325123252338e-09
-0.000156546362207973 5.07701024277107e-09
-0.000156546071160021 4.68785998908317e-09
-0.000156545780111838 4.28931998253113e-09
-0.000156545489063439 3.88195569439587e-09
-0.000156545314430304 3.47005437578707e-09
-0.000156545168901148 3.06335269650848e-09
-0.000156545023372127 2.6620810417155e-09
-0.000156544906947067 2.26601237773849e-09
-0.00015654490693775 1.88452400212702e-09
-0.000156544906928877 1.52113688312028e-09
-0.000156544906920424 1.17494613344205e-09
-0.000156544921464293 8.45385823844413e-10
-0.000156545066976037 5.39002391330978e-10
-0.000156545212488501 2.62260713146389e-10
-0.000156545358001645 1.31229402344779e-11
-0.000156545503515418 -2.10106515519115e-10
-0.000156545649029795 -4.0867325495908e-10
-0.000156545809096655 -5.8404740765905e-10
-0.000156546100131567 -7.28890975354446e-10
-0.000156546391167324 -8.39228818383386e-10
-0.000156546682203893 -9.163049000116e-10
-0.000156546973241233 -9.61816945532767e-10
-0.00015654726427931 -9.77121862588692e-10
-0.000156547555318091 -9.63577530266324e-10
-0.000156547846357537 -9.22767695588078e-10
-0.000156548137397624 -8.55824335010968e-10
-0.000156548428438324 -7.63651412938327e-10
-0.000156548719479604 -6.47720301005794e-10
-0.000156548952313729 -5.10289595301305e-10
-0.000156549097836563 -3.6255234925342e-10
-0.000156549243359564 -2.07913658512027e-10
-0.000156549388882731 -4.64868976646216e-11
-0.000156549534406051 1.21275559039624e-10
-0.000156549679929516 2.949206989733e-10
-0.00015654982545312 4.73995148686512e-10
-0.000156549970976819 6.57256929437189e-10
-0.000156550116500656 8.4617549078736e-10
-0.000156550145609151 1.0363496935617e-09
-0.000156550145613583 1.21781681960975e-09
-0.000156550145617802 1.3905726778396e-09
-0.000156550145621822 1.55518303096569e-09
-0.000156550145625651 1.71210061405969e-09
-0.000156550145629299 1.86143758046375e-09
-0.00015655014563277 2.0036474077112e-09
-0.000156550145636077 2.13906915791373e-09
-0.000156550145639228 2.2681555800208e-09
-0.000156550087434503 2.38909980687652e-09
-0.00015654994191782 2.49331306295675e-09
-0.000156549796400682 2.57874503695188e-09
-0.000156549650883102 2.64618930934102e-09
-0.000156549505365106 2.69654996248869e-09
-0.000156549359846707 2.73039302972622e-09
-0.000156549214327925 2.74851013476463e-09
-0.000156549068808781 2.75180690040289e-09
-0.000156548923289289 2.74096213087605e-09
-0.000156548777769472 2.71665394346865e-09
-0.000156548632249338 2.67944870457892e-09
-0.00015654848672891 2.63025155128327e-09
-0.000156548341208184 2.56872188797441e-09
-0.000156548195687201 2.49678481362148e-09
-0.000156548050165948 2.41364644243403e-09
-0.000156547933748283 2.32043843861884e-09
-0.000156547933746007 2.22732948751414e-09
-0.000156547933743852 2.13908482593617e-09
-0.000156547933741801 2.05502567046656e-09
-0.000156547933739844 1.97492699971491e-09
-0.00015654793373798 1.89856121102228e-09
-0.000156547933736207 1.82592891501132e-09
-0.000156547933734519 1.75680382047405e-09
-0.000156547933732914 1.69107289976766e-09
-0.000156547933731382 1.62839671608017e-09
-0.000156547933729926 1.56866147849044e-09
-0.000156547933728537 1.5118682972215e-09
-0.000156547933727215 1.45767696524413e-09
-0.000156547933725956 1.40608757970284e-09
-0.000156547933724755 1.3569877374553e-09
-0.000156547933723614 1.31026333533013e-09
-0.000156547933722525 1.26557476304301e-09
-0.000156547933721489 1.22314949835278e-09
-0.000156547933720502 1.18276072963441e-09
-0.000156547933719562 1.14429521413939e-09
-0.000156547933718665 1.10752638310396e-09
-0.000156547933717811 1.07256806214373e-09
-0.000156547933717 1.03930639788752e-09
-0.000156547933716222 1.00751599424465e-09
-0.000156547933715488 9.77422032200082e-10
-0.000156547933714787 9.48685852097952e-10
-0.000156547933714116 9.21194114045232e-10
-0.000156547933713478 8.95060053851537e-10
-0.000156548021024452 8.72425631737173e-10
-0.000156548166543462 8.63585071508854e-10
-0.000156548312062823 8.69226218780383e-10
-0.000156548443030605 8.88442666657774e-10
-0.000156548443031204 9.12992889623432e-10
-0.000156548443031773 9.36298462372864e-10
-0.000156548443032318 9.5858605775323e-10
-0.000156548443032834 9.79741995865702e-10
-0.000156548443033329 9.99992921801862e-10
-0.000156548443033796 1.01922635609153e-09
-0.000156548443034242 1.03744077217804e-09
-0.000156548443034668 1.05486327311999e-09
-0.000156548443035075 1.07149385197847e-09
-0.00015654844303546 1.08733300835384e-09
-0.000156548443035825 1.10226656274692e-09
-0.00015654844303618 1.11674750002955e-09
-0.00015654844303651 1.13032403575852e-09
-0.000156548443036829 1.14333416345591e-09
-0.000156548443037131 1.15577934722833e-09
-0.00015654844303742 1.16754491491511e-09
-0.000156548443037695 1.17885869121981e-09
-0.000156548443037955 1.18949301103344e-09
-0.000156548443038203 1.19967524803144e-09
-0.000156548443038445 1.20951758331156e-09
-0.000156548443038665 1.21856853774194e-09
-0.000156548443038885 1.22761959625572e-09
-0.000156548443039088 1.23587804573555e-09
-0.00015654844303928 1.24379762739268e-09
-0.000156548443039473 1.25171726456097e-09
-0.000156548443039646 1.25873111239683e-09
-0.000156548443039811 1.2655193351585e-09
-0.000156548443039976 1.2723075371035e-09
-0.000156548443040133 1.27864269866551e-09
-0.00015654844304027 1.28429951395947e-09
-0.000156548443040407 1.28995643333685e-09
-0.000156548443040546 1.2956132625086e-09
-0.000156548443040677 1.30093007894017e-09
-0.000156548443040787 1.30545558391093e-09
-0.000156548443040897 1.30998104030944e-09
-0.000156548443041007 1.31450647589126e-09
-0.000156548443041117 1.31903198086203e-09
-0.000156548443041224 1.32333065339107e-09
-0.000156548443041307 1.32672475089413e-09
-0.000156548443041389 1.33011885533607e-09
-0.000156548443041472 1.33351307773921e-09
-0.000156548443041554 1.33690710585332e-09
-0.000156548443041636 1.34030121029527e-09
-0.000156548443041719 1.34369529392053e-09
-0.000156548443041796 1.34674951052238e-09
-0.000156548443041851 1.34901213810767e-09
-0.000156548443041906 1.35127497385978e-09
-0.000156548443041961 1.35353769858959e-09
-0.000156548443042016 1.35580039556382e-09
-0.000156548443042071 1.35806323825483e-09
-0.000156548443042126 1.36032597686242e-09
-0.000156548443042181 1.36258863914218e-09
-0.000156548443042236 1.36485138468867e-09
-0.00015654844304229 1.36711406084622e-09
-0.000156548443042345 1.36926302934937e-09
-0.000156548443042373 1.37039456171717e-09
-0.000156548443042401 1.3715259553071e-09
-0.000156548443042428 1.37265731420255e-09
-0.000156548443042456 1.37378870779248e-09
-0.000156548443042483 1.37492012913798e-09
-0.000156548443042511 1.37605134925556e-09
-0.000156548443042538 1.37718281917332e-09
-0.000156548443042566 1.37831419888546e-09
-0.000156548443042593 1.37944551614755e-09
-0.000156548443042621 1.38057680565407e-09
-0.000156548443042648 1.38170822699957e-09
-0.000156548443042675 1.38283962752839e-09
-0.000156548443042703 1.38397098642384e-09
-0.000156548443042731 1.38510238695266e-09
-0.000156548443042758 1.38623372503144e-09
-0.000156548443042785 1.38736511168247e-09
-0.000156548443042813 1.38849641506678e-09
-0.000156548443042841 1.38962785722896e-09
-0.000156548443042868 1.39075920224663e-09
-0.000156548443042896 1.39189061665324e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
};
\addplot [very thick, learnedWithSideInfo, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131150103691391 0.0251356025722856
0.126968029637955 -0.0389804261332939
0.0957675894598062 -0.0816976800135551
0.0496518577121472 -0.0983119976459421
0.00166806992534072 -0.0898541185842259
-0.0371370056327868 -0.0631135958967026
-0.0600700498393938 -0.0280962719098358
-0.0654696369696904 0.00559551711088195
-0.0558866875201988 0.0309292179767128
-0.0365666577808287 0.0442227151578759
-0.0137321839008316 0.0452006162944087
0.00698383215913619 0.0363297262510094
0.0216265057250144 0.0216428457900281
0.0283908765637439 0.00551823968443439
0.027535429326037 -0.00830632854027768
0.020886424338161 -0.017371618583699
0.0111200524515847 -0.0207473553077486
0.00101159339167783 -0.0189222740868918
-0.00718510845982325 -0.0134099406372933
-0.0121158366743519 -0.00619952482223503
-0.0134249406584718 0.000785631880188264
-0.0116138695183155 0.00609222525533532
-0.00774549174928579 0.00894587306707921
-0.00309321318041546 0.00926711191239
0.00117765796366853 0.00753569814801625
0.00423565619726028 0.0045660254807805
0.00568851247326772 0.00126090185956265
0.00557214551225802 -0.00159979243846421
0.00425077301871133 -0.003499012772493
0.00226833893441109 -0.0042368867479724
0.000193216390004797 -0.00390578797742794
-0.00150909778165114 -0.0028078138052163
-0.00255379527281427 -0.00134459233289906
-0.00285887633844492 9.07287829478298e-05
-0.00251882537744825 0.00119620137224664
-0.00174607567033335 0.0018061198761635
-0.000799873914693128 0.00189696031755512
7.94459684350497e-05 0.00156154768965615
0.000717867687156066 0.000963951718335833
0.00103063403826324 0.000288940254225559
0.00102111428487492 -0.000302055964745571
0.000761040007346363 -0.000700484120182525
0.000360365890520573 -0.000862526717435627
-6.45709769197744e-05 -0.000804531010161653
-0.000417380216292881 -0.000586512929480414
-0.000637985670917476 -0.000289841593445535
-0.00070766037157574 4.83889397479009e-06
-0.000644099406082603 0.000234758316079317
-0.000489745271047211 0.000364616974774697
-0.000297330722469933 0.000388209796275872
-0.000116344653157536 0.000323459609324804
1.68765986880176e-05 0.000203354253879393
8.40958024133673e-05 6.56164116021041e-05
8.51716376600468e-05 -5.64065610709832e-05
3.41764836758652e-05 -0.000139946626705877
-4.66939409032135e-05 -0.000175409916124109
-0.000133636573553106 -0.000165587119903783
-0.000206693314794136 -0.000122377531015773
-0.00025319974408545 -6.22672684521403e-05
-0.000268923583615845 -1.80194051907501e-06
-0.000257149829553526 4.59747966077562e-05
-0.000226349467519108 7.35614571892376e-05
-0.00018724160952521 7.94084546856255e-05
-0.000150009076680395 6.69631091142486e-05
-0.00012223046832028 4.2849758518218e-05
-0.000107818344048852 1.47624482328898e-05
-0.000106972793537941 -1.0416456823488e-05
-0.000116941437143246 -2.79164571271445e-05
-0.000133248038175071 -3.56452715723626e-05
-0.000151025156596855 -3.40584590927673e-05
-0.000166142630077174 -2.55107461858903e-05
-0.000175933751834973 -1.33403689139625e-05
-0.000179450599519718 -9.4060938343743e-07
-0.00017729580394971 8.97986741542345e-06
-0.000171157844038109 1.48297993158852e-05
-0.00016321443495499 1.62349446021018e-05
-0.000155559308879333 1.3855170188197e-05
-0.000149771643794407 9.01924632216305e-06
-0.000146688824726192 3.29531032408625e-06
-0.000146386992898027 -1.89715397129475e-06
-0.000148329686970693 -5.55955489804638e-06
-0.000151614640639987 -7.23738558202486e-06
-0.000155247533898543 -6.99995616382926e-06
-0.000158373750080902 -5.31235674408603e-06
-0.000160432499802102 -2.85010212466852e-06
-0.000161213156099341 -3.0874846624479e-07
-0.000160824757352509 1.7496435105388e-06
-0.000159603313774134 2.98808059601835e-06
-0.000157991056134501 3.31831068611788e-06
-0.000156418055020617 2.8659692593927e-06
-0.000155213234038445 1.89723239755329e-06
-0.000154555269493829 7.31505238625585e-07
-0.000154467029602515 -3.38648198740243e-07
-0.000154844240388078 -1.10439415795111e-06
-0.000155505543643123 -1.46733837110002e-06
-0.000156247677889957 -1.43664439538477e-06
-0.000156893762269683 -1.10404784173929e-06
-0.000157326082942725 -6.06229758712273e-07
-0.000157498128484554 -8.56801503079652e-08
-0.000157429322864563 3.41025923049354e-07
-0.000157186617740454 6.02731884201402e-07
-0.000156859390519541 6.78931122849447e-07
-0.000156536262989841 5.93362610643022e-07
-0.000156285776010069 3.99400962226848e-07
-0.000156145882584633 1.62164964172262e-07
-0.000156122448606871 -5.82160321685454e-08
-0.000156195699080866 -2.180628568757e-07
-0.000156328920025493 -2.96108393346706e-07
-0.000156480536575415 -2.93280662040651e-07
-0.000156614008411233 -2.27673277911067e-07
-0.00015670452382907 -1.26963831496851e-07
-0.00015674191032058 -2.04055370933709e-08
-0.000156729659756974 6.78357726935364e-08
-0.00015668114498868 1.22759202920986e-07
-0.000156614614014173 1.39763631834544e-07
-0.000156548256847601 1.23393025047713e-07
-0.000156496320083298 8.43820273585538e-08
-0.000156466836706922 3.60136277743894e-08
-0.000156461291318011 -9.28817317502606e-09
-0.000156475711463355 -4.24481138155963e-08
-0.000156502661220482 -5.89649062632258e-08
-0.0001565336713693 -5.88869522727409e-08
-0.000156561174822281 -4.58096189315249e-08
-0.000156580020061514 -2.53557864288156e-08
-0.000156588009600173 -3.52483014304239e-09
-0.000156585783600859 1.4688421305642e-08
-0.00015657601954076 2.61492946601605e-08
-0.000156562559102992 2.98579456159409e-08
-0.000156549011187356 2.6756044761711e-08
-0.000156538242573386 1.89234758904422e-08
-0.00015653201410982 9.06757435109595e-09
-0.000156530675105129 -2.60414044495061e-10
-0.000156533468905463 -7.17140360290136e-09
-0.000156538853030577 -1.07018903530709e-08
-0.000156545386841462 -1.07970703766558e-08
-0.000156550989395615 -8.17761009602735e-09
-0.000156554889412327 -4.02296015250547e-09
-0.000156556577544409 4.42938470623933e-10
-0.000156556170182103 4.19009688751304e-09
-0.000156554249386414 6.5684997996307e-09
-0.000156551397228825 7.35565887366452e-09
-0.000156548486828296 6.6994588418523e-09
-0.000156546362207973 5.07701024277107e-09
-0.000156545168901148 3.06335269650848e-09
-0.000156544906920424 1.17494613344205e-09
-0.000156545503515418 -2.10106515519115e-10
-0.000156546682203893 -9.163049000116e-10
-0.000156548137397624 -8.55824335010968e-10
-0.000156549243359564 -2.07913658512027e-10
-0.000156549970976819 6.57256929437189e-10
-0.000156550145621822 1.55518303096569e-09
-0.000156550145639228 2.2681555800208e-09
-0.000156549505365106 2.69654996248869e-09
-0.000156548777769472 2.71665394346865e-09
-0.000156548050165948 2.41364644243403e-09
-0.000156547933739844 1.97492699971491e-09
-0.000156547933731382 1.62839671608017e-09
-0.000156547933724755 1.3569877374553e-09
-0.000156547933719562 1.14429521413939e-09
-0.000156547933715488 9.77422032200082e-10
-0.000156548166543462 8.63585071508854e-10
-0.000156548443032318 9.5858605775323e-10
-0.000156548443034668 1.05486327311999e-09
-0.00015654844303651 1.13032403575852e-09
-0.000156548443037955 1.18949301103344e-09
-0.000156548443039088 1.23587804573555e-09
-0.000156548443039976 1.2723075371035e-09
-0.000156548443040677 1.30093007894017e-09
-0.000156548443041224 1.32333065339107e-09
-0.000156548443041636 1.34030121029527e-09
-0.000156548443041961 1.35353769858959e-09
-0.000156548443042236 1.36485138468867e-09
-0.000156548443042428 1.37265731420255e-09
-0.000156548443042566 1.37831419888546e-09
-0.000156548443042703 1.38397098642384e-09
-0.000156548443042841 1.38962785722896e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
-0.000156548443042912 1.39245572711166e-09
};
\addplot [very thick, learnedWithoutSideInfo]
table {%
0.1 0.1
0.10967932420608 0.0853612655471494
0.117846078614853 0.0701550867044975
0.12454144799639 0.0545181662632341
0.129800347697544 0.0387601448532751
0.133528090222383 0.02343668743955
0.135477078256225 0.00936511961486453
0.135432661291088 -0.00255290932033247
0.133497284052023 -0.0117084821335345
0.130152468702303 -0.0180654901844322
0.126023624976199 -0.0220743564223311
0.121624347633132 -0.0243648581241587
0.117268406712279 -0.0255058654566693
0.113104689952105 -0.0259188668067045
0.109181086202137 -0.025885428204647
0.105493863100789 -0.0255834931024941
0.102016964146712 -0.025122130006682
0.0987171612634667 -0.0245669260401424
0.095561143475829 -0.023956682641292
0.0925184657742908 -0.0233138869997229
0.0895625203457153 -0.0226511468317252
0.0866706342875285 -0.0219751171771785
0.0838238313866047 -0.0212888975105847
0.0810065080732341 -0.0205935021841723
0.0782061319423626 -0.0198887702852439
0.075413002593975 -0.0191739361398406
0.0726200816442564 -0.0184479941713138
0.0698228829777925 -0.0177099389824851
0.067019406574695 -0.0169589294458561
0.0642100952985758 -0.0161944059030046
0.0613977920615434 -0.0154161773321486
0.0585876742325073 -0.0146244876138595
0.0557871430911563 -0.0138200650885283
0.0530056488733868 -0.0130041564569692
0.0502544368232574 -0.0121785441598985
0.0475462067695069 -0.0113455453744327
0.0448946878180521 -0.0105079905258938
0.0423141400636475 -0.00966917964477831
0.0398188055826627 -0.00883281593053598
0.0374223398604538 -0.00800291741349834
0.0351372606613425 -0.00718370946482416
0.0329744528954694 -0.00637950284518585
0.0309427646531342 -0.00559456369975386
0.0290487215260975 -0.00483298308489744
0.027296374787944 -0.00409855400101744
0.0256872858132411 -0.00339466338674521
0.0242206363945554 -0.00272420515712968
0.0228934442586364 -0.0020895183580949
0.0217008563583829 -0.00149235218874599
0.020636489875574 -0.000933857364801227
0.0196927919766865 -0.000414601363438738
0.0188613933242432 6.53963024257465e-05
0.0181334360032572 0.000506613412824208
0.0174998627481937 0.000909963811393411
0.0169516602478321 0.00127673020194941
0.0164800542756898 0.00160849498425719
0.0160766581668916 0.00190707239973875
0.0157335787111488 0.00217444446547921
0.0154434849936247 0.00241270241940583
0.015199646310128 0.00262399473544939
0.0149959452507202 0.00281048221969371
0.0148268716058304 0.00297430027222045
0.0146875020818937 0.00311752808541188
0.0145734700521047 0.0032421643334688
0.0144809288042866 0.00335010877107855
0.0144065110375768 0.00344314908526266
0.0143472867319656 0.00352295231688737
0.0143007209817458 0.00359106017520228
0.014264632943942 0.00364888759885496
0.0142371566992847 0.00369772396240231
0.0142167045453103 0.0037387363822563
0.0142019330269703 0.00377297463537651
0.0141917118489649 0.0038013772646277
0.0141850956947662 0.00382477850447094
0.0141812988922947 0.00384391571713172
0.0141796728069297 0.00385943708215164
0.0141796858039407 0.00387190933047332
0.0141809055987157 0.00388182535697812
0.0141829838013305 0.00388961158362289
0.0141856424583318 0.00389563497807277
0.0141886623973879 0.00390020966086224
0.0141918731869879 0.00390360305753434
0.0141951445334541 0.00390604157198604
0.0141983789489193 0.00390771577243143
0.0142015055365587 0.00390878509429538
0.0142044747524239 0.00390938207347791
0.014207254016338 0.00390961613072616
0.01420982405689 0.00390957693275062
0.0142121758878422 0.00390933735886012
0.0142143083247164 0.00390895610392805
0.0142162259609577 0.00390847994898191
0.014217937532969 0.00390794573075137
0.0142194546123533 0.00390738204046182
0.0142207905716432 0.00390681068094034
0.0142219597773643 0.00390624790946692
0.0142229769706685 0.00390570549172375
0.0142238568015909 0.00390519159038583
0.0142246134880604 0.00390471150967242
0.0142252605754338 0.0039042683152708
0.0142258107759909 0.00390386334691062
0.0142262758714327 0.00390349663912559
0.0142266666641868 0.00390316726380435
0.0142269929659165 0.00390287360661068
0.0142272636137326 0.00390261358779576
0.0142274865064196 0.00390238483649119
0.0142276686545033 0.00390218482639515
0.0142278162392828 0.0039020109796466
0.014227934676966 0.00390186074463905
0.0142280286850274 0.00390173165268948
0.0142281023484827 0.00390162135777405
0.0142281591845257 0.00390152766270102
0.0142282022042615 0.00390144853471863
0.0142282339708375 0.00390138211290081
0.0142282566534342 0.00390132670931598
0.0142282720768736 0.00390128080558139
0.0142282817667305 0.00390124304608097
0.0142282869900701 0.00390121222892903
0.0142282887919016 0.00390118729546973
0.0142282880275291 0.00390116731896617
0.0142282853911713 0.0039011514930003
0.0142282814410382 0.0039011391198942
0.0142282766212198 0.0039011295995075
0.0142282712806305 0.00390112241850282
0.0142282656893533 0.0039011171403236
0.0142282600526733 0.00390111339583576
0.0142282545229806 0.00390111087483014
0.0142282492099106 0.00390110931822862
0.0142282441888626 0.00390110851107828
0.0142282395081179 0.00390110827630341
0.0142282351947682 0.00390110846916336
0.014228231259636 0.00390110897234308
0.0142282277012615 0.00390110969165525
0.0142282245091825 0.00390111055231079
0.0142282216665701 0.0039011114956824
0.0142282191523053 0.00390111247649827
0.0142282169426475 0.00390111346046851
0.0142282150125173 0.00390111442223784
0.0142282133364571 0.00390111534368121
0.0142282118893844 0.00390111621246136
0.0142282106471088 0.00390111702078011
0.014228209586709 0.00390111776440127
0.0142282086867564 0.0039011184418194
0.0142282079274501 0.00390111905357227
0.0142282072907149 0.00390111960169914
0.0142282067601647 0.00390112008927712
0.0142282063210795 0.00390112052008629
0.014228205960336 0.00390112089832639
0.0142282056663197 0.00390112122841257
0.0142282054287914 0.00390112151478172
0.014228205238811 0.00390112176180057
0.0142282050885987 0.00390112197367021
0.0142282049714404 0.00390112215436123
0.014228204881555 0.00390112230757556
0.0142282048140068 0.00390112243671759
0.0142282047646054 0.00390112254489949
0.0142282047298039 0.00390112263495102
0.0142282047066264 0.00390112270939547
0.0142282046925954 0.00390112277048216
0.0142282046856548 0.00390112282020416
0.0142282046841089 0.00390112286031252
0.0142282046865811 0.00390112289233358
0.0142282046919529 0.00390112291761069
0.0142282046993154 0.0039011229372683
0.0142282047079685 0.00390112295230782
0.0142282047173627 0.00390112296356815
0.0142282047270665 0.00390112297175671
0.0142282047367552 0.00390112297748546
0.014228204746189 0.00390112298125889
0.0142282047552023 0.0039011229834931
0.0142282047636844 0.00390112298454026
0.0142282047715616 0.00390112298468459
0.0142282047787932 0.00390112298416545
0.0142282047853692 0.00390112298316048
0.0142282047913005 0.00390112298183132
0.0142282047966118 0.00390112298028811
0.0142282048013276 0.00390112297863032
0.0142282048054896 0.00390112297692902
0.0142282048091471 0.00390112297524503
0.0142282048123343 0.00390112297360146
0.014228204815093 0.00390112297204359
0.014228204817472 0.00390112297057721
0.014228204819509 0.00390112296921519
0.0142282048212476 0.00390112296797129
0.0142282048227136 0.00390112296683887
0.0142282048239486 0.00390112296581924
0.0142282048249842 0.00390112296491507
0.0142282048258493 0.00390112296410816
0.0142282048265545 0.00390112296339939
0.0142282048271407 0.00390112296278078
0.0142282048276194 0.00390112296223633
0.0142282048280054 0.00390112296176204
0.0142282048283122 0.00390112296135126
0.014228204828552 0.00390112296099998
0.0142282048287434 0.00390112296069711
0.0142282048288842 0.00390112296044487
0.0142282048289863 0.00390112296023526
0.014228204829061 0.00390112296006118
0.0142282048291156 0.00390112295991196
0.0142282048291493 0.00390112295978984
0.0142282048291671 0.00390112295969036
0.0142282048291746 0.00390112295960998
0.0142282048291746 0.00390112295954559
0.0142282048291671 0.00390112295949585
0.0142282048291538 0.00390112295945677
0.0142282048291431 0.00390112295942657
0.0142282048291302 0.00390112295940348
0.0142282048291107 0.00390112295938394
0.0142282048290947 0.00390112295937373
0.0142282048290778 0.00390112295936174
0.0142282048290601 0.00390112295935419
0.0142282048290405 0.00390112295935774
0.0142282048290241 0.00390112295935685
0.0142282048290099 0.00390112295935108
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
};
\addplot [very thick, learnedWithoutSideInfo, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.133528090222383 0.02343668743955
0.126023624976199 -0.0220743564223311
0.105493863100789 -0.0255834931024941
0.0895625203457153 -0.0226511468317252
0.075413002593975 -0.0191739361398406
0.0613977920615434 -0.0154161773321486
0.0475462067695069 -0.0113455453744327
0.0351372606613425 -0.00718370946482416
0.0256872858132411 -0.00339466338674521
0.0196927919766865 -0.000414601363438738
0.0164800542756898 0.00160849498425719
0.0149959452507202 0.00281048221969371
0.0144065110375768 0.00344314908526266
0.0142167045453103 0.0037387363822563
0.0141796728069297 0.00385943708215164
0.0141886623973879 0.00390020966086224
0.0142044747524239 0.00390938207347791
0.0142162259609577 0.00390847994898191
0.0142229769706685 0.00390570549172375
0.0142262758714327 0.00390349663912559
0.0142276686545033 0.00390218482639515
0.0142281591845257 0.00390152766270102
0.0142282817667305 0.00390124304608097
0.0142282814410382 0.0039011391198942
0.0142282545229806 0.00390111087483014
0.014228231259636 0.00390110897234308
0.0142282169426475 0.00390111346046851
0.014228209586709 0.00390111776440127
0.0142282063210795 0.00390112052008629
0.0142282050885987 0.00390112197367021
0.0142282047298039 0.00390112263495102
0.0142282046865811 0.00390112289233358
0.0142282047270665 0.00390112297175671
0.0142282047715616 0.00390112298468459
0.0142282048013276 0.00390112297863032
0.014228204817472 0.00390112297057721
0.0142282048249842 0.00390112296491507
0.0142282048280054 0.00390112296176204
0.0142282048289863 0.00390112296023526
0.0142282048291746 0.00390112295960998
0.0142282048291302 0.00390112295940348
0.0142282048290405 0.00390112295935774
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
0.014228204829005 0.00390112295934886
};

==> figures/smd_phase_plots/phase_plot_10_full_space_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
-0.0851167887449265 -0.0186469480395317
-0.0454825237393379 -0.0466751903295517
-0.0707155764102936 0.0543140470981598
0.0425342917442322 -0.0603686273097992
-0.0346308201551437 0.0210207104682922
0.0864222571253777 0.0394710972905159
-0.140851497650146 -0.0788728967308998
0.00558629212900996 -0.106390342116356
-0.110396720468998 0.0222673658281565
0.127625793218613 -0.132599860429764
};
\addplot [very thick, trueDynamics]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, approxDynamics, dashed]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, learnedWithSideInfo]
table {%
0.1 0.1
0.109298212332738 0.0858932882874477
0.117167928359414 0.0714627413978735
0.123586441875491 0.0569005084712115
0.128549782942737 0.0423883890689869
0.132071489995752 0.02809459702527
0.134181135077563 0.0141716256566531
0.134922804316429 0.000755069396633106
0.134353071662648 -0.0120366599980824
0.132539702674864 -0.0241020089711906
0.129559747251902 -0.0353555220273739
0.125498034612993 -0.0457268391117878
0.120445712922918 -0.0551596487228051
0.114498878288696 -0.0636106045225834
0.107757390006854 -0.0710484272898966
0.100323648554039 -0.0774529852837571
0.0923015673011908 -0.0828146113476468
0.0837955069832445 -0.087133384809145
0.0749093740979889 -0.0904186261790915
0.0657456522606472 -0.0926883300610257
0.0564046943449772 -0.0939687512825418
0.0469837501414803 -0.0942939139733632
0.0375763740097978 -0.0937051028136946
0.0282715941264075 -0.0922504334501136
0.0191533369252618 -0.0899842047130429
0.0102998012583958 -0.0869663230429857
0.00178296073530153 -0.0832615469835412
-0.00633191460963969 -0.0789387384862903
-0.0139865984678881 -0.0740699807229076
-0.0211301990541392 -0.0687295631334546
-0.0277193275585942 -0.0629931393143706
-0.0337181718502524 -0.05693670871757
-0.03909852024805 -0.0506356748699363
-0.0438396320985625 -0.0441640358164866
-0.0479280496881645 -0.0375935277043589
-0.0513573486889852 -0.0309930070157768
-0.0541278401763763 -0.0244278347318974
-0.0562461534314214 -0.0179594623981467
-0.0577248634416273 -0.0116450487994629
-0.0585820364360278 -0.00553720844181636
-0.058840775412335 0.000316175696405431
-0.0585287097762977 0.00587206921635005
-0.057677533402868 0.011092360247901
-0.0563225166147977 0.0159438887598892
-0.0545019697286986 0.020398459135851
-0.0522568109067203 0.0244328176908738
-0.0496300073477819 0.0280286231197147
-0.0466661319625935 0.0311723788048728
-0.0434108567207828 0.0338553758957931
-0.0399105056041794 0.0360735857957715
-0.0362115740342448 0.0378275411231307
-0.0323602743805124 0.0391221823499631
-0.0284021131343157 0.0399666764378538
-0.0243814718119292 0.0403742160226185
-0.0203412344233839 0.0403617292826177
-0.016322416807138 0.0399496115166069
-0.0123638220407959 0.0391614047632513
-0.0085017638387879 0.0380234140072674
-0.00476980717943878 0.0365643457518725
-0.00119854117662396 0.0348148949273852
0.00218459915405326 0.0328072982537952
0.00535545956108105 0.0305749293771146
0.00829326039339035 0.0281518455063184
0.0109806495785905 0.0255723776226434
0.0134036978597809 0.0228707096271518
0.0155518738942232 0.0200805118463859
0.0174179692942119 0.0172345691070385
0.0189980064385788 0.0143644730914093
0.0202910848170065 0.0115003277508299
0.0212992320300409 0.00867050762152777
0.0220272305737175 0.00590145365886435
0.0224823812930891 0.00321750259898674
0.0226743227130429 0.000640762648612512
0.022614783312655 -0.00180898348282667
0.0223173561493383 -0.00411433793074024
0.0217972492670084 -0.00626031753983369
0.0210710491412093 -0.00823435487760718
0.020156471084224 -0.0100262724229116
0.0190721431771538 -0.0116282478608561
0.0178373492220466 -0.0130347378197315
0.0164718368866448 -0.0142424067220266
0.0149955578611443 -0.0152500196019418
0.0134284918344731 -0.0160583432068209
0.0117904546371273 -0.0166700240070318
0.0101009073154156 -0.0170894587377457
0.00837878383188234 -0.0173226417120668
0.00664234763717792 -0.01737705488499
0.00490904963780677 -0.0172614678000947
0.00319539920426137 -0.0169858321569544
0.00151686253504582 -0.016561102214627
-0.000112235296431007 -0.0159990847503397
-0.00167878579792329 -0.015312287199762
-0.00317095850116051 -0.0145137500124431
-0.00457824954014393 -0.01361690682237
-0.00589150946360896 -0.0126354371177033
-0.00710296461582395 -0.0115831217610697
-0.00820622063250059 -0.0104737086376295
-0.0091962466119744 -0.00932077927705322
-0.0100693606824185 -0.0081376404313722
-0.0108231876297084 -0.00693720454244209
-0.0114566263037299 -0.00573188874735375
-0.0119697844280892 -0.00453352499803939
-0.0123639217912364 -0.00335327846490373
-0.0126413776052052 -0.00220157317823678
-0.0128054941384047 -0.00108803150786565
-0.0128605347603412 -2.14240085014449e-05
-0.0128115926727885 0.000990371443870076
-0.0126645033659917 0.00194039973169971
-0.0124257561433137 0.00282264994164087
-0.0121023860878432 0.00363206509700687
-0.0117018921058195 0.00436454257674453
-0.0112321335494796 0.00501692789900194
-0.0107012352216593 0.00558699968703378
-0.0101175035559358 0.00607344142963845
-0.00948932975827118 0.00647581184129115
-0.0088251087810844 0.00679450824844852
-0.00813315736561226 0.00703071980899903
-0.00742163115303296 0.00718637559248258
-0.00669846135323914 0.00726409221937767
-0.00597128396293011 0.00726711174169201
-0.00524738295343483 0.00719924094196876
-0.00453363532115847 0.0070647855143203
-0.00383646847791465 0.00686847961645072
-0.00316181205347543 0.00661542377296565
-0.00251507554200407 0.00631100933801238
-0.00190111547128555 0.00596085316718689
-0.00132421793892281 0.00557073552029308
-0.000788085513642532 0.00514652688115547
-0.000295832810057617 0.00469412771283713
0.000150015375581486 0.00421941150206328
0.000547517547719063 0.00372816314431914
0.000895304278863885 0.00322602987333387
0.00119256150527675 0.00271847192526275
0.00143901050485155 0.0022107173998139
0.00163488205404424 0.0017077233705449
0.0017808873250097 0.00121414243402616
0.00187818639619474 0.000734290999246505
0.00192835321201622 0.000272126345947353
0.00193333833060069 -0.000168774536653873
0.0018954306235777 -0.00058522870227203
0.00181721699672829 -0.000974458324718751
0.00170154222687785 -0.00133409613400323
0.00155146600472036 -0.00166218660894554
0.00137022475050791 -0.00195718272031624
0.00116118760893291 -0.00221794060132458
0.000927819486968255 -0.00244370878036102
0.000673640773803344 -0.00263411451683467
0.000402191484414962 -0.0027891462083421
0.000116995257697649 -0.00290913729549103
-0.000178474099052177 -0.00299474264598753
-0.000480823358966136 -0.00304691632973521
-0.000786768456272152 -0.00306688591619537
-0.00109316091326652 -0.00305612700200747
-0.00139701076039459 -0.00301633520148898
-0.00169550797191051 -0.00294939950896542
-0.00198603920142453 -0.00285737266554331
-0.00226620367334886 -0.00274244406889218
-0.00253382587291176 -0.00260691035264909
-0.0027869632303388 -0.00245314946344879
-0.00302391415427549 -0.00228359054605781
-0.00324322152489093 -0.00210069102197101
-0.00344367409154814 -0.00190690983477665
-0.00362430647342766 -0.0017046846410574
-0.00378439357223367 -0.00149640784069399
-0.00392344824436072 -0.00128440781220411
-0.00404121035840367 -0.00107092795155051
-0.00413764050915527 -0.000858111215614327
-0.00421290674665781 -0.000647983438004001
-0.00426737409919356 -0.000442439898685714
-0.00430158920673867 -0.000243234159612422
-0.00431626774835405 -5.19683967407565e-05
-0.0043122795412293 0.000129914711751128
-0.00429062572341806 0.000301137625920123
-0.00425242850937441 0.000460591383267144
-0.00419891396054349 0.000607338042845037
-0.00413139196193364 0.000740611284160768
-0.00405124271787612 0.000859814149783647
-0.00395989579722046 0.0009645172795107
-0.00385881523203985 0.00105445396040535
-0.00374948438346932 0.00112951387449979
-0.00363338987623961 0.00118973695923299
-0.0035120080942773 0.00123530501198785
-0.00338679004646244 0.00126653242707574
-0.00325914762937073 0.00128385623410323
-0.00313044617645072 0.00128782706610132
-0.00300198885802953 0.00127909549086468
-0.00287500923045963 0.00125840275232492
-0.00275066285390588 0.00122656767764766
-0.00263002053991363 0.0011844742895172
-0.00251406136623098 0.0011330619625648
-0.00240366848548558 0.00107331106224194
-0.0022996253996229 0.00100623252177459
-0.00220261432976855 0.000932856207053308
-0.00211321249067698 0.00085422054972693
-0.00203189441870946 0.00077136033104659
-0.00195902964330278 0.000685298286747183
-0.00189489002086863 0.0005970352648899
-0.00183964635853693 0.000507542119262654
-0.00179337470034616 0.000417750880087971
-0.00175605947028224 0.000328548473426349
-0.00172760034060837 0.000240770032969722
-0.0017078150256876 0.000155193690357116
-0.0016964474309315 7.25358923369798e-05
-0.00169317230930674 -6.55239060937379e-06
-0.00169760306108628 -8.14885232642823e-05
-0.00170929802021563 -0.000151760376281816
-0.00172776860334913 -0.000216927621406186
-0.00175248489777447 -0.000276622209538677
-0.00178288439255608 -0.00033054837694117
-0.00181837814857878 -0.000378481662072298
-0.00185835894765906 -0.000420267239923137
-0.00190220734619653 -0.000455817968519995
-0.0019492978452598 -0.000485111697063801
-0.00199900657407725 -0.000508188080483494
-0.00205071501542939 -0.000525145078321896
-0.00210382013388505 -0.000536134842692431
-0.00215773356101761 -0.000541359231900109
-0.00221189137439576 -0.000541066105953733
-0.00226575572753764 -0.000535543679265546
-0.00231881973949442 -0.000525115833894447
-0.0023706105217652 -0.000510137311622791
-0.00242069150674136 -0.000490988793916656
-0.00246866570748647 -0.000468071315096949
-0.00251417711482746 -0.00044180206374427
-0.00255691162882683 -0.000412608912028798
-0.00259659962003728 -0.000380925899021878
-0.00263301243715925 -0.000347188946768941
-0.00266596729660702 -0.000311831170000247
-0.00269532309165946 -0.00027527908397479
-0.0027209810910492 -0.000237948854997695
-0.00274288400774273 -0.000200242522880405
-0.00276101367071315 -0.000162544975430241
-0.00277538916236689 -0.000125221234309842
-0.00278606542163 -8.86137987956357e-05
-0.00279313045003667 -5.30405251366389e-05
-0.00279670158648636 -1.87928275015443e-05
-0.00279692550728147 1.38657674318124e-05
-0.0027939728710528 4.47007431223399e-05
-0.00278803645613438 7.35073850039497e-05
-0.00277932836660874 0.000100111242207563
-0.00276807584135547 0.000124368163480456
-0.00275451962423431 0.000146164243119081
-0.00273891070444526 0.00016541535022954
-0.00272150635838436 0.000182066274843777
-0.00270256782131613 0.000196089975477709
-0.00268235865752586 0.000207486290663041
-0.00266114033649848 0.000216280447896167
-0.00263917083589639 0.000222521718006019
-0.00261670231320631 0.000226281503653544
-0.00259397807889175 0.000227651632064052
-0.00257123213068182 0.000226742371400253
-0.00254868566105432 0.000223680346760648
-0.00252654659152205 0.000218606542507332
-0.00250500933974626 0.000211674101554914
-0.00248425155985059 0.000203046343200686
-0.00246443414236713 0.000192894591117426
-0.00244570051568669 0.000181396118554867
-0.00242817711166798 0.000168732063268143
-0.00241197080444851 0.000155085546222515
-0.00239717030737696 0.000140639760994095
-0.00238384687145548 0.000125576033768451
-0.00237205312114904 0.000110072448369342
-0.0023618244513228 9.4302123896678e-05
-0.00235317949286587 7.84317888640486e-05
-0.00234611964699681 6.26205436330505e-05
-0.00234063187920034 4.70186660834592e-05
-0.00233668755504724 3.17666456550736e-05
-0.00233424569980024 1.69942966324378e-05
-0.00233325206707352 2.8200941775585e-06
-0.00233364146712275 -1.06494526894709e-05
-0.00233533846532766 -2.33201399545634e-05
-0.00233825901199689 -3.51104239858535e-05
-0.00234231207218167 -4.59514680182628e-05
-0.00234739962567437 -5.57871825504249e-05
-0.00235341852965484 -6.45741884233431e-05
-0.00236026214851308 -7.22814995706457e-05
-0.00236782175084109 -7.8890221776399e-05
-0.00237598674227748 -8.43930588784621e-05
-0.00238464652816219 -8.87939145154641e-05
-0.00239369284186724 -9.21069948015249e-05
-0.00240301555385449 -9.43564718285531e-05
-0.0024125117520936 -9.55755860701837e-05
-0.00242208061981443 -9.58057130866262e-05
-0.00243162483250456 -9.5095791448765e-05
-0.00244105311907496 -9.35012734602364e-05
-0.00245028026187952 -9.10834087492723e-05
-0.00245922826089727 -8.79081150385251e-05
-0.00246782260845863 -8.40454029697464e-05
-0.00247599973985431 -7.95682758864853e-05
-0.00248370144542295 -7.45518867584512e-05
-0.00249087836303167 -6.90727383949009e-05
-0.00249748671846826 -6.32078909433421e-05
-0.00250349251641439 -5.70341804423198e-05
-0.00250886921215823 -5.06274349902167e-05
-0.00251359654746074 -4.40617965241918e-05
-0.00251766194755411 -3.74091598501751e-05
-0.00252106075398927 -3.07385289263415e-05
-0.00252379459483504 -2.41155146447373e-05
-0.00252587091902811 -1.76018958158335e-05
-0.00252730416053918 -1.12551569174414e-05
-0.00252811294441341 -5.1281578227042e-06
-0.00252832241508024 7.30989925368025e-07
-0.00252796097673584 6.27933996966384e-06
-0.00252706192315889 1.14791740736128e-05
-0.00252566204072875 1.62980736014746e-05
-0.0025237997457837 2.07090497939852e-05
-0.00252151811141421 2.46903428816211e-05
-0.00251886021085445 2.82256031201218e-05
-0.00251587167861051 3.13035505937705e-05
-0.00251259884781811 3.39180655856859e-05
-0.00250908735324531 3.60677183575589e-05
-0.00250538376110429 3.77556387060105e-05
-0.00250153347356938 3.898929165737e-05
-0.00249758305707645 3.9780216929589e-05
-0.00249357628419524 4.01437720045491e-05
-0.00248955343512179 4.0098542280575e-05
-0.00248555455730013 3.96660733023664e-05
-0.00248161643861612 3.88705740073383e-05
-0.00247777447002815 3.77383739430079e-05
-0.0024740617142453 3.62979303588505e-05
-0.00247050750872425 3.45791627106738e-05
-0.00246713816415515 3.2613144619545e-05
-0.00246397696445179 3.04318002554561e-05
-0.00246104183843053 2.80673288374808e-05
-0.0024583514134042 2.55520960283117e-05
-0.00245591942723903 2.29183553593687e-05
-0.00245375449551138 2.01977596431958e-05
-0.00245186406962048 1.74210824536506e-05
-0.00245025397112717 1.46181781141075e-05
-0.00244892396796253 1.18176706791186e-05
-0.00244787243102937 9.04651963365801e-06
-0.00244709610137414 6.33009940779203e-06
-0.00244658799470462 3.69197696750733e-06
-0.00244633740138174 1.1535951248377e-06
-0.00244633570718987 -1.26558100791818e-06
-0.00244656987407499 -3.54818508205507e-06
-0.00244702430278534 -5.67913961031145e-06
-0.00244768292834526 -7.64570835744684e-06
-0.00244853038421466 -9.43728203968712e-06
-0.00244954850982628 -1.10454822749703e-05
-0.00245071821323084 -1.24641625117176e-05
-0.00245201970392952 -1.36893447228621e-05
-0.0024534322600408 -1.47193025863649e-05
-0.00245493865209346 -1.55541689380152e-05
-0.00245651908943111 -1.61958859754497e-05
-0.00245815447984115 -1.66482007104322e-05
-0.00245982619672874 -1.69164985462692e-05
-0.00246151561345899 -1.70076684577737e-05
-0.00246320526751272 -1.69300061878552e-05
-0.00246487932615327 -1.6693015274591e-05
-0.00246652218944739 -1.6307220624926e-05
-0.00246811918876013 -1.57840536170609e-05
-0.00246965751808085 -1.51357363702873e-05
-0.00247112483704631 -1.43750130090481e-05
-0.00247251090075611 -1.3515108936915e-05
-0.00247380755977958 -1.25694830049308e-05
-0.00247500689751693 -1.15515813932528e-05
-0.0024761012301951 -1.0475003187977e-05
-0.00247708496951884 -9.35326423715671e-06
-0.00247795462267646 -8.19959545889635e-06
-0.00247870786101883 -7.02687494622879e-06
-0.00247934258874098 -5.84747145756582e-06
-0.00247985927118951 -4.67320915183448e-06
-0.00248026023637468 -3.51521740740907e-06
-0.00248054734666896 -2.38374991507872e-06
-0.00248072293012306 -1.28841073971037e-06
-0.00248079071179396 -2.37973522013266e-07
-0.00248075558091442 7.59645772968002e-07
-0.00248062312523433 1.69747019258457e-06
-0.00248040056234349 2.56948357718221e-06
-0.0024800937128736 3.37063049678796e-06
-0.00247971049295671 4.09678375002786e-06
-0.00247925975007401 4.74481670623074e-06
-0.0024787489347499 5.31261232880023e-06
-0.00247818573036018 5.79883886986832e-06
-0.00247757735464165 6.20300413872754e-06
-0.00247693288799746 6.52540112887562e-06
-0.00247625954820606 6.767108204174e-06
-0.0024755661828798 6.92992015486325e-06
-0.00247486047549658 7.01634470280437e-06
-0.00247415034238204 7.02952643923756e-06
-0.00247344183723084 6.97314191701673e-06
-0.00247274217790197 6.85129110080556e-06
-0.00247205788377501 6.66853711627435e-06
-0.00247139547424015 6.42985205914575e-06
-0.00247075867472576 6.14042151022122e-06
-0.00247015353897293 5.8056698791025e-06
-0.00246958379242106 5.43119708260173e-06
-0.00246905339334234 5.02268810358922e-06
-0.002468565368688 4.58588763977113e-06
-0.00246812204691592 4.12648064002119e-06
-0.00246772389383397 3.64998752485604e-06
-0.00246737393638479 3.16181818868977e-06
-0.00246707333886416 2.66733559527686e-06
-0.0024668225670705 2.17169279270962e-06
-0.00246662115547196 1.67974969917252e-06
-0.00246646887136007 1.19610029739622e-06
-0.00246636408503432 7.25029165443095e-07
-0.00246630586527559 2.70422806141141e-07
-0.00246629258236548 -1.6410910303659e-07
-0.00246632144242086 -5.75383862972062e-07
-0.00246639011720936 -9.60620477998778e-07
-0.00246649604565776 -1.317416085494e-06
-0.0024666364338511 -1.64379123963963e-06
-0.00246680802220418 -1.93809576404073e-06
-0.00246700755111963 -2.19914452018861e-06
-0.0024672319938218 -2.4260798294133e-06
-0.00246747669370878 -2.6184927524194e-06
-0.00246773908964537 -2.77630725169415e-06
-0.00246801568916504 -2.89978385974014e-06
-0.00246830299979351 -2.98947259074075e-06
-0.00246859752904737 -3.04626543253038e-06
-0.00246889625009787 -3.07130224772392e-06
-0.00246919660177146 -3.06595451280887e-06
-0.00246949392741188 -3.03185242680776e-06
-0.00246978682998563 -2.97085960653952e-06
-0.00247007228264243 -2.884928334803e-06
-0.00247034795701873 -2.77620267303451e-06
-0.00247061175757969 -2.64690087293932e-06
-0.00247086158878767 -2.49934977485816e-06
-0.00247109582076465 -2.33593408187631e-06
-0.00247131305646268 -2.1590620432315e-06
-0.0024715118988337 -1.97114370312245e-06
-0.00247169141649148 -1.77457466398671e-06
-0.00247185091088105 -1.57172154421166e-06
-0.00247198991628 -1.36488223768591e-06
-0.00247210796696819 -1.1562677725307e-06
-0.00247220529571981 -9.48000534504046e-07
-0.00247228166965086 -7.42085288461163e-07
-0.00247233755437237 -5.40409191877259e-07
-0.00247237364832984 -3.44714649594055e-07
-0.0024723904171426 -1.56586709745528e-07
-0.00247238879209488 2.25416513413134e-08
-0.00247236970447504 1.9138032905468e-07
-0.00247233408557619 3.48823807402128e-07
-0.00247228333235709 4.93927584110172e-07
-0.00247221884178086 6.25911813166178e-07
-0.00247214201081583 7.44193874593468e-07
-0.00247205377077304 8.4833769110719e-07
-0.00247195575145898 9.38046539191145e-07
-0.00247184981551586 1.01320639785281e-06
-0.00247173689426694 1.07384258481061e-06
-0.00247161838470013 1.12010889572302e-06
-0.00247149614946803 1.15228395171731e-06
-0.00247137111990435 1.17078388408632e-06
-0.00247124539149877 1.17613522237895e-06
-0.00247111966276117 1.16900922007813e-06
-0.00247099486503177 1.15006990709238e-06
-0.00247087262814661 1.12012605228717e-06
-0.00247075388345095 1.08002803587406e-06
-0.00247063956229154 1.03068778679665e-06
-0.00247053059601648 9.7306243560186e-07
-0.00247042791597478 9.0814349659827e-07
-0.00247033198785445 8.36938797213731e-07
-0.00247024397583648 7.60490510370209e-07
-0.00247016364711751 6.79822729028525e-07
-0.00247009146738496 5.95919753417678e-07
-0.00247002766949578 5.09767669319271e-07
-0.00246997271913638 4.22310960323169e-07
-0.00246992638350041 3.34463359625572e-07
-0.00246988889544176 2.47096969636191e-07
-0.00246986002215151 1.6102962469987e-07
-0.00246983999648105 7.70411663620057e-08
-0.00246982788712696 -4.15009837411405e-09
-0.00246982369410556 -8.19289700520077e-08
-0.00246982718460139 -1.55725508226034e-07
-0.00246983812579839 -2.24993290314965e-07
-0.00246985558638567 -2.89292629878984e-07
-0.00246987933354219 -3.48259835364871e-07
-0.00246990890161505 -4.01583707718796e-07
-0.00246994312645665 -4.49048903398497e-07
-0.00246998177524014 -4.90514302776924e-07
-0.00247002461513762 -5.25880402959221e-07
-0.0024700704819967 -5.55110982436305e-07
-0.00247011914298636 -5.78222335704094e-07
-0.00247016989961185 -5.95319394436182e-07
-0.00247022158771558 -6.0656861992827e-07
-0.00247027513861611 -6.12116559775056e-07
-0.00247032868966301 -6.12165863896497e-07
-0.00247038224084792 -6.07029550687651e-07
-0.00247043392951704 -5.97031471671157e-07
-0.0024704851526437 -5.82566068556994e-07
-0.00247053404757332 -5.6399160501899e-07
-0.00247058131278751 -5.41695285095076e-07
-0.00247062624978368 -5.16075146013211e-07
-0.00247066839288892 -4.87567236633611e-07
-0.00247070727643085 -4.56591344999034e-07
-0.00247074313322833 -4.23587124522224e-07
-0.00247077549760892 -3.88977986835325e-07
-0.00247080460239213 -3.53178253458247e-07
-0.00247082974907538 -3.16591427869774e-07
-0.00247085163613961 -2.79626403160843e-07
-0.00247086933225267 -2.42646880676861e-07
-0.00247088353589619 -2.0603642655458e-07
-0.00247089401423102 -1.70118934912015e-07
-0.00247090100007941 -1.35205600294234e-07
-0.00247090449343348 -1.01594975570728e-07
-0.00247090495994758 -6.95494297453005e-08
-0.00247090193395478 -3.9275202290065e-08
-0.00247089611394121 -1.09985028129249e-08
-0.00247088773273321 1.51269071504978e-08
-0.0024708767903272 3.89616838505566e-08
-0.00247086351955077 6.03900203399949e-08
-0.00247084815323189 7.93178608604053e-08
-0.00247083115703059 9.56927039766223e-08
-0.00247081253094571 1.09472947444644e-07
-0.00247079250780894 1.20694755921785e-07
-0.00247077155328036 1.2931653192781e-07
-0.00247075059868584 1.35459482629744e-07
-0.00247072871270563 1.39230367694667e-07
-0.00247070542967747 1.40593008200523e-07
-0.00247068214658734 1.39628823342592e-07
-0.00247065979476125 1.36462629275573e-07
-0.00247063883986827 1.3139117910929e-07
-0.00247061788492821 1.24548354414177e-07
-0.00247059692994332 1.16022835452479e-07
-0.0024705780703944 1.05999144323727e-07
-0.00247055944364171 9.46835726108042e-08
-0.00247054244667235 8.21955224807915e-08
-0.00247052614816983 6.876297004878e-08
-0.00247051217795289 5.45505863648946e-08
-0.00247049913904298 3.97501349669099e-08
-0.00247048749710592 2.45371433922094e-08
-0.00247047771780693 9.05816429372722e-09
-0.0024704691026584 -6.52577456872541e-09
-0.00247046211732645 -2.20319272266171e-08
-0.00247045699464493 -3.73372396123613e-08
-0.00247045303612589 -5.22988065546461e-08
-0.00247045070743445 -6.67646039948736e-08
-0.00247045000857274 -8.06622938345335e-08
-0.00247045000822179 -9.38488946486404e-08
-0.00247045233619862 -1.06235787942707e-07
-0.0024704546641985 -1.17755997394568e-07
-0.00247045932052985 -1.28335355747576e-07
-0.00247046397688765 -1.37921381119718e-07
-0.00247047026308653 -1.46508649723708e-07
-0.00247047724780699 -1.53981359402402e-07
-0.00247048423255586 -1.60386545614119e-07
-0.00247049214865459 -1.65767648301366e-07
-0.00247050146176736 -1.70014293142916e-07
-0.00247051077491011 -1.73135522919072e-07
-0.00247052008808116 -1.75189210070616e-07
-0.00247052940127937 -1.76226056401198e-07
-0.00247053871450325 -1.76296696661549e-07
-0.00247054802775112 -1.75468098138421e-07
-0.00247055734102174 -1.73781848682381e-07
-0.00247056665431396 -1.71285012015923e-07
-0.00247057596762677 -1.68015585806452e-07
-0.00247058528095908 -1.64011548509741e-07
-0.00247059226600072 -1.59415839517344e-07
-0.00247059925105408 -1.54378639234155e-07
-0.00247060623611855 -1.48923474659101e-07
-0.00247061322119351 -1.43077506154572e-07
-0.00247061880929358 -1.36891354575409e-07
-0.00247062346607508 -1.30555017525849e-07
-0.00247062812285984 -1.24095640527725e-07
-0.00247063277964795 -1.17511423850533e-07
-0.00247063510812935 -1.10936230946716e-07
-0.00247063743660776 -1.04475035852462e-07
-0.00247063976508326 -9.81205768052929e-08
-0.00247064116223307 -9.18855438982163e-08
-0.0024706411623914 -8.59363744340827e-08
-0.0024706411625414 -8.03002235171208e-08
-0.00247064116268354 -7.49589968926118e-08
-0.00247064069715701 -6.9894595794472e-08
-0.00247063836897461 -6.52318510663882e-08
-0.00247063604077981 -6.10359247069873e-08
-0.00247063371257299 -5.72941603229748e-08
-0.00247063138435482 -5.39775882914262e-08
-0.00247062905612606 -5.1057258049908e-08
-0.00247062672788729 -4.85150945517526e-08
-0.00247062276982316 -4.63800202481993e-08
-0.00247061811325239 -4.47967877087712e-08
-0.00247061345666767 -4.37364556770672e-08
-0.0024706088000695 -4.31845680287472e-08
-0.0024706041434585 -4.3113964401419e-08
-0.00247059948683537 -4.34975036408495e-08
-0.00247059483020076 -4.43134824546637e-08
-0.00247059017355518 -4.55438162169424e-08
-0.0024705855168991 -4.71667729478632e-08
-0.0024705824900491 -4.91063760528357e-08
-0.00247058016168744 -5.11816941337409e-08
-0.00247057783332258 -5.33764237130221e-08
-0.0024705755049547 -5.56851461890225e-08
-0.00247057317658404 -5.80988145096805e-08
-0.0024705708482107 -6.06119908157406e-08
-0.00247056851983515 -6.3208399993242e-08
-0.00247056619145721 -6.5895279683769e-08
-0.00247056386307688 -6.8672629886888e-08
-0.00247056200035569 -7.15295892766542e-08
-0.00247056200028136 -7.43232424864609e-08
-0.00247056200021087 -7.69721428754266e-08
-0.00247056200014406 -7.94835376639533e-08
-0.00247056200008065 -8.18664642736767e-08
-0.00247056200002045 -8.4128160345422e-08
-0.00247056199996346 -8.62704449698572e-08
-0.00247056199990939 -8.83023555178775e-08
-0.00247056199985838 -9.02166448191709e-08
-0.00247056199981016 -9.20296263056796e-08
-0.00247056199976442 -9.37485184072506e-08
-0.00247056362953687 -9.53280949766207e-08
-0.00247056595780916 -9.66127660389669e-08
-0.00247056828608925 -9.7602503178109e-08
-0.00247057061437668 -9.83172194872484e-08
-0.00247057294267114 -9.87677714263217e-08
-0.00247057527097226 -9.89668153411356e-08
-0.00247057759927965 -9.89306453992025e-08
-0.00247057992759304 -9.86701182157171e-08
-0.00247058225591207 -9.81978995095219e-08
-0.00247058458423646 -9.75230268552337e-08
-0.00247058691256589 -9.66599850619294e-08
-0.00247058924090001 -9.56196210635286e-08
-0.00247059156923887 -9.44019443883254e-08
-0.00247059180210392 -9.31082539949073e-08
-0.00247059180213663 -9.18797025952975e-08
-0.00247059180216767 -9.07126615141193e-08
-0.00247059180219712 -8.96053310222786e-08
-0.0024705918022249 -8.85631488282187e-08
-0.00247059180225095 -8.75842864644406e-08
-0.00247059180227566 -8.66560875876317e-08
-0.00247059180229913 -8.57731144391499e-08
-0.0024705918023214 -8.49371954855186e-08
-0.00247059180234247 -8.41446928497372e-08
-0.00247059180236249 -8.33919972400123e-08
-0.00247059180238146 -8.26809276448801e-08
-0.00247059180239942 -8.20060366759235e-08
-0.00247059180241642 -8.13655149223399e-08
-0.00247059180243256 -8.07593815434996e-08
-0.00247059180244788 -8.01840081385459e-08
-0.00247059180246244 -7.96375853480673e-08
-0.00247059180247619 -7.91201034925238e-08
-0.00247059180248931 -7.86261440206739e-08
-0.00247059180250171 -7.81611446418282e-08
-0.00247059180251345 -7.77196580674247e-08
-0.00247059180252461 -7.72998844159305e-08
-0.00247059180253519 -7.69036426770744e-08
-0.0024705918025452 -7.65272948214171e-08
-0.00247059180255468 -7.61708505295829e-08
-0.00247059180256369 -7.58325003399202e-08
-0.00247059180257226 -7.55104348419515e-08
-0.0024705918025804 -7.5204654087827e-08
-0.00247059180258806 -7.49151483959466e-08
-0.00247059180259534 -7.46419369755539e-08
-0.00247059180260224 -7.43832008373536e-08
-0.00247059180260885 -7.41353211603912e-08
-0.00247059180261507 -7.3900097827392e-08
-0.00247059180262092 -7.36811687147062e-08
-0.00247059180262657 -7.34694772426287e-08
-0.00247059180263184 -7.32704421139724e-08
-0.00247059180263686 -7.30822729759321e-08
-0.00247059180264165 -7.29013319500978e-08
-0.00247059180264616 -7.27330663247063e-08
-0.00247059180265047 -7.25702194018024e-08
-0.00247059180265454 -7.24182384683218e-08
-0.00247059180265837 -7.22734856479145e-08
-0.0024705918026621 -7.21341705865828e-08
-0.00247059180266546 -7.20075118685638e-08
-0.00247059180266881 -7.1880853150328e-08
-0.00247059180267192 -7.17650604227082e-08
-0.00247059180267479 -7.16564958072943e-08
-0.00247059180267767 -7.154793119123e-08
-0.00247059180268035 -7.144842315628e-08
-0.00247059180268274 -7.13579526430376e-08
-0.00247059180268514 -7.12674821303372e-08
-0.00247059180268744 -7.11824493764956e-08
-0.00247059180268935 -7.11100729661835e-08
-0.00247059180269127 -7.10376965558715e-08
-0.00247059017287609 -7.10630145271153e-08
-0.00247059017287369 -7.11534850401409e-08
-0.00247059017287149 -7.1234898972811e-08
-0.00247059017286958 -7.13072753832315e-08
-0.00247059017286766 -7.13796517934351e-08
-0.00247059017286574 -7.14520282038555e-08
-0.00247059017286407 -7.15135386238769e-08
-0.00247059017286263 -7.15678209314754e-08
-0.00247059017286119 -7.16221032395076e-08
-0.00247059017285976 -7.16763855471061e-08
-0.00247059017285832 -7.17306678551383e-08
-0.00247059017285688 -7.17849501627368e-08
-0.00247059017285554 -7.1833794711585e-08
-0.00247059017285459 -7.18699829163616e-08
-0.00247059017285363 -7.1906171121355e-08
-0.00247059017285267 -7.19423593269989e-08
-0.00247059017285171 -7.19785475322091e-08
-0.00247059017285075 -7.20147357368773e-08
-0.0024705901728498 -7.20509239423043e-08
-0.00247059017284884 -7.20871121467556e-08
-0.00247059017284788 -7.21233003523995e-08
-0.00247059017284692 -7.21594885573929e-08
-0.0024705901728463 -7.2181191951683e-08
-0.00247059017284582 -7.21992860543965e-08
-0.00247059017284534 -7.22173801573269e-08
-0.00247059017284486 -7.22354742598236e-08
-0.00247059017284438 -7.22535683623203e-08
-0.00247059017284391 -7.22716624644917e-08
-0.00247059017284343 -7.22897565674221e-08
-0.00247059017284295 -7.23078506701356e-08
-0.00247059017284247 -7.23259447726323e-08
-0.00247059017284199 -7.23440388755627e-08
-0.00247059017284151 -7.23621329777342e-08
-0.00247059017284103 -7.23802270802308e-08
-0.00247059017284055 -7.23983211831612e-08
-0.00247059017284007 -7.24164152857663e-08
-0.0024705901728396 -7.2434509388263e-08
-0.00247059017283912 -7.24526034909766e-08
-0.00247059017283864 -7.2470697593148e-08
-0.00247059017283816 -7.248879169597e-08
-0.00247059017283768 -7.25068857987919e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
};
\addplot [very thick, learnedWithSideInfo, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.132071489995752 0.02809459702527
0.129559747251902 -0.0353555220273739
0.100323648554039 -0.0774529852837571
0.0564046943449772 -0.0939687512825418
0.0102998012583958 -0.0869663230429857
-0.0277193275585942 -0.0629931393143706
-0.0513573486889852 -0.0309930070157768
-0.058840775412335 0.000316175696405431
-0.0522568109067203 0.0244328176908738
-0.0362115740342448 0.0378275411231307
-0.016322416807138 0.0399496115166069
0.00218459915405326 0.0328072982537952
0.0155518738942232 0.0200805118463859
0.0220272305737175 0.00590145365886435
0.0217972492670084 -0.00626031753983369
0.0164718368866448 -0.0142424067220266
0.00837878383188234 -0.0173226417120668
-0.000112235296431007 -0.0159990847503397
-0.00710296461582395 -0.0115831217610697
-0.0114566263037299 -0.00573188874735375
-0.0128605347603412 -2.14240085014449e-05
-0.0117018921058195 0.00436454257674453
-0.0088251087810844 0.00679450824844852
-0.00524738295343483 0.00719924094196876
-0.00190111547128555 0.00596085316718689
0.000547517547719063 0.00372816314431914
0.0017808873250097 0.00121414243402616
0.00181721699672829 -0.000974458324718751
0.000927819486968255 -0.00244370878036102
-0.000480823358966136 -0.00304691632973521
-0.00198603920142453 -0.00285737266554331
-0.00324322152489093 -0.00210069102197101
-0.00404121035840367 -0.00107092795155051
-0.00431626774835405 -5.19683967407565e-05
-0.00413139196193364 0.000740611284160768
-0.00363338987623961 0.00118973695923299
-0.00300198885802953 0.00127909549086468
-0.00240366848548558 0.00107331106224194
-0.00195902964330278 0.000685298286747183
-0.00172760034060837 0.000240770032969722
-0.00170929802021563 -0.000151760376281816
-0.00185835894765906 -0.000420267239923137
-0.00210382013388505 -0.000536134842692431
-0.0023706105217652 -0.000510137311622791
-0.00259659962003728 -0.000380925899021878
-0.00274288400774273 -0.000200242522880405
-0.00279670158648636 -1.87928275015443e-05
-0.00276807584135547 0.000124368163480456
-0.00268235865752586 0.000207486290663041
-0.00257123213068182 0.000226742371400253
-0.00246443414236713 0.000192894591117426
-0.00238384687145548 0.000125576033768451
-0.00234063187920034 4.70186660834592e-05
-0.00233533846532766 -2.33201399545634e-05
-0.00236026214851308 -7.22814995706457e-05
-0.00240301555385449 -9.43564718285531e-05
-0.00245028026187952 -9.10834087492723e-05
-0.00249087836303167 -6.90727383949009e-05
-0.00251766194755411 -3.74091598501751e-05
-0.00252811294441341 -5.1281578227042e-06
-0.0025237997457837 2.07090497939852e-05
-0.00250908735324531 3.60677183575589e-05
-0.00248955343512179 4.0098542280575e-05
-0.00247050750872425 3.45791627106738e-05
-0.00245591942723903 2.29183553593687e-05
-0.00244787243102937 9.04651963365801e-06
-0.00244656987407499 -3.54818508205507e-06
-0.00245071821323084 -1.24641625117176e-05
-0.00245815447984115 -1.66482007104322e-05
-0.00246652218944739 -1.6307220624926e-05
-0.00247380755977958 -1.25694830049308e-05
-0.00247870786101883 -7.02687494622879e-06
-0.00248072293012306 -1.28841073971037e-06
-0.0024800937128736 3.37063049678796e-06
-0.00247757735464165 6.20300413872754e-06
-0.00247415034238204 7.02952643923756e-06
-0.00247075867472576 6.14042151022122e-06
-0.00246812204691592 4.12648064002119e-06
-0.00246662115547196 1.67974969917252e-06
-0.00246632144242086 -5.75383862972062e-07
-0.00246700755111963 -2.19914452018861e-06
-0.00246830299979351 -2.98947259074075e-06
-0.00246978682998563 -2.97085960653952e-06
-0.00247109582076465 -2.33593408187631e-06
-0.00247198991628 -1.36488223768591e-06
-0.00247237364832984 -3.44714649594055e-07
-0.00247228333235709 4.93927584110172e-07
-0.00247184981551586 1.01320639785281e-06
-0.00247124539149877 1.17613522237895e-06
-0.00247063956229154 1.03068778679665e-06
-0.00247016364711751 6.79822729028525e-07
-0.00246988889544176 2.47096969636191e-07
-0.00246982718460139 -1.55725508226034e-07
-0.00246994312645665 -4.49048903398497e-07
-0.00247016989961185 -5.95319394436182e-07
-0.00247043392951704 -5.97031471671157e-07
-0.00247066839288892 -4.87567236633611e-07
-0.00247082974907538 -3.16591427869774e-07
-0.00247090100007941 -1.35205600294234e-07
-0.00247088773273321 1.51269071504978e-08
-0.00247081253094571 1.09472947444644e-07
-0.00247070542967747 1.40593008200523e-07
-0.00247059692994332 1.16022835452479e-07
-0.00247051217795289 5.45505863648946e-08
-0.00247046211732645 -2.20319272266171e-08
-0.00247045000822179 -9.38488946486404e-08
-0.00247047026308653 -1.46508649723708e-07
-0.00247051077491011 -1.73135522919072e-07
-0.00247055734102174 -1.73781848682381e-07
-0.00247059925105408 -1.54378639234155e-07
-0.00247062812285984 -1.24095640527725e-07
-0.00247064116223307 -9.18855438982163e-08
-0.00247063836897461 -6.52318510663882e-08
-0.00247062672788729 -4.85150945517526e-08
-0.0024706041434585 -4.3113964401419e-08
-0.0024705824900491 -4.91063760528357e-08
-0.0024705708482107 -6.06119908157406e-08
-0.00247056200028136 -7.43232424864609e-08
-0.00247056199996346 -8.62704449698572e-08
-0.00247056362953687 -9.53280949766207e-08
-0.00247057527097226 -9.89668153411356e-08
-0.00247058691256589 -9.66599850619294e-08
-0.00247059180216767 -9.07126615141193e-08
-0.00247059180229913 -8.57731144391499e-08
-0.00247059180239942 -8.20060366759235e-08
-0.00247059180247619 -7.91201034925238e-08
-0.00247059180253519 -7.69036426770744e-08
-0.0024705918025804 -7.5204654087827e-08
-0.00247059180261507 -7.3900097827392e-08
-0.00247059180264165 -7.29013319500978e-08
-0.0024705918026621 -7.21341705865828e-08
-0.00247059180267767 -7.154793119123e-08
-0.00247059180268935 -7.11100729661835e-08
-0.00247059017286958 -7.13072753832315e-08
-0.00247059017286119 -7.16221032395076e-08
-0.00247059017285459 -7.18699829163616e-08
-0.0024705901728498 -7.20509239423043e-08
-0.00247059017284582 -7.21992860543965e-08
-0.00247059017284343 -7.22897565674221e-08
-0.00247059017284103 -7.23802270802308e-08
-0.00247059017283864 -7.2470697593148e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
-0.00247059017283763 -7.2506876269739e-08
};
\addplot [very thick, learnedWithoutSideInfo]
table {%
0.1 0.1
0.0668753270132454 0.0460863503913297
0.0726735309436108 0.037240702076267
0.0798342613352712 0.0276159482417389
0.0885307109485782 0.0133399086812288
0.100635747764291 -0.0131918495230911
0.115645992257787 -0.0681395031655277
0.116478566905227 -0.117272744993738
0.112268028240126 -0.124621962240746
0.111399850901932 -0.125133656896663
0.111287714920967 -0.12517317742043
0.111275018645082 -0.125176743684119
0.111273645493237 -0.125177095644017
0.111273499425655 -0.125177131790367
0.1112734839822 -0.125177135561906
0.111273482353059 -0.125177135957814
0.111273482181343 -0.125177135999468
0.111273482163248 -0.125177136003854
0.111273482161342 -0.125177136004316
0.111273482161141 -0.125177136004364
0.11127348216112 -0.125177136004369
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
};
\addplot [very thick, learnedWithoutSideInfo, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.100635747764291 -0.0131918495230911
0.111287714920967 -0.12517317742043
0.111273482353059 -0.125177135957814
0.11127348216112 -0.125177136004369
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
0.111273482161118 -0.12517713600437
};

==> figures/smd_phase_plots/phase_plot_10_quarter_space_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.0829243212938309 0.116129510104656
0.0997821465134621 0.089897409081459
0.112891390919685 0.117963708937168
0.106157816946507 0.139007225632668
0.0986010059714317 0.0330617986619473
0.104692600667477 0.0903725251555443
0.0223752297461033 0.0962871387600899
0.0350027941167355 0.0742338597774506
0.0147444102913141 0.144461542367935
0.0977527648210526 0.0138454213738441
};
\addplot [very thick, trueDynamics]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, approxDynamics, dashed]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, learnedWithSideInfo]
table {%
0.1 0.1
0.109246891902101 0.084914927517825
0.116980995532932 0.0697691646872414
0.123203418575138 0.0547031419313173
0.127928353772489 0.0398381922563755
0.131181321129939 0.0252802280005022
0.132997774378514 0.0111231080391361
0.1334221022234 -0.00254849196773825
0.132506830739095 -0.0156569026372208
0.130311877949362 -0.0281299848485477
0.12690421079167 -0.0399002670706551
0.122357300977047 -0.0509045596498113
0.116750737369661 -0.0610840069574923
0.110169756459695 -0.0703843426535668
0.102704757976724 -0.0787564514166558
0.0944507981809875 -0.0861568334898107
0.0855069565221604 -0.0925483878665909
0.0759756799616332 -0.0979010173500858
0.0659620602535032 -0.102192212208347
0.0555730292789813 -0.105407639329851
0.0449165171346369 -0.107541588477213
0.0341005878740124 -0.108597357920483
0.0232324970217475 -0.108587527595937
0.0124177900696299 -0.107534112312336
0.00175933659628831 -0.105468491180177
-0.00864360324664406 -0.102431373693198
-0.0186962869857124 -0.0984724602318954
-0.0283093882957803 -0.0936501170373234
-0.0373998143289571 -0.0880308128204814
-0.0458915167564997 -0.0816885030979434
-0.0537161660234296 -0.074703806054975
-0.060813814429061 -0.0671631117102399
-0.067133369217166 -0.0591577133195827
-0.072633091749373 -0.0507825637676941
-0.0772808768859553 -0.0421352553790907
-0.0810544466896602 -0.0333148106836566
-0.0839414472758715 -0.0244204087658127
-0.0859393966538032 -0.0155502006178446
-0.0870555357144479 -0.00680005922954217
-0.0873065302104723 0.00173763887656978
-0.0867180535301455 0.00997515787192305
-0.0853242800682377 0.0178305078768723
-0.08316723703973 0.0252284646980006
-0.0802961190447008 0.0321014686097309
-0.0767664536261246 0.038390435619605
-0.0726392072282452 0.0440454186803454
-0.0679798911599638 0.0490261077134689
-0.0628575111007892 0.053302162910791
-0.057343643271376 0.0568533813196332
-0.0515113615966065 0.0596696875134836
-0.045434243099127 0.0617508561744349
-0.0391854030967764 0.0631061673110092
-0.0328366235245104 0.063753709129404
-0.0264574123345562 0.0637197077654227
-0.0201143124773589 0.0630375654510921
-0.0138702043514642 0.0617468935926043
-0.00778374421022894 0.0598923889124946
-0.00190890814351632 0.0575228017382382
0.00370536034616586 0.0546898365445531
0.00901539230202574 0.0514470922709448
0.0139829346956975 0.0478491679837557
0.0185752102077072 0.0439508030394866
0.0227648827129328 0.039806162810264
0.0265299926102969 0.0354682465002651
0.0298537929603683 0.0309884278219908
0.0327245828214036 0.0264160705211209
0.0351354837652969 0.0217982556391661
0.0370842014813626 0.017179612746318
0.0385727687461372 0.0126021571201901
0.0396073014221314 0.00810522652761087
0.040197700433741 0.00372541049531807
0.0403573947159785 -0.000503491106602102
0.0401030394552395 -0.00455048569622574
0.0394542739326407 -0.00838741638415025
0.0384333750575896 -0.0119889881436663
0.0370650301101962 -0.0153327825436378
0.0353760238023984 -0.0183992919601497
0.0333949365156167 -0.0211719460886621
0.0311518537152585 -0.0236371070610727
0.028678082818005 -0.0257841293142881
0.0260058495702296 -0.0276053197620182
0.0231679907035981 -0.029095956145915
0.0201976857075503 -0.0302542715921963
0.0171281308605925 -0.0310813980291809
0.0139922635550088 -0.0315813315566381
0.0108224950035826 -0.0317608344644175
0.00765041547403799 -0.0316293275915438
0.00450654702180515 -0.0311988048625381
0.00142009272952326 -0.030483630638766
-0.00158129484242707 -0.0295004241137495
-0.00447172890865356 -0.0282678285067166
-0.00722728054383281 -0.0268063210344887
-0.00982614864913263 -0.025137968917566
-0.0122488109429529 -0.0232861928402506
-0.0144781437522567 -0.0212755117636888
-0.0164995109551214 -0.0191312470169684
-0.0183008487310245 -0.0168792857300569
-0.0198726916397066 -0.0145457701408821
-0.0212081977685558 -0.0121568269178729
-0.0223031124126712 -0.00973830392666843
-0.0231557531767589 -0.00731548213391928
-0.0237669187080844 -0.0049128391002722
-0.0241398141942701 -0.00255379661591045
-0.0242799172565623 -0.000260493678777581
-0.024194840118083 0.00194641032105899
-0.0238941843217746 0.00404791763589505
-0.0233893768221233 0.00602684970218023
-0.0226934427468361 0.00786797321471545
-0.0218208470764846 0.00955810068673342
-0.0207872618181002 0.0110861615479159
-0.0196093536674299 0.0124432386379356
-0.0183045753964738 0.0136225953890206
-0.0168909442013158 0.014619635260116
-0.0153868424017413 0.0154318835142283
-0.0138107780927552 0.0160589040491269
-0.0121812184387883 0.0165022200475997
-0.0105163773317511 0.0167651957819033
-0.00883405054634792 0.0168529128681271
-0.00715144390905919 0.0167720291079588
-0.00548502335243007 0.0165306207213004
-0.00385038662228969 0.0161380265051567
-0.00226213777747325 0.0156046736588387
-0.000733792424005221 0.0149419295225829
0.000722311406499312 0.0141619127228602
0.00209507711562398 0.013277333051369
0.00337470367658196 0.0123013388585754
0.0045527176537454 0.0112473504790615
0.00562199736375074 0.0101289252436883
0.00657677759540972 0.00895960855458354
0.00741264076631305 0.00775281644046888
0.00812650062886289 0.00652170600659563
0.00871656874615149 0.00527906949604781
0.00918231165397225 0.00403723800151549
0.00952440615984979 0.00280799139632814
0.00974467182407459 0.0016024755976129
0.00984600856252865 0.000431136118287229
0.00983232866108502 -0.000696343880601424
0.00970846550654096 -0.00177109406375284
0.00948010187498957 -0.00278510082678046
0.00915367493673563 -0.00373123832847988
0.00873629057430193 -0.00460329867693221
0.00823562652422719 -0.00539600649618784
0.00765984250359815 -0.00610502607928734
0.00701748614569053 -0.00672696992616201
0.00631739614135951 -0.00725938964299045
0.00556860724297454 -0.00770075894547253
0.00478026318483653 -0.0080504626675516
0.00396152401523918 -0.00830875977725676
0.00312148274218949 -0.00847675887869958
0.00226908011607191 -0.0085563733072685
0.00141302628122065 -0.00855028219758464
0.00056172877172062 -0.00846187114370434
-0.000276777397043758 -0.00829517839285487
-0.00109489131298931 -0.00805484193949005
-0.00188550274644885 -0.00774603412114899
-0.00264204273366186 -0.00737438219745297
-0.00335852484699553 -0.00694591686000873
-0.00402958291465294 -0.00646698724560115
-0.00465049942705439 -0.00594419595261487
-0.00521722532836651 -0.00538432844575825
-0.00572639654889225 -0.00479426719204738
-0.00617534145636245 -0.00418093918358101
-0.00656207713187304 -0.00355123352849641
-0.0068853065771004 -0.00291193602968788
-0.00714440381400844 -0.00226967021965731
-0.00733939339687693 -0.0016308339065648
-0.00747092666462628 -0.00100154315585582
-0.00754024961111037 -0.000387582619800458
-0.00754917028978024 0.000205640852366177
-0.00750001504239615 0.000773138159504929
-0.00739558752163135 0.00131037239369908
-0.00723912119435106 0.00181328739068351
-0.00703422905081302 0.00227832933215478
-0.00678485471077647 0.00270246347370944
-0.00649521840718403 0.00308318303086116
-0.00616976529808186 0.00341851365492709
-0.00581311098441185 0.00370701153816962
-0.00542998795904827 0.00394775641227798
-0.00502519764356377 0.00414033806885087
-0.00460355683701508 0.00428483893071854
-0.00416984835557044 0.00438181594676535
-0.00372877819108538 0.00443226601771127
-0.00328493243707938 0.00443760883781691
-0.0028427342142755 0.00439964235005966
-0.00240640967665169 0.00432051587301572
-0.00197995448310235 0.00420269532172055
-0.00156710294641111 0.00404891683522595
-0.00117130381800244 0.00386215528415782
-0.000795698750219034 0.00364558160770101
-0.000443103639739358 0.00340252227387412
-0.000115995479051329 0.00313642220094937
0.000183497081433566 0.00285080443882355
0.00045360044267548 0.00254923541697642
0.000692898167949277 0.00223528438225728
0.000900329201044521 0.00191249189588222
0.0010751840034559 0.00158433714911927
0.00121709678441321 0.00125420575038066
0.00132603394726372 0.000925362662833099
0.00140228180824265 0.000600925429824362
0.00144642983314265 0.000283841394379873
0.00145935282620546 -2.31337050325465e-05
0.00144219067419179 -0.000317453386171195
0.00139632715907535 -0.000596796122666984
0.00132336574386261 -0.000859077981125913
0.00122510652250574 -0.00110246290010849
0.00110352060861369 -0.00132536967513527
0.000960724174841258 -0.00152647629411034
0.000798952084811413 -0.00170472331492393
0.000620532630884896 -0.00185931155837711
0.000427860729431436 -0.00198970131358046
0.00022337278949325 -0.00209560632025662
9.52118760079828e-06 -0.00217698624496234
-0.000211249360238143 -0.0022340361370329
-0.000436525163675641 -0.00226717948743826
-0.00066394553718964 -0.00227705176135364
-0.00089122370150761 -0.00226448742495482
-0.00111616532217224 -0.00223050301594264
-0.00133668601579802 -0.002176282070185
-0.00155082788146489 -0.00210315611331998
-0.00175677213207255 -0.00201258795543522
-0.00195285259895834 -0.00190614954397887
-0.00213756481263252 -0.00178550550091096
-0.00230957426865638 -0.00165239131478176
-0.00246772352933878 -0.00150859525241457
-0.00261103513448647 -0.00135593817617273
-0.00273871393008829 -0.00119625487671362
-0.00285014962978616 -0.00103137574622755
-0.00294491215860246 -0.000863109151398046
-0.0030227525845938 -0.000693224619472083
-0.00308359566858377 -0.000523436602803952
-0.00312753404366284 -0.000355390765964705
-0.00315481960073975 -0.000190650000178945
-0.0031658583665056 -3.06824156456782e-05
-0.00316119606814992 0.000123149075410508
-0.00314151021730934 0.000269595952006541
-0.0031075959075637 0.000407531831196872
-0.00306035603568706 0.000535958613228156
-0.00300078477076985 0.000654011097742782
-0.00292995777541855 0.000760960226106077
-0.00284901707180388 0.000856214586871936
-0.00275915520919036 0.000939320791552229
-0.00266160362239578 0.00100996213757475
-0.00255761959322729 0.00106795605680315
-0.00244847111644049 0.00111325104042685
-0.00233542502525754 0.00114592101671524
-0.00221973558256385 0.00116616001634381
-0.00210263120941529 0.00117427486754257
-0.00198530493883373 0.00117067777520177
-0.00186890347259354 0.0011558790214295
-0.00175451740211286 0.00113047536845329
-0.00164317399055587 0.00109514391820482
-0.0015358292563336 0.00105062959101464
-0.00143336180289364 0.000997736084911372
-0.00133656723056791 0.000937316198357326
-0.00124615417821946 0.000870260177009762
-0.00116274048132507 0.000797486966759387
-0.00108685095986204 0.00071993308232217
-0.00101891625394236 0.000638543278352071
-0.000959273172864275 0.000554261158710478
-0.000908164054621351 0.000468019642650278
-0.00086573891941777 0.000380732994916474
-0.000832057623168523 0.000293288160355947
-0.000807093058776594 0.000206537880593005
-0.000790734706651597 0.000121293375046697
-0.000782793524032668 3.83186243157665e-05
-0.000783006543281085 -4.16753462240284e-05
-0.000791042459723557 -0.000118035055505723
-0.000806507685171812 -0.000190168578604208
-0.000828952634291313 -0.000257548630945716
-0.000857878534852238 -0.000319715147689078
-0.000892743946956706 -0.000376277025642792
-0.000932971573326944 -0.000426912994777399
-0.000977955884504305 -0.000471372010252894
-0.00102706923067636 -0.000509472674912333
-0.00107967004897817 -0.000541102341316322
-0.00113510792760089 -0.00056621563591109
-0.00119273198774961 -0.000584831792439281
-0.0012518958895654 -0.000597032074385665
-0.00131196446786681 -0.000602956354389141
-0.0013723197858242 -0.000602799811968786
-0.00143236520958295 -0.000596808759987947
-0.00149153181120721 -0.000585275600847587
-0.00154928186122705 -0.000568535060508463
-0.00160511301969287 -0.000546958562954219
-0.00165856136308155 -0.000520949769784508
-0.00170920499328183 -0.000490938577834057
-0.00175666613316117 -0.000457376917356218
-0.00180061287291588 -0.000420732635199443
-0.00184076138205961 -0.000381485003210678
-0.00187687509462648 -0.000340118948670277
-0.00190876633907785 -0.000297120678076027
-0.00193629645481559 -0.00025297269089559
-0.00195937381321647 -0.000208149272893753
-0.00197795439979249 -0.000163112176426396
-0.00199203925313586 -0.000118306656894018
-0.00200167330083745 -7.41578854866872e-05
-0.00200694175068409 -3.10674138739808e-05
-0.00200796962505078 1.05894408092843e-05
-0.00200491850133039 5.04665055100244e-05
-0.00199798138969977 8.82487859646639e-05
-0.00198738273315904 0.000123654276914274
-0.00197337281962408 0.000156435436268413
-0.00195622522081188 0.00018638019020045
-0.00193623260130035 0.000213312614797257
-0.00191370310965695 0.000237092986310654
-0.00188895770088517 0.000257617868696219
-0.0018623255962202 0.000274819620227971
-0.00183414090706079 0.000288665525162063
-0.00180473960815752 0.000299156865114293
-0.00177445546303698 0.000306327238969615
-0.00174361792849878 0.00031024120045013
-0.00171254784720684 0.000310992287452826
-0.00168155605066363 0.000308700993165434
-0.0016509391682048 0.000303512273929704
-0.00162097927771173 0.000295593462061305
-0.00159194018026048 0.00028513157137716
-0.00156406600308757 0.000272330717040041
-0.00153757980254425 0.000257409275764905
-0.00151268205065005 0.000240597596090583
-0.00148955016936681 0.00022213491176975
-0.00146833690072849 0.000202266704458325
-0.00144917042320473 0.000181242269375847
-0.00143215365315382 0.000159311946897648
-0.00141736471043226 0.000136724790061836
-0.00140485726759171 0.000113726085990126
-0.00139466031700326 9.05552403333926e-05
-0.00138677933496632 6.74436251845182e-05
-0.0013811973294101 4.4612760088456e-05
-0.00137787553834638 2.22724499572744e-05
-0.00137675505965361 6.19257741619187e-07
-0.00137775801520397 -2.01647922894118e-05
-0.00138078859857586 -3.99134704701247e-05
-0.00138573621824929 -5.84772812529983e-05
-0.00139247526476059 -7.57242087780126e-05
-0.00140086837032034 -9.15403199467642e-05
-0.00141076757295986 -0.000105830101867344
-0.00142201617917309 -0.000118516703129328
-0.00143445097581027 -0.00012954187249304
-0.00144790316140357 -0.000138865799422943
-0.00146220172222014 -0.000146466773890708
-0.00147717413076824 -0.000152340585299879
-0.00149264809203871 -0.000156499942765635
-0.00150845305692042 -0.000158973685286977
-0.00152442301619204 -0.00015980576794039
-0.00154039650054078 -0.000159054290655806
-0.00155621844323136 -0.000156790367938154
-0.0015717419263639 -0.0001530968539334
-0.00158682876297551 -0.000148067095948984
-0.00160134984631173 -0.000141803702660848
-0.00161518759457965 -0.000134417051541668
-0.00162823513606853 -0.00012602397021465
-0.00164039817182274 -0.000116746352320751
-0.00165159451000965 -0.000106709751807741
-0.00166175441519419 -9.60419916900272e-05
-0.00167082130685604 -8.48719248982149e-05
-0.00167875152658978 -7.33279852631396e-05
-0.00168551387246354 -6.15371474017522e-05
-0.00169109006470783 -4.96235970861883e-05
-0.00169547369799826 -3.77077567560187e-05
-0.00169867059072332 -2.59051784814365e-05
-0.00170069750443332 -1.43256943454043e-05
-0.00170158202744359 -3.07252248616138e-06
-0.00170136152711007 7.75843325611178e-06
-0.00170008268418168 1.80792208898276e-05
-0.00169780067790343 2.78103875317799e-05
-0.00169457802187239 3.68813986771943e-05
-0.00169048386555061 4.5230947371121e-05
-0.00168559294653349 5.28072112470628e-05
-0.00167998489205914 5.95679577794668e-05
-0.00167374305485445 6.54805226099519e-05
-0.00166695299973633 7.05218567458611e-05
-0.0016597032020975 7.46781785641992e-05
-0.00165208167185848 7.79449163310731e-05
-0.0016441787474294 8.03263237709805e-05
-0.00163608104210169 8.18350167299603e-05
-0.00162787482008418 8.24915528133492e-05
-0.0016196445995089 8.23239459749909e-05
-0.00161147105694347 8.13670722510349e-05
-0.00160343149303799 7.96620541951415e-05
-0.0015955976206218 7.72556448533332e-05
-0.00158803731091643 7.4199401677935e-05
-0.00158081273087902 7.05491795038209e-05
-0.00157398045960069 6.63642899328906e-05
-0.00156759078980096 6.17068637787216e-05
-0.00156168784422702 5.66410612084642e-05
-0.00155630899356386 5.1232463206072e-05
-0.00155148555491122 4.55472960557394e-05
-0.00154724151120087 3.96518084410208e-05
-0.00154359490816724 3.36115974284359e-05
-0.00154055692301303 2.74910251187691e-05
-0.00153813244647348 2.13526463114282e-05
-0.00153632019922059 1.52566432115641e-05
-0.00153511296468429 9.26037255995208e-06
-0.00153449793828869 3.41789465482464e-06
-0.00153445742593706 -2.22039088459702e-06
-0.00153496884400465 -7.60808474221508e-06
-0.00153600448650188 -1.27030870303752e-05
-0.00153753373696125 -1.74678415652914e-05
-0.00153952155503444 -2.18694885954064e-05
-0.00154192975705786 -2.58800397431339e-05
-0.00154471852945157 -2.94764086497314e-05
-0.00154784584664148 -3.26404684916267e-05
-0.00155126700539972 -3.53589661348059e-05
-0.00155493753522798 -3.76235522193762e-05
-0.00155881191779323 -3.94305582741895e-05
-0.00156284370334404 -4.07809496165171e-05
-0.00156698795543887 -4.16800574673384e-05
-0.00157120008679663 -4.21373705147847e-05
-0.00157543644137951 -4.21662487651857e-05
-0.00157965487647423 -4.17836952743942e-05
-0.00158381534477658 -4.10100066822008e-05
-0.00158787942873606 -3.98684542496879e-05
-0.00159181278528607 -3.83849253952147e-05
-0.00159558165339114 -3.65875430749073e-05
-0.0015991559972663 -3.45064159101354e-05
-0.0016025096228028 -3.21731545990441e-05
-0.00160561854776042 -2.96205167529064e-05
-0.00160846286441943 -2.68820935759488e-05
-0.00161102522619006 -2.39918759548362e-05
-0.00161329236101626 -2.09840375430972e-05
-0.00161525425647915 -1.7892439421293e-05
-0.00161690427621526 -1.47504403537456e-05
-0.0016182386942643 -1.15904991161699e-05
-0.00161925809205717 -8.44395431631988e-06
-0.00161996433162265 -5.3407566413085e-06
-0.00162036393163776 -2.3092179266622e-06
-0.00162046469138555 6.24147840628831e-07
-0.00162027813548335 3.43488967060129e-06
-0.0016198175348229 6.10069223899137e-06
-0.00161909872148262 8.60159678231993e-06
-0.00161813822608174 1.0920006716147e-05
-0.00161695642099775 1.30408178331232e-05
-0.00161557239809152 1.49514512037095e-05
-0.00161400815965949 1.66418421431371e-05
-0.00161228698862091 1.8104523517501e-05
-0.00161043077096221 1.93345336539015e-05
-0.00160846302253413 2.03292946927285e-05
-0.00160640760848309 2.1088638075715e-05
-0.00160428781192611 2.16146959225397e-05
-0.00160212668319439 2.19117705246415e-05
-0.00159994703983019 2.1986204016099e-05
-0.00159777053526136 2.18462297948292e-05
-0.00159561847370633 2.15018674683465e-05
-0.00159351087884717 2.09647127268589e-05
-0.00159146614457942 2.02477599398517e-05
-0.00158950161708537 1.93652063515989e-05
-0.00158763324558456 1.83323036372417e-05
-0.00158587546591437 1.71651586433972e-05
-0.00158423968712547 1.58804907101173e-05
-0.001582737434692 1.44954268252686e-05
-0.00158137825503465 1.30274581923634e-05
-0.00158016983193053 1.14941921269888e-05
-0.00157911635669316 9.9131021462225e-06
-0.00157822283553764 8.30139186974564e-06
-0.00157749171353491 6.67594256345226e-06
-0.00157692299102151 5.0530832457154e-06
-0.00157651550416479 3.44839307287638e-06
-0.00157626727420932 1.87670125551936e-06
-0.00157617434331964 3.51936890135402e-07
-0.00157623007608513 -1.1130413857779e-06
-0.00157642911764059 -2.50649444554282e-06
-0.0015767637847917 -3.81776636884421e-06
-0.00157722534658018 -5.03743019772027e-06
-0.00157780332579019 -6.15738218632709e-06
-0.00157848771083939 -7.17085999069514e-06
-0.00157926814087464 -8.07231502317588e-06
-0.00158013320727717 -8.85751917846002e-06
-0.00158107091932497 -9.52352413285091e-06
-0.00158206940268491 -1.0068671399911e-05
-0.00158311631733653 -1.0492551011795e-05
-0.00158419967248111 -1.07959386801335e-05
-0.00158530759371232 -1.09807260323265e-05
-0.00158642809018542 -1.10499205659738e-05
-0.0015875501023587 -1.10074972154738e-05
-0.00158866245425596 -1.08583615826661e-05
-0.00158975466837552 -1.06082702596691e-05
-0.00159081684927691 -1.0263740733816e-05
-0.00159184026566037 -9.831925096408e-06
-0.00159281630263022 -9.32051388735092e-06
-0.0015937376258498 -8.73768959575074e-06
-0.00159459713380581 -8.09198978453019e-06
-0.0015953891219636 -7.39223200904273e-06
-0.00159610870069286 -6.64738967883174e-06
-0.00159675179526942 -5.86650465667714e-06
-0.00159731631003128 -5.05857094388217e-06
-0.0015977987523351 -4.23244753377402e-06
-0.00159819807426159 -3.39690384250119e-06
-0.00159851357714393 -2.5604213758761e-06
-0.0015987453772293 -1.73115921393805e-06
-0.00159889498775728 -9.16885245041472e-07
-0.00159896392197734 -1.24894585599474e-07
-0.00159895602145769 6.38077241299026e-07
-0.00159887338154732 1.36583557054702e-06
-0.00159871996025252 2.05274626871189e-06
-0.00159849994842297 2.69378565435145e-06
-0.00159821800258309 3.28458218229726e-06
-0.00159787959417825 3.82140549144571e-06
-0.00159749007825288 4.30122628291272e-06
-0.00159705562477257 4.72168004764816e-06
-0.00159658205447114 5.08109065047022e-06
-0.001596075653757 5.37842502884453e-06
-0.00159554282546782 5.61332036333107e-06
-0.0015949905545319 5.7860840463807e-06
-0.00159442419607407 5.89758697714572e-06
-0.0015938494544756 5.94920727527695e-06
-0.00159327226695934 5.94284291887461e-06
-0.00159269868717376 5.88089550265513e-06
-0.00159213395386902 5.76621230978846e-06
-0.00159158318938816 5.60203370065253e-06
-0.00159105035192608 5.39188642832976e-06
-0.00159054068025444 5.13965211207836e-06
-0.00159005813258041 4.84944622190008e-06
-0.00158960643428563 4.52562876438226e-06
-0.00158918849584678 4.17268844289385e-06
-0.00158880722774287 3.79522808751013e-06
-0.00158846484196181 3.39790311847322e-06
-0.00158816308482981 2.98535812835798e-06
-0.00158790323701143 2.56222686885522e-06
-0.00158768611350774 2.13304712666681e-06
-0.00158751218007101 1.70222265520164e-06
-0.00158738120395815 1.27400691910895e-06
-0.00158729283600635 8.52439627350472e-07
-0.00158724626138702 4.41354020332721e-07
-0.00158724019960451 4.43098309159298e-08
-0.00158727185675679 -3.35459178644261e-07
-0.00158734076724289 -6.9500921777145e-07
-0.0015874446028111 -1.03164639189529e-06
-0.00158758080237142 -1.34303816067948e-06
-0.00158774703765791 -1.62717626818438e-06
-0.00158794016548987 -1.88240474603658e-06
-0.00158815750834115 -2.1073991519591e-06
-0.00158839569018572 -2.30120816127209e-06
-0.00158865156782141 -2.46321288048927e-06
-0.00158892199803925 -2.59313047786332e-06
-0.00158920395403885 -2.69099963844956e-06
-0.00158949429259877 -2.75714075733329e-06
-0.00158978963766021 -2.79219120848006e-06
-0.00159008684598936 -2.79707190535952e-06
-0.00159038312359318 -2.77295556190462e-06
-0.00159067567647409 -2.72124226674536e-06
-0.00159096171063012 -2.64353950870223e-06
-0.00159123878130148 -2.54165228486905e-06
-0.00159150456014048 -2.41753501600016e-06
-0.00159175683521181 -2.27329069552218e-06
-0.001591993743824 -2.11113466629626e-06
-0.00159221365611466 -1.93335836004067e-06
-0.00159241482580455 -1.74233020621583e-06
-0.00159259643793667 -1.54044313103763e-06
-0.00159275744472357 -1.33008918400563e-06
-0.00159289679837774 -1.11365131665706e-06
-0.00159301438243542 -8.93479058496167e-07
-0.00159310984760328 -6.71863045685015e-07
-0.00159318307742034 -4.51016940686131e-07
-0.0015932343046738 -2.33052081619653e-07
-0.00159326411139943 -1.99621005705182e-08
-0.00159327377812905 1.8644499460673e-07
-0.00159326318841216 3.84470036009248e-07
-0.00159323327353919 5.72533291213009e-07
-0.00159318508121905 7.49209010460661e-07
-0.00159311977557933 9.13232664969955e-07
-0.00159303875358231 1.06353354122604e-06
-0.00159294329577825 1.19919670323168e-06
-0.00159283526479842 1.31951733536951e-06
-0.00159271594120062 1.42394824023768e-06
-0.00159258683837643 1.51209985294653e-06
-0.00159244970255219 1.58376367921022e-06
-0.00159230616354249 1.63891422643772e-06
-0.00159215808399599 1.67768720890701e-06
-0.00159200686090297 1.70037237122675e-06
-0.00159185435691804 1.70739345654278e-06
-0.00159170185262259 1.69934633296995e-06
-0.00159155074501442 1.67688303924336e-06
-0.00159140254750973 1.6408041566087e-06
-0.00159125865711157 1.59201169680488e-06
-0.00159112023799368 1.53148379898233e-06
-0.00159098845433184 1.46028914481278e-06
-0.00159086435388751 1.37955260826991e-06
-0.00159074863517699 1.29044255469367e-06
-0.00159064234596323 1.19415813892862e-06
-0.00159054583551758 1.09192391120546e-06
-0.00159045991877295 9.84969830151479e-07
-0.00159038482858514 8.74511401606736e-07
-0.00159032137988737 7.61793069275902e-07
-0.0015902686413812 6.48001445066978e-07
-0.00159022731158136 5.34232452371742e-07
-0.00159019762334175 4.21611028470363e-07
-0.00159017922743856 3.11215036515522e-07
-0.00159017165823001 2.04002826423611e-07
-0.0015901745664893 1.00905519829966e-07
-0.00159018748657158 2.73837594562247e-09
-0.00159020890509175 -8.97992874651177e-08
-0.00159023928772376 -1.7609154954642e-07
-0.0015902780524032 -2.55538761187874e-07
-0.00159032438423256 -3.27653561142107e-07
-0.00159037746831271 -3.9202830229835e-07
-0.0015904368389887 -4.48344104166947e-07
-0.00159050121569611 -4.96379868295731e-07
-0.00159057013277616 -5.36005129528702e-07
-0.00159064242607595 -5.67181747029166e-07
-0.001590717513518 -5.8994228172753e-07
-0.00159079434736137 -6.04411632880772e-07
-0.0015908723455254 -6.10781797241714e-07
-0.00159095034385057 -6.09331635691775e-07
-0.00159102810949964 -6.00379966836302e-07
-0.0015911044783111 -5.84307112581873e-07
-0.00159117886819874 -5.61567715252708e-07
-0.00159125081349107 -5.32645402804768e-07
-0.00159131949926963 -4.98074527159354e-07
-0.00159138445986143 -4.58411177568747e-07
-0.00159144522959289 -4.14244059191652e-07
-0.00159150134278973 -3.66190846465641e-07
-0.00159155245019303 -3.14878315438999e-07
-0.00159159831895915 -2.60933233329618e-07
-0.00159163848341359 -2.04985963499579e-07
-0.00159167340920491 -1.47659691729937e-07
-0.00159170251424421 -8.95467672129996e-08
-0.00159172579851928 -3.12359145651457e-08
-0.00159174407692639 2.67293610819091e-08
-0.00159175688379449 8.38762587074997e-08
-0.00159176386986661 1.3967947806113e-07
-0.001591765267963 1.93631779230144e-07
-0.0015917614273205 2.45283877183677e-07
-0.00159175246434625 2.94233595046539e-07
-0.00159173884469394 3.40111377570131e-07
-0.00159172080118781 3.82592901461865e-07
-0.00159169856665302 4.21413696109882e-07
-0.00159167272316141 4.56330964727436e-07
-0.00159164361995548 4.8716895945901e-07
-0.00159161160627867 5.1379721519528e-07
-0.00159157714779025 5.36116090001147e-07
-0.00159154059373582 5.54092913458525e-07
-0.00159150252619203 5.67724034853566e-07
-0.00159146329440602 5.77056512877174e-07
-0.00159142371328719 5.82182681312557e-07
-0.00159138296793015 5.83204035487932e-07
-0.0015913428045678 5.80245461955379e-07
-0.00159130322320548 5.73556912274187e-07
-0.00159126445667773 5.6332678000437e-07
-0.00159122673782027 5.49797792800543e-07
-0.00159119053229991 5.33230778721318e-07
-0.00159115618936871 5.13910095217029e-07
-0.00159112394186357 4.92138263665147e-07
-0.00159109402262168 4.68228654558229e-07
-0.00159106654806506 4.42503709571985e-07
-0.00159104186744638 4.1528404464634e-07
-0.00159101974794166 3.86890289302383e-07
-0.00159100053880336 3.57641284347873e-07
-0.00159098424003816 3.2785219622724e-07
-0.00159097120089851 2.97838227885161e-07
-0.00159096095572956 2.67914602394609e-07
-0.00159095373736743 2.38345791071714e-07
-0.00159094931298713 2.09408968512197e-07
-0.00159094791542444 1.81352309498744e-07
-0.00159094931185396 1.54431242594598e-07
-0.00159095326944934 1.2885773171486e-07
-0.00159095967179917 1.04825626875309e-07
-0.00159096840249139 8.24961626685308e-08
-0.0015909794615293 6.20287554510914e-08
-0.00159099238325406 4.3550240561664e-08
-0.00159100705125231 2.71548185723958e-08
-0.00159102311627939 1.29168047401568e-08
-0.00159104057833631 8.8511090278365e-10
-0.00159105885534687 -8.91487437462615e-09
-0.00159107724881706 -1.65627685589482e-08
-0.00159109587516152 -2.21020911352629e-08
-0.00159111566570248 -2.55582441587585e-08
-0.00159113545628589 -2.6956520671076e-08
-0.00159115524691001 -2.63802452870015e-08
-0.0015911750375732 -2.39091262145189e-08
-0.00159119424619679 -1.96318801876333e-08
-0.00159121287277757 -1.37006566039584e-08
-0.00159123126655976 -6.20969773072343e-09
-0.00159124966037277 2.77212266505775e-09
-0.00159126712289084 1.3118115112622e-08
-0.00159128342128051 2.46851449369856e-08
-0.00159129843912308 3.73138173840389e-08
-0.00159131217641477 5.08266288853248e-08
-0.001591324516737 6.50623440102917e-08
-0.00159133546008625 7.98524961239831e-08
-0.00159134489004384 9.50340531796605e-08
-0.00159135269019078 1.10434945598849e-07
-0.00159135909335482 1.25908410191731e-07
-0.00159136398311731 1.41296863809574e-07
-0.00159136712664479 1.56460808945652e-07
-0.00159136887318009 1.71249895099523e-07
-0.00159136922272075 1.85542741795583e-07
-0.00159136817526435 1.99219779297561e-07
-0.0015913657308087 2.12174126938539e-07
-0.00159136200576712 2.24309779311106e-07
-0.00159135711655324 2.35541580068484e-07
-0.00159135117958071 2.45786191277724e-07
-0.00159134419484837 2.54987454208314e-07
-0.00159133627877083 2.63107313609856e-07
-0.00159132789700864 2.70102257292053e-07
-0.00159131858389993 2.75952399153323e-07
-0.00159130915435228 2.80657663970067e-07
-0.0015912986770425 2.84209090872382e-07
-0.00159128819970881 2.86599329318586e-07
-0.00159127772235211 2.87873675543769e-07
-0.00159126724497351 2.88084657012826e-07
-0.0015912567675738 2.87270316265349e-07
-0.00159124629015379 2.85472326440046e-07
-0.00159123581271437 2.82732345673953e-07
-0.00159122568450239 2.79088395663973e-07
-0.00159121637118186 2.74659983602767e-07
-0.00159120705784641 2.69508778118357e-07
-0.0015911986758203 2.63699925709534e-07
-0.00159119052661347 2.57333095933602e-07
-0.00159118342513475 2.50473456108634e-07
-0.00159117678930944 2.43224306241134e-07
-0.0015911709683855 2.35670740145446e-07
-0.00159116596236435 2.27890690058746e-07
-0.00159116165483256 2.19971088063185e-07
-0.00159115816220749 2.12007932963711e-07
-0.00159115560090561 2.04061019934751e-07
-0.00159115362168262 1.96211874727936e-07
-0.0015911524573708 1.8853838131363e-07
-0.00159115222438676 1.81100312638327e-07
-0.00159115245707033 1.73961107904403e-07
-0.00159115362108438 1.67185934572223e-07
-0.00159115536718337 1.60805629898227e-07
-0.00159115769536893 1.54898084537346e-07
-0.00159116060564119 1.49468731671181e-07
-0.00159116409800154 1.44586411677969e-07
-0.00159116770678833 1.40242107061594e-07
-0.00159117236332532 1.36473770893868e-07
-0.0015911770198747 1.33306861802536e-07
-0.00159118167643608 1.30723264235653e-07
-0.00159118656583982 1.2870302955346e-07
-0.00159119238657896 1.272895813449e-07
-0.00159119820733093 1.26495660770449e-07
-0.00159120402809514 1.26297740037112e-07
-0.00159120984887112 1.26670442542363e-07
-0.00159121566965852 1.27595652791109e-07
-0.0015912214904567 1.29046212420689e-07
-0.00159122614711061 1.30949734761823e-07
-0.00159123080377225 1.3322823965727e-07
-0.001591235460441 1.35854569493997e-07
-0.00159124011711699 1.38832332520714e-07
-0.00159124430813833 1.4213800618657e-07
-0.0015912478006721 1.45670185356043e-07
-0.00159125129320982 1.49392569812041e-07
-0.00159125455292076 1.5330699266856e-07
-0.00159125688131082 1.57321126000932e-07
-0.00159125920970218 1.61400482554929e-07
-0.00159126107243313 1.65526959546144e-07
-0.00159126223667122 1.69624520973867e-07
-0.00159126340090824 1.73669547466176e-07
-0.00159126398306712 1.7764758093703e-07
-0.00159126398314611 1.81482571917272e-07
-0.00159126398322195 1.85161762232474e-07
-0.00159126351763314 1.88685194292315e-07
-0.00159126235354731 1.91976817246202e-07
-0.00159126118945631 1.9501845381124e-07
-0.00159126002536037 1.97819154264776e-07
-0.00159125816276725 2.00375343974426e-07
-0.00159125583450604 2.02614575755991e-07
-0.00159125350623839 2.04540409446644e-07
-0.00159125117796443 2.06158279725173e-07
-0.00159124884968441 2.0748268636632e-07
-0.00159124652139859 2.08526310308563e-07
-0.0015912441931073 2.0930363641565e-07
-0.0015912418648107 2.09825548925483e-07
-0.001591239536509 2.10097460167323e-07
-0.00159123720820247 2.10135688904611e-07
-0.00159123487989122 2.09945669877893e-07
-0.00159123255157547 2.09536453332857e-07
-0.00159123022325541 2.08918916007518e-07
-0.00159122789493123 2.0810029668927e-07
-0.00159122556660318 2.07093276194555e-07
-0.00159122323827103 2.05888804276708e-07
-0.00159122090993547 2.04519488735354e-07
-0.00159121858159649 2.02983510641291e-07
-0.00159121625325405 2.01279058445236e-07
-0.00159121392490834 1.9941518989504e-07
-0.00159121241146757 1.97428088234279e-07
-0.00159121124727219 1.95402902340025e-07
-0.0015912100830761 1.93345116025225e-07
-0.00159120891887953 1.91261960577686e-07
-0.0015912077546824 1.89153450846642e-07
-0.00159120670690007 1.87017760433739e-07
-0.0015912067068568 1.84918211603401e-07
-0.00159120670681531 1.82905617206381e-07
-0.0015912067067755 1.80972723515927e-07
-0.00159120670673728 1.79119545472777e-07
-0.00159120670670063 1.77340633518566e-07
-0.00159120670666542 1.75632371994386e-07
-0.00159120787078639 1.74047205675514e-07
-0.0015912090349111 1.72643187644825e-07
-0.00159121019903927 1.71405824757041e-07
-0.00159121136317083 1.70333312872291e-07
-0.00159121252730558 1.69414775283568e-07
-0.00159121369144342 1.68646596302423e-07
-0.00159121485558423 1.68023341279555e-07
-0.0015912160197279 1.67539575567292e-07
-0.00159121718387429 1.67186234008304e-07
-0.00159121834802331 1.66961512462326e-07
-0.00159121951217487 1.66858157291794e-07
-0.0015912206763288 1.66872560308307e-07
-0.00159122184048504 1.66997460403321e-07
-0.00159122300464351 1.67229234478053e-07
-0.0015912241688041 1.67566085862133e-07
-0.00159122533296673 1.6800075350963e-07
-0.00159122649713137 1.68535063818382e-07
-0.0015912276612979 1.691599441613e-07
-0.00159122882546622 1.69869959889965e-07
-0.00159122998963625 1.70665125914571e-07
-0.00159123115380796 1.71539992646107e-07
-0.00159123231798126 1.72494575025639e-07
-0.00159123348215612 1.73523423493879e-07
-0.00159123464633243 1.74621103402192e-07
-0.00159123557767945 1.75787636376806e-07
-0.00159123557770324 1.76943390158371e-07
-0.0015912355777261 1.78052036213863e-07
-0.00159123557774803 1.79117212490933e-07
-0.00159123557776907 1.80137092590903e-07
-0.00159123557778922 1.81115314523084e-07
-0.00159123557780859 1.82055493885955e-07
-0.00159123557782718 1.82957630709722e-07
-0.00159123557784499 1.83821724993816e-07
-0.00159123557786212 1.84653211387633e-07
-0.00159123557787855 1.8545027834144e-07
-0.00159123557789432 1.86214737373419e-07
-0.00159123557790941 1.86948407534976e-07
-0.00159123476301588 1.87625967377775e-07
-0.00159123359887343 1.88171333212069e-07
-0.00159123243472823 1.88580825365376e-07
-0.00159123127058036 1.88861704944669e-07
-0.00159123010642992 1.89019406599314e-07
-0.00159122894227703 1.89055726968255e-07
-0.00159122777812179 1.88979738709248e-07
-0.00159122661396429 1.88793245931986e-07
-0.00159122544980459 1.88499871734831e-07
-0.00159122428564282 1.88106869756431e-07
-0.00159122312147907 1.87617855624848e-07
-0.00159122219014418 1.8703824983352e-07
-0.00159122219013183 1.86440453353384e-07
-0.00159122219012005 1.85868011096172e-07
-0.00159122219010871 1.85317307462897e-07
-0.00159122219009782 1.84788342423619e-07
-0.00159122219008737 1.84282934967552e-07
-0.00159122219007737 1.83797447085045e-07
-0.00159122219006778 1.83331886277366e-07
-0.00159122219005856 1.82884440964618e-07
-0.00159122219004971 1.8245511114661e-07
-0.0015912221900412 1.82042085273789e-07
-0.00159122219003302 1.81645363377163e-07
-0.00159122219002522 1.81264937955584e-07
-0.00159122219001771 1.80900823918892e-07
-0.0015912221900105 1.80551202278172e-07
-0.00159122219000358 1.80216073033477e-07
-0.00159122218999689 1.79891813115949e-07
-0.00159122218999057 1.79583849673143e-07
-0.00159122218998447 1.79288574516956e-07
-0.00159122218997856 1.7900235710793e-07
-0.00159122218997299 1.78730624685627e-07
-0.00159122218996756 1.78467957420464e-07
-0.00159122218996235 1.7821434049278e-07
-0.00159122218995741 1.77975223370099e-07
-0.00159122218995258 1.77739721937264e-07
-0.00159122218994804 1.77520531859229e-07
-0.00159122218994358 1.7730314592146e-07
-0.00159122218993942 1.77102071338545e-07
-0.00159122218993533 1.76902800895083e-07
-0.00159122218993128 1.76707160960682e-07
-0.00159122218992756 1.76526006012218e-07
-0.00159122218992384 1.76344851063808e-07
-0.00159122218992038 1.76178195921201e-07
-0.00159122218991707 1.76018786975644e-07
-0.0015912221899141 1.75873863017664e-07
-0.00159122218991113 1.75728939058654e-07
-0.00159122218990819 1.75587645608245e-07
-0.00159122312122908 1.75489752623158e-07
-0.00159122428538302 1.75504155639386e-07
-0.00159122498387773 1.75623648677708e-07
-0.00159122498388066 1.75764942127941e-07
-0.00159122498388327 1.7589175059141e-07
-0.00159122498388587 1.76018559055585e-07
-0.00159122498388847 1.7614536751919e-07
-0.00159122498389081 1.76257676177629e-07
-0.00159122498389304 1.76366369146507e-07
-0.00159122498389516 1.76467808508138e-07
-0.00159122498389702 1.76558385982342e-07
-0.00159122498389888 1.7664896345652e-07
-0.00159122498390074 1.76739540930861e-07
-0.0015912249839026 1.768301184047e-07
-0.00159122498390446 1.76920695879108e-07
-0.00159122498390617 1.7700220819624e-07
-0.00159122498390765 1.77074670175664e-07
-0.00159122498390914 1.77147132154694e-07
-0.00159122498391063 1.77219594134172e-07
-0.00159122498391211 1.77292056113555e-07
-0.0015912249839136 1.77364518092789e-07
-0.00159122498391494 1.77427914915275e-07
-0.00159122498391605 1.77482261399674e-07
-0.00159122498391717 1.77536607884289e-07
-0.00159122498391828 1.77590954368714e-07
-0.0015912249839194 1.77645300852882e-07
-0.00159122498392051 1.77699647337754e-07
-0.00159122498392163 1.7775399382222e-07
-0.00159122498392275 1.77808340306551e-07
-0.00159122498392375 1.77855433183783e-07
-0.00159122498392449 1.77891664173536e-07
-0.00159122498392524 1.77927895163166e-07
-0.00159122498392598 1.77964126152851e-07
-0.00159122498392672 1.78000357142264e-07
-0.00159122498392747 1.78036588131922e-07
-0.00159122498392821 1.78072819121674e-07
-0.00159122498392895 1.78109050111644e-07
-0.0015912249839297 1.78145281101369e-07
-0.00159122498393044 1.78181512090633e-07
-0.00159122498393118 1.78217743080399e-07
-0.00159122498393193 1.78253974069921e-07
-0.00159122498393263 1.78286574551101e-07
-0.00159122498393301 1.78304690046086e-07
-0.00159122498393338 1.78322805540881e-07
-0.00159122498393375 1.78340921035648e-07
-0.00159122498393412 1.7835903653047e-07
-0.00159122498393449 1.78377152025441e-07
-0.00159122498393486 1.78395267520033e-07
-0.00159122498393524 1.78413383014909e-07
-0.00159122498393561 1.78431498509731e-07
-0.00159122498393598 1.78449614004648e-07
-0.00159122498393635 1.78467729499619e-07
-0.00159122498393672 1.78485844994509e-07
-0.0015912249839371 1.78503960488938e-07
-0.00159122498393747 1.78522075984004e-07
-0.00159122498393784 1.78540191478853e-07
-0.00159122498393821 1.78558306973743e-07
-0.00159122498393858 1.78576422468673e-07
-0.00159122498393895 1.78594537963333e-07
-0.00159122498393933 1.78612653457978e-07
-0.0015912249839397 1.78630768952895e-07
-0.00159122498394007 1.78648884447934e-07
-0.00159122498394044 1.78666999942973e-07
-0.00159122498394081 1.78685115437348e-07
-0.00159122498394118 1.78703230932481e-07
-0.00159122498394156 1.78721346427303e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
};
\addplot [very thick, learnedWithSideInfo, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131181321129939 0.0252802280005022
0.12690421079167 -0.0399002670706551
0.0944507981809875 -0.0861568334898107
0.0449165171346369 -0.107541588477213
-0.00864360324664406 -0.102431373693198
-0.0537161660234296 -0.074703806054975
-0.0810544466896602 -0.0333148106836566
-0.0867180535301455 0.00997515787192305
-0.0726392072282452 0.0440454186803454
-0.045434243099127 0.0617508561744349
-0.0138702043514642 0.0617468935926043
0.0139829346956975 0.0478491679837557
0.0327245828214036 0.0264160705211209
0.040197700433741 0.00372541049531807
0.0370650301101962 -0.0153327825436378
0.0260058495702296 -0.0276053197620182
0.0108224950035826 -0.0317608344644175
-0.00447172890865356 -0.0282678285067166
-0.0164995109551214 -0.0191312470169684
-0.0231557531767589 -0.00731548213391928
-0.0238941843217746 0.00404791763589505
-0.0196093536674299 0.0124432386379356
-0.0121812184387883 0.0165022200475997
-0.00385038662228969 0.0161380265051567
0.00337470367658196 0.0123013388585754
0.00812650062886289 0.00652170600659563
0.00984600856252865 0.000431136118287229
0.00873629057430193 -0.00460329867693221
0.00556860724297454 -0.00770075894547253
0.00141302628122065 -0.00855028219758464
-0.00264204273366186 -0.00737438219745297
-0.00572639654889225 -0.00479426719204738
-0.00733939339687693 -0.0016308339065648
-0.00739558752163135 0.00131037239369908
-0.00616976529808186 0.00341851365492709
-0.00416984835557044 0.00438181594676535
-0.00197995448310235 0.00420269532172055
-0.000115995479051329 0.00313642220094937
0.0010751840034559 0.00158433714911927
0.00145935282620546 -2.31337050325465e-05
0.00110352060861369 -0.00132536967513527
0.00022337278949325 -0.00209560632025662
-0.00089122370150761 -0.00226448742495482
-0.00195285259895834 -0.00190614954397887
-0.00273871393008829 -0.00119625487671362
-0.00312753404366284 -0.000355390765964705
-0.0031075959075637 0.000407531831196872
-0.00275915520919036 0.000939320791552229
-0.00221973558256385 0.00116616001634381
-0.00164317399055587 0.00109514391820482
-0.00116274048132507 0.000797486966759387
-0.00086573891941777 0.000380732994916474
-0.000783006543281085 -4.16753462240284e-05
-0.000892743946956706 -0.000376277025642792
-0.00113510792760089 -0.00056621563591109
-0.00143236520958295 -0.000596808759987947
-0.00170920499328183 -0.000490938577834057
-0.00190876633907785 -0.000297120678076027
-0.00200167330083745 -7.41578854866872e-05
-0.00198738273315904 0.000123654276914274
-0.00188895770088517 0.000257617868696219
-0.00174361792849878 0.00031024120045013
-0.00159194018026048 0.00028513157137716
-0.00146833690072849 0.000202266704458325
-0.00139466031700326 9.05552403333926e-05
-0.00137775801520397 -2.01647922894118e-05
-0.00141076757295986 -0.000105830101867344
-0.00147717413076824 -0.000152340585299879
-0.00155621844323136 -0.000156790367938154
-0.00162823513606853 -0.00012602397021465
-0.00167875152658978 -7.33279852631396e-05
-0.00170069750443332 -1.43256943454043e-05
-0.00169457802187239 3.68813986771943e-05
-0.00166695299973633 7.05218567458611e-05
-0.00162787482008418 8.24915528133492e-05
-0.00158803731091643 7.4199401677935e-05
-0.00155630899356386 5.1232463206072e-05
-0.00153813244647348 2.13526463114282e-05
-0.00153496884400465 -7.60808474221508e-06
-0.00154471852945157 -2.94764086497314e-05
-0.00156284370334404 -4.07809496165171e-05
-0.00158381534477658 -4.10100066822008e-05
-0.0016025096228028 -3.21731545990441e-05
-0.00161525425647915 -1.7892439421293e-05
-0.00162036393163776 -2.3092179266622e-06
-0.00161813822608174 1.0920006716147e-05
-0.00161043077096221 1.93345336539015e-05
-0.00159994703983019 2.1986204016099e-05
-0.00158950161708537 1.93652063515989e-05
-0.00158137825503465 1.30274581923634e-05
-0.00157692299102151 5.0530832457154e-06
-0.00157642911764059 -2.50649444554282e-06
-0.00157926814087464 -8.07231502317588e-06
-0.00158419967248111 -1.07959386801335e-05
-0.00158975466837552 -1.06082702596691e-05
-0.00159459713380581 -8.09198978453019e-06
-0.0015977987523351 -4.23244753377402e-06
-0.00159896392197734 -1.24894585599474e-07
-0.00159821800258309 3.28458218229726e-06
-0.001596075653757 5.37842502884453e-06
-0.00159327226695934 5.94284291887461e-06
-0.00159054068025444 5.13965211207836e-06
-0.00158846484196181 3.39790311847322e-06
-0.00158738120395815 1.27400691910895e-06
-0.00158734076724289 -6.9500921777145e-07
-0.00158815750834115 -2.1073991519591e-06
-0.00158949429259877 -2.75714075733329e-06
-0.00159096171063012 -2.64353950870223e-06
-0.00159221365611466 -1.93335836004067e-06
-0.00159301438243542 -8.93479058496167e-07
-0.00159327377812905 1.8644499460673e-07
-0.00159303875358231 1.06353354122604e-06
-0.00159244970255219 1.58376367921022e-06
-0.00159170185262259 1.69934633296995e-06
-0.00159098845433184 1.46028914481278e-06
-0.00159045991877295 9.84969830151479e-07
-0.00159019762334175 4.21611028470363e-07
-0.00159020890509175 -8.97992874651177e-08
-0.0015904368389887 -4.48344104166947e-07
-0.00159079434736137 -6.04411632880772e-07
-0.00159117886819874 -5.61567715252708e-07
-0.00159150134278973 -3.66190846465641e-07
-0.00159170251424421 -8.95467672129996e-08
-0.001591765267963 1.93631779230144e-07
-0.00159169856665302 4.21413696109882e-07
-0.00159154059373582 5.54092913458525e-07
-0.0015913428045678 5.80245461955379e-07
-0.00159115618936871 5.13910095217029e-07
-0.00159101974794166 3.86890289302383e-07
-0.00159095373736743 2.38345791071714e-07
-0.00159095967179917 1.04825626875309e-07
-0.00159102311627939 1.29168047401568e-08
-0.00159111566570248 -2.55582441587585e-08
-0.00159121287277757 -1.37006566039584e-08
-0.00159129843912308 3.73138173840389e-08
-0.00159135269019078 1.10434945598849e-07
-0.00159136922272075 1.85542741795583e-07
-0.00159135117958071 2.45786191277724e-07
-0.00159130915435228 2.80657663970067e-07
-0.0015912567675738 2.87270316265349e-07
-0.00159120705784641 2.69508778118357e-07
-0.0015911709683855 2.35670740145446e-07
-0.00159115362168262 1.96211874727936e-07
-0.00159115536718337 1.60805629898227e-07
-0.00159117236332532 1.36473770893868e-07
-0.00159119820733093 1.26495660770449e-07
-0.00159122614711061 1.30949734761823e-07
-0.0015912478006721 1.45670185356043e-07
-0.00159126107243313 1.65526959546144e-07
-0.00159126398322195 1.85161762232474e-07
-0.00159125816276725 2.00375343974426e-07
-0.00159124652139859 2.08526310308563e-07
-0.00159123487989122 2.09945669877893e-07
-0.00159122323827103 2.05888804276708e-07
-0.00159121241146757 1.97428088234279e-07
-0.00159120670690007 1.87017760433739e-07
-0.00159120670670063 1.77340633518566e-07
-0.00159121136317083 1.70333312872291e-07
-0.00159121718387429 1.67186234008304e-07
-0.00159122300464351 1.67229234478053e-07
-0.00159122882546622 1.69869959889965e-07
-0.00159123464633243 1.74621103402192e-07
-0.00159123557776907 1.80137092590903e-07
-0.00159123557786212 1.84653211387633e-07
-0.00159123359887343 1.88171333212069e-07
-0.00159122777812179 1.88979738709248e-07
-0.00159122219014418 1.8703824983352e-07
-0.00159122219008737 1.84282934967552e-07
-0.0015912221900412 1.82042085273789e-07
-0.00159122219000358 1.80216073033477e-07
-0.00159122218997299 1.78730624685627e-07
-0.00159122218994804 1.77520531859229e-07
-0.00159122218992756 1.76526006012218e-07
-0.00159122218991113 1.75728939058654e-07
-0.00159122498388066 1.75764942127941e-07
-0.00159122498389304 1.76366369146507e-07
-0.0015912249839026 1.768301184047e-07
-0.00159122498391063 1.77219594134172e-07
-0.00159122498391717 1.77536607884289e-07
-0.00159122498392275 1.77808340306551e-07
-0.00159122498392672 1.78000357142264e-07
-0.00159122498393044 1.78181512090633e-07
-0.00159122498393338 1.78322805540881e-07
-0.00159122498393524 1.78413383014909e-07
-0.0015912249839371 1.78503960488938e-07
-0.00159122498393895 1.78594537963333e-07
-0.00159122498394081 1.78685115437348e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
-0.00159122498394163 1.78723150567162e-07
};
\addplot [very thick, learnedWithoutSideInfo]
table {%
0.1 0.1
0.109269053436191 0.0889836670136178
0.111595353042118 0.073315306235741
0.109752164231319 0.0564314083268954
0.104955590269717 0.0407671064958819
0.0989451238411656 0.0288326424941496
0.093742453768592 0.0215864759760053
0.0903086667490493 0.0179732265370429
0.0884358538567978 0.0164044957272623
0.0875395027805738 0.0157830100855219
0.0871487421216078 0.0155526143463554
0.0869902282491686 0.0154719346263465
0.0869296868275382 0.015445262126123
0.086907796519388 0.0154370147237411
0.0869003004883217 0.0154346840906263
0.0868978822616964 0.0154341159007051
0.0868971575683226 0.0154340181263381
0.0868969622849617 0.0154340225811133
0.0868969189646004 0.0154340381225577
0.0868969137501729 0.0154340483459331
0.0868969156452665 0.0154340534653856
0.0868969176249443 0.015434055718233
0.0868969187581697 0.0154340566305992
0.0868969192929268 0.0154340569772319
0.0868969195199318 0.0154340571017402
0.0868969196094586 0.0154340571440544
0.0868969196427155 0.0154340571575811
0.0868969196544077 0.0154340571615856
0.0868969196582914 0.0154340571626435
0.0868969196594992 0.0154340571628682
0.0868969196598432 0.0154340571628896
0.0868969196599285 0.0154340571628759
0.0868969196599438 0.0154340571628636
0.0868969196599436 0.0154340571628568
0.0868969196599415 0.0154340571628535
0.0868969196599401 0.0154340571628522
0.0868969196599393 0.0154340571628518
0.0868969196599391 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
};
\addplot [very thick, learnedWithoutSideInfo, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.0989451238411656 0.0288326424941496
0.0871487421216078 0.0155526143463554
0.0868978822616964 0.0154341159007051
0.0868969156452665 0.0154340534653856
0.0868969196094586 0.0154340571440544
0.0868969196598432 0.0154340571628896
0.0868969196599401 0.0154340571628522
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
0.086896919659939 0.0154340571628516
};

==> figures/smd_phase_plots/phase_plot_500_full_space_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.0814326703548431 -0.0593703389167786
0.0146933533251286 0.0994157120585442
-0.113948777318001 -0.149170473217964
-0.102269671857357 -0.059582743793726
0.14642345905304 0.00800876971334219
-0.120429024100304 0.0734910815954208
0.0575935244560242 -0.118745096027851
0.107369937002659 -0.0946406647562981
-0.10917304456234 0.0248330533504486
0.0790728628635406 0.110723488032818
0.135007947683334 0.0542426444590092
0.094056211411953 -0.00504271266981959
-0.0806920900940895 0.0256969090551138
-0.011313253082335 0.0146123403683305
0.0781108066439629 -0.0587609969079494
0.0027543012984097 0.0900809317827225
0.0130529431626201 0.10588750988245
0.046719815582037 -0.118236042559147
0.00119913986418396 0.0214361492544413
-0.11741641908884 0.13514618575573
0.10690388828516 0.101515702903271
-0.109577775001526 0.130772441625595
0.1446193754673 0.0739124044775963
0.0602454729378223 0.131513342261314
0.119452342391014 0.0353347770869732
-0.0453976280987263 0.103371299803257
0.103148713707924 0.103881813585758
-0.0106587847694755 0.12862141430378
0.0305761378258467 0.148217782378197
0.0271146483719349 -0.0453120619058609
0.0154461329802871 -0.0592566542327404
-0.1022744551301 0.0224678944796324
0.106574460864067 -0.0994370207190514
0.0177052356302738 0.0954219922423363
-0.0708518624305725 -0.116321220993996
0.0909851714968681 -0.0404467508196831
0.0655272826552391 0.1428382396698
0.00655771605670452 -0.0415804907679558
0.090212382376194 -0.0269190799444914
0.0353434346616268 0.0693309679627419
0.122076123952866 -0.0534803569316864
-0.115993440151215 0.0696566328406334
0.0889185965061188 0.000178730828338303
-0.00645797653123736 0.0832215324044228
0.00555702205747366 -0.114664785563946
-0.038790125399828 0.125341832637787
-0.110549204051495 0.0725014954805374
0.000527397729456425 0.0933233499526978
-0.0971920117735863 0.102553881704807
-0.0165495947003365 -0.122671686112881
0.0103683480992913 0.0604769848287106
0.140656501054764 -0.0965601950883865
0.130132988095284 -0.065050832927227
0.0271369144320488 -0.140705555677414
-0.0997730568051338 0.147792503237724
-0.0446485057473183 -0.0373512804508209
0.056681826710701 0.0153243187814951
-0.147529870271683 0.0877882689237595
-0.10355319082737 -0.0902270451188087
-0.0846454650163651 0.0965598002076149
0.109903492033482 0.113588035106659
0.0629415512084961 0.0818918719887733
-0.0386061482131481 -0.0599000118672848
-0.0191563609987497 -0.0254993848502636
-0.0314483940601349 0.0302908457815647
-0.083296000957489 0.0287481136620045
0.143578186631203 0.0555927827954292
0.0792634338140488 -0.00019858822633978
0.0404624193906784 -0.00977848283946514
0.122218430042267 0.0976669192314148
0.120517171919346 0.13444621860981
0.0165893789380789 0.0491799786686897
-0.0139660863205791 0.118689060211182
-0.149381875991821 -0.138376742601395
-0.0999322682619095 0.0452727824449539
0.130411967635155 0.0708538144826889
-0.12773634493351 0.0542285479605198
-0.0932100340723991 -0.0937420576810837
0.0293169189244509 0.0323986858129501
0.063817597925663 -0.0317535549402237
-0.0782464295625687 -0.0203660242259502
0.0291480701416731 -0.0172720178961754
0.130338102579117 0.0822987332940102
-0.00978419091552496 -0.0772585049271584
0.0790134966373444 -0.0760266184806824
-0.101918995380402 -0.0402511470019817
0.0819889307022095 0.0886669754981995
0.0250810422003269 -0.0899845138192177
-0.0709231421351433 0.0478549860417843
0.0446740351617336 0.058364812284708
0.125222742557526 0.08504618704319
-0.117338508367538 -0.128298491239548
-0.123497426509857 0.00833962298929691
0.0299272388219833 -0.0787191540002823
-0.0559124685823917 0.069234773516655
-0.0579375252127647 0.0427027195692062
-0.127630233764648 0.0812363028526306
0.0438803397119045 -0.133779242634773
-0.0491093546152115 -0.117659315466881
0.120132282376289 0.0760952010750771
0.111750409007072 -0.098501056432724
0.133140876889229 0.102654881775379
0.141061782836914 -0.0415398478507996
-0.00235026073642075 0.0704079568386078
0.0418831370770931 -0.0566052347421646
-0.0181647818535566 0.148291915655136
-0.0608454868197441 -0.0484543740749359
0.134074002504349 0.13143502175808
-0.0351838655769825 -0.126895889639854
0.0855192095041275 0.140031665563583
0.0665320307016373 -0.0204962529242039
0.0890595614910126 -0.0902296751737595
0.0910286977887154 -0.0192707572132349
-0.107841305434704 -0.0257825907319784
-0.116941198706627 0.0828272998332977
-0.0155808636918664 0.135335937142372
0.102494217455387 0.0502970591187477
-0.131086871027946 0.0892383307218552
-0.0515573024749756 0.0309658870100975
-0.0619089528918266 -0.105189882218838
0.0959845930337906 0.0117737986147404
0.149509832262993 0.0252959579229355
0.132936209440231 0.12021604180336
0.141098365187645 -0.00829494465142488
-0.0621836334466934 0.0245888847857714
0.143374502658844 0.0973092615604401
-0.0102873388677835 -0.122469715774059
0.1456548422575 -0.0254117771983147
-0.0159943532198668 0.114598177373409
-0.146915227174759 0.0535781607031822
-0.0720073580741882 -0.0417797490954399
-0.136376321315765 -0.0876572355628014
0.0461657494306564 0.138538435101509
0.0446432381868362 -0.00264690071344376
-0.0102718826383352 -0.0103019075468183
0.065925344824791 -0.0498036332428455
0.102205969393253 0.100773677229881
-0.0866624489426613 0.110951729118824
-0.132234320044518 -0.0301581267267466
-0.0972800478339195 0.0388097800314426
-0.0684895515441895 0.00873029138892889
-0.0440820604562759 -0.0175117813050747
-0.00771126337349415 0.0953196585178375
-0.101588614284992 0.0807499438524246
-0.105301693081856 0.105374023318291
-0.116278044879436 -0.0210556406527758
-0.0610739663243294 0.108533397316933
0.100288569927216 0.144903406500816
0.0841476023197174 -0.100920043885708
-0.124338895082474 0.063747450709343
-0.143232211470604 0.123638860881329
-0.0969955325126648 0.022976340726018
0.0142960771918297 0.0609227865934372
-0.147298201918602 -0.0841598138213158
-0.0715576410293579 -0.128080621361732
-0.0036234431900084 0.148193493485451
0.100458174943924 -0.11040922999382
0.0881727933883667 0.0272351801395416
-0.105349451303482 0.075864389538765
-0.0707892850041389 -0.130759283900261
0.0658958181738853 -0.015867680311203
0.142866492271423 -0.104903139173985
0.126255467534065 -0.110785998404026
0.0517466329038143 0.135463774204254
-0.133124977350235 0.0761690512299538
-0.10710209608078 -0.135331377387047
0.0503630787134171 0.0604815669357777
-0.1248679459095 -0.126721307635307
-0.046244915574789 0.11755033582449
0.10224262624979 -0.052689041942358
0.0806207954883575 -0.0186737887561321
-0.0501299239695072 -0.113121747970581
0.0907574221491814 0.141406342387199
-0.0964571759104729 0.0206002946943045
0.0510854050517082 -0.048865482211113
-0.0180330276489258 -0.138730987906456
0.0124803353101015 -0.0513679720461369
-0.0977554842829704 -0.100361287593842
-0.0437440425157547 -0.0589756965637207
0.0716508328914642 -0.0984773188829422
0.10940620303154 -0.14807602763176
0.111441135406494 0.118549041450024
-0.0119260419160128 -0.044714018702507
-0.0642928257584572 -0.0490027330815792
-0.0230935644358397 -0.14142832159996
-0.115285232663155 -0.0143733844161034
-0.122860759496689 -0.142361253499985
0.016326704993844 0.119710713624954
0.144426241517067 -0.102049253880978
0.146456748247147 -0.118975579738617
0.028433071449399 0.141128718852997
-0.0508259236812592 0.0311124846339226
0.124751426279545 0.144675731658936
-0.136397451162338 -0.046972494572401
-0.00640422059223056 0.147944390773773
-0.0579056516289711 -0.143006190657616
-0.00931815151125193 -0.0863844007253647
0.0349511839449406 -0.0148998172953725
-0.0441649816930294 -0.116150505840778
-0.051563236862421 0.0492984130978584
-0.0462164357304573 0.114726431667805
-0.0629955157637596 0.0834572017192841
-0.0105311488732696 -0.0581123754382133
0.106499582529068 -0.0361297093331814
0.0133021529763937 0.0575268417596817
0.0267595890909433 -0.123620733618736
-0.0625667795538902 0.139353945851326
0.091122604906559 -0.053092934191227
-0.00931020639836788 0.000349793583154678
-0.0628024563193321 0.0352978222072124
0.0242545660585165 0.0118094021454453
-0.0889072641730309 -0.0666353777050972
0.132203623652458 -0.145331308245659
0.0509638972580433 0.127525925636292
0.0861383751034737 0.0621699132025242
-0.0802535116672516 -0.0472251735627651
0.0227831043303013 -0.0566614791750908
0.129797831177711 0.0676167085766792
0.113636896014214 0.033496517688036
0.000676832336466759 -0.0161677803844213
0.0640725269913673 -0.13554485142231
-0.0251235738396645 0.0371036604046822
-0.00541039602831006 0.0858017280697823
0.0564108304679394 -0.102225139737129
-0.0880882292985916 0.0235155615955591
-0.00318166450597346 0.120643101632595
-0.0906504765152931 0.0101812370121479
0.119322694838047 0.146022245287895
-0.0182829704135656 0.0230381656438112
0.12359356880188 -0.0325963385403156
0.0437033884227276 0.0722462683916092
-0.14692696928978 0.0119784530252218
0.148210138082504 -0.0812464728951454
0.137650087475777 -0.0536919087171555
-0.0380140654742718 0.0638589039444923
0.138613313436508 -0.0193035863339901
-0.125325411558151 -0.128827884793282
0.119153268635273 0.12590280175209
-0.0794371515512466 -0.146404966711998
-0.0787628963589668 0.00394094223156571
-0.0490477830171585 -0.051899254322052
-0.132736191153526 0.0341022349894047
-0.00430327421054244 0.124260179698467
0.0144909387454391 -0.120198711752892
0.100959427654743 0.00287476764060557
-0.0314806625247002 -0.045861829072237
-0.115493096411228 0.144621193408966
-0.0034806455951184 -0.0228118505328894
0.102145701646805 -0.121153891086578
0.086247481405735 0.0767332315444946
0.0941749885678291 0.0748733729124069
0.0816269218921661 0.0494536571204662
0.0546775236725807 -0.0130183519795537
0.0742503255605698 0.00281393388286233
-0.0786206275224686 -0.0455583855509758
-0.124060854315758 -0.0258026067167521
0.00236071227118373 0.0487877726554871
0.0531653873622417 0.00921503826975822
0.0867809653282166 0.026841938495636
-0.0687994360923767 -0.0868481397628784
-0.0415815562009811 -0.0863775536417961
0.139494717121124 -0.135749876499176
-0.110114701092243 0.0349842384457588
-0.0975954830646515 -0.0697546079754829
0.124704450368881 -0.0414840094745159
-0.0504336655139923 0.0967046469449997
-0.0609969757497311 0.0320977009832859
0.133477419614792 -0.0355774834752083
0.0197620652616024 0.0006569919642061
-0.00841342378407717 -0.0466318726539612
-0.0185893196612597 -0.0161062330007553
-0.00468633789569139 0.0952178314328194
-0.0128527488559484 0.0283450148999691
-0.0536055937409401 -0.0213118605315685
0.135631456971169 0.0287079401314259
0.02979751303792 -0.0562561750411987
-0.122948214411736 0.000678254291415215
0.102111861109734 0.0788853839039803
0.114814706146717 -0.0597033873200417
0.0479279235005379 -0.0479442402720451
-0.0113884881138802 -0.0492476969957352
0.0672290697693825 0.101719886064529
-0.0116038080304861 -0.0112737128511071
-0.136941865086555 0.0702601969242096
0.00682632438838482 0.0738862156867981
0.0360274873673916 -0.0768134444952011
0.140637263655663 0.0510349161922932
0.0693568736314774 -0.0534942150115967
0.141999587416649 0.0607307329773903
0.108503550291061 0.0668395683169365
-0.0572645775973797 -0.0880151763558388
-0.0664508268237114 0.035179678350687
0.00425110664218664 0.0584234856069088
-0.110814906656742 -0.0399999804794788
-0.0704799965023994 -0.0626941323280334
0.0940591841936111 0.113330997526646
0.10878823697567 0.0587702840566635
-0.0026677381247282 0.0209531839936972
-0.0121087096631527 0.0925518572330475
0.148966774344444 0.101072132587433
-0.0803850144147873 -0.108786776661873
0.0904676243662834 0.0759864971041679
0.0576965846121311 0.114742666482925
0.147017851471901 0.0614680834114552
0.0919522792100906 -0.129343450069427
0.00984007213264704 -0.115185789763927
0.0444618761539459 0.0374648422002792
0.0971507653594017 -0.0423904545605183
0.0379268378019333 0.12441511452198
-0.126282393932343 -0.0531500652432442
-0.0250144749879837 0.0532527342438698
-0.124320335686207 0.108781293034554
-0.130832955241203 0.0303250830620527
0.0495852753520012 0.0718026682734489
-0.141139224171638 -0.0305178929120302
-0.0590286143124104 -0.0669989958405495
0.130871921777725 -0.143426775932312
-0.0544187650084496 -0.060585793107748
-0.130419209599495 0.121816605329514
0.0928976461291313 -0.124701969325542
0.0331819094717503 -0.0825595036149025
-0.0440905541181564 0.0421023778617382
0.0764059275388718 0.0408030301332474
-0.126158446073532 -0.101422190666199
-0.0720105022192001 -0.042324535548687
0.137450039386749 0.00614312756806612
0.129837229847908 -0.110992208123207
0.0291331447660923 0.053099125623703
-0.0529982335865498 5.32445192220621e-05
0.0591607987880707 -0.0133686987683177
0.0306670386344194 0.0598593950271606
0.14211094379425 -0.11742041260004
0.041024774312973 -0.0314294472336769
0.021834721788764 -0.102927885949612
0.0269061829894781 0.00630054716020823
-0.108675420284271 0.127976313233376
-0.0756035968661308 -0.124013312160969
0.0917599871754646 -0.0086032934486866
0.0611596703529358 0.0481299571692944
0.0745210349559784 -0.0349623709917068
-0.0350433550775051 -0.0148177817463875
-0.0789738744497299 0.00854022242128849
-0.106329880654812 0.000117260089609772
-0.0127034289762378 0.0853822529315948
-0.0760677754878998 0.0238396655768156
0.0913535058498383 -0.111014276742935
0.148311093449593 -0.0213220063596964
0.0419443659484386 -0.0856405273079872
-0.0371860451996326 0.0314251556992531
0.112230077385902 0.0270198043435812
-0.0227748211473227 -0.0916523188352585
0.062744989991188 -0.145499885082245
-0.0279310327023268 -0.064011313021183
-0.0872489586472511 -0.0740789622068405
-0.103859134018421 0.0171443708240986
-0.0323463566601276 -0.0442918986082077
0.14215649664402 0.0618775151669979
-0.111256517469883 -0.0284862965345383
-0.128426879644394 -0.0571339316666126
0.0131475115194917 0.0857531428337097
-0.145662173628807 0.056579478085041
0.0709336921572685 -0.0556470677256584
-0.13193416595459 -0.0879579484462738
0.113287001848221 -0.00138089363463223
0.0688846260309219 -0.00458211963996291
-0.0697247684001923 0.135269120335579
0.0236607361584902 0.0775254145264626
0.052603654563427 0.0175650510936975
0.117793053388596 -0.0163944140076637
0.119585327804089 0.0294885858893394
0.147319540381432 -0.0295007079839706
0.0263188220560551 -0.0535395964980125
0.0486718937754631 -0.015268774703145
-0.123143874108791 0.0117415580898523
0.0874399542808533 0.065573938190937
0.0330676287412643 0.148246169090271
0.134500712156296 -0.102188684046268
0.032833855599165 -0.0574734918773174
-0.0706480145454407 0.0452279485762119
-0.110211685299873 -0.107292659580708
-0.0708674341440201 0.11238931119442
-0.0742549300193787 0.137602865695953
-0.085900753736496 0.101730816066265
-0.149601146578789 0.142118096351624
-0.0358127504587173 -0.0895499065518379
-0.0935561582446098 -0.0100143477320671
-0.00842844974249601 -0.115829937160015
0.0660711377859116 0.021761192008853
0.0420148074626923 0.0807169675827026
0.0963384956121445 -0.0299271605908871
0.0154269300401211 0.0422649160027504
0.145154610276222 0.0357353985309601
0.0033715704921633 -0.132509276270866
-0.113240271806717 0.0302418675273657
0.0440898314118385 0.0290577262639999
-0.00732152350246906 -0.0734173879027367
-0.0193355940282345 0.0108235571533442
0.0689747482538223 0.00365877407602966
0.112367525696754 0.100797437131405
0.00317283812910318 0.0759765654802322
0.0141596300527453 0.147148877382278
-0.118861101567745 0.0686717927455902
-0.0278211906552315 0.116942420601845
0.00291815330274403 -0.0654763355851173
-0.0989378914237022 -0.0803195312619209
0.136120393872261 -0.0929654687643051
0.00966317858546972 -0.135932624340057
-0.0192937273532152 0.12455815076828
0.0501009114086628 0.011316666379571
0.111659094691277 -0.114619873464108
-0.0112117119133472 -0.0155883692204952
0.118089698255062 0.0981784909963608
0.0563453696668148 0.0722696259617805
0.0440736599266529 -0.0513753704726696
-0.110677324235439 -0.0886931717395782
0.140043616294861 0.0736287161707878
0.0663435682654381 0.140947550535202
-0.117483988404274 -0.0855392068624496
0.135215133428574 0.0714751034975052
0.0143675431609154 -0.0190817229449749
0.120617486536503 -0.0334810093045235
0.0145629141479731 0.0810388326644897
0.106732226908207 -0.138984069228172
0.0837345197796822 -0.079064317047596
0.124547876417637 -0.131926372647285
-0.0281435698270798 -0.0616427026689053
-0.0244269222021103 0.0699432715773582
0.130066484212875 0.0451244525611401
0.0799028873443604 0.0984253957867622
0.0232702493667603 -0.0291866809129715
0.0880905762314796 0.0476272702217102
0.053692277520895 -0.0528824925422668
-0.118884541094303 0.0148967290297151
-0.00930488202720881 -0.0755145326256752
-0.109715968370438 -0.0984668135643005
-0.110809065401554 -0.0675843879580498
-0.00871904939413071 -0.140193626284599
0.00694030430167913 -0.126158729195595
-0.0843608826398849 0.0857486948370934
-0.149928271770477 0.101228661835194
-0.114080965518951 -0.112304635345936
0.146607965230942 0.00927557237446308
0.120588377118111 -0.0239985790103674
0.0435369983315468 0.0759091004729271
0.0498009026050568 0.0339340418577194
-0.00194591004401445 0.0864440426230431
0.0498273931443691 0.0439288206398487
0.127475574612617 -0.0378741584718227
-0.0752971395850182 -0.111249729990959
0.147313758730888 0.0025496284943074
-0.112871751189232 -0.116903394460678
0.12224805355072 -0.123986504971981
-0.0193813070654869 -0.112171739339828
-0.0369525626301765 -0.110101625323296
-0.0270735751837492 -0.0389575622975826
-0.0461766086518764 0.0722459033131599
-0.0130763817578554 0.0820803791284561
-0.0802235379815102 -0.00908475462347269
-0.0134952627122402 -0.0577773153781891
0.0671334192156792 0.066381648182869
0.00768333114683628 0.0950867086648941
-0.145623177289963 -0.00206449092365801
0.0496808886528015 -0.0640359595417976
-0.0491824448108673 0.0584856867790222
-0.100028909742832 0.126350045204163
0.0593772791326046 0.136161848902702
-0.144051000475883 0.11689156293869
-0.0359612554311752 -0.013783797621727
0.0710039287805557 0.102705329656601
-0.123135082423687 0.0593811832368374
-0.0713121667504311 -0.106601670384407
-0.107270754873753 -0.0177913252264261
0.0871856734156609 -0.0508868992328644
0.0862780287861824 -0.0714460238814354
0.0621834471821785 0.053574338555336
-0.10174011439085 -0.0342920944094658
0.00418711872771382 0.10406331717968
-0.0867998823523521 0.114847913384438
0.137330874800682 -0.0107976254075766
0.136133000254631 0.0191466137766838
-0.130580320954323 0.0012527781073004
0.0962633937597275 0.0960155054926872
-0.0821665152907372 -0.0737583115696907
0.0629534274339676 -0.116225816309452
0.106584519147873 -0.0637359842658043
-0.0463633388280869 -0.149244651198387
-0.0110519574955106 -0.0200161952525377
-0.0387497060000896 0.0450341627001762
-0.068908579647541 -0.0940155163407326
-0.00926343351602554 -0.130028992891312
-0.125001817941666 -0.0950935333967209
-0.0843332037329674 0.128655999898911
-0.0893610790371895 -0.0058577130548656
0.0683804899454117 0.0184905752539635
-0.0318516232073307 -0.110582813620567
0.0139986537396908 -0.137995585799217
-0.0801320746541023 -0.00918674562126398
-0.112506575882435 -0.0367870554327965
-0.061914000660181 0.0977432504296303
-0.0859289988875389 -0.0371700115501881
};
\addplot [very thick, trueDynamics]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, approxDynamics, dashed]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, learnedWithSideInfo]
table {%
0.1 0.1
0.109247060338725 0.0849121646659476
0.116979193994005 0.069727185003237
0.123194298531671 0.0545956522504545
0.127904955654806 0.0396627828885316
0.131138066888461 0.0250668494778665
0.132933877331238 0.0109373529199281
0.133345029471286 -0.00260706169268232
0.132435490544648 -0.0154602611527039
0.130279152151059 -0.0275296091253203
0.126958370228723 -0.0387362145725874
0.122562862541352 -0.0490145965559314
0.117188166441684 -0.0583120138549322
0.110934528654079 -0.0665877477070858
0.103905653433372 -0.0738124547285857
0.0962076816831238 -0.0799677416217452
0.0879480061934715 -0.0850458083631658
0.0792343402584379 -0.0890492736177748
0.0701735702741065 -0.0919908643012217
0.0608708430725857 -0.0938930297943585
0.0514285750345394 -0.0947873978478473
0.0419456437297886 -0.0947139198025599
0.0325164938611228 -0.0937202423307735
0.0232304815887314 -0.0918605801066565
0.0141712579586734 -0.089194940935613
0.00541620819818422 -0.0857881819880451
-0.00296396625949515 -0.0817092290099755
-0.0109056308158194 -0.0770302338494311
-0.0183524975853179 -0.071825832493845
-0.0252558270333283 -0.0661723712734972
-0.0315745730289673 -0.0601470459207984
-0.0372754221901027 -0.0538272151297159
-0.0423327557066223 -0.047289422055206
-0.0467285450424743 -0.040608733112462
-0.0504521675545019 -0.0338579300056265
-0.053500127120455 -0.0271068796408596
-0.0558757561440224 -0.0204218824556275
-0.0575887983463394 -0.0138652397092125
-0.0586550250828488 -0.00749480678291015
-0.0590957547972659 -0.00136366967480672
-0.058937357568482 0.0044801075830172
-0.058210752202106 0.00999366528151135
-0.0569508995930061 0.0151394850728446
-0.0551962029523424 0.0198854592189264
-0.0529880272419984 0.0242049271458935
-0.0503701441008396 0.0280766365454896
-0.0473881618708191 0.031484716355922
-0.0440890040492287 0.0344185394180139
-0.0405204398970537 0.0368726098555152
-0.0367305032866204 0.0388463539936037
-0.0327670493873017 0.040343903365712
-0.0286773132133936 0.0413738834096069
-0.0245074365060351 0.0419490459069776
-0.0203021101002074 0.0420860129705538
-0.0161041715865385 0.0418048835411255
-0.0119542951748453 0.0411288918780395
-0.00789068993749462 0.0400840329373056
-0.00394884368614611 0.038698628427527
-0.000161308948129331 0.0370029709057054
0.00344246586227995 0.0350288493323108
0.00683627682037743 0.0328092751489546
0.009997261855867 0.0303779725557956
0.0129059524364365 0.0277690842964819
0.0155462991456224 0.0250167992967523
0.0179056640087703 0.0221550173999621
0.0199747692790102 0.0192170251465349
0.021747623870463 0.0162352160500063
0.0232214088121834 0.0132408246269922
0.0243963729464433 0.0102636715603381
0.0252756671586005 0.00733194542241122
0.0258651618422722 0.00447202193918628
0.0261732811280025 0.00170828703266679
0.0262107756438444 -0.000936999956763884
0.0259905027257508 -0.00344381642669944
0.025527223391249 -0.0057944626152473
0.0248373378451905 -0.00797362233498156
0.0239386545123438 -0.00996839295077123
0.0228501590696421 -0.0117682995928945
0.0215917611257585 -0.013365271313118
0.0201840651149573 -0.0147536142351736
0.0186481132503404 -0.0159299420498478
0.0170051899441407 -0.016893103763957
0.01527656941727 -0.0176440891115828
0.0134833452638062 -0.0181859035206422
0.01164620134341 -0.0185234633188127
0.00978524320786334 -0.018663430771884
0.00791982766610835 -0.0186140935971366
0.00606841423371317 -0.0183851684383392
0.00424841798073038 -0.0179876729771955
0.00247609846672645 -0.0174337294424838
0.00076645443961626 -0.016736414436
-0.000866863480652215 -0.0159095587304368
-0.00241161782413365 -0.0149675841713943
-0.00385703712715786 -0.0139253544767808
-0.00519384847513437 -0.0127979750148448
-0.00641429822828272 -0.0116006501406751
-0.0075121505703001 -0.0103485247117021
-0.00848267354224545 -0.00905653861442879
-0.00932261413331181 -0.00773928733097762
-0.0100301591682848 -0.00641090007151135
-0.0106048761717457 -0.00508492259963589
-0.0110476542317322 -0.00377421159067026
-0.0113606294964098 -0.0024908424606167
-0.0115471069450288 -0.00124602945031604
-0.0116114653948578 -5.0058060356406e-05
-0.0115590597136756 0.00108776791866028
-0.0113961295513662 0.00215917206896421
-0.0111296847880321 0.00315693297548769
-0.0107674040203371 0.00407490573913982
-0.0103175330475734 0.0049080260611607
-0.00978876100568455 0.00565230828005703
-0.00919013096001584 0.00630483355469735
-0.00853091697009901 0.00686372042298622
-0.00782053747594617 0.0073280984013806
-0.00706844493523814 0.00769806303396692
-0.00628403827777424 0.00797462445063424
-0.00547656930636265 0.00815966290251247
-0.00465506586109568 0.00825585877024793
-0.00382824543740684 0.00826662446718984
-0.0030044520875386 0.00819604698348719
-0.00219159099308304 0.00804880447712186
-0.00139707304947325 0.00783009585661354
-0.000627765853151205 0.00754556061820288
0.000110045743116016 0.00720120980586891
0.000810692861716811 0.00680334169727992
0.00146914782053416 0.00635846627490189
0.00208104216448753 0.00587323665160611
0.00264267517312451 0.00535437403269157
0.00315102022874256 0.00480859586976834
0.00360371998681042 0.00424255565575571
0.00399907531817971 0.00366277527128211
0.00433603040916992 0.00307559587323958
0.00461415250681395 0.00248711812627889
0.00483360584296379 0.00190315691136433
0.00499511857347539 0.00132919719812108
0.00509995204546387 0.000770358194014165
0.00514985376632962 0.000231361157776888
0.00514702993042811 -0.00028349780681225
0.00509408860893736 -0.000770368888305839
0.0049940038943277 -0.00122586394458502
0.00485006141828298 -0.00164706760603295
0.00466581597663528 -0.00203154148828943
0.0044450440319531 -0.00237732601815921
0.0041916924907261 -0.00268293550098875
0.00390983260266253 -0.00294734990252721
0.0036036166538649 -0.00317000094415754
0.00327723093467047 -0.00335075657730499
0.00293485452812565 -0.00348990106045122
0.00258061670144902 -0.00358811294631067
0.00221856314483711 -0.00364643449823454
0.00185261499271986 -0.00366624991457165
0.00148654204740063 -0.0036492512696995
0.00112392855219056 -0.00359740723413182
0.000768150373175659 -0.00351293064422364
0.00042235116238834 -0.00339824559826774
8.94231120232569e-05 -0.00325595387144872
-0.000228009264499646 -0.0030887989925148
-0.000527601415248227 -0.00289963359371548
-0.000807298398502104 -0.00269138487997012
-0.00106534010041997 -0.00246702405622656
-0.00130026456091241 -0.00222953458154684
-0.00151090726139917 -0.00198188229404117
-0.00169639862255348 -0.00172698679109828
-0.00185615707828984 -0.00146769514264555
-0.00198988174218568 -0.00120675825971617
-0.00209754076650688 -0.000946808537895194
-0.00217935900273632 -0.000690339012583863
-0.00223580205307056 -0.000439687343973816
-0.00226756206817949 -0.000197019080307115
-0.00227553772407837 3.56840494148969e-05
-0.00226081629444996 0.000256635084234347
-0.0022246540930714 0.000464249496475944
-0.0021684557520398 0.000657151018518931
-0.00209375233577582 0.000834174474466209
-0.00200218085196351 0.000994367159391274
-0.0018954636460237 0.00113698791087735
-0.00177538593288788 0.00126150360139832
-0.0016437767047422 0.00136758398676839
-0.00150248742688264 0.00145509538965172
-0.00135337376029283 0.00152409201202985
-0.00119827728422745 0.00157480678047861
-0.0010390073351127 0.00160763988326096
-0.000877325755865938 0.00162314695047172
-0.000714931354097101 0.0016220250386052
-0.000553446630457172 0.00160510035149031
-0.000394405787459293 0.00157331272080974
-0.000239243844303329 0.00152770112273259
-8.92877525635813e-05 0.0014693894325557
5.42515823208356e-05 0.0013995693960176
0.000190285271297524 0.00131948777264768
0.000317851120553166 0.00123042988745681
0.000436116906021342 0.00113370642453958
0.000544382196386459 0.00103063883430643
0.000642078415274722 0.000922545199532721
0.000728768361353098 0.00081072836539775
0.00080414385120204 0.000696464179723577
0.000868022198072194 0.00058098939154938
0.000920342545024704 0.000465492498818776
0.000961159171319316 0.000351103150142862
0.000990636952385854 0.000238885717442017
0.00100904321096438 0.000129830679989951
0.00101674044129173 2.48492271719414e-05
0.00101417798553299 -7.52318913264105e-05
0.00100188365198416 -0.000169674342432202
0.000980454401921738 -0.0002578310944088
0.000950546978214548 -0.000339148217408436
0.000912869407037623 -0.000413165854231679
0.00086817075331691 -0.000479518047010075
0.000817231982101665 -0.000537931505215639
0.000760856761718109 -0.000588224099766776
0.000699862499720774 -0.000630302082619494
0.000635071902697411 -0.000664156349380107
0.00056730447785304 -0.000689858937368726
0.000497368442024887 -0.000707557810740056
0.000426053823959077 -0.000717472169096567
0.000354125421029111 -0.000719886424594307
0.000282316512670758 -0.000715144525264222
0.00021132327228026 -0.000703643236166229
0.000141799790308567 -0.000685826232288633
7.43537812744333e-05 -0.000662177031788502
9.54289468844266e-06 -0.000633212626105717
-5.21283555638338e-05 -0.000599476702083379
-0.00011021084694926 -0.000561532693396316
-0.000164312558275259 -0.000519957812684879
-0.00021409955213024 -0.000475336540237237
-0.000259296586198526 -0.000428254306445552
-0.000299686531335643 -0.000379292021358779
-0.000335110117050029 -0.00032902045673211
-0.000365464301808706 -0.000277995380434604
-0.000390700730662323 -0.000226752532563879
-0.000410823377939087 -0.000175803542685316
-0.000425886102619219 -0.000125632165365985
-0.000435989592519698 -7.66908271145894e-05
-0.00044127798832435 -2.93977471237383e-05
-0.000441935594912339 1.58654499244903e-05
-0.000438182835976075 5.87556916649135e-05
-0.000430272528769135 9.8969920339087e-05
-0.000418485693182036 0.00013624612600438
-0.000403127448114063 0.000170363720688016
-0.000384522966051154 0.000201143980259388
-0.000363013282104516 0.000228449518772322
-0.000338950957523017 0.000252183622498237
-0.000312696354379333 0.00027228920716027
-0.000284613531897501 0.000288747514350263
-0.000255066666638763 0.00030157640343198
-0.000224416341714002 0.000310828280142061
-0.000193016257997669 0.000316587953776093
-0.000161210119953584 0.000318970030644294
-0.000129328797961244 0.000318117032394483
-9.76877234335691e-05 0.000314195572158837
-6.65844440436644e-05 0.000307394531358085
-3.62966591298391e-05 0.000297921322619743
-7.08054479418851e-06 0.000285999516545843
2.08307763954613e-05 0.000271865742345057
4.7228364168761e-05 0.000255766444203331
7.19282909885585e-05 0.000237955377242471
9.47722637653081e-05 0.000218690522817866
0.000115627871759373 0.00019823151142262
0.000134388661230854 0.00017683679914704
0.000150973869925686 0.000154761394833614
0.000165327874159876 0.000132254557662748
0.000177419715943122 0.000109557379166958
0.000187242026181277 8.69010966422223e-05
0.0001948099624327 6.4505210916721e-05
0.000200160001140648 4.25759152964389e-05
0.000203348424267828 2.13047420238865e-05
0.000204450053309539 8.67415383964953e-07
0.000203556357569371 -1.85771210468033e-05
0.000200773795259936 -3.68874082141701e-05
0.000196222110941537 -5.39400056087658e-05
0.00019003251654312 -6.96298358064951e-05
0.000182345814166894 -8.38702354926113e-05
0.000173310431581516 -9.65930280507621e-05
0.000163080763297359 -0.000107748197324398
0.000151815409772771 -0.000117303442561223
0.000139675242000155 -0.000125243765600302
0.000126821786224356 -0.000131570666962233
0.000113415666865589 -0.000136301299026087
9.96150130661913e-05 -0.000139467684078909
8.55740835034105e-05 -0.000141115468831998
7.14419348658846e-05 -0.000141302925221964
5.7361195823287e-05 -0.000140099792467652
4.34669901546794e-05 -0.000137585987930677
2.98860290393263e-05 -0.000133850304241179
1.67357451851327e-05 -0.000128989076804586
4.12360703971881e-06 -0.000123105025979342
-7.85345331813514e-06 -0.00011630577972177
-1.91094558485219e-05 -0.000108702650326364
-2.9569681810511e-05 -0.000100409345627384
-3.91708720635514e-05 -9.15407602484208e-05
-4.78612207286538e-05 -8.2211809710131e-05
-5.56003961382431e-05 -7.25362433087184e-05
-6.23593571428133e-05 -6.26256452243013e-05
-6.81200348130878e-05 -5.25884170539115e-05
-7.2875015959227e-05 -4.25289021936948e-05
-7.66270993175153e-05 -3.25465385611068e-05
-7.93887316834149e-05 -2.27351385486685e-05
-8.11814622295598e-05 -1.31822472049237e-05
-8.20352003733302e-05 -3.96859955742457e-06
-8.19876555393784e-05 4.83234964754331e-06
-8.10834131225041e-05 1.31547774149254e-05
-7.93732942103373e-05 2.09407647737692e-05
-7.69135188529377e-05 2.81404751056868e-05
-7.37648620543138e-05 3.4712240459811e-05
-6.9991846142016e-05 4.062258550519e-05
-6.56619767890818e-05 4.58461342240923e-05
-6.08448407922318e-05 5.03654615862104e-05
-5.56114112134215e-05 5.41708924242101e-05
-5.003325429178e-05 5.72601938593209e-05
-4.4181798203459e-05 5.96382567330522e-05
-3.81276381969525e-05 6.13166899654516e-05
-3.19398999344411e-05 6.23133356647543e-05
-2.56856264836819e-05 6.26518781263741e-05
-1.94292180537292e-05 6.23612428221065e-05
-1.323194722163e-05 6.14751042178341e-05
-7.15150326206088e-06 6.00313028691346e-05
-1.2416090075934e-06 5.8071280731653e-05
4.44831317760602e-06 5.56394839712482e-05
9.87341244147732e-06 5.27828017258258e-05
1.49936236445644e-05 4.95499943973243e-05
1.97738267636374e-05 4.59910852903533e-05
2.4183948996101e-05 4.21568467583455e-05
2.81990052458936e-05 3.80982499077476e-05
3.17991054123931e-05 3.38659688008391e-05
3.49693561765563e-05 2.95099043263747e-05
3.76998646509225e-05 2.5078701050063e-05
3.99854564469213e-05 2.06193617326988e-05
4.18255992862826e-05 1.61768600026591e-05
4.32241010576775e-05 1.17938072996537e-05
4.41889461153949e-05 7.51013898536712e-06
4.47319642300353e-05 3.36286518631823e-06
4.48684995377618e-05 -6.14149874067493e-07
4.46171340584625e-05 -4.39036682209348e-06
4.39993202637351e-05 -7.93870495208182e-06
4.30390682131451e-05 -1.1235639012952e-05
4.17625344636338e-05 -1.42612527866959e-05
4.01977092047284e-05 -1.69992545053788e-05
3.83740051659726e-05 -1.94369821784335e-05
3.63219301980772e-05 -2.15653076232059e-05
3.40727489380396e-05 -2.33785749763626e-05
3.16581008197939e-05 -2.48745038398113e-05
2.91096944793692e-05 -2.60540081526983e-05
2.6459011256301e-05 -2.692106609814e-05
2.37369650377892e-05 -2.74825098784959e-05
2.09736712417016e-05 -2.77478267918241e-05
1.81981648673599e-05 -2.77289202355036e-05
1.54381822119881e-05 -2.74399088642241e-05
1.27199434948044e-05 -2.68968513701395e-05
1.00679818649321e-05 -2.61175040368045e-05
7.50497377598192e-06 -2.51210673667401e-05
5.05161892458417e-06 -2.39279144604865e-05
2.72653019565278e-06 -2.25593504374899e-05
5.46156178921064e-07 -2.10373444975431e-05
-1.47527801169778e-06 -1.93843019324902e-05
-3.32579746033929e-06 -1.76228070216666e-05
-4.99568439078779e-06 -1.57753824243656e-05
-6.47746219733375e-06 -1.38643072276068e-05
-7.76586162961473e-06 -1.19113870997722e-05
-8.85776031489538e-06 -9.93776065350005e-06
-9.75211045877583e-06 -7.96373924849547e-06
-1.04498492630375e-05 -6.0086419377825e-06
-1.09537884260338e-05 -4.09065643047768e-06
-1.12684950017913e-05 -2.2267142387733e-06
-1.14001622546836e-05 -4.32390983462483e-07
-1.13564741469688e-05 1.2781817844143e-06
-1.11464489069291e-05 2.89238393236246e-06
-1.07802935116127e-05 4.39915514327538e-06
-1.02692308833752e-05 5.78902948511484e-06
-9.62535891866484e-06 7.05414513646474e-06
-8.86148223159383e-06 8.18824654835737e-06
-7.99094753489715e-06 9.18666363247667e-06
-7.02748993457875e-06 1.0046286028853e-05
-5.98508240752527e-06 1.07655082661751e-05
-4.8777834597627e-06 1.13441791071978e-05
-3.71960047296227e-06 1.17835255739607e-05
-2.52434918555228e-06 1.20860768628717e-05
-1.30553045446513e-06 1.22555837744898e-05
-7.62156201691844e-08 1.22969039004772e-05
1.15106279808402e-06 1.22159128359556e-05
2.36440570709068e-06 1.20193954895598e-05
3.55263394327676e-06 1.17149350664647e-05
4.70535984901932e-06 1.13107960171277e-05
5.81305511075658e-06 1.08158164966454e-05
6.86709498665117e-06 1.02392798950746e-05
7.85980446511153e-06 9.59082328222394e-06
8.78448259743897e-06 8.88031089907315e-06
9.63542296419928e-06 8.11772540920686e-06
1.04079168606677e-05 7.31307663315306e-06
1.10982596656373e-05 6.47629462591226e-06
1.17037235599499e-05 5.61713116731255e-06
1.22225493417588e-05 4.74508410874819e-06
1.26539091405212e-05 3.86930878448766e-06
1.29978709478007e-05 2.99855183882869e-06
1.32553540541577e-05 2.14107963358856e-06
1.34280808472484e-05 1.30462413139298e-06
1.35185113289762e-05 4.9633332821486e-07
1.3529796733483e-05 -2.77269922577261e-07
1.34657022194257e-05 -1.01032222055153e-06
1.33305495738645e-05 -1.6976435013305e-06
1.31291417239179e-05 -2.33475489608281e-06
1.28666936156027e-05 -2.91788779094304e-06
1.25487603633498e-05 -3.44398541329838e-06
1.21811708580361e-05 -3.91069884742024e-06
1.17699504581029e-05 -4.3163748948416e-06
1.13212536878085e-05 -4.66003885080113e-06
1.08413105757085e-05 -4.9413675604626e-06
1.03363402520901e-05 -5.16066591060849e-06
9.81250729267108e-06 -5.31882785104187e-06
9.27585714335238e-06 -5.41730345027247e-06
8.73226427776375e-06 -5.4580549697647e-06
8.18738126513729e-06 -5.44351154374567e-06
7.64660238850717e-06 -5.37652453935777e-06
7.1150099839809e-06 -5.26031895375922e-06
6.59735306574039e-06 -5.09844197793541e-06
6.09801003644689e-06 -4.89471270448405e-06
5.62096412858731e-06 -4.65317508613339e-06
5.16978703285487e-06 -4.3780435952101e-06
4.74762207133828e-06 -4.07365305221674e-06
4.35717601039026e-06 -3.7444120906116e-06
4.0007117839691e-06 -3.39475835176017e-06
3.68004849223003e-06 -3.02911009164575e-06
3.39656822174322e-06 -2.6518257989494e-06
3.15122013730407e-06 -2.26716440110408e-06
2.94453457815036e-06 -1.87924767658387e-06
2.77663874549e-06 -1.49202725374664e-06
2.64727216382071e-06 -1.10925571306097e-06
2.55581282779943e-06 -7.34456129691807e-07
2.50129675589961e-06 -3.70903244117926e-07
2.48244823043003e-06 -2.15999200747774e-08
2.49770298971913e-06 3.10736970376979e-07
2.54524096873071e-06 6.23689494716473e-07
2.62301517638813e-06 9.15147946756178e-07
2.72878534556681e-06 1.18331610998723e-06
2.86014430949527e-06 1.42671283853701e-06
3.01455483547874e-06 1.6441727304084e-06
3.18937691012183e-06 1.83484011273549e-06
3.38190207303801e-06 1.99816390455965e-06
3.58938070177395e-06 2.13388667447134e-06
3.80905157058853e-06 2.24203440524207e-06
4.03816936324353e-06 2.32290065937946e-06
4.27403173075547e-06 2.37703197925043e-06
4.5140024839338e-06 2.40520808425515e-06
4.75553319426864e-06 2.40842547860609e-06
4.99618593205464e-06 2.38787609774249e-06
5.2336519111712e-06 2.3449251678187e-06
5.46576604205234e-06 2.2810901860737e-06
5.69052102920853e-06 2.1980182633996e-06
5.90607873993815e-06 2.09746411172773e-06
6.11078339339544e-06 1.98126763706341e-06
6.30316565339295e-06 1.85133094809942e-06
6.48194808616082e-06 1.70959807732629e-06
6.64604879851982e-06 1.55803196300042e-06
6.79458416737166e-06 1.39859661807407e-06
6.92686292745603e-06 1.23323610345949e-06
7.04238890207598e-06 1.06385763842809e-06
7.14085508993906e-06 8.92313943623435e-07
7.22213093357071e-06 7.20388245056824e-07
7.28626823152251e-06 5.49780081016138e-07
7.33347749109353e-06 3.82092746775697e-07
7.36412702004308e-06 2.18822652442441e-07
7.37872746452151e-06 6.13496697887683e-08
7.37792407937143e-06 -8.9070708142458e-08
7.36247853762306e-06 -2.31313407539346e-07
7.33325847205452e-06 -3.64388489160206e-07
7.29122519665948e-06 -4.87443987395864e-07
7.23741915530096e-06 -5.99767764342118e-07
7.17294036688826e-06 -7.00787595064867e-07
7.09894478796713e-06 -7.90069593747944e-07
7.01662066542735e-06 -8.67316199304469e-07
6.92718080595733e-06 -9.32361750471955e-07
6.83184847838358e-06 -9.85168178146978e-07
6.73184422645551e-06 -1.02581877214902e-06
6.62837495440938e-06 -1.05451153231684e-06
6.52262301220619e-06 -1.07155254269742e-06
6.41573255444339e-06 -1.07734534182669e-06
6.30880499111891e-06 -1.07238476232396e-06
6.20288671002167e-06 -1.05724619103853e-06
6.09896498367929e-06 -1.03257612593666e-06
5.99795841930983e-06 -9.99082978125898e-07
5.90070922795033e-06 -9.5752639062141e-07
5.80798640698738e-06 -9.08707253444163e-07
5.72047300803624e-06 -8.53459177108107e-07
5.63877204746294e-06 -7.92637480984126e-07
5.56339468284206e-06 -7.27109568998685e-07
5.4947693079524e-06 -6.57746561216754e-07
5.43323564095033e-06 -5.85414595022371e-07
5.37904790692129e-06 -5.10966337685659e-07
5.33237665694547e-06 -4.35233456386186e-07
5.29330876820194e-06 -3.59019097118107e-07
5.26185471901724e-06 -2.83092070674229e-07
5.23794858955928e-06 -2.08180752636622e-07
5.22145351802838e-06 -1.34967555354137e-07
5.21216943170227e-06 -6.4085181605833e-08
5.20983168216665e-06 3.88758891745056e-09
5.21412377858799e-06 6.84287986274512e-08
5.22467875171267e-06 1.29075727883787e-07
5.24108642962345e-06 1.8542619173445e-07
5.26290071381497e-06 2.37139653691543e-07
5.28964321736686e-06 2.83937758638331e-07
5.32080963107362e-06 3.25603799922192e-07
5.35587972806673e-06 3.61981880914186e-07
5.39431872796647e-06 3.92975511687155e-07
5.43558502790614e-06 4.18545509361934e-07
5.47913793307042e-06 4.3870757338027e-07
5.52443993070972e-06 4.53529665378483e-07
5.57096214665043e-06 4.63128172256688e-07
5.61818843882594e-06 4.67665534742423e-07
5.66562449179353e-06 4.67345273591491e-07
5.71279463414121e-06 4.62408511481271e-07
5.75925184229803e-06 4.53129747057801e-07
5.80457728642514e-06 4.39812419372743e-07
5.84838305892066e-06 4.2278455048006e-07
5.89031353862013e-06 4.02394347176482e-07
5.93005266716351e-06 3.79006078077282e-07
5.96731894651759e-06 3.52995263241951e-07
6.0018690772809e-06 3.24744569013546e-07
6.03349750401272e-06 2.94640042142191e-07
6.06203914364778e-06 2.6306681810695e-07
6.08736574798235e-06 2.30405571954861e-07
6.10938772258041e-06 1.97028846571357e-07
6.12805139785927e-06 1.63297977806565e-07
6.14333903019293e-06 1.29560161710174e-07
6.15526743673322e-06 9.61454933445793e-08
6.16388253910777e-06 6.33648111758589e-08
6.16926345611835e-06 3.15075627810302e-08
6.17151522777637e-06 8.40014280356627e-10
6.17077108867881e-06 -2.83963110803143e-08
6.16718382859954e-06 -5.59856836446215e-08
6.16092761092368e-06 -8.17391612173424e-08
6.15219433479364e-06 -1.05494859070632e-07
6.14119136175401e-06 -1.2711833896617e-07
6.12813742226215e-06 -1.46502722842001e-07
6.11326034297838e-06 -1.63568213196186e-07
6.09679522656226e-06 -1.78261686301084e-07
6.07898081469299e-06 -1.90555592638475e-07
6.06005630438694e-06 -2.00447237475032e-07
6.04026225745763e-06 -2.07957723930008e-07
6.01983332446099e-06 -2.1313008247148e-07
5.99900370186479e-06 -2.16028571031757e-07
5.97799530840243e-06 -2.16736259162076e-07
5.95702096835293e-06 -2.15353713528543e-07
5.93628441124261e-06 -2.11996670884673e-07
5.91597436060826e-06 -2.06794604551419e-07
5.89627226398048e-06 -1.99888715357588e-07
5.87734046996607e-06 -1.91430197915565e-07
5.85932450174187e-06 -1.81577583191483e-07
5.84235714949644e-06 -1.704956940074e-07
5.82655164969165e-06 -1.58352905899051e-07
5.81200623189088e-06 -1.45320045774611e-07
5.79880184554266e-06 -1.31568077321731e-07
5.78700215948802e-06 -1.17266719001918e-07
5.77665310731723e-06 -1.02582649930127e-07
5.76778470646327e-06 -8.76783374792467e-08
5.76041196753002e-06 -7.27102733577567e-08
5.75453216583588e-06 -5.78279948371119e-08
5.75013029837507e-06 -4.3172617480991e-08
5.74717726446045e-06 -2.88762773692497e-08
5.74563032097741e-06 -1.5061228708646e-08
5.74543581071535e-06 -1.83891835092709e-09
5.74653007138354e-06 1.06904476382397e-08
5.74883943638138e-06 2.24382663560618e-08
5.75227977937798e-06 3.33280194553254e-08
5.75676515453261e-06 4.3295314000602e-08
5.76219779259424e-06 5.22878820241601e-08
5.76848128849838e-06 6.02654020021021e-08
5.77550832231433e-06 6.71997248957723e-08
5.78317748575752e-06 7.30740774557148e-08
5.79138191358214e-06 7.7882994276024e-08
5.80001110200845e-06 8.16316951812723e-08
5.80896227789229e-06 8.43356247060001e-08
5.81813357704991e-06 8.60195079610548e-08
5.82742404482001e-06 8.67168399310003e-08
5.83673681903846e-06 8.64690345991903e-08
5.8459795847024e-06 8.53248742771484e-08
5.8550650291686e-06 8.33394739885307e-08
5.86391175096124e-06 8.05734750031206e-08
5.87244426047961e-06 7.70922525816786e-08
5.88059934606561e-06 7.29648572672659e-08
5.88831197711331e-06 6.82630929560446e-08
5.89552712735447e-06 6.30611274310411e-08
5.90219977488621e-06 5.7434565658987e-08
5.90829399269022e-06 5.14589295619317e-08
5.91377521824699e-06 4.52097710379462e-08
5.91862025749873e-06 3.87617458130762e-08
5.92281546615142e-06 3.21874775721653e-08
5.92634856426411e-06 2.55574654772772e-08
5.92921864062124e-06 1.89393691840678e-08
5.93143160538406e-06 1.23971339860418e-08
5.93299382342649e-06 5.99109917231999e-09
5.93392666660419e-06 -2.22661000748303e-10
5.93424968759609e-06 -6.19303364146617e-09
5.93398926063832e-06 -1.18734035936541e-08
5.93317721695602e-06 -1.72224989825054e-08
5.93184902598215e-06 -2.22043521347359e-08
5.93004152127374e-06 -2.6788111284759e-08
5.92779517502584e-06 -3.09484775584679e-08
5.92515818972211e-06 -3.46654758232035e-08
5.92217149218699e-06 -3.79247708792718e-08
5.91888101171556e-06 -4.07168130323043e-08
5.9153349515062e-06 -4.30370743487174e-08
5.91158015053606e-06 -4.48859740487251e-08
5.9076639023492e-06 -4.6268537445826e-08
5.90363168230523e-06 -4.71940992952113e-08
5.89952896518781e-06 -4.76758348355588e-08
5.89539895248098e-06 -4.7730893015796e-08
5.89128393615329e-06 -4.73794870003985e-08
5.88722393461e-06 -4.66451322012063e-08
5.88325578301102e-06 -4.55536905974441e-08
5.87941313341667e-06 -4.41333476430827e-08
5.87572827343702e-06 -4.24142161392638e-08
5.87222985314051e-06 -4.04276434551321e-08
5.86894152013878e-06 -3.82063269910304e-08
5.86588783160757e-06 -3.57835041597809e-08
5.86308515926337e-06 -3.31928120544944e-08
5.8605471464912e-06 -3.04678025031535e-08
5.85828516266873e-06 -2.76415192956847e-08
5.85630966778994e-06 -2.47464342351122e-08
5.85462702928918e-06 -2.18142961472267e-08
5.85323906680812e-06 -1.88757596220057e-08
5.85214441685411e-06 -1.59598592119892e-08
5.85133989679937e-06 -1.30941018028352e-08
5.8508155029377e-06 -1.03038857446336e-08
5.85056532417805e-06 -7.61263585502547e-09
5.85057890177543e-06 -5.04191000061383e-09
5.85084350335913e-06 -2.61095323139671e-09
5.85134457742331e-06 -3.36793704036609e-10
5.85206393446946e-06 1.76604331159069e-09
5.85298474919255e-06 3.68533648043012e-09
5.85408837713852e-06 5.41128208908503e-09
5.85535117169494e-06 6.93669832685373e-09
5.85675721680862e-06 8.25655455116703e-09
5.85828468461363e-06 9.36799793294085e-09
5.85991265684982e-06 1.02704049709246e-08
5.86162157945741e-06 1.09651292490298e-08
5.86338916942764e-06 1.14555600561062e-08
5.86519632741339e-06 1.17468896831951e-08
5.86702213497409e-06 1.18460050657632e-08
5.86884885656752e-06 1.17614789019171e-08
5.87065830224415e-06 1.15030776015601e-08
5.87243364591483e-06 1.10818412224489e-08
5.87415988070189e-06 1.05098045821705e-08
5.87582109023987e-06 9.79995284922097e-09
5.87740545049398e-06 8.96603502553717e-09
5.87890068302899e-06 8.02224420226594e-09
5.88029587358235e-06 6.98325841597125e-09
5.88158283648665e-06 5.86394577339888e-09
5.88275429503488e-06 4.67920457936088e-09
5.8838088850266e-06 3.44358674908563e-09
5.88473751089724e-06 2.17148077297225e-09
5.88553744376025e-06 8.77182770864238e-10
5.88620686450131e-06 -4.25565360728797e-10
5.88674622736818e-06 -1.72350667071441e-09
5.88715598690698e-06 -3.00423863563992e-09
5.88743932593283e-06 -4.25607105114523e-09
5.88759851809922e-06 -5.46817346958051e-09
5.88763811035231e-06 -6.63048638216424e-09
5.8875644691897e-06 -7.73409247756263e-09
5.88738350582041e-06 -8.77109584962454e-09
5.88710249636165e-06 -9.73450653418695e-09
5.88672962593961e-06 -1.06186774928574e-08
5.88627080617271e-06 -1.14187166389002e-08
5.88573695095573e-06 -1.21308367795336e-08
5.88513579075078e-06 -1.27524941717638e-08
5.88447687537713e-06 -1.32819479858881e-08
5.88377339247326e-06 -1.37186848547799e-08
5.88303170853677e-06 -1.4063282094412e-08
5.88225955411303e-06 -1.43167699917512e-08
5.88146647922949e-06 -1.44812233315861e-08
5.88066157858336e-06 -1.45593670453081e-08
5.87985212842368e-06 -1.45546401597585e-08
5.87904813331708e-06 -1.44711442828793e-08
5.87825641437667e-06 -1.43136222874318e-08
5.87748333844007e-06 -1.40872007392545e-08
5.8767366362053e-06 -1.37974573988231e-08
5.87602176495977e-06 -1.34503750359727e-08
5.87534236253656e-06 -1.30521140562223e-08
5.87470343153818e-06 -1.26087940088837e-08
5.87410997437282e-06 -1.21269234654164e-08
5.87356699319197e-06 -1.16130287608485e-08
5.87307676210014e-06 -1.10737836678254e-08
5.87264155495898e-06 -1.05156914287363e-08
5.87226273621178e-06 -9.94515936270091e-09
5.87194167013527e-06 -9.36830879538775e-09
5.87167835695845e-06 -8.79113670748666e-09
5.87147234194091e-06 -8.21935941530683e-09
5.87132362558224e-06 -7.65824736959075e-09
5.87122993393752e-06 -7.11279035670032e-09
5.87118990291735e-06 -6.58758381177904e-09
5.8712017137405e-06 -6.08680039704268e-09
5.87126309269798e-06 -5.61416513278346e-09
5.87136994711218e-06 -5.1729074357354e-09
5.87151909405698e-06 -4.76586414777103e-09
5.87170689519967e-06 -4.39528236029219e-09
5.87193062250024e-06 -4.06305034061916e-09
5.87218527357131e-06 -3.77049858002465e-09
5.8724667556867e-06 -3.51860762748402e-09
5.87277143104109e-06 -3.30780203228187e-09
5.87309611623649e-06 -3.13813686148023e-09
5.8734353544504e-06 -3.0092284220018e-09
5.87378505275543e-06 -2.92048518701904e-09
5.87414202807973e-06 -2.87066193038754e-09
5.87450127804284e-06 -2.85836776470205e-09
5.87486052892189e-06 -2.88182633312317e-09
5.87521614275888e-06 -2.93914759197378e-09
5.87556402656397e-06 -3.02809510799307e-09
5.87590145188777e-06 -3.14626724673417e-09
5.87622614513922e-06 -3.2909959202243e-09
5.87653492276075e-06 -3.45966988390956e-09
5.87682551093927e-06 -3.64943986141952e-09
5.87709609082415e-06 -3.85736242947132e-09
5.87734620734193e-06 -4.08055456091461e-09
5.87757222261787e-06 -4.31611724138747e-09
5.8777745913785e-06 -4.56106263868605e-09
5.87795149436382e-06 -4.81256456907886e-09
5.87810338629341e-06 -5.06785369225327e-09
5.87822935778359e-06 -5.32422994581339e-09
5.87832986333886e-06 -5.57908386156214e-09
5.87840490295227e-06 -5.83000492326846e-09
5.87845493134342e-06 -6.07473715774631e-09
5.87848040310701e-06 -6.31122176741883e-09
5.87848268257529e-06 -6.53741771827754e-09
5.8784635885642e-06 -6.751681880246e-09
5.87842357583496e-06 -6.95254698257486e-09
5.87836400865738e-06 -7.13864878321147e-09
5.87828670591678e-06 -7.30894100797741e-09
5.87819348665114e-06 -7.46251593852776e-09
5.87808526023026e-06 -7.59871277011825e-09
5.87796475522151e-06 -7.71699859569708e-09
5.8778328810502e-06 -7.81712294894987e-09
5.87769191148779e-06 -7.8990165519599e-09
5.87754366553062e-06 -7.96268118108401e-09
5.87738996208481e-06 -8.00846500226271e-09
5.87723216546182e-06 -8.03676769578487e-09
5.87707300426371e-06 -8.04813282684336e-09
5.87691384264233e-06 -8.04338995408216e-09
5.87675468062543e-06 -8.02329580551486e-09
5.87659915618488e-06 -7.98872257234962e-09
5.87644726947334e-06 -7.94078935939524e-09
5.8763008392998e-06 -7.88064369316999e-09
5.87616168491734e-06 -7.80946329825838e-09
5.87602980610391e-06 -7.72853603336898e-09
5.8759065674277e-06 -7.63901475409057e-09
5.87579242342096e-06 -7.54227791333051e-09
5.87568828371021e-06 -7.43961514615421e-09
5.8755946030567e-06 -7.33231964034076e-09
5.87551183631185e-06 -7.22163129296405e-09
5.87543998338547e-06 -7.10882552823477e-09
5.87537995396653e-06 -6.99508895252166e-09
5.87533083841463e-06 -6.88160817219341e-09
5.8752935462314e-06 -6.76950584477254e-09
5.87526716821357e-06 -6.65976607194807e-09
5.87525215888646e-06 -6.55338894262059e-09
5.87524715398718e-06 -6.45123066078668e-09
5.87525215380719e-06 -6.3541456540861e-09
5.87526670339789e-06 -6.26268992220957e-09
5.87528989338254e-06 -6.17755624432448e-09
5.8753217237334e-06 -6.0992899619805e-09
5.87536083019452e-06 -6.02838312602216e-09
5.87540675800469e-06 -5.96510218997537e-09
5.8754585978496e-06 -5.90971538372287e-09
5.87551544000559e-06 -5.86233817045922e-09
5.87557682990569e-06 -5.82307002616744e-09
5.87564094849113e-06 -5.79188252913809e-09
5.87570915997621e-06 -5.7687543630891e-09
5.87577737168332e-06 -5.75343328534927e-09
5.87584876672598e-06 -5.74564928967902e-09
5.87592152641314e-06 -5.74529934738166e-09
5.87599337653621e-06 -5.75209746500605e-09
5.87606158894416e-06 -5.76537217966688e-09
5.87612980152558e-06 -5.78469006029536e-09
5.87619574050902e-06 -5.80972603358987e-09
5.87625940592224e-06 -5.83981041302195e-09
5.87631852391746e-06 -5.87433390819569e-09
5.87637445876449e-06 -5.91293236595902e-09
5.87642675581312e-06 -5.95491123078773e-09
5.87647450534662e-06 -5.99977134640994e-09
5.87651770752456e-06 -6.04683236815617e-09
5.87655590750247e-06 -6.09558270525667e-09
5.87658955995829e-06 -6.14546991073439e-09
5.87661821033897e-06 -6.19592377404388e-09
5.87664185844328e-06 -6.24647356062269e-09
5.87666050440999e-06 -6.2966130087716e-09
5.87667369343625e-06 -6.3458323040777e-09
5.87668187998491e-06 -6.39369268640166e-09
5.87668551919884e-06 -6.43979625181146e-09
5.87668461071722e-06 -6.48372378009299e-09
5.87667960968291e-06 -6.52524789757081e-09
5.8766705155755e-06 -6.56401510923388e-09
5.87665732883907e-06 -6.5998406739709e-09
5.87664095877405e-06 -6.63247945453804e-09
5.87662186012083e-06 -6.66176980246291e-09
5.87659912339861e-06 -6.68749855492479e-09
5.87657502237882e-06 -6.70973854255408e-09
5.87654773792634e-06 -6.72833877501944e-09
5.87652045354325e-06 -6.74331701588926e-09
5.87649044048177e-06 -6.75481715006754e-09
5.87645860846558e-06 -6.76273970157126e-09
5.87642677621347e-06 -6.76710243396883e-09
5.87639494395442e-06 -6.76817535349983e-09
5.87636311158435e-06 -6.76606148886094e-09
5.8763312791657e-06 -6.7609242648814e-09
5.87629944671236e-06 -6.75295908081353e-09
5.87626988785006e-06 -6.74227784713821e-09
5.87624260271757e-06 -6.72942057633463e-09
5.87621531750182e-06 -6.71451516609523e-09
5.87618939641016e-06 -6.6977197121787e-09
5.8761666585222e-06 -6.67937527509821e-09
5.87614392071056e-06 -6.65973942659548e-09
5.8761252756459e-06 -6.6389969077818e-09
5.87610708513431e-06 -6.61752252995029e-09
5.87609207798601e-06 -6.59536070202194e-09
5.87607843506588e-06 -6.57295018413606e-09
5.87606797522455e-06 -6.55047038833345e-09
5.876058879771e-06 -6.52810783208224e-09
5.87605296747257e-06 -6.50611298169679e-09
5.87604841945089e-06 -6.48472209263673e-09
5.87604659994106e-06 -6.46400266646197e-09
5.87604659943453e-06 -6.44430286911302e-09
5.87604796320473e-06 -6.4255782916689e-09
5.87605251026191e-06 -6.40808117680081e-09
5.87605705720112e-06 -6.39193054041698e-09
5.87606433281873e-06 -6.37704999917332e-09
5.8760734274535e-06 -6.36373798101886e-09
5.87608252216459e-06 -6.35204600030193e-09
5.87609161682712e-06 -6.34176444691548e-09
5.87610434950314e-06 -6.33300878405407e-09
5.87611799169468e-06 -6.32601349082051e-09
5.87613163401113e-06 -6.32068797301599e-09
5.87614527631369e-06 -6.31693453101434e-09
5.87615891869953e-06 -6.31471586132193e-09
5.87617256103679e-06 -6.31396090966518e-09
5.87618620354058e-06 -6.31458796362949e-09
5.87619984600274e-06 -6.31647090187926e-09
5.87621348847878e-06 -6.31962393526919e-09
5.87622713103808e-06 -6.32393515331842e-09
5.87624077363902e-06 -6.32937435796066e-09
5.87625441616363e-06 -6.33589003484758e-09
5.87626578500006e-06 -6.34341290606244e-09
5.87627488012749e-06 -6.35152019867746e-09
5.87628397535206e-06 -6.36008756771389e-09
5.87629307052806e-06 -6.36911323681488e-09
5.87630216568324e-06 -6.37859898233728e-09
5.87630989662413e-06 -6.38847375000751e-09
5.87631444444459e-06 -6.39845332273126e-09
5.87631899211238e-06 -6.40834585396988e-09
5.87632353982181e-06 -6.41827213598845e-09
5.876328087559e-06 -6.42813802187447e-09
5.87632899728963e-06 -6.43777298137138e-09
5.87632899754637e-06 -6.4469034555259e-09
5.87632899773372e-06 -6.45565734203046e-09
5.87632899789331e-06 -6.46397424475254e-09
5.8763289982125e-06 -6.47189324354258e-09
5.87632672455901e-06 -6.47938591669117e-09
5.8763221772451e-06 -6.48607922926203e-09
5.87631762986873e-06 -6.49204068281506e-09
5.87631308258257e-06 -6.497195670363e-09
5.87630853528254e-06 -6.50167031324145e-09
5.87630398785066e-06 -6.50549836223036e-09
5.87629944051593e-06 -6.50870646268231e-09
5.87629489316038e-06 -6.5112892855268e-09
5.87629034565218e-06 -6.51327880518693e-09
5.87628579826194e-06 -6.51474074686575e-09
5.87628125076761e-06 -6.51572307219794e-09
5.87627670331492e-06 -6.51624709746557e-09
5.87627215588304e-06 -6.51623999203821e-09
5.87626760842341e-06 -6.51573728305266e-09
5.87626306088745e-06 -6.51485621006032e-09
5.87625851340007e-06 -6.51359144399066e-09
5.87625396583635e-06 -6.51195364298474e-09
5.87624941831427e-06 -6.50996412332461e-09
5.87624487087546e-06 -6.50758380515981e-09
5.87624032323542e-06 -6.5048872954776e-09
5.87623577569946e-06 -6.50187459427798e-09
5.87623122812186e-06 -6.49861497947768e-09
5.87622668064142e-06 -6.49503384408945e-09
5.87622213303607e-06 -6.49118092610479e-09
5.87621758543766e-06 -6.48703846195531e-09
5.87621303788782e-06 -6.48264730784831e-09
5.87620849030329e-06 -6.47806963627318e-09
5.87620621641388e-06 -6.47335696157825e-09
5.87620621626816e-06 -6.46878639543047e-09
5.87620621620571e-06 -6.46443787388762e-09
5.87620621611551e-06 -6.46027231709922e-09
5.87620621601836e-06 -6.45631459406104e-09
5.87620621583795e-06 -6.45256825748675e-09
5.87620621579632e-06 -6.44894981860489e-09
5.87620621572693e-06 -6.44561026774682e-09
5.87620621567836e-06 -6.44241104907906e-09
5.87620621560203e-06 -6.43932196453534e-09
5.87620621546325e-06 -6.43637676489561e-09
5.87620621542856e-06 -6.43360031915563e-09
5.87620621537999e-06 -6.4309659819628e-09
5.87620985331716e-06 -6.4286034273664e-09
5.87621440073516e-06 -6.42678799067653e-09
5.87621894817397e-06 -6.4255196718932e-09
5.87622349558503e-06 -6.42472741674283e-09
5.87622804299609e-06 -6.42444497600536e-09
5.87623259051817e-06 -6.42462794075982e-09
5.87623713803331e-06 -6.42526565286516e-09
5.87624168555539e-06 -6.42625685998155e-09
5.87624623299421e-06 -6.42762287839105e-09
5.87625078059262e-06 -6.42938502437573e-09
5.87625350909754e-06 -6.43143671652524e-09
5.87625350906978e-06 -6.43358788465775e-09
5.8762535092155e-06 -6.43555075896529e-09
5.8762535092155e-06 -6.43743014450138e-09
5.87625350936122e-06 -6.43924025212073e-09
5.87625350932652e-06 -6.44096331825494e-09
5.87625350929877e-06 -6.4426206591861e-09
5.87625350940979e-06 -6.44416786599322e-09
5.87625350948612e-06 -6.44567244023619e-09
5.87625350954163e-06 -6.44706332764144e-09
5.87625350952081e-06 -6.44840092434151e-09
5.87625350964571e-06 -6.44969233576376e-09
5.87625350952081e-06 -6.45096065454709e-09
5.87625350963183e-06 -6.45211883920638e-09
5.87625350965265e-06 -6.45324860215624e-09
5.87625350968041e-06 -6.45430020540516e-09
5.87625350963183e-06 -6.45527720166683e-09
5.87625350972204e-06 -6.45620623629384e-09
5.87625350972898e-06 -6.45715303448924e-09
5.8762535097498e-06 -6.45799858034479e-09
5.87625350979837e-06 -6.45881392813408e-09
5.87625350979837e-06 -6.45960440692761e-09
5.87625350981225e-06 -6.46039488572114e-09
5.87625350986082e-06 -6.46107700674747e-09
5.87625350988857e-06 -6.46173958784857e-09
5.87625350984e-06 -6.46236131274236e-09
5.87625350985388e-06 -6.46300435391822e-09
5.87625350991633e-06 -6.46359055167522e-09
5.87625350993715e-06 -6.46412168237021e-09
5.87625350992327e-06 -6.46458531150529e-09
5.87625350988857e-06 -6.46512532398447e-09
5.87625350990245e-06 -6.4656049403311e-09
5.87625350990245e-06 -6.46602060783152e-09
5.8762535099649e-06 -6.4664433807593e-09
5.8762535099996e-06 -6.46689812811019e-09
5.87625350995102e-06 -6.46728537390118e-09
5.8762535099649e-06 -6.46764419798274e-09
5.87625351004817e-06 -6.46802433834637e-09
5.87625351007592e-06 -6.46838493878477e-09
5.87625351002041e-06 -6.4686975775885e-09
5.87625351000653e-06 -6.4690492962427e-09
5.87625351006205e-06 -6.46929620984338e-09
5.87625351000653e-06 -6.46955378158509e-09
5.87625351004817e-06 -6.46979358975841e-09
5.87625351002735e-06 -6.47002629250437e-09
5.87625351010368e-06 -6.47026787703453e-09
5.8762535100898e-06 -6.47052900148992e-09
5.87625351010368e-06 -6.47068532089179e-09
5.87625351006205e-06 -6.47089493099884e-09
5.87625351004817e-06 -6.47108322482381e-09
5.87625351001347e-06 -6.47125553143724e-09
5.87625351011062e-06 -6.47137810005916e-09
5.8762535100898e-06 -6.47151487953579e-09
5.87625351016613e-06 -6.4716640935103e-09
5.87625351015919e-06 -6.47182041291217e-09
5.87625351014531e-06 -6.47193409974989e-09
5.8762535101245e-06 -6.47207087922652e-09
5.87625351008286e-06 -6.4722005532758e-09
5.87625351011756e-06 -6.47233555639559e-09
5.87625351015919e-06 -6.4724172688102e-09
5.87625351018001e-06 -6.47256825914155e-09
5.87625351008286e-06 -6.47265352426984e-09
5.87625351006898e-06 -6.47271036768871e-09
5.87625351015225e-06 -6.47282050181275e-09
5.8762535101245e-06 -6.47287379251793e-09
5.87625351016613e-06 -6.47294662314835e-09
5.87625351016613e-06 -6.47303721734716e-09
5.87625351015919e-06 -6.47310827162073e-09
5.87625351006898e-06 -6.47317577318063e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
};
\addplot [very thick, learnedWithSideInfo, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131138066888461 0.0250668494778665
0.126958370228723 -0.0387362145725874
0.0962076816831238 -0.0799677416217452
0.0514285750345394 -0.0947873978478473
0.00541620819818422 -0.0857881819880451
-0.0315745730289673 -0.0601470459207984
-0.053500127120455 -0.0271068796408596
-0.058937357568482 0.0044801075830172
-0.0503701441008396 0.0280766365454896
-0.0327670493873017 0.040343903365712
-0.0119542951748453 0.0411288918780395
0.00683627682037743 0.0328092751489546
0.0199747692790102 0.0192170251465349
0.0258651618422722 0.00447202193918628
0.0248373378451905 -0.00797362233498156
0.0186481132503404 -0.0159299420498478
0.00978524320786334 -0.018663430771884
0.00076645443961626 -0.016736414436
-0.00641429822828272 -0.0116006501406751
-0.0106048761717457 -0.00508492259963589
-0.0115590597136756 0.00108776791866028
-0.00978876100568455 0.00565230828005703
-0.00628403827777424 0.00797462445063424
-0.00219159099308304 0.00804880447712186
0.00146914782053416 0.00635846627490189
0.00399907531817971 0.00366277527128211
0.00509995204546387 0.000770358194014165
0.00485006141828298 -0.00164706760603295
0.0036036166538649 -0.00317000094415754
0.00185261499271986 -0.00366624991457165
8.94231120232569e-05 -0.00325595387144872
-0.00130026456091241 -0.00222953458154684
-0.00209754076650688 -0.000946808537895194
-0.00226081629444996 0.000256635084234347
-0.0018954636460237 0.00113698791087735
-0.00119827728422745 0.00157480678047861
-0.000394405787459293 0.00157331272080974
0.000317851120553166 0.00123042988745681
0.00080414385120204 0.000696464179723577
0.00100904321096438 0.000129830679989951
0.000950546978214548 -0.000339148217408436
0.000699862499720774 -0.000630302082619494
0.000354125421029111 -0.000719886424594307
9.54289468844266e-06 -0.000633212626105717
-0.000259296586198526 -0.000428254306445552
-0.000410823377939087 -0.000175803542685316
-0.000438182835976075 5.87556916649135e-05
-0.000363013282104516 0.000228449518772322
-0.000224416341714002 0.000310828280142061
-6.65844440436644e-05 0.000307394531358085
7.19282909885585e-05 0.000237955377242471
0.000165327874159876 0.000132254557662748
0.000203348424267828 2.13047420238865e-05
0.00019003251654312 -6.96298358064951e-05
0.000139675242000155 -0.000125243765600302
7.14419348658846e-05 -0.000141302925221964
4.12360703971881e-06 -0.000123105025979342
-4.78612207286538e-05 -8.2211809710131e-05
-7.66270993175153e-05 -3.25465385611068e-05
-8.10834131225041e-05 1.31547774149254e-05
-6.56619767890818e-05 4.58461342240923e-05
-3.81276381969525e-05 6.13166899654516e-05
-7.15150326206088e-06 6.00313028691346e-05
1.97738267636374e-05 4.59910852903533e-05
3.76998646509225e-05 2.5078701050063e-05
4.47319642300353e-05 3.36286518631823e-06
4.17625344636338e-05 -1.42612527866959e-05
3.16581008197939e-05 -2.48745038398113e-05
1.81981648673599e-05 -2.77289202355036e-05
5.05161892458417e-06 -2.39279144604865e-05
-4.99568439078779e-06 -1.57753824243656e-05
-1.04498492630375e-05 -6.0086419377825e-06
-1.11464489069291e-05 2.89238393236246e-06
-7.99094753489715e-06 9.18666363247667e-06
-2.52434918555228e-06 1.20860768628717e-05
3.55263394327676e-06 1.17149350664647e-05
8.78448259743897e-06 8.88031089907315e-06
1.22225493417588e-05 4.74508410874819e-06
1.35185113289762e-05 4.9633332821486e-07
1.28666936156027e-05 -2.91788779094304e-06
1.08413105757085e-05 -4.9413675604626e-06
8.18738126513729e-06 -5.44351154374567e-06
5.62096412858731e-06 -4.65317508613339e-06
3.68004849223003e-06 -3.02911009164575e-06
2.64727216382071e-06 -1.10925571306097e-06
2.54524096873071e-06 6.23689494716473e-07
3.18937691012183e-06 1.83484011273549e-06
4.27403173075547e-06 2.37703197925043e-06
5.46576604205234e-06 2.2810901860737e-06
6.48194808616082e-06 1.70959807732629e-06
7.14085508993906e-06 8.92313943623435e-07
7.37872746452151e-06 6.13496697887683e-08
7.23741915530096e-06 -5.99767764342118e-07
6.83184847838358e-06 -9.85168178146978e-07
6.30880499111891e-06 -1.07238476232396e-06
5.80798640698738e-06 -9.08707253444163e-07
5.43323564095033e-06 -5.85414595022371e-07
5.23794858955928e-06 -2.08180752636622e-07
5.22467875171267e-06 1.29075727883787e-07
5.35587972806673e-06 3.61981880914186e-07
5.57096214665043e-06 4.63128172256688e-07
5.80457728642514e-06 4.39812419372743e-07
6.0018690772809e-06 3.24744569013546e-07
6.12805139785927e-06 1.63297977806565e-07
6.17151522777637e-06 8.40014280356627e-10
6.14119136175401e-06 -1.2711833896617e-07
6.06005630438694e-06 -2.00447237475032e-07
5.95702096835293e-06 -2.15353713528543e-07
5.85932450174187e-06 -1.81577583191483e-07
5.78700215948802e-06 -1.17266719001918e-07
5.75013029837507e-06 -4.3172617480991e-08
5.74883943638138e-06 2.24382663560618e-08
5.77550832231433e-06 6.71997248957723e-08
5.81813357704991e-06 8.60195079610548e-08
5.86391175096124e-06 8.05734750031206e-08
5.90219977488621e-06 5.7434565658987e-08
5.92634856426411e-06 2.55574654772772e-08
5.93424968759609e-06 -6.19303364146617e-09
5.92779517502584e-06 -3.09484775584679e-08
5.91158015053606e-06 -4.48859740487251e-08
5.89128393615329e-06 -4.73794870003985e-08
5.87222985314051e-06 -4.04276434551321e-08
5.85828516266873e-06 -2.76415192956847e-08
5.85133989679937e-06 -1.30941018028352e-08
5.85134457742331e-06 -3.36793704036609e-10
5.85675721680862e-06 8.25655455116703e-09
5.86519632741339e-06 1.17468896831951e-08
5.87415988070189e-06 1.05098045821705e-08
5.88158283648665e-06 5.86394577339888e-09
5.88620686450131e-06 -4.25565360728797e-10
5.88763811035231e-06 -6.63048638216424e-09
5.88627080617271e-06 -1.14187166389002e-08
5.88303170853677e-06 -1.4063282094412e-08
5.87904813331708e-06 -1.44711442828793e-08
5.87534236253656e-06 -1.30521140562223e-08
5.87264155495898e-06 -1.05156914287363e-08
5.87132362558224e-06 -7.65824736959075e-09
5.87136994711218e-06 -5.1729074357354e-09
5.8724667556867e-06 -3.51860762748402e-09
5.87414202807973e-06 -2.87066193038754e-09
5.87590145188777e-06 -3.14626724673417e-09
5.87734620734193e-06 -4.08055456091461e-09
5.87822935778359e-06 -5.32422994581339e-09
5.87848268257529e-06 -6.53741771827754e-09
5.87819348665114e-06 -7.46251593852776e-09
5.87754366553062e-06 -7.96268118108401e-09
5.87675468062543e-06 -8.02329580551486e-09
5.87602980610391e-06 -7.72853603336898e-09
5.87551183631185e-06 -7.22163129296405e-09
5.87526716821357e-06 -6.65976607194807e-09
5.87528989338254e-06 -6.17755624432448e-09
5.87551544000559e-06 -5.86233817045922e-09
5.87584876672598e-06 -5.74564928967902e-09
5.87619574050902e-06 -5.80972603358987e-09
5.87647450534662e-06 -5.99977134640994e-09
5.87664185844328e-06 -6.24647356062269e-09
5.87668461071722e-06 -6.48372378009299e-09
5.87662186012083e-06 -6.66176980246291e-09
5.87649044048177e-06 -6.75481715006754e-09
5.8763312791657e-06 -6.7609242648814e-09
5.87618939641016e-06 -6.6977197121787e-09
5.87609207798601e-06 -6.59536070202194e-09
5.87604841945089e-06 -6.48472209263673e-09
5.87605705720112e-06 -6.39193054041698e-09
5.87610434950314e-06 -6.33300878405407e-09
5.87617256103679e-06 -6.31396090966518e-09
5.87624077363902e-06 -6.32937435796066e-09
5.87629307052806e-06 -6.36911323681488e-09
5.87632353982181e-06 -6.41827213598845e-09
5.87632899789331e-06 -6.46397424475254e-09
5.87631308258257e-06 -6.497195670363e-09
5.87629034565218e-06 -6.51327880518693e-09
5.87626760842341e-06 -6.51573728305266e-09
5.87624487087546e-06 -6.50758380515981e-09
5.87622213303607e-06 -6.49118092610479e-09
5.87620621626816e-06 -6.46878639543047e-09
5.87620621579632e-06 -6.44894981860489e-09
5.87620621542856e-06 -6.43360031915563e-09
5.87622349558503e-06 -6.42472741674283e-09
5.87624623299421e-06 -6.42762287839105e-09
5.8762535092155e-06 -6.43743014450138e-09
5.87625350948612e-06 -6.44567244023619e-09
5.87625350963183e-06 -6.45211883920638e-09
5.87625350972898e-06 -6.45715303448924e-09
5.87625350986082e-06 -6.46107700674747e-09
5.87625350993715e-06 -6.46412168237021e-09
5.8762535099649e-06 -6.4664433807593e-09
5.87625351007592e-06 -6.46838493878477e-09
5.87625351004817e-06 -6.46979358975841e-09
5.87625351006205e-06 -6.47089493099884e-09
5.87625351016613e-06 -6.4716640935103e-09
5.87625351011756e-06 -6.47233555639559e-09
5.87625351015225e-06 -6.47282050181275e-09
5.87625351006898e-06 -6.47317577318063e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
5.87625351011756e-06 -6.4732148530311e-09
5.87625351006205e-06 -6.47322373481529e-09
};
\addplot [very thick, learnedWithoutSideInfo]
table {%
0.1 0.1
0.109334025213846 0.0849673078156741
0.117135881364824 0.069773198427912
0.123404117518257 0.0545891084372343
0.128156396134152 0.0395817716057412
0.131424007867825 0.024908268591485
0.13324953875692 0.0107127451168285
0.133686673454327 -0.00287658660230328
0.132800147128097 -0.0157497948474266
0.130664526074201 -0.0278159116982106
0.127361814924592 -0.0390014571068367
0.122978840139616 -0.049247314238773
0.117605497557325 -0.0585051982137337
0.111334440228831 -0.0667350506363977
0.104262052724081 -0.0739042169399529
0.0964899782021611 -0.0799885131599041
0.0881262267605836 -0.0849745663383423
0.0792850395619729 -0.0888623570641549
0.0700851385971326 -0.0916668502607507
0.0606465786714825 -0.0934179784993443
0.0510868986954378 -0.0941588759832221
0.0415174501844398 -0.0939428699591414
0.0320406183490629 -0.0928300677350222
0.0227482689817329 -0.090884342621667
0.0137213544465116 -0.0881712160700765
0.00503035303231059 -0.0847567444322799
-0.00326385264357221 -0.0807072121841195
-0.0111089763435785 -0.0760892867933833
-0.018460390673674 -0.0709702960787943
-0.0252803131359105 -0.0654183906782535
-0.0315371096831694 -0.0595024855983048
-0.0372046966453059 -0.0532919839546935
-0.042262042521001 -0.0468563466722038
-0.0466927974192917 -0.0402645830582138
-0.0504850883285766 -0.0335847151900488
-0.0536315044814835 -0.0268832365856682
-0.0561292635749489 -0.0202245613908794
-0.0579805094703474 -0.0136704533314749
-0.0591926598079375 -0.00727943277088272
-0.0597787082071424 -0.00110617753448139
-0.0597573936546141 0.00479905075189535
-0.0591531753928773 0.0103909150697632
-0.0579959865677875 0.015629408770458
-0.0563207745652434 0.0204801320635681
-0.0541668631065013 0.0249144275835107
-0.0515771873658508 0.0289093783258281
-0.0485974588539282 0.0324476832292966
-0.0452753140558073 0.0355174335200239
-0.0416594929388188 0.0381118167318526
-0.0377990830465951 0.040228775748183
-0.033742853699148 0.0418706480412503
-0.029538693804577 0.0430438061452989
-0.0252331566042221 0.0437583148768432
-0.0208711058755275 0.0440276145458434
-0.0164954512629052 0.0438682331518869
-0.0121469559333525 0.0432995251041746
-0.00786409785957431 0.0423434300161283
-0.00368296656013456 0.0410242429666887
0.000362820394657071 0.0393683873210087
0.00424219307245099 0.037404182417184
0.00792670480038549 0.0351616005981406
0.011390611402029 0.0326720105532736
0.0146109543191075 0.0299679061854583
0.017567645335971 0.027082621897307
0.0202435489299413 0.0240500362066527
0.0226245572827164 0.0209042661007395
0.0246996525044576 0.0176793547925911
0.026460950465502 0.0144089558393823
0.0279037207214579 0.011126017121704
0.0290263773632411 0.00786246899872722
0.0298304362899913 0.00464892193514288
0.0303204354685658 0.00151437979716462
0.0305038162197278 -0.0015140244219225
0.030390765399428 -0.00441126368688316
0.0299940203632616 -0.00715461672616158
0.0293286406062645 -0.00972382777396774
0.0284117517246099 -0.0121012232668605
0.027262268660607 -0.0142717845700631
0.0259006059400821 -0.0162231778811623
0.0243483827460516 -0.0179457443019402
0.0226281302405198 -0.0194324545254325
0.0207630076402623 -0.0206788335384651
0.0187765323185189 -0.0216828611808886
0.0166923277937006 -0.0224448543437816
0.0145338920305313 -0.0229673361270244
0.0123243871336527 -0.0232548965002977
0.0100864503714515 -0.0233140480537024
0.00784202556307001 -0.0231530793869865
0.00561221325258643 -0.0227819076910549
0.00341713774797014 -0.0222119311950486
0.00127582901799528 -0.0214558814581842
-0.000793882436548543 -0.0205276750091699
-0.00277545933485079 -0.0194422635891272
-0.00465374118977735 -0.0182154822218159
-0.00641501844175529 -0.0168638944941684
-0.00804709741293408 -0.0154046347294141
-0.0095393558848258 -0.0138552471408744
-0.0108827887017924 -0.0122335225097103
-0.0120700424891176 -0.0105573333898619
-0.0130954383638233 -0.00884446927545213
-0.0139549814367541 -0.00711247352334965
-0.0146463559554597 -0.00537848409222974
-0.0151689051197597 -0.00365908030791928
-0.015523594908565 -0.0019701378964605
-0.0157129616545113 -0.000326694428434138
-0.015741043568938 0.00125717288688421
-0.0156132969104075 0.00276845542563464
-0.0153364979647019 0.00419530612853691
-0.0149186324296906 0.00552711638741243
-0.0143687741399017 0.00675457641090205
-0.0136969553043578 0.00786971904672384
-0.012914030556324 0.00886594739294821
-0.0120315371294861 0.00973804683614787
-0.0110615533893856 0.0104821823775438
-0.0100165577818636 0.0110958822698599
-0.00890929003656371 0.0115780090759898
-0.00775261620273771 0.0119287192900046
-0.0065593988268775 0.0121494126510591
-0.00534237332000398 0.012242672233036
-0.0041140313271999 0.0122121963322037
-0.00288651171152488 0.0120627231111037
-0.00167149960363933 0.0117999488944811
-0.000480133848396846 0.0114304409685104
0.000677076904009866 0.0109615457012708
0.0017903292675987 0.010401292792082
0.00285059118867537 0.00975829645942028
0.00384965886680089 0.00904165439368754
0.00478020439705773 0.00826084532787164
0.00563581401797464 0.00742562610759734
0.00641101687473444 0.00654592917247498
0.00710130424527833 0.00563176137981358
0.00770313923251642 0.00469310511652665
0.00821395699332861 0.0037398226381633
0.00863215566360509 0.00278156455590661
0.00895707823456959 0.00182768334710914
0.00918898574042082 0.000887152706518179
0.00932902222866616 -3.15065283729155e-05
0.00937917208998762 -0.000920293244679016
0.00934221042302497 -0.0017717851961514
0.00922164720013186 -0.00257919002622131
0.00902166606709542 -0.0033363879134285
0.00874705866394621 -0.00403796571136539
0.00840315538287761 -0.00467924258644814
0.00799575348710491 -0.00525628727476146
0.00753104350355827 -0.00576592719067293
0.00701553476812578 -0.00620574970898602
0.00645598095796984 -0.00657409602034775
0.00585930638373 -0.00687004801871538
0.00523253374598021 -0.00709340871931374
0.00458271398936105 -0.00724467673535401
0.00391685881112025 -0.00732501535372165
0.00324187631132133 -0.00733621675604113
0.00256451020175774 -0.00728066192746368
0.00189128292851848 -0.00716127678871104
0.00122844300922154 -0.00698148507716212
0.000581916834507368 -0.00674515849326696
-4.27348588676324e-05 -0.006456564619441
-0.000640355672254955 -0.00612031311212391
-0.00120622725262542 -0.00574130066105738
-0.00173609791705154 -0.00532465520789316
-0.00222620612120927 -0.00487567991070748
-0.00267329872814059 -0.00439979733841156
-0.00307464406681213 -0.00390249437295864
-0.00342803980258566 -0.00338926828856856
-0.00373181568173031 -0.00286557446468194
-0.00398483124872939 -0.00233677617069361
-0.00418646867808548 -0.00180809683925176
-0.00433662090642173 -0.00128457521442726
-0.00443567529153555 -0.00077102372737059
-0.00448449307068621 -0.000271990412105794
-0.00448438492835379 0.000208275369345756
-0.00443708302195844 0.000665853171504693
-0.00434470984657764 0.00109717750698834
-0.00420974434615751 0.00149905956649476
-0.00403498569891525 0.00186870454638566
-0.00382351522096869 0.00220372456412576
-0.00357865683564462 0.00250214719176256
-0.00330393655903194 0.00276241968097324
-0.00300304144657559 0.00298340899373173
-0.00267977843133949 0.00316439779597033
-0.00233803347034467 0.00330507659926482
-0.00198173139307301 0.00340553227101381
-0.00161479682100918 0.00346623315577332
-0.00124111650219838 0.00348801107577756
-0.000864503372127956 0.00347204049463201
-0.000488662624871239 0.00341981514555201
-0.000117160044805331 0.00333312243486006
0.000246607182532443 0.00321401594328208
0.000599436992485991 0.00306478635111418
0.000938346142255853 0.00288793111838359
0.00126059096781006 0.00268612325008277
0.00156368510471694 0.00246217947535143
0.00184541411286254 0.00221902816531383
0.00210384697546928 0.00195967730457625
0.00233734447199829 0.00168718282388625
0.00254456445476769 0.00140461758657295
0.00272446408650673 0.00111504130721229
0.00287629912346432 0.000821471663169149
0.00299962035550294 0.000526856838554579
0.00309426733569929 0.000234049719175289
0.00316035955842686 -5.4216067209012e-05
0.00319828526043686 -0.000335348097003418
0.00320868804119634 -0.000606914940401992
0.0031924515106887 -0.000866663679463642
0.00315068218686498 -0.00111253506766218
0.00308469087346985 -0.00134267626996376
0.00299597275627761 -0.00155545114990829
0.00288618645910788 -0.00174944809788613
0.00275713230073471 -0.00192348541731491
0.00261072999416179 -0.00207661431027617
0.00244899602396487 -0.0022081195264434
0.00227402092941098 -0.00231751775825728
0.00208794671593004 -0.00240455388452077
0.00189294460451173 -0.00246919517998023
0.001691193315839 -0.00251162362400592
0.00148485807555154 -0.00253222645102014
0.00127607051010692 -0.00253158510012241
0.00106690958853761 -0.0025104627262138
0.000859383750061227 -0.00246979044115037
0.000655414340814175 -0.00241065246295591
0.000456820465124963 -0.00233427034899947
0.000265305342402655 -0.00224198649405594
8.24442430218397e-05 -0.00213524707361046
-9.03259415494517e-05 -0.00201558460987528
-0.000251715453700285 -0.00188460033860238
-0.000400588726410689 -0.00174394654681365
-0.000535969735404151 -0.00159530904809202
-0.000657045653099431 -0.00144038995612661
-0.000763168830079763 -0.00128089090735273
-0.000853857140700853 -0.00111849687544208
-0.000928792746016427 -0.000954860710418615
-0.000987819337474605 -0.000791588524599263
-0.00103093794109022 -0.00063022603305285
-0.00105830136831742 -0.000472245948174077
-0.00107020741320518 -0.000319036510074255
-0.00106709090333013 -0.000171891224155729
-0.00104951471902304 -3.19998625144535e-05
-0.00101815990195853 9.95592297812209e-05
-0.000973814980039123 0.000221825493579075
-0.000917364637048834 0.000333961166255392
-0.000849777858798362 0.000435254942750873
-0.000772095688564178 0.000525124298704327
-0.000685418722568443 0.000603116500244028
-0.000590894475337223 0.000668908337448926
-0.00048970474122001 0.000722304627434056
-0.000383053074086703 0.00076323554668889
-0.000272152500286893 0.000791752857011829
-0.000158213577549304 0.000808025102024601
-4.24328994981238e-05 0.000812331855879478
7.40178575355799e-05 0.000805057112490459
0.000190002259499167 0.000786681909715981
0.000304428735448781 0.000757776284938672
0.000416259425749743 0.000718990664513086
0.000524518201149959 0.000671046788141894
0.000628297804295741 0.000614728271962406
0.000726766077331575 0.000550870914828749
0.000819171247542272 0.000480352848441612
0.000904846254943692 0.00040408463205921
0.000983212113677467 0.000322999389037903
0.0010537803098547 0.000238043078280015
0.00111615424741274 0.000150164988934165
0.00117002976220881 6.03085423200866e-05
0.00121519473238507 -3.05975219561105e-05
0.00125152782212723 -0.000121647504435884
0.00127899640098228 -0.000211966585251133
0.00129765368903634 -0.000300718087114404
0.00130763518301436 -0.000387110113692302
0.00130915442337098 -0.000470401521425856
0.0013024981670835 -0.000549907191796706
0.00128802103297154 -0.00062500257890008
0.00126613969133871 -0.000695127514255489
0.00123732666847332 -0.000759789260097676
0.00120210384014108 -0.000818564808430011
0.0011610356870797 -0.000871102431478477
0.00111472238582699 -0.000917122495984302
0.00106379280647673 -0.000956417559411449
0.0010088974873117 -0.000988851773954025
0.000950701654740982 -0.00101435962911367
0.000889878353071083 -0.00103294406748233
0.000827101744949488 -0.0010446740161747
0.000763040640949342 -0.00104968137656059
0.000698352311250261 -0.00104815752180087
0.000633676627792568 -0.0010403493526141
0.000569630581034986 -0.00102655496443305
0.000506803210054585 -0.00100711898171113
0.000445750979155335 -0.000982427614626857
0.000386993628929133 -0.000952903496056479
0.000331010524879716 -0.000919000355231958
0.000278237519479418 -0.00088119758419225
0.000229064340670604 -0.00083999475275931
0.000183832512004045 -0.000795906126413115
0.000142833805497844 -0.000749455238427288
0.000106309223905754 -0.000701169565971327
7.44485022305952e-05 -0.00065157535772542
4.73901162436619e-05 -0.000601192656397131
2.52217785696729e-05 -0.000550530556417073
7.98140216318188e-06 -0.000500082734554042
-4.34149570338604e-06 -0.000450323285321019
-1.1803977249869e-05 -0.000401702890975741
-1.45074877142548e-05 -0.000354645350139293
-1.25953128424783e-05 -0.000309544486299274
-6.24972697771398e-06 -0.000266761451094055
4.31113056009735e-06 -0.000226622435874901
1.88366108169191e-05 -0.000189416797290676
3.70471024631058e-05 -0.000155395601183272
5.86377302607133e-05 -0.000124770583990852
8.32821640628367e-05 -9.77135260882278e-05
0.000110636497650418 -7.43560291667222e-05
0.0001403431582645 -5.47896857447938e-05
0.000172034808459287 -3.90666240512871e-05
0.000205338202539096 -2.72004116403934e-05
0.000239877962680879 -1.91672947664756e-05
0.000275280241794462 -1.49077506534923e-05
0.000311176241510225 -1.43283268769778e-05
0.000347205556817443 -1.73037393658149e-05
0.000383019321828826 -2.36792001295782e-05
0.000418283133639008 -3.32729449041835e-05
0.000452679733236039 -4.58789285247008e-05
0.000485911427769992 -6.12696566442139e-05
0.000517702239394069 -7.91991218775934e-05
0.000547799769950785 -9.94058128611641e-05
0.000575976774079834 -0.000121615764314242
0.000602032435264022 -0.000145545617648679
0.000625793344529058 -0.000170905662542964
0.00064711418148633 -0.000197402831130233
0.000665878103593087 -0.000224743617316392
0.000681996848109989 -0.000252636897062786
0.000695410558574139 -0.000280796624796409
0.000706087344468642 -0.000308944385523091
0.000714022590946328 -0.000336811783231639
0.00071923803118068 -0.000364142648251686
0.000721780601288913 -0.000390695048906764
0.000721721093878358 -0.000416243095841651
0.000719152633124054 -0.000440578528774438
0.000714188989661579 -0.000463512077818251
0.000706962759343455 -0.000484874595354512
0.000697623426784588 -0.000504517954990291
0.000686335336578026 -0.00052231571780581
0.000673275594804679 -0.000538163567981087
0.000658631923915465 -0.000551979521148382
0.000642600492653855 -0.000563703912575875
0.00062538374228005 -0.000573299172305752
0.000607188230789646 -0.000580749397485647
0.000588222514291914 -0.000586059733219457
0.000568695085199522 -0.000589255574539038
0.000548812383712516 -0.000590381603146284
0.000528776900534211 -0.000589500674731624
0.000508785384072397 -0.000586692572628777
0.000489027166633349 -0.000582052643583353
0.000469682620913403 -0.000575690334141399
0.000450921756449674 -0.000567727644437355
0.00043290296544285 -0.000558297516974449
0.000415771923528041 -0.000547542178530591
0.000399660651261513 -0.000535611452047391
0.000384686739135276 -0.00052266105659271
0.000370952737851482 -0.0005088509109612
0.000358545713774916 -0.00049434345771715
0.000347536967936435 -0.000479302022785788
0.000337981915723873 -0.000463889224651126
0.000329920121792782 -0.000448265446909346
0.000323375485869803 -0.000432587386644201
0.000318356570975453 -0.000417006689140464
0.000314857066618046 -0.000401668679621991
0.000312856377565396 -0.00038671120014655
0.000312320327676474 -0.000372263559675901
0.000313201969120769 -0.000358445602049784
0.000315442484126294 -0.000345366898400812
0.000318972168862786 -0.000333126065555689
0.000323711485236799 -0.00032181021390798
0.0003295721705463 -0.000311494523945299
0.000336458390036043 -0.00030224195251094
0.000344267921388308 -0.000294103065943574
0.000352893358218864 -0.000287115997494425
0.000362223319612553 -0.000281306524737346
0.000372143655654966 -0.000276688262829339
0.000382538636205965 -0.000273262966342003
0.000393292111883881 -0.000271020934349053
0.000404288638936379 -0.000269941510083527
0.000415414556588445 -0.000269993667600943
0.000426559009479632 -0.000271136677028494
0.000437614906502404 -0.000273320838104496
0.000448479809934454 -0.000276488273961206
0.000459056748821851 -0.000280573774762871
0.000469254950544951 -0.000285505681080878
0.000478990487186692 -0.000291206797754739
0.000488186834179061 -0.000297595327872102
0.000496775337913036 -0.000304585817886505
0.000504695591342141 -0.000312090103900431
0.000511895717824729 -0.000320018249833964
0.000518332562965185 -0.000328279469830051
0.000523971796987155 -0.00033678302515483
0.000528787928441687 -0.000345439089677768
0.00053276423311388 -0.000354159574936119
0.000535892602282928 -0.000362858910008867
0.00053817331356143 -0.000371454768863799
0.000539614729767379 -0.000379868741596567
0.000540232931520279 -0.000388026943689113
0.000540051289405596 -0.000395860560956862
0.000539099980922941 -0.000403306326060004
0.000537415460636126 -0.000410306925761716
0.000535039888548638 -0.000416811336418021
0.000532020524648402 -0.00042277508723032
0.000528409096013149 -0.000428160452120352
0.000524261144059679 -0.000432936570206266
0.00051963535861077 -0.000437079495988257
0.000514592905375366 -0.000440572182267118
0.0005091967535229 -0.000443404397636016
0.000503511011000768 -0.000445572581508458
0.000497600271218701 -0.00044707964111268
0.000491528979150502 -0.000447934693646346
0.000485360821205205 -0.00044815275824206
0.000479158144447211 -0.000447754402795653
0.000472981408453421 -0.000446765349987999
0.000466888675427768 -0.000445216048934327
0.000460935140782937 -0.00044314121589295
0.000455172708260676 -0.000440579350797776
0.000449649611262259 -0.000437572235792771
0.000444410082552693 -0.000434164418987137
0.000439494074672808 -0.00043040269104111
0.000434937030100002 -0.000426335558383784
0.00043076970348821 -0.000422012719333509
0.000427018034375948 -0.000417484546908042
0.000423703071009029 -0.000412801583831168
0.000420840942856771 -0.000408014054201544
0.000418442881784387 -0.000403171394804502
0.000416515288666375 -0.000398321811410085
0.000415059844067756 -0.000393511861691564
0.00041407366011903 -0.000388786069947855
0.000413549470197339 -0.000384186573530343
0.000413475854283973 -0.000379752805926614
0.00041383749555024 -0.000375521215666197
0.000414615465139434 -0.00037152502494564
0.000415787531174772 -0.000367794026651325
0.000417328488754976 -0.000364354422007551
0.000419210506267476 -0.000361228698071869
0.000421403484599736 -0.000358435544864477
0.000423875424857556 -0.000355989811826163
0.000426592801950676 -0.00035390250279832
0.000429520938894257 -0.000352180807443148
0.000432624378628788 -0.000350828168155459
0.000435867250818234 -0.000349844380608033
0.000439213628720125 -0.00034922572515228
0.000442627874646107 -0.000348965127461298
0.000446074969829624 -0.000349052345157475
0.000449520826816041 -0.000349474178499065
0.000452932582202692 -0.000350214701516194
0.000456278866495907 -0.000351255510970816
0.000459530051115209 -0.000352575990287818
0.000462658469100319 -0.000354153584979144
0.00046563860959381 -0.000355964087106031
0.000468447284877271 -0.000357981925247941
0.00047106376937478 -0.000360180457139592
0.000473469909811897 -0.000362532262180082
0.000475650207286904 -0.000365009431174457
0.000477591870676974 -0.000367583849936182
0.000479284842779037 -0.000370227475197993
0.000480721798833628 -0.000372912600099085
0.000481898119589985 -0.000375612106473966
0.000482811839127351 -0.000378299703321261
0.000483463569112885 -0.000380950148066717
0.00048385640141646 -0.000383539450652393
0.00048399579046432 -0.000386045057780393
0.000483889417058236 -0.000388446017559829
0.000483547035852183 -0.0003907231223792
0.000482980308351699 -0.000392859030498016
0.000482202623938832 -0.000394838365259886
0.000481228910501841 -0.000396647791802707
0.000480075436939842 -0.000398276072282044
0.000478759610533785 -0.00039971409817241
0.000477299769803707 -0.000400954901692785
0.000475714976587938 -0.00040199364635285
0.000474024808099216 -0.000402827597298483
0.000472249151689752 -0.000403456072366026
0.00047040800409448 -0.000403880376008914
0.000468521276204115 -0.000404103716075355
0.000466608606375374 -0.000404131105437244
0.000464689182395617 -0.00040396925002284
0.000462781574235294 -0.000403626424521519
0.000460903578781924 -0.000403112337473033
0.000459072077196865 -0.000402437987798265
0.000457302906701429 -0.000401615513730746
0.000455610745799362 -0.000400658036411983
0.000454009016056744 -0.00039957949984526
0.000452509797883138 -0.000398394508039246
0.000451123763507866 -0.000397118162542398
0.000449860124701829 -0.000395765900172762
0.00044872659677786 -0.000394353333948771
0.000447729378487693 -0.000392896097650919
0.000446873146206173 -0.000391409695602363
0.00044616106395523 -0.000389909359743257
0.000445594806436134 -0.000388409913053778
0.000445174596199749 -0.000386925643368841
0.000444899253409403 -0.000385470185271686
0.000444766256681106 -0.000384056413533784
0.000444771814645861 -0.000382696347074329
0.000444910947894783 -0.000381401064693421
0.00044517757839202 -0.000380180632522098
0.000445564626545547 -0.000379044043864241
0.000446064114594691 -0.000377999171796262
0.000446667274482948 -0.000377052733561811
0.00044736466028894 -0.000376210267315713
0.000448146261605942 -0.000375476121721618
0.000449001620093981 -0.000374853456222013
0.000449919944653487 -0.000374344253234682
0.000450890226618483 -0.000373949341280877
0.000451901352629847 -0.000373668427883445
0.000452942214453245 -0.000373500142401895
0.000454001814723881 -0.000373442087230558
0.00045506936834272 -0.000373490897505491
0.000456134397422758 -0.00037364230728798
0.000457186821105182 -0.000373891222622547
0.000458217037028419 -0.000374231799412428
0.000459215996624351 -0.000374657526059252
0.000460175271289387 -0.000375161309300154
0.000461087111226277 -0.000375735562773372
0.000461944495246058 -0.000376372296781113
0.000462741171832093 -0.00037706320902231
0.000463471691372064 -0.000377799775137078
0.000464131430035764 -0.000378573337627586
0.000464716604193782 -0.000379375193766407
0.000465224276830156 -0.000380196680090705
0.000465652355499557 -0.000381029253482268
0.000465999582285548 -0.000381864568861801
0.000466265516065434 -0.00038269455168205
0.000466450507879301 -0.00038351146539739
0.000466555669090596 -0.000384307973366305
0.000466582834068419 -0.00038507719478531
0.000466534516579742 -0.000385812753933124
0.000466413861984094 -0.000386508823353893
0.000466224594671161 -0.000387160159981192
0.000465970961705864 -0.000387762134167247
0.000465657673819564 -0.000388310752526877
0.00046528984412042 -0.000388802672979693
0.000464872924448301 -0.000389235213891226
0.000464412641811407 -0.000389606355859939
0.000463914933682474 -0.000389914737873198
0.000463385883751499 -0.000390159646435961
0.000462831658687435 -0.000390340999548044
0.000462258446393804 -0.000390459325341652
0.000461672395923429 -0.000390515734899566
0.000461079560391653 -0.000390511890955736
0.000460485842520342 -0.000390449972762497
0.000459896943494797 -0.000390332636456492
0.000459318315687796 -0.000390162973161523
0.000458755119694843 -0.000389944463577763
0.000458212185121099 -0.000389680931260017
0.000457693976507301 -0.000389376493703963
0.000457204563458546 -0.000389035512643687
0.000456747595693585 -0.000388662543787888
0.000456326283568842 -0.00038826228626121
0.000455943382682733 -0.000387839532638878
0.000455601183890764 -0.000387399119986753
0.000455301507914285 -0.000386945882077327
0.0004550457046264 -0.000386484603083659
0.000454834656760994 -0.000386019974211393
0.000454668788572477 -0.000385556551478317
0.000454548077481576 -0.000385098717675447
0.000454472070732237 -0.000384650646243045
0.000454439904792991 -0.000384216269004867
0.000454450327751488 -0.000383799247199335
0.000454501725911882 -0.000383402946226852
0.000454592151447386 -0.000383030413853902
0.000454719353157884 -0.000382684362595143
0.000454880808728575 -0.000382367155530972
0.000455073758216074 -0.000382080796345718
0.000455295239280673 -0.000381826922829731
0.000455542122312025 -0.000381606804367607
0.00045581114650517 -0.000381421342691368
0.000456098955478268 -0.000381271076744127
0.000456402132734013 -0.000381156190083942
0.000456717236660964 -0.000381076521922097
0.000457040833911293 -0.000381031580825919
0.000457369532261609 -0.000381020561086132
0.000457700011434525 -0.000381042361990325
0.000458029052030184 -0.000381095608208426
0.000458353562903469 -0.000381178673233507
0.000458670606121814 -0.00038128970348339
0.000458977419658169 -0.000381426644338489
0.000459271437177833 -0.000381587266790717
0.000459550305816236 -0.000381769194934378
0.000459811901148299 -0.000381969933695103
0.000460054339157523 -0.000382186897347481
0.000460275985783909 -0.000382417437045035
0.000460475463672338 -0.000382658868371522
0.000460651656101874 -0.000382908498508527
0.000460803708486779 -0.000383163652092122
0.000460931027058464 -0.000383421696035668
0.000461033275353628 -0.000383680063222869
0.00046111036835228 -0.000383936274968022
0.000461162464301168 -0.00038418796112083
0.000461189954513941 -0.000384432878998808
0.00046119345145712 -0.000384668930347942
0.000461173774677803 -0.000384894176185924
0.000461131936178916 -0.000385106849698502
0.000461069123526059 -0.000385305367011313
0.000460986682274012 -0.000385488335680861
0.0004608860975992 -0.000385654561156912
0.000460768975335313 -0.000385803051493383
0.000460637021893362 -0.000385933019177997
0.000460492024810577 -0.000386043881611897
0.000460335832457304 -0.000386135259500264
0.000460170334488197 -0.000386206973033154
0.000459997442396443 -0.000386259036456948
0.000459819070078638 -0.000386291651295778
0.000459637115746148 -0.00038630519774685
0.000459453444364044 -0.000386300224345604
0.000459269871086576 -0.000386277437051774
0.000459088145444042 -0.000386237687003188
0.000458909937222529 -0.000386181956777421
0.000458736823151895 -0.000386111346937668
0.000458570275249315 -0.000386027060770289
0.000458411650626545 -0.000385930389541045
0.000458262182439384 -0.000385822696699734
0.000458122972320396 -0.000385705402653258
0.000457994985065824 -0.00038557996894184
0.00045787904385719 -0.000385447882756296
0.000457775827548801 -0.000385310642084136
0.000457685869303504 -0.000385169740805935
0.000457609556837824 -0.000385026654598164
0.000457547133756009 -0.000384882827624722
0.000457498702388648 -0.000384739659754274
0.000457464227675786 -0.000384598494719057
0.00045744354256172 -0.000384460609438975
0.000457436354345475 -0.000384327204049129
0.000457442251711626 -0.000384199393266726
0.000457460713068514 -0.000384078198742088
0.000457491115408715 -0.000383964542507442
0.000457532743791234 -0.000383859241921414
0.000457584801500488 -0.00038376300555143
0.000457646420620961 -0.000383676430104174
0.000457716672729092 -0.000383599998869499
0.000457794579894255 -0.000383534081059622
0.000457879126059879 -0.000383478932366899
0.000457969267781522 -0.000383434696452412
0.000458063945103504 -0.000383401407752615
0.00045816209271976 -0.000383378994925465
0.00045826264992499 -0.000383367285362368
0.000458364570793179 -0.000383366010282771
0.000458466833464399 -0.000383374810752457
0.000458568449271723 -0.000383393244611341
0.000458668470663781 -0.000383420793284017
0.000458765999255206 -0.000383456869528231
0.000458860192335209 -0.00038350082560612
0.000458950268976466 -0.00038355196158335
0.000459035515362416 -0.000383609533884055
0.000459115289029199 -0.000383672763799581
0.000459189022777196 -0.000383740846423564
0.000459256227387073 -0.000383812958919094
0.000459316493097717 -0.000383888269421817
0.000459369491119688 -0.000383965944912745
0.000459414973773775 -0.000384045159645297
0.000459452773956315 -0.000384125102325328
0.000459482803766065 -0.00038420498363223
0.000459505052830878 -0.000384284042972638
0.000459519585255919 -0.000384361554580437
0.000459526536586097 -0.000384436833272161
0.000459526110127229 -0.000384509239463426
0.000459518572174744 -0.000384578183954432
0.000459504247675824 -0.000384643131308593
0.000459483514696046 -0.000384703603437231
0.000459456799129399 -0.000384759182097127
0.000459424568665767 -0.000384809510350692
0.00045938732730022 -0.000384854294360082
0.000459345608884831 -0.000384893303561284
0.000459299970943405 -0.000384926370749383
0.000459250988731341 -0.00038495339145328
0.000459199248904696 -0.000384974322727771
0.000459145343654654 -0.000384989181007711
0.000459089864678575 -0.000384998040477313
0.000459033397692821 -0.000385001029659549
0.000458976517151655 -0.000384998328943453
0.000458919780928824 -0.000384990166288901
0.000458863725777192 -0.000384976813954552
0.000458808862699556 -0.000384958583829587
0.000458755673335531 -0.000384935823589672
0.000458704606092653 -0.000384908911644999
0.000458656073092811 -0.000384878252564391
0.000458610447873653 -0.000384844272446117
0.000458568062617459 -0.000384807413738031
0.000458529206943226 -0.000384768130942348
0.000458494126423403 -0.00038472688527591
0.000458463021818289 -0.000384684140477987
0.000458436048692334 -0.000384640358017663
0.000458413317840467 -0.000384595992922954
0.000458394895455072 -0.000384551489634788
0.000458380804317926 -0.00038450727797823
0.000458371025043647 -0.00038446376979806
0.000458365497561175 -0.000384421355576592
0.000458364123606003 -0.000384380401548867
0.000458366768587126 -0.00038434124682496
0.000458373264311973 -0.000384304201364927
0.000458383411842789 -0.000384269543875604
0.000458396984457821 -0.000384237520467678
0.000458413730690665 -0.000384208343323422
0.000458433377739098 -0.000384182189890225
0.000458455634928967 -0.000384159202369005
0.000458480196881439 -0.000384139487721313
0.00045850674707637 -0.000384123117882496
0.000458534961309098 -0.000384110130280391
0.000458564510893211 -0.000384100528446396
0.00045859506622925 -0.000384094283866432
0.000458626299746356 -0.000384091336830039
0.000458657888994907 -0.000384091598252922
0.00045868951981376 -0.000384094951463965
0.000458720888442343 -0.000384101254457647
0.000458751704808691 -0.000384110342356081
0.000458781694213428 -0.000384122029284839
0.000458810599688775 -0.000384136111108546
0.000458838183700294 -0.000384152368276602
0.000458864229763378 -0.000384170568239028
0.000458888543896308 -0.000384190467968892
0.000458910955460468 -0.000384211817063829
0.000458931318076949 -0.000384234360112146
0.000458949510260709 -0.000384257839378677
0.00045896543536017 -0.000384281997405367
0.000458979021900063 -0.000384306579213956
0.000458990223238587 -0.000384331335137489
0.000458999017284967 -0.000384356022493648
0.000459005405680557 -0.000384380408007701
0.000459009412971056 -0.000384404269571093
0.000459011085364835 -0.00038442739784017
0.000459010490031275 -0.000384449598023195
0.000459007713359938 -0.000384470691219718
0.000459002859397373 -0.000384490515212832
0.000458996048246618 -0.000384508925986182
0.00045898741468875 -0.000384525797883839
0.000458977105779468 -0.000384541024516238
0.000458965279715784 -0.000384554518955582
0.000458952103318921 -0.00038456621389571
0.00045893775050132 -0.000384576061673414
0.000458922400056849 -0.000384584033927382
0.000458906234110046 -0.000384590121218054
0.000458889436004029 -0.000384594332434318
0.00045887218863605 -0.000384596694008366
0.000458854672642062 -0.000384597249226459
0.00045883706493477 -0.000384596056939301
0.000458819536854449 -0.000384593190695171
0.000458802252978785 -0.000384588737485814
0.00045878536971955 -0.000384582796137067
0.000458769034150208 -0.000384575476402915
0.00045875338259016 -0.000384566897132288
0.000458738540247694 -0.000384557185061141
0.00045872462012575 -0.000384546473128466
0.000458711722405525 -0.000384534899279032
0.000458699933849616 -0.000384522604715443
0.00045868932765103 -0.00038450973241666
0.000458679962997977 -0.000384496425798631
0.000458671885182227 -0.000384482827481492
0.000458665125607993 -0.000384469077641114
0.000458659701955355 -0.000384455313032106
0.000458655618562176 -0.000384441665566726
0.000458652866704767 -0.000384428261423153
0.000458651425297774 -0.000384415219986778
0.0004586512615532 -0.000384402652876759
0.000458652331584375 -0.00038439066321061
0.000458654581304785 -0.000384379344996688
0.000458657947330465 -0.000384368782452071
0.000458662357793571 -0.000384359049547811
0.000458667733463258 -0.000384350209714057
0.00045867398860544 -0.000384342315719266
0.000458681032228014 -0.000384335409208347
0.000458688769088056 -0.000384329521043725
0.000458697100697236 -0.000384324671340863
0.000458705926217107 -0.000384320869358135
0.000458715143825117 -0.000384318114118543
0.000458724651652531 -0.000384316394846707
0.000458734348452339 -0.000384315691061232
0.000458744135096723 -0.000384315973409599
0.000458753914706733 -0.000384317204087381
0.000458763594282985 -0.000384319337669581
0.000458773084933028 -0.000384322321643538
0.000458782302702687 -0.000384326097300658
0.000458791169229755 -0.000384330600383009
0.000458799612356842 -0.000384335762205978
0.000458807566548813 -0.000384341509821695
0.000458814973193 -0.000384347767557358
0.000458821781117891 -0.000384354457640512
0.000458827946463458 -0.000384361500749719
0.000458833433281569 -0.000384368816952474
0.000458838213251767 -0.000384376326806546
0.000458842265874893 -0.000384383951651301
0.00045884557831144 -0.000384391614641544
0.000458848145257207 -0.000384399241170286
0.000458849968794084 -0.000384406759703637
0.000458851057862475 -0.00038441410238832
0.000458851428106755 -0.00038442120523996
0.000458851101701185 -0.000384428009006399
0.000458850106387132 -0.000384434459363092
0.00045884847544464 -0.000384440507200878
0.000458846247081368 -0.000384446109155334
0.000458843464031133 -0.000384451227620985
0.000458840172345987 -0.000384455830776176
0.0004588364216076 -0.000384459893073341
0.000458832263978692 -0.000384463394894397
0.0004588277536417 -0.000384466322756793
0.000458822946169946 -0.000384468669150095
0.000458817897998287 -0.000384470432340578
0.000458812666021657 -0.000384471616150961
0.000458807306571885 -0.000384472229828958
0.000458801875542036 -0.000384472287965565
0.000458796427199815 -0.000384471809635301
0.00045879101440427 -0.000384470818552529
0.000458785687307284 -0.000384469342382232
0.000458780493886479 -0.000384467412459344
0.000458775479021512 -0.000384465063316242
0.000458770684121035 -0.000384462332355895
0.000458766147209744 -0.000384459259144876
0.000458761902464744 -0.000384455885303225
0.000458757979924229 -0.000384452253680223
0.00045875440584453 -0.000384448408194515
0.000458751201763974 -0.000384444393056071
0.000458748385177898 -0.000384440252748419
0.000458745969146079 -0.000384436031204416
0.000458743962553854 -0.000384431771614402
0.000458742369946918 -0.000384427516078034
0.000458741191867063 -0.000384423305018089
0.000458740424923221 -0.000384419177077433
0.00045874006175417 -0.000384415168753094
0.000458740091406895 -0.000384411314044542
0.00045874049963146 -0.000384407644300921
0.000458741269085294 -0.000384404188061183
0.00045874237962451 -0.000384400970620646
0.000458743808467332 -0.000384398014269038
0.00045874553069325 -0.000384395338006271
0.000458747519379799 -0.000384392957375468
0.000458749746163889 -0.000384390884619279
0.000458752181209832 -0.000384389128541329
0.000458754793859484 -0.000384387694719379
0.00045875755288094 -0.000384386585281504
0.000458760426734983 -0.000384385799442555
0.000458763383804239 -0.000384385333084936
0.000458766392979371 -0.000384385179383884
0.000458769423731908 -0.000384385328576542
0.000458772446187083 -0.000384385768612105
0.000458775431832592 -0.000384386484800103
0.000458778353451095 -0.000384387460552915
0.000458781185585622 -0.00038438867735735
0.000458783904122129 -0.000384390114991362
0.000458786487325114 -0.00038439175182603
0.000458788915256747 -0.000384393565187935
0.000458791170277806 -0.000384395531494164
0.000458793237008592 -0.0003843976265685
0.000458795102312948 -0.000384399825758663
0.000458796755671287 -0.000384402104337767
0.000458798188777365 -0.000384404437806296
0.000458799395850917 -0.000384406801881454
0.000458800373214885 -0.000384409172916378
0.000458801119822994 -0.000384411527935669
0.000458801636773032 -0.000384413845189613
0.000458801927173624 -0.000384416103706542
0.000458801996416014 -0.000384418284088639
0.00045880185170688 -0.000384420368327199
0.000458801502100314 -0.000384422339841706
0.000458800958151429 -0.000384424184002086
0.000458800231882606 -0.000384425887492768
0.000458799336806592 -0.000384427439232837
0.000458798287411355 -0.000384428829690364
0.000458797099259556 -0.000384430051369122
0.000458795788595978 -0.000384431098567006
0.000458794372349303 -0.000384431967582088
0.00045879286773598 -0.000384432656346689
0.00045879129226023 -0.000384433164803966
0.000458789663511538 -0.000384433494378555
0.000458787998931953 -0.000384433648299876
0.00045878631568641 -0.000384433631381853
0.000458784630531284 -0.00038443344980621
0.00045878295971491 -0.000384433111268123
0.000458781318544155 -0.000384432624542796
0.000458779721631331 -0.000384431999492563
0.000458778182736097 -0.000384431247084649
0.000458776714452824 -0.000384430379078537
0.000458775328286976 -0.000384429407731091
0.000458774034559184 -0.000384428346038135
0.000458772842327093 -0.000384427207279714
0.000458771759399568 -0.000384426005215488
0.000458770792226559 -0.000384424753509194
0.000458769945979043 -0.000384423465909833
0.000458769224399802 -0.000384422155914166
0.000458768629858497 -0.000384420836894606
0.000458768163616341 -0.000384419521807899
0.000458767825444184 -0.000384418223006833
0.000458767614226474 -0.00038441695237168
0.000458767527279136 -0.000384415720866116
0.000458767561063667 -0.000384414539027489
0.000458767710977526 -0.000384413416306018
0.000458767971426965 -0.000384412361309927
0.000458768336088156 -0.000384411381737948
0.00045876879771356 -0.000384410484301156
0.000458769348398391 -0.000384409674644814
0.000458769979832852 -0.000384408957344817
0.000458770683014365 -0.000384408335985853
0.000458771448691664 -0.000384407813065479
0.000458772267368346 -0.000384407390043862
0.000458773129324186 -0.000384407067443249
0.000458774024881592 -0.000384406844858631
0.000458774944188889 -0.000384406720691288
0.000458775877598683 -0.000384406692806039
0.000458776815751349 -0.000384406757895306
0.000458777749539507 -0.000384406912093738
0.00045877867013111 -0.000384407150757937
0.000458779569180834 -0.000384407468686732
0.000458780438922446 -0.000384407859936431
0.00045878127214749 -0.000384408318240048
0.000458782062120022 -0.000384408836701766
0.000458782802885693 -0.000384409408322739
0.000458783489085235 -0.000384410025660031
0.000458784116100119 -0.000384410681313341
0.000458784680143154 -0.000384411367683413
0.000458785177888998 -0.000384412077000462
0.000458785607047929 -0.000384412801722078
0.000458785965987474 -0.000384413534352035
0.000458786253716426 -0.000384414267610822
0.000458786470010963 -0.000384414994655913
0.000458786615361362 -0.000384415708577279
0.000458786690931134 -0.000384416402972931
0.000458786698491309 -0.000384417072051946
0.000458786640384901 -0.000384417710343143
0.000458786519349275 -0.000384418312737722
0.000458786339034845 -0.000384418874720183
0.000458786103120445 -0.000384419392474911
0.000458785815784069 -0.000384419862580643
0.000458785481736612 -0.000384420282266262
0.000458785105706738 -0.000384420649307771
0.000458784692977332 -0.000384420962014076
0.000458784248511535 -0.000384421219404629
0.00045878377790487 -0.000384421420935865
0.000458783286440223 -0.000384421566756998
0.000458782779556799 -0.000384421657422251
0.000458782262722224 -0.000384421693976122
0.000458781741230041 -0.000384421678024438
0.00045878122026366 -0.000384421611606456
0.000458780704747141 -0.000384421497063414
0.000458780199299014 -0.000384421337269458
0.000458779708477408 -0.00038442113532966
0.000458779236447882 -0.000384420894761206
0.000458778787027825 -0.000384420619159442
0.00045877836372199 -0.000384420312435907
0.000458777969662094 -0.000384419978484374
0.000458777607590832 -0.00038441962169955
0.000458777279666478 -0.000384419246234557
0.000458776987944276 -0.000384418856210544
0.000458776733944788 -0.000384418455883662
0.00045877651873738 -0.000384418049563351
0.000458776342902922 -0.000384417641328128
0.000458776206841094 -0.000384417235075318
0.000458776110438208 -0.00038441683460988
0.000458776053106291 -0.00038441644360887
0.00045877603406197 -0.000384416065468685
0.000458776052138177 -0.000384415703301499
0.00045877610576639 -0.000384415360038304
0.000458776193168475 -0.000384415038222841
0.000458776312443732 -0.000384414740139505
0.000458776461162103 -0.000384414467898608
0.000458776637028535 -0.000384414223155716
0.000458776837247044 -0.000384414007267964
0.000458777059151316 -0.000384413821212348
0.000458777299728652 -0.000384413665766914
0.000458777556087142 -0.000384413541262063
0.000458777825325996 -0.000384413447850562
0.000458778104242441 -0.00038441338533346
0.000458778389843317 -0.000384413353156532
0.000458778679245597 -0.000384413350460022
0.000458778969525397 -0.000384413376462334
0.000458779257781927 -0.000384413429681985
0.00045877954154605 -0.000384413508818682
0.000458779818067967 -0.000384413612025014
0.000458780085082822 -0.000384413737542388
0.000458780340348852 -0.000384413883431023
0.000458780581805485 -0.000384414047445603
0.000458780807649717 -0.000384414227490026
0.000458781016330789 -0.000384414421198187
0.000458781206440051 -0.00038441462624661
0.000458781376790895 -0.00038441484031182
0.000458781526507579 -0.000384415060974419
0.000458781654845808 -0.000384415285950013
0.000458781761333071 -0.000384415512868941
0.00045878184583259 -0.000384415739596022
0.000458781908221795 -0.000384415963889495
0.000458781948701414 -0.000384416183749181
0.000458781967708433 -0.000384416397189113
0.000458781965795296 -0.000384416602411619
0.000458781943702746 -0.000384416797761133
0.00045878190242199 -0.000384416981667357
0.000458781842919365 -0.000384417152901051
0.000458781766552008 -0.000384417310225871
0.000458781674513631 -0.000384417452515606
0.000458781568243083 -0.000384417579113006
0.000458781449326651 -0.000384417689275551
0.000458781319391477 -0.000384417782502311
0.000458781180068257 -0.000384417858615649
0.000458781033000122 -0.000384417917416613
0.000458780879768028 -0.000384417958990468
0.000458780722132346 -0.000384417983536167
0.000458780561720218 -0.000384417991341479
0.000458780400251158 -0.000384417983124052
0.000458780239261714 -0.000384417959402583
0.000458780080212051 -0.000384417920997748
0.00045877992465293 -0.000384417868779963
0.000458779773897078 -0.000384417803736881
0.000458779629113337 -0.000384417726898789
0.000458779491609107 -0.000384417639473611
};
\addplot [very thick, learnedWithoutSideInfo, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131424007867825 0.024908268591485
0.127361814924592 -0.0390014571068367
0.0964899782021611 -0.0799885131599041
0.0510868986954378 -0.0941588759832221
0.00503035303231059 -0.0847567444322799
-0.0315371096831694 -0.0595024855983048
-0.0536315044814835 -0.0268832365856682
-0.0597573936546141 0.00479905075189535
-0.0515771873658508 0.0289093783258281
-0.033742853699148 0.0418706480412503
-0.0121469559333525 0.0432995251041746
0.00792670480038549 0.0351616005981406
0.0226245572827164 0.0209042661007395
0.0298304362899913 0.00464892193514288
0.0293286406062645 -0.00972382777396774
0.0226281302405198 -0.0194324545254325
0.0123243871336527 -0.0232548965002977
0.00127582901799528 -0.0214558814581842
-0.00804709741293408 -0.0154046347294141
-0.0139549814367541 -0.00711247352334965
-0.015741043568938 0.00125717288688421
-0.0136969553043578 0.00786971904672384
-0.00890929003656371 0.0115780090759898
-0.00288651171152488 0.0120627231111037
0.00285059118867537 0.00975829645942028
0.00710130424527833 0.00563176137981358
0.00918898574042082 0.000887152706518179
0.00902166606709542 -0.0033363879134285
0.00701553476812578 -0.00620574970898602
0.00391685881112025 -0.00732501535372165
0.000581916834507368 -0.00674515849326696
-0.00222620612120927 -0.00487567991070748
-0.00398483124872939 -0.00233677617069361
-0.00448438492835379 0.000208275369345756
-0.00382351522096869 0.00220372456412576
-0.00233803347034467 0.00330507659926482
-0.000488662624871239 0.00341981514555201
0.00126059096781006 0.00268612325008277
0.00254456445476769 0.00140461758657295
0.00316035955842686 -5.4216067209012e-05
0.00308469087346985 -0.00134267626996376
0.00244899602396487 -0.0022081195264434
0.00148485807555154 -0.00253222645102014
0.000456820465124963 -0.00233427034899947
-0.000400588726410689 -0.00174394654681365
-0.000928792746016427 -0.000954860710418615
-0.00106709090333013 -0.000171891224155729
-0.000849777858798362 0.000435254942750873
-0.000383053074086703 0.00076323554668889
0.000190002259499167 0.000786681909715981
0.000726766077331575 0.000550870914828749
0.00111615424741274 0.000150164988934165
0.00129765368903634 -0.000300718087114404
0.00126613969133871 -0.000695127514255489
0.00106379280647673 -0.000956417559411449
0.000763040640949342 -0.00104968137656059
0.000445750979155335 -0.000982427614626857
0.000183832512004045 -0.000795906126413115
2.52217785696729e-05 -0.000550530556417073
-1.25953128424783e-05 -0.000309544486299274
5.86377302607133e-05 -0.000124770583990852
0.000205338202539096 -2.72004116403934e-05
0.000383019321828826 -2.36792001295782e-05
0.000547799769950785 -9.94058128611641e-05
0.000665878103593087 -0.000224743617316392
0.00071923803118068 -0.000364142648251686
0.000706962759343455 -0.000484874595354512
0.000642600492653855 -0.000563703912575875
0.000548812383712516 -0.000590381603146284
0.000450921756449674 -0.000567727644437355
0.000370952737851482 -0.0005088509109612
0.000323375485869803 -0.000432587386644201
0.000313201969120769 -0.000358445602049784
0.000336458390036043 -0.00030224195251094
0.000382538636205965 -0.000273262966342003
0.000437614906502404 -0.000273320838104496
0.000488186834179061 -0.000297595327872102
0.000523971796987155 -0.00033678302515483
0.000539614729767379 -0.000379868741596567
0.000535039888548638 -0.000416811336418021
0.000514592905375366 -0.000440572182267118
0.000485360821205205 -0.00044815275824206
0.000455172708260676 -0.000440579350797776
0.00043076970348821 -0.000422012719333509
0.000416515288666375 -0.000398321811410085
0.00041383749555024 -0.000375521215666197
0.000421403484599736 -0.000358435544864477
0.000435867250818234 -0.000349844380608033
0.000452932582202692 -0.000350214701516194
0.000468447284877271 -0.000357981925247941
0.000479284842779037 -0.000370227475197993
0.00048385640141646 -0.000383539450652393
0.000482202623938832 -0.000394838365259886
0.000475714976587938 -0.00040199364635285
0.000466608606375374 -0.000404131105437244
0.000457302906701429 -0.000401615513730746
0.000449860124701829 -0.000395765900172762
0.000445594806436134 -0.000388409913053778
0.000444910947894783 -0.000381401064693421
0.00044736466028894 -0.000376210267315713
0.000451901352629847 -0.000373668427883445
0.000457186821105182 -0.000373891222622547
0.000461944495246058 -0.000376372296781113
0.000465224276830156 -0.000380196680090705
0.000466555669090596 -0.000384307973366305
0.000465970961705864 -0.000387762134167247
0.000463914933682474 -0.000389914737873198
0.000461079560391653 -0.000390511890955736
0.000458212185121099 -0.000389680931260017
0.000455943382682733 -0.000387839532638878
0.000454668788572477 -0.000385556551478317
0.000454501725911882 -0.000383402946226852
0.000455295239280673 -0.000381826922829731
0.000456717236660964 -0.000381076521922097
0.000458353562903469 -0.000381178673233507
0.000459811901148299 -0.000381969933695103
0.000460803708486779 -0.000383163652092122
0.000461189954513941 -0.000384432878998808
0.000460986682274012 -0.000385488335680861
0.000460335832457304 -0.000386135259500264
0.000459453444364044 -0.000386300224345604
0.000458570275249315 -0.000386027060770289
0.00045787904385719 -0.000385447882756296
0.000457498702388648 -0.000384739659754274
0.000457460713068514 -0.000384078198742088
0.000457716672729092 -0.000383599998869499
0.00045816209271976 -0.000383378994925465
0.000458668470663781 -0.000383420793284017
0.000459115289029199 -0.000383672763799581
0.000459414973773775 -0.000384045159645297
0.000459526536586097 -0.000384436833272161
0.000459456799129399 -0.000384759182097127
0.000459250988731341 -0.00038495339145328
0.000458976517151655 -0.000384998328943453
0.000458704606092653 -0.000384908911644999
0.000458494126423403 -0.00038472688527591
0.000458380804317926 -0.00038450727797823
0.000458373264311973 -0.000384304201364927
0.000458455634928967 -0.000384159202369005
0.00045859506622925 -0.000384094283866432
0.000458751704808691 -0.000384110342356081
0.000458888543896308 -0.000384190467968892
0.000458979021900063 -0.000384306579213956
0.000459011085364835 -0.00038442739784017
0.00045898741468875 -0.000384525797883839
0.000458922400056849 -0.000384584033927382
0.00045883706493477 -0.000384596056939301
0.00045875338259016 -0.000384566897132288
0.00045868932765103 -0.00038450973241666
0.000458655618562176 -0.000384441665566726
0.000458654581304785 -0.000384379344996688
0.000458681032228014 -0.000384335409208347
0.000458724651652531 -0.000384316394846707
0.000458773084933028 -0.000384322321643538
0.000458814973193 -0.000384347767557358
0.000458842265874893 -0.000384383951651301
0.000458851428106755 -0.00038442120523996
0.000458843464031133 -0.000384451227620985
0.000458822946169946 -0.000384468669150095
0.000458796427199815 -0.000384471809635301
0.000458770684121035 -0.000384462332355895
0.000458751201763974 -0.000384444393056071
0.000458741191867063 -0.000384423305018089
0.000458741269085294 -0.000384404188061183
0.000458749746163889 -0.000384390884619279
0.000458763383804239 -0.000384385333084936
0.000458778353451095 -0.000384387460552915
0.000458791170277806 -0.000384395531494164
0.000458799395850917 -0.000384406801881454
0.000458801996416014 -0.000384418284088639
0.000458799336806592 -0.000384427439232837
0.00045879286773598 -0.000384432656346689
0.000458784630531284 -0.00038443344980621
0.000458776714452824 -0.000384430379078537
0.000458770792226559 -0.000384424753509194
0.000458767825444184 -0.000384418223006833
0.000458767971426965 -0.000384412361309927
0.000458770683014365 -0.000384408335985853
0.000458774944188889 -0.000384406720691288
0.000458779569180834 -0.000384407468686732
0.000458783489085235 -0.000384410025660031
0.000458785965987474 -0.000384413534352035
0.000458786698491309 -0.000384417072051946
0.000458785815784069 -0.000384419862580643
0.00045878377790487 -0.000384421420935865
0.00045878122026366 -0.000384421611606456
0.000458778787027825 -0.000384420619159442
0.000458776987944276 -0.000384418856210544
0.000458776110438208 -0.00038441683460988
0.000458776193168475 -0.000384415038222841
0.000458777059151316 -0.000384413821212348
0.000458778389843317 -0.000384413353156532
0.000458779818067967 -0.000384413612025014
0.000458781016330789 -0.000384414421198187
0.000458781761333071 -0.000384415512868941
0.000458781965795296 -0.000384416602411619
0.000458781674513631 -0.000384417452515606
0.000458781033000122 -0.000384417917416613
0.000458780239261714 -0.000384417959402583
0.000458779491609107 -0.000384417639473611
};

==> figures/smd_phase_plots/phase_plot_500_quarter_space_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.126059710979462 0.0896271765232086
0.0154455490410328 0.131384283304214
0.0513721480965614 0.0313997976481915
0.082636721432209 0.0110023710876703
0.106708213686943 0.0700695589184761
0.0293074287474155 0.120401069521904
0.0685335397720337 0.0215303190052509
0.144762814044952 0.101747281849384
0.0755311325192451 0.104764722287655
0.147041350603104 0.0762226358056068
0.0460380166769028 0.143301129341125
0.0638903304934502 0.0122154261916876
0.134745746850967 0.114434517920017
0.0611746348440647 0.13946844637394
0.124260194599628 0.0229866653680801
0.092472605407238 0.0679329335689545
0.130701825022697 0.057284202426672
0.139173373579979 0.00289910193532705
0.0123289907351136 0.0772732347249985
0.0338512100279331 0.0217431019991636
0.11681666970253 0.0987960994243622
0.019643509760499 0.0305930413305759
0.0362244434654713 0.094357930123806
0.0514646656811237 0.114206053316593
0.0903850048780441 0.0880887508392334
0.0561763308942318 0.0693369060754776
0.015913438051939 0.108600042760372
0.10721368342638 0.0280223060399294
0.052905511111021 0.138107284903526
0.149418815970421 0.130520418286324
0.0487065240740776 0.0394486486911774
0.0133920982480049 0.108594790101051
0.0300552304834127 0.10216810554266
0.083167240023613 0.126957446336746
0.0068960408680141 0.13059501349926
0.0688064098358154 0.0293086785823107
0.128035753965378 0.105342656373978
0.138893440365791 0.0664708465337753
0.141436785459518 0.0683240294456482
0.0461075492203236 0.149200320243835
0.0724221542477608 0.00792080536484718
0.0820045247673988 0.116448394954205
0.148474469780922 0.0441175550222397
0.0539027415215969 0.00797526631504297
0.112296730279922 0.0759547427296638
0.109676398336887 0.116531275212765
0.1372240036726 0.148393988609314
0.110134422779083 0.0771380960941315
0.104038491845131 0.0749923512339592
0.0175050124526024 0.10516145825386
0.024103844538331 0.0981674492359161
0.140440478920937 0.0912992581725121
0.0576616004109383 0.010666947811842
0.0583279244601727 0.0196904204785824
0.137431055307388 0.00756669929251075
0.06688442081213 0.147586598992348
0.109511204063892 0.00507567916065454
0.0349652804434299 0.148427858948708
0.0178876612335443 0.0865505784749985
0.136710658669472 0.117487624287605
0.075613871216774 0.0544831566512585
0.0856964364647865 0.0611775368452072
0.13248947262764 0.125426143407822
0.0594214424490929 0.0662747919559479
0.103569827973843 0.139848530292511
0.0919174775481224 0.0613835975527763
0.112664744257927 0.134701326489449
0.00285930675454438 0.0291176587343216
0.0745778903365135 0.0293563809245825
0.0165614597499371 0.0183865521103144
0.115193545818329 0.0815011113882065
0.107758432626724 0.0732208266854286
0.128057509660721 0.0652069225907326
0.0588799454271793 0.0158282443881035
0.0830262675881386 0.11742989718914
0.130864664912224 0.0956629291176796
0.120479449629784 0.00228296942077577
0.0539159402251244 0.127905458211899
0.022627092897892 0.0272417869418859
0.0681142285466194 0.00683047017082572
0.0742683038115501 0.105974525213242
0.0565901063382626 0.0479470379650593
0.0980423241853714 0.015290985815227
0.0401987135410309 0.140855029225349
0.139310926198959 0.080925777554512
0.0808979347348213 0.0823404118418694
0.0110648758709431 0.0494692660868168
0.038238137960434 0.137579694390297
0.0494386330246925 0.0750015452504158
0.146910011768341 0.0268907304853201
0.0473635382950306 0.0928224921226501
0.10964597761631 0.0277776028960943
0.145380571484566 0.100799761712551
0.136597111821175 0.0142897916957736
0.129612073302269 0.115576088428497
0.027934230864048 0.139315441250801
0.0814925283193588 0.0268165394663811
0.025308707728982 0.0987330973148346
0.137443214654922 0.0994996279478073
0.0416265316307545 0.0676908269524574
0.115691103041172 0.127621173858643
0.130340605974197 0.0709564313292503
0.089205414056778 0.106597431004047
0.100015394389629 0.0299089774489403
0.133798167109489 0.0126308314502239
0.119059391319752 0.0380210690200329
0.0579026751220226 0.00500079290941358
0.0307372566312551 0.0731149241328239
0.0643376931548119 0.137868314981461
0.0500246435403824 0.0473833121359348
0.00941361393779516 0.113410979509354
0.0722644329071045 0.000439742201706395
0.05632508918643 0.0638177841901779
0.114261090755463 0.0361735820770264
0.0257379449903965 0.109901405870914
0.0260166767984629 0.143626004457474
0.147024631500244 0.0860518887639046
0.0371474176645279 0.0158483777195215
0.0918784886598587 0.103078469634056
0.0741936340928078 0.00995106343179941
0.14351961016655 0.0189803019165993
0.0818610638380051 0.0360670238733292
0.0165939014405012 0.00125702773220837
0.0875000283122063 0.137915790081024
0.126323267817497 0.019434716552496
0.102820537984371 0.00600335048511624
0.06215450912714 0.129702866077423
2.92798722512089e-05 0.112838350236416
0.028193986043334 0.101814277470112
0.144707158207893 0.00698395865038037
0.0588852427899837 0.1409512758255
0.0404016189277172 0.0536858662962914
0.0755366235971451 0.083427868783474
0.0943731442093849 0.0302713122218847
0.136291086673737 0.0061657028272748
0.117966637015343 0.00828273314982653
0.0394405089318752 0.116517707705498
0.0686425864696503 0.14555861055851
0.0900317281484604 0.0150341847911477
0.0179184600710869 0.144305214285851
0.0778645724058151 0.00688879238441586
0.0364701375365257 0.105173520743847
0.0799032002687454 0.117069385945797
0.0559075772762299 0.13134354352951
0.0315456055104733 0.0707686692476273
0.124008066952229 0.0345919020473957
0.131636053323746 0.0130611835047603
0.0772032663226128 0.140912249684334
0.0668815299868584 0.055417213588953
0.127132132649422 0.0250769034028053
0.0544450394809246 0.0788068175315857
0.102669641375542 0.0423268750309944
0.0339352637529373 0.116766363382339
0.0119242370128632 0.0105324424803257
0.063947319984436 0.0970716774463654
0.116275772452354 0.0584417432546616
0.0931801348924637 0.00652110204100609
0.144701391458511 0.00398875074461102
0.0323194675147533 0.142206847667694
0.00255645927973092 0.0422582216560841
0.104891747236252 0.0458429493010044
0.00203249137848616 0.0490928441286087
0.113421373069286 0.143587291240692
0.010949706658721 0.0841038227081299
0.087025560438633 0.0143569214269519
0.0826852321624756 0.0405703112483025
0.0282575879245996 0.0553455650806427
0.0892534181475639 0.0725297853350639
0.0990475863218307 0.067402221262455
0.0393516048789024 0.0371562950313091
0.0987444221973419 0.126150771975517
0.0895861089229584 0.0349774025380611
0.0981228873133659 0.103975132107735
0.0995391830801964 0.136937618255615
0.0392169766128063 0.079342894256115
0.0635829716920853 0.0714120045304298
0.0573591068387032 0.0441724583506584
0.00399817293509841 0.027719508856535
0.0472894571721554 0.108411237597466
0.139184609055519 0.0352317579090595
0.039487037807703 0.134357094764709
0.04927858710289 0.0557515248656273
0.0629367902874947 0.139280945062637
0.0559024028480053 0.103459298610687
0.0512955375015736 0.11118983477354
0.110399201512337 0.109098613262177
0.147616147994995 0.147672459483147
0.130930230021477 0.129355058073997
0.0110514787957072 0.0861547887325287
0.087624117732048 0.0500809289515018
0.0525178276002407 0.0503235422074795
0.107802905142307 0.0342200174927711
0.144859209656715 0.149191468954086
0.0965857282280922 0.069718636572361
0.133650496602058 0.0181353706866503
0.0232196804136038 0.0543846152722836
0.0771027579903603 0.034818310290575
0.0280842650681734 0.0638328120112419
0.0305586792528629 0.0215371940284967
0.0564399808645248 0.052959930151701
0.0825752019882202 0.0352355651557446
0.00323400855995715 0.0110028693452477
0.134850814938545 0.0710656121373177
0.113447733223438 0.102790378034115
0.0183068942278624 0.0845214203000069
0.0943416282534599 0.0029987976886332
0.0780192837119102 0.108922958374023
0.0130812805145979 0.135874226689339
0.0778335630893707 0.0673545822501183
0.0754760801792145 0.121723957359791
0.104789540171623 0.135212048888206
0.131876677274704 0.00577232660725713
0.0273294467478991 0.112905003130436
0.127185791730881 0.0294300820678473
0.140331611037254 0.088337354362011
0.0134508656337857 0.0923119634389877
0.107934698462486 0.127206057310104
0.0332373827695847 0.131498664617538
0.0884316489100456 0.009884437546134
0.139608263969421 0.113304823637009
0.0874997153878212 0.0480843372642994
0.102625727653503 0.0196156110614538
0.127110525965691 0.116724252700806
0.117654114961624 0.0744862854480743
0.0705315619707108 0.0844371467828751
0.106263644993305 0.096696637570858
0.118559308350086 0.0606270916759968
0.129830583930016 0.0441520884633064
0.00608945125713944 0.0101298028603196
0.135277435183525 0.0698283910751343
0.0598524026572704 0.0372473932802677
0.123445868492126 0.0624548457562923
0.0519788302481174 0.0669865012168884
0.0746084600687027 0.0475160852074623
0.0187756326049566 0.0198752582073212
0.0930349752306938 0.0255921166390181
0.135448530316353 0.11924797296524
0.0332409404218197 0.0173890236765146
0.0983608886599541 0.012799066491425
0.0811338573694229 0.0607983954250813
0.110670827329159 0.0315677784383297
0.0420897789299488 0.0853832215070724
0.145949989557266 0.125874191522598
0.0890120789408684 0.128904163837433
0.119280248880386 0.103596016764641
0.134758979082108 0.0725098177790642
0.110508181154728 0.00913384091109037
0.0367444902658463 0.0823377147316933
0.140674754977226 0.109226763248444
0.0087839113548398 0.0116941295564175
0.149475917220116 0.102646231651306
0.0611467845737934 0.0877566784620285
0.014616240747273 0.102400206029415
0.00365043641068041 0.116095997393131
0.104546174407005 0.124319173395634
0.0558921135962009 0.0260963346809149
0.0680077970027924 0.0481640808284283
0.0592110194265842 0.103612042963505
0.10720357298851 0.0452930703759193
0.094660609960556 0.132892847061157
0.0703367590904236 0.145737692713737
0.0353243984282017 0.0911879912018776
0.113876454532146 0.0499691739678383
0.0145607171580195 0.0295654945075512
0.00797984190285206 0.0542757920920849
0.046673446893692 0.106444783508778
0.0715144798159599 0.140088066458702
0.144057899713516 0.0651383399963379
0.0403448157012463 0.10668983310461
0.0992514789104462 0.126214608550072
0.0346443876624107 0.138838112354279
0.136902883648872 0.0576081201434135
0.0277352947741747 0.0138150649145246
0.023222591727972 0.0417274422943592
0.118676163256168 0.00368626089766622
0.00339692342095077 0.0329431369900703
0.00287827290594578 0.0937284901738167
0.016902094706893 0.0878584906458855
0.0749416276812553 0.00526650017127395
0.0631038099527359 0.0799967870116234
0.0862356126308441 0.0826869904994965
0.132068917155266 0.0817722305655479
0.0351773872971535 0.0843994095921516
0.01625089161098 0.0961326211690903
0.0787480548024178 0.00716962572187185
0.0284889843314886 0.11749766767025
0.0169215649366379 0.0706115588545799
0.0375914201140404 0.00847049616277218
0.0328514315187931 0.0110723450779915
0.102549724280834 0.0351182855665684
0.0884641781449318 0.0516972653567791
0.0425934083759785 0.146630465984344
0.0441946014761925 0.134773567318916
0.0959240198135376 0.143332064151764
0.125903353095055 0.0813931003212929
0.119150720536709 0.114419922232628
0.0176883395761251 0.0636279508471489
0.0234459303319454 0.119738832116127
0.0174427069723606 0.0171949211508036
0.0733274966478348 0.0199265871196985
0.0458904355764389 0.073303185403347
0.130436137318611 0.0296708531677723
0.0401402860879898 0.0695049688220024
0.0186323113739491 0.13330203294754
0.0709266662597656 0.0793338716030121
0.0415680110454559 0.0235833432525396
0.00719246780499816 0.133822724223137
0.134537279605865 0.0346012338995934
0.0650278851389885 0.142925545573235
0.126786753535271 0.011379811912775
0.0617317296564579 0.103906311094761
0.0362310111522675 0.0187228061258793
0.114746779203415 0.134810552000999
0.0228101536631584 0.0789918228983879
0.0802884697914124 0.0823595747351646
0.059972420334816 0.0320621244609356
0.133487150073051 0.111020177602768
0.111444659531116 0.0944196060299873
0.0416592508554459 0.0427777394652367
0.121785871684551 0.0298886708915234
0.0461387373507023 0.0925521180033684
0.0195743646472692 0.122662410140038
0.0849164724349976 0.106576763093472
0.149990871548653 0.0330822505056858
0.138996779918671 0.0833243131637573
0.0170145574957132 0.108051754534245
0.0947175696492195 0.135231927037239
0.038900651037693 0.0904524549841881
0.013232558965683 0.0491798371076584
0.0831334516406059 0.133155509829521
0.0716870874166489 0.0062324577011168
0.0735354498028755 0.130344569683075
0.0580229833722115 0.0956618636846542
0.0361713506281376 0.0283010564744473
0.0698787197470665 0.031686145812273
0.0721690878272057 0.0733439326286316
0.0869070068001747 0.00557503383606672
0.0210013538599014 0.149996533989906
0.130354359745979 0.136712476611137
0.0871507003903389 0.0587546117603779
0.143877133727074 0.120860129594803
0.0502694062888622 0.144558787345886
0.0603035390377045 0.0641627460718155
0.0774569064378738 0.0547872260212898
0.0770427659153938 0.11682890355587
0.0270195305347443 0.0870320498943329
0.0611060671508312 0.100208766758442
0.0471886172890663 0.102302029728889
0.0879396498203278 0.000172155065229163
0.105693317949772 0.110890135169029
0.0961147099733353 0.0303957145661116
0.0400939099490643 0.0751709565520287
0.082476980984211 0.0403577163815498
0.0908571630716324 0.0247443839907646
0.0061498717404902 0.117735609412193
0.0629345923662186 0.0524636544287205
0.0340719223022461 0.0148865608498454
0.104461774230003 0.00340684107504785
0.0936172530055046 0.073521301150322
0.0367082096636295 0.148055359721184
0.0213599912822247 0.100676573812962
0.0833155140280724 0.06899643689394
0.0851347520947456 0.085747167468071
0.0623382218182087 0.0135454088449478
0.110467061400414 0.0384368300437927
0.053184486925602 0.124934569001198
0.00394439231604338 0.0832507461309433
0.0241723507642746 0.111580811440945
0.0334352403879166 0.0920310020446777
0.0306403879076242 0.0675907507538795
0.0787986367940903 0.117038086056709
0.0812554806470871 0.10290739685297
0.138604283332825 0.0897893682122231
0.00836394820362329 0.128217935562134
0.0107820946723223 0.148429870605469
0.0527913458645344 0.0263644922524691
0.0297252032905817 0.105325244367123
0.103513553738594 0.0222739037126303
0.0229387022554874 0.0168540049344301
0.00535693718120456 0.146236583590508
0.113584041595459 0.0013116744812578
0.00515737617388368 0.132100149989128
0.0106764696538448 0.0587610602378845
0.0860553234815598 0.0970920026302338
0.0711185410618782 0.0851156041026115
0.0020372299477458 0.120011836290359
0.125589102506638 0.1359993070364
0.0318211130797863 0.0764337703585625
0.00900029297918081 0.0831089690327644
0.046272948384285 0.110544860363007
0.114149764180183 0.141921043395996
0.0748816132545471 0.0435789972543716
0.119466349482536 0.0437573306262493
0.0989110171794891 0.142660290002823
0.105135254561901 0.0631821230053902
0.139594405889511 0.14543491601944
0.121478401124477 0.104247368872166
0.0650747939944267 0.116749368607998
0.0627402439713478 0.0150257106870413
0.143203511834145 0.0372284986078739
0.048188891261816 0.120444238185883
0.0429414920508862 0.122409336268902
0.106966882944107 0.0448797531425953
0.0219821147620678 0.0817307308316231
0.13392348587513 0.0991086512804031
0.106201320886612 0.0590249188244343
0.0662129744887352 0.00215323315933347
0.0483030267059803 0.147724688053131
0.0161626376211643 0.144342690706253
0.0407830998301506 0.0435872152447701
0.0921577662229538 0.0103915110230446
0.0810827314853668 0.000292450393317267
0.106350757181644 0.115394964814186
0.00499444268643856 0.14299388229847
0.100007116794586 0.0316224433481693
0.100871287286282 0.0105326762422919
0.00792212504893541 0.098140761256218
0.0155767826363444 0.0131912408396602
0.0854057893157005 0.14283312857151
0.147979021072388 0.131334632635117
0.0051477593369782 0.0166497118771076
0.0319727063179016 0.0282296929508448
0.0594884157180786 0.0572985783219337
0.0997360497713089 0.115266658365726
0.0795639902353287 0.147407308220863
0.0295596029609442 0.0173367988318205
0.0429823063313961 0.00401025358587503
0.0551168359816074 0.146465122699738
0.0444938018918037 0.0510862059891224
0.121826648712158 0.117350533604622
0.118147939443588 0.103984646499157
0.0620878636837006 0.127478435635567
0.0852085202932358 0.116016052663326
0.0668653473258018 0.00399146042764187
0.140021875500679 0.149759903550148
0.0654582753777504 0.100761443376541
0.0925060585141182 0.14207823574543
0.138199433684349 0.0855318084359169
0.0349211543798447 0.113135181367397
0.0343535132706165 0.0136902444064617
0.114601656794548 0.0587180554866791
0.0595807172358036 0.135587930679321
0.13538932800293 0.041206955909729
0.130657732486725 0.0337637476623058
0.0875058546662331 2.33375430980232e-05
0.107514634728432 0.00173759856261313
0.136927887797356 0.0269481409341097
0.0942110791802406 0.118043951690197
0.0373597405850887 0.0604476593434811
0.0632051602005959 0.00123380648437887
0.0589385963976383 0.0393770299851894
0.0379896648228168 0.10621327906847
0.04679274559021 0.00120695412624627
0.0143889328464866 0.144143864512444
0.0432168170809746 0.088054820895195
0.0222741980105639 0.0796655863523483
0.0533686727285385 0.0657552033662796
0.0509073175489902 0.0819379910826683
0.106498666107655 0.148161128163338
0.0884660556912422 0.106790542602539
0.0701580122113228 0.12667527794838
0.119334295392036 0.00485182553529739
0.0910911038517952 0.0105965491384268
0.122818037867546 0.00966267939656973
0.0372047238051891 0.0193484406918287
0.0642773285508156 0.137530460953712
0.149363055825233 0.0343220010399818
0.0167273599654436 0.0360086895525455
0.0257122777402401 0.127217307686806
0.0633836835622787 0.100316017866135
0.102375917136669 0.0615031011402607
0.0964506641030312 0.0187380742281675
0.113762378692627 0.0763056725263596
0.0412802696228027 0.12709829211235
0.0494297556579113 0.0910094454884529
0.0418439619243145 0.142465129494667
0.00669558765366673 0.0254317577928305
0.0254420470446348 0.0969804152846336
0.0869837552309036 0.133150428533554
0.0763218030333519 0.122853569686413
0.125443875789642 0.130300208926201
0.090585820376873 0.0550371147692204
0.0789790228009224 0.091693252325058
0.0675503015518188 0.142915800213814
0.0464116632938385 0.121719568967819
0.0532164759933949 0.0198866818100214
0.0829681679606438 0.1006029099226
0.00630428362637758 0.144192755222321
0.0116050187498331 0.104811608791351
0.042180985212326 0.0818893685936928
0.0585090965032578 0.0728256553411484
0.0352655090391636 0.100919537246227
0.0256189592182636 0.0331419333815575
0.12321775406599 0.122193612158298
0.0633485391736031 0.149149090051651
0.113337457180023 0.0654397010803223
0.145155310630798 0.101265214383602
0.093443438410759 0.00619239080697298
0.0518850013613701 0.102707609534264
};
\addplot [very thick, trueDynamics]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, approxDynamics, dashed]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, learnedWithSideInfo]
table {%
0.1 0.1
0.109246787884187 0.0849056879037491
0.116977856282425 0.0697118587300309
0.123191033969249 0.0545740180148684
0.127899505297662 0.0396419982526908
0.131130967030441 0.0250559077740711
0.132926466543096 0.0109425638129075
0.133338957170253 -0.00258659573409048
0.132431823733722 -0.0154359873737953
0.130277109831185 -0.0275248658381102
0.126954415385522 -0.0387854337854492
0.122549540600166 -0.0491606042490318
0.117153442639939 -0.0586020289505456
0.110861609433211 -0.0670685710712853
0.103773306784947 -0.0745256139450596
0.0959909596281738 -0.0809449603276278
0.0876194439393209 -0.0863054317720273
0.0787653936450396 -0.0905938243314601
0.0695362319568042 -0.0938060357641053
0.0600394635743245 -0.0959482451638003
0.0503812628900897 -0.0970377168106555
0.0406655726221058 -0.0971032922093258
0.0309928727906974 -0.0961852720839342
0.0214590428313642 -0.0943347621127941
0.0121543941123799 -0.0916125267172614
0.00316271916885161 -0.0880875118528515
-0.00543940813987145 -0.0838349665832521
-0.0135831863179909 -0.0789346835837001
-0.0212079420740005 -0.0734691784276578
-0.028261335324715 -0.0675221453208579
-0.03469939238653 -0.0611773146571117
-0.0404864991170488 -0.0545173801440768
-0.045595196125536 -0.047623456219906
-0.050006065223115 -0.0405745021067823
-0.0537074630967319 -0.0334471091811608
-0.0566952679898909 -0.0263151914150761
-0.0589726040049098 -0.0192497179924942
-0.0605495467640373 -0.0123183734813388
-0.0614427359322527 -0.00558515133463544
-0.0616750138219479 0.000890133856376707
-0.0612749820527788 0.00705238800848562
-0.0602764799959969 0.0128517940104054
-0.0587180334330828 0.0182443320280719
-0.0566422883285354 0.0231922298639624
-0.0540953216803389 0.0276643337454772
-0.0511259784534823 0.0316363000069835
-0.047785212241898 0.035090676520344
-0.0441253700484958 0.038016833668987
-0.0401995254876873 0.0404107419670865
-0.0360608343316592 0.0422746619200858
-0.031761942199843 0.0436166573162033
-0.0273544108664889 0.0444501624276725
-0.0228882190634416 0.0447933912120213
-0.0184113079789198 0.0446687741425116
-0.0139691770413678 0.0441023702634595
-0.00960457562654017 0.0431233245649061
-0.00535720221141361 0.0417632814117894
-0.0012634887463996 0.0400559167262173
0.00264358260898538 0.03803643291592
0.00633460733375517 0.0357411202579492
0.00978384610990571 0.0332069362135208
0.0129692751306613 0.0304711213377402
0.0158725905372584 0.0275708703061177
0.0184791881740466 0.0245429597757365
0.0207781240158055 0.0214234390085508
0.0227619949645598 0.018247375890077
0.0244268438607565 0.015048571276786
0.0257720272408522 0.011859299282218
0.0268000365271607 0.00871011522685095
0.0275163341193549 0.00562964925140008
0.0279291373310218 0.00264443654341662
0.0280491967376518 -0.000221219379703541
0.0278895931502436 -0.0029453593340385
0.0274654712583346 -0.00550845715453718
0.0267938123875864 -0.00789348272423496
0.0258931662785029 -0.0100859387020868
0.0247834126663143 -0.0120738644086593
0.023485491195907 -0.0138478400478625
0.0220211704513414 -0.0154009471070289
0.020412772281695 -0.0167287213381861
0.0186829594563317 -0.0178290667225589
0.0168544842052114 -0.0187021888749932
0.0149499665605168 -0.0193504718441986
0.0129916838748873 -0.0197783724687319
0.0110013724457415 -0.0199922609492909
0.00900004124768462 -0.0200002836084217
0.00700780242804734 -0.0198122015864293
0.00504371437558999 -0.0194392350786607
0.00312565389184369 -0.0188938500848437
0.00127019325363215 -0.018189626778284
-0.000507501539022737 -0.0173410445085445
-0.0021937487646886 -0.0163633037450275
-0.00377641594446666 -0.0152721528144397
-0.00524496664486505 -0.0140837099240514
-0.00659048353213659 -0.0128142796304687
-0.00780568723499855 -0.0114801980385337
-0.00888492330987051 -0.0100976584971271
-0.00982414617856747 -0.0086825734564826
-0.0106208772219098 -0.00725042795815511
-0.0112741633388076 -0.00581614192472912
-0.0117845089621703 -0.00439395423118327
-0.0121538015556109 -0.00299730934072784
-0.0123852343157014 -0.0016387660745707
-0.0124832046599297 -0.000329908170929372
-0.0124532145769211 0.000918723697118651
-0.0123017709765788 0.00209769180047914
-0.0120362636882028 0.00319870423313873
-0.0116648546342103 0.00421464308833208
-0.011196357690499 0.00513958404315318
-0.0106401166838484 0.00596879944469819
-0.0100058964273524 0.00669874361943812
-0.00930374581614789 0.00732703585816452
-0.0085439056262695 0.00785242879998904
-0.00773668371666839 0.00827476016040052
-0.00689234978887268 0.00859490215490766
-0.00602103852842832 0.00881470582310939
-0.00513265414259295 0.00893692081754338
-0.00423678095194276 0.00896514073954791
-0.00334260818403498 0.00890370668711782
-0.00245885593103784 0.0087576313286597
-0.00159371240002289 0.00853252010690397
-0.000754779602700734 0.00823447767487906
5.09720452380596e-05 0.0078700236061664
0.00081724169587559 0.00744601319633276
0.00153842684789625 0.00696954434490493
0.0022096438162143 0.00644787699847171
0.0028267394737793 0.005888355791555
0.00338629626317195 0.00529833316384298
0.00388562899719269 0.00468509571940956
0.00432277543103037 0.00405579706585968
0.00469648019858945 0.00341739667362972
0.00500616920275093 0.00277659687142062
0.00525192610077112 0.0021397949083557
0.00543445528540751 0.00151303453164786
0.00555504696145145 0.000901963779757153
0.00561553523699802 0.000311801030164816
0.00561825202374754 -0.000252694764508732
0.00556598233406944 -0.000787248179729971
0.00546191445564967 -0.00128808458279295
0.00530958733203175 -0.00175194253396072
0.00511283794299555 -0.00217608016681581
0.00487575613542536 -0.00255827704680911
0.00460262408716404 -0.00289682914110045
0.00429787113764388 -0.00319054141165154
0.00396601977082765 -0.00343871484549041
0.00361163997995589 -0.00364112931397997
0.00323929827704959 -0.00379802203640978
0.00285351694695105 -0.00391006232083058
0.00245873190432767 -0.00397832748010529
0.00205924938639482 -0.00400426899518536
0.00165921591695453 -0.00398968264241617
0.00126258081994778 -0.00393667557635169
0.000873069850384225 -0.00384762788133486
0.00049415760310921 -0.00372515734380841
0.000129047182869976 -0.00357208284851041
-0.000219348990524268 -0.00339138730056732
-0.00054842353127639 -0.00318618241432134
-0.000855884886029626 -0.00295966745283494
-0.0011397642177694 -0.00271509726819019
-0.00139841987404406 -0.00245574753495248
-0.00163053744599401 -0.00218488068954414
-0.00183512627670487 -0.00190571384686677
-0.0020115150380329 -0.00162139156480023
-0.00215934020624883 -0.00133495654360161
-0.00227853907767933 -0.00104932517466949
-0.00236933021152091 -0.000767265131614181
-0.0024322027201357 -0.000491374748762041
-0.00246789578038804 -0.000224065863640988
-0.00247737930908909 3.24506875131192e-05
-0.00246183510403454 0.000276177593860893
-0.00242263262988182 0.000505340418690992
-0.00236130713225408 0.000718394068197625
-0.00227953705331338 0.000914027274394158
-0.00217912074874668 0.0010911639685709
-0.00206195134208977 0.00124896248962614
-0.00192999576988896 0.00138681205049451
-0.00178526917027226 0.00150432914162124
-0.00162981555782114 0.00160134825553371
-0.00146568384180583 0.0016779135472369
-0.00129490896668598 0.00173426886649963
-0.00111949188836696 0.00177084454872656
-0.000941381878773628 0.00178824501830022
-0.000762459412428571 0.00178723361249666
-0.000584521672378713 0.00176871740439566
-0.000409268347140446 0.00173373156420453
-0.000238289741352843 0.00168342198344362
-7.30570183521961e-05 0.00161903033073685
8.50869316534747e-05 0.0015418745938689
0.000234934302218728 0.00145333517741975
0.000375417580729287 0.00135483579100182
0.000505613310437858 0.00124782931955281
0.00062474394625979 0.00113378079566573
0.000732178248031373 0.00101415291887363
0.000827431310005594 0.000890391465745211
0.000910160544823999 0.000763912777006936
0.000980163413757951 0.000636090728832528
0.00103737201369662 0.000508244860398577
0.00108184731481964 0.000381631135770277
0.0011137724087663 0.000257432071322228
0.00113344470901044 0.000136748714041346
0.00114126652138702 2.05941029776113e-05
0.0011377381757324 -9.01124332770564e-05
0.00112344615163958 -0.000194549782563058
0.00109905423097602 -0.000291998274128957
0.00106529290414537 -0.00038184170644584
0.00102294912556597 -0.000463568540769899
0.000972856010917705 -0.000536771682302373
0.000915881777669006 -0.000601147566964499
0.000852920257148185 -0.000656493325461582
0.000784880300729596 -0.000702705302913387
0.000712676699304401 -0.0007397737889967
0.00063722028788965 -0.000767779485094877
0.000559409854640883 -0.000786888232223504
0.000480123496864118 -0.000797344812877299
0.000400211315810084 -0.000799467101320062
0.000320487878612399 -0.000793639229122789
0.000241726499224743 -0.00078030480706559
0.000164653519332439 -0.000759959279253763
8.99433896306423e-05 -0.000733143031219186
1.8214516892559e-05 -0.000700433859275762
-4.99739285566847e-05 -0.000662438977578006
-0.000114124712387143 -0.000619788125273857
-0.000173804380899034 -0.000573126326472106
-0.000228644459917424 -0.000523106475892376
-0.000278341918796485 -0.000470382881356812
-0.000322658817703977 -0.000415604370697764
-0.000361421696584277 -0.000359408674455608
-0.000394520003694679 -0.000302416429999397
-0.000421904247649096 -0.000245225999417897
-0.000443583465504965 -0.00018840844397161
-0.000459622137862825 -0.000132503557978225
-0.000470137016645014 -7.80158935249631e-05
-0.000475293632720114 -2.54115994984261e-05
-0.000475301813984363 2.48843510419761e-05
-0.000470411843711091 7.24903088595852e-05
-0.000460910036814061 0.000117069605966691
-0.00044711387953808 0.00015833164260215
-0.000429367663905375 0.000196032603767549
-0.000408037889314122 0.000229975489208556
-0.000383508169360239 0.000260009649636572
-0.000356174982670474 0.000286030351745126
-0.000326443016254521 0.000307977257360648
-0.000294721090940975 0.000325833119454444
-0.000261417271878062 0.000339621581481708
-0.000226935521548108 0.000349405091036203
-0.00019167169792797 0.000355282438565752
-0.00015601010561897 0.000357385889731887
-0.00012032019249375 0.000355878462922732
-8.49537410987505e-05 0.000350950714850029
-5.02422710555034e-05 0.00034281735149122
-1.64946906665991e-05 0.00033171404267307
1.60045476143705e-05 0.00031789455576714
4.69971043772915e-05 0.000301626641864061
7.62520011587109e-05 0.00028318908282543
0.000103566568215405 0.000262868563709162
0.000128767023046414 0.000240956124734737
0.000151708799705275 0.000217744338289805
0.0001722765306853 0.000193524224666675
0.000190383828705051 0.00016858264550379
0.000205972522804521 0.000143199582396392
0.000219012163638607 0.000117645652895959
0.000229498684756996 9.21800118192095e-05
0.000237453325811557 6.7048360090638e-05
0.000242921177411731 4.24811314871931e-05
0.000245969507689944 1.86920446445527e-05
0.000246686088867659 -4.1232572485228e-06
0.000245177101803926 -2.57881660061798e-05
0.000241565811793437 -4.61459708169798e-05
0.000235989876477799 -6.50604235410412e-05
0.00022859952686495 -8.24160658119411e-05
0.000219555602824884 -9.81183396007168e-05
0.000209027253885941 -0.000112093501943633
0.000197190062032171 -0.000124288386043503
0.000184223844353085 -0.00013466987961408
0.000170310804933363 -0.000143224237159956
0.000155633526672944 -0.000149956340877111
0.000140373341445468 -0.000154888709438694
0.000124708336466217 -0.000158060497835066
0.000108811964546263 -0.000159526107896824
9.2851545223982e-05 -0.000159354188753014
7.69868677398533e-05 -0.000157625985934828
6.13689904729042e-05 -0.000154434125445135
4.61392768422025e-05 -0.000149881150523612
3.14283402537419e-05 -0.00014407798736471
1.73553546651134e-05 -0.000137142351913866
4.02745883358591e-06 -0.000129197403261117
-8.46074576482669e-06 -0.000120370194387931
-2.0027496010433e-05 -0.000110790296453445
-3.06040527131568e-05 -0.000100588358005638
-4.01347415743269e-05 -8.98947659280225e-05
-4.8576854990004e-05 -7.88384142360599e-05
-5.59004529035179e-05 -6.75454735983294e-05
-6.20880335947399e-05 -5.61383415700334e-05
-6.7134097149868e-05 -4.47345421328293e-05
-7.1044628890779e-05 -3.34458678530325e-05
-7.38364481969039e-05 -2.23775545400429e-05
-7.55365755165105e-05 -1.16275448007741e-05
-7.61813810942064e-05 -1.28589651637867e-06
-7.58158864922476e-05 8.56571926277638e-06
-7.44928041748749e-05 1.7854410245377e-05
-7.22716716766852e-05 2.65163702692917e-05
-6.92179930445319e-05 3.44970241741294e-05
-6.5402242035037e-05 4.17511591770392e-05
-6.08989198775806e-05 4.82429113510818e-05
-5.57857003471857e-05 5.39456061048327e-05
-5.01424402306466e-05 5.88416259326152e-05
-4.40503098433076e-05 6.29221391079682e-05
-3.75909599239777e-05 6.61867590920906e-05
-3.08456521486561e-05 6.86431244893981e-05
-2.3894522427903e-05 7.03064249414354e-05
-1.68158260134277e-05 7.11988797164054e-05
-9.68525263762843e-06 7.13492525932224e-05
-2.57533123115827e-06 7.07921495468611e-05
4.44514216245417e-06 6.95674176753869e-05
1.13115950744896e-05 6.77196096994237e-05
1.79641115486823e-05 6.52971436814198e-05
2.43477882241605e-05 6.23517386912908e-05
3.04130262986368e-05 5.893776662802e-05
3.61157684693886e-05 5.51115173479388e-05
4.14176672057232e-05 5.09306159273137e-05
4.628616298058e-05 4.64533492881003e-05
5.06945515890561e-05 4.17380798154454e-05
5.46219204966975e-05 3.68426842669578e-05
5.80531088375247e-05 3.18239782508556e-05
6.09785655434347e-05 2.67372311313352e-05
6.33941601827226e-05 2.16356863269596e-05
6.53010010705918e-05 1.65701452630174e-05
6.67050933100266e-05 1.15885844493846e-05
6.76171096064132e-05 6.73582561105945e-06
6.80520155638825e-05 2.05323926394385e-06
6.80287568248089e-05 -2.42148050944024e-06
6.75698516216378e-05 -6.65451729275901e-06
6.67009687742998e-05 -1.06160690371837e-05
6.54505930000882e-05 -1.42804480347536e-05
6.38495447007892e-05 -1.76261353495022e-05
6.19306161658284e-05 -2.06357857130968e-05
5.97280840825276e-05 -2.32961980444202e-05
5.72773712025076e-05 -2.55982391372811e-05
5.46145988675473e-05 -2.7536741441736e-05
5.17762341224887e-05 -2.91103510718926e-05
4.87986713438582e-05 -3.03213664523128e-05
4.57179048163753e-05 -3.11755323068041e-05
4.25692122242721e-05 -3.16818166012922e-05
3.93867944842169e-05 -3.18521647102443e-05
3.62035501856456e-05 -3.17012439410291e-05
3.30507518032791e-05 -3.12461686249321e-05
2.99578692475599e-05 -3.05061920471417e-05
2.69523697697394e-05 -2.95024353889062e-05
2.40594905799446e-05 -2.82575833026044e-05
2.13021678995839e-05 -2.6795578119021e-05
1.87008659687515e-05 -2.5141328496403e-05
1.6273538841205e-05 -2.33204287702904e-05
1.40355585256935e-05 -2.13588567916645e-05
1.19996813293388e-05 -1.9282714987412e-05
1.01760660397021e-05 -1.71179480759065e-05
8.57229574748042e-06 -1.489012681688e-05
7.19342013173752e-06 -1.26241845563868e-05
6.04203730859842e-06 -1.03442209997695e-05
5.11838841492362e-06 -8.07329848129257e-06
4.4204653777552e-06 -5.83327276615364e-06
3.94414096889506e-06 -3.64463294033612e-06
3.68331613932738e-06 -1.5263654269404e-06
3.63006985545922e-06 5.04156638214681e-07
3.77482985455813e-06 2.43126674703831e-06
4.10654408247724e-06 4.24107522434269e-06
4.61286486518053e-06 5.921519072416e-06
5.28032966960745e-06 7.4623942687424e-06
6.09454959632494e-06 8.85535927608316e-06
7.04039400735434e-06 1.00939336711292e-05
8.10217378945099e-06 1.11734651859763e-05
9.26382871094256e-06 1.2091093836375e-05
1.05090956802195e-05 1.28456836705482e-05
1.18216856434261e-05 1.34377557117205e-05
1.31854377464907e-05 1.38694038227527e-05
1.45844739511264e-05 1.41441897021366e-05
1.60033472853677e-05 1.42670424274627e-05
1.74271628087252e-05 1.42441489252576e-05
1.88416994879037e-05 1.40828209680421e-05
2.02335220672312e-05 1.37913783078147e-05
2.15900702031507e-05 1.33790058356453e-05
2.28997475971854e-05 1.28556340399655e-05
2.41519711121491e-05 1.22318005573163e-05
2.5337247173185e-05 1.15185161497777e-05
2.64471917799242e-05 1.07271318015023e-05
2.74745741649512e-05 9.86921649825945e-06
2.84133222543115e-05 8.95642772391625e-06
2.92585335842921e-05 8.00039488879634e-06
3.00064607524492e-05 7.01260741919896e-06
3.06544914107643e-05 6.00430482577963e-06
3.12011191654082e-05 4.98638362245174e-06
3.16459053790324e-05 3.96930508728133e-06
3.19894464318182e-05 2.96301321611736e-06
3.22332882305293e-05 1.97686220104742e-06
3.23798934682568e-05 1.01955374276486e-06
3.2432532486748e-05 9.90828574742864e-08
3.23952760010182e-05 -7.77305540822226e-07
3.22728568580288e-05 -1.60315200403716e-06
3.20706191040826e-05 -2.37280699977305e-06
3.17944343136284e-05 -3.08144808158772e-06
3.14505997248415e-05 -3.7250852678028e-06
3.10457836701777e-05 -4.30056036293536e-06
3.05869346268195e-05 -4.80554059478777e-06
3.00811775342663e-05 -5.23849680433841e-06
2.95357574043725e-05 -5.59868126259744e-06
2.89579647423238e-05 -5.88609649199157e-06
2.83550391400184e-05 -6.10146083346308e-06
2.77341292562044e-05 -6.24616367517206e-06
2.71022000475352e-05 -6.32222194596466e-06
2.64659854735672e-05 -6.33222634505159e-06
2.5831943020721e-05 -6.2792901402986e-06
2.52062045879436e-05 -6.16699580646696e-06
2.45944964500505e-05 -5.9993320888907e-06
2.40021428943721e-05 -5.78063709966159e-06
2.34340207440481e-05 -5.51553925731696e-06
2.28945247961049e-05 -5.208901011855e-06
2.23875623630992e-05 -4.86574935010253e-06
2.19165278055461e-05 -4.49123034940158e-06
2.14842988928154e-05 -4.09054554495469e-06
2.1093227706756e-05 -3.66889972980289e-06
2.07451551921534e-05 -3.23145475178421e-06
2.04414038800782e-05 -2.78327159719538e-06
2.01828033516843e-05 -2.32927204990574e-06
1.99696938761873e-05 -1.87419701447311e-06
1.98019555130852e-05 -1.4225654041411e-06
1.96790335773717e-05 -9.78643306837057e-07
1.95999513716572e-05 -5.46414614888135e-07
1.95633502032694e-05 -1.2955329609099e-07
1.95675294016456e-05 2.68595520935833e-07
1.96104608693459e-05 6.45033011892338e-07
1.96898363762077e-05 9.9711989065554e-07
1.98031112140229e-05 1.32258379181849e-06
1.9947520568081e-05 1.61952405619559e-06
2.0120130448234e-05 1.88641316256621e-06
2.03178777070656e-05 2.12209261718499e-06
2.05375973244548e-05 2.32576629244363e-06
2.07760678834629e-05 2.49699061072306e-06
2.10300297590338e-05 2.63566385783065e-06
2.12962378706716e-05 2.74200714400763e-06
2.15714853288446e-05 2.81654926581609e-06
2.18526307201872e-05 2.86010569183759e-06
2.21366326692979e-05 2.87375436158754e-06
2.24205589340332e-05 2.85881516148834e-06
2.27016246048956e-05 2.81682531522165e-06
2.29771993815187e-05 2.74951393208767e-06
2.32448585052863e-05 2.65877360305922e-06
2.35023572939669e-05 2.54663393661758e-06
2.37476602460152e-05 2.41523559552093e-06
2.39789519557582e-05 2.26680636217225e-06
2.41946443892138e-05 2.10363178609896e-06
2.43933787042461e-05 1.92803042153855e-06
2.45740270698597e-05 1.74233062821827e-06
2.47356963052336e-05 1.54884640934938e-06
2.48777242417564e-05 1.34985608823968e-06
2.49996724478035e-05 1.14758063674003e-06
2.51013171342074e-05 9.44165645222483e-07
2.518264915502e-05 7.41663352954447e-07
2.52438576363867e-05 5.42017662752414e-07
2.52853208823622e-05 3.47049283533352e-07
2.53075863666102e-05 1.58445235598492e-07
2.53113780078612e-05 -2.22523617310344e-08
2.52975543341277e-05 -1.93654344116112e-07
2.5267106663035e-05 -3.54530406809772e-07
2.52211445514183e-05 -5.03812810137561e-07
2.5160868508442e-05 -6.40599846946088e-07
2.50875736358958e-05 -7.64156560251195e-07
2.50026077899118e-05 -8.73913528209869e-07
2.49073715812287e-05 -9.69464288402833e-07
2.48033001856024e-05 -1.05056142629678e-06
2.46918487912667e-05 -1.11711189632047e-06
2.45744725903829e-05 -1.16917001236061e-06
2.44526031316361e-05 -1.20692937599642e-06
2.43276646909596e-05 -1.23071520974349e-06
2.42010215207311e-05 -1.24097302389714e-06
2.40740051342253e-05 -1.2382599621219e-06
2.39478852019082e-05 -1.22323344697861e-06
2.38238513607103e-05 -1.19664002085074e-06
2.37030259469806e-05 -1.1593038706792e-06
2.35864312543022e-05 -1.11211344133721e-06
2.34750077232754e-05 -1.05601123223664e-06
2.33696012078982e-05 -9.91981135456399e-07
2.32709520618657e-05 -9.2103739035565e-07
2.31796987757438e-05 -8.44213040807062e-07
2.30963797959866e-05 -7.62548101107541e-07
2.3021428067857e-05 -6.77080020494714e-07
2.29551710347747e-05 -5.88832719472521e-07
2.2897834276267e-05 -4.98807654736311e-07
2.28495469644513e-05 -4.07974919625076e-07
2.28103400457674e-05 -3.1726530380638e-07
2.27801680673101e-05 -2.27563404564535e-07
2.27588800738726e-05 -1.39701121781854e-07
2.27462541681767e-05 -5.44513767408716e-08
2.27419884156616e-05 2.74761191576545e-08
2.2745724491971e-05 1.05438683561943e-07
2.27570349489309e-05 1.78863704292098e-07
2.27754414052067e-05 2.47250880214267e-07
2.28004163646267e-05 3.10173863482532e-07
2.28313941307151e-05 3.6728088659288e-07
2.28677817201983e-05 4.18293716109019e-07
2.29089606821331e-05 4.63008007045573e-07
2.29542852789449e-05 5.01291282262173e-07
2.300311704731e-05 5.33080111608797e-07
2.30547975132861e-05 5.58378928872116e-07
2.3108691848378e-05 5.77254780864678e-07
2.31641615844602e-05 5.89834090902741e-07
2.32205682519221e-05 5.96300143484996e-07
2.32773261308883e-05 5.96887488768516e-07
2.33338604138933e-05 5.9187616585632e-07
2.33896290344759e-05 5.81587670467343e-07
2.34441263049501e-05 5.66378851374338e-07
2.34968701836313e-05 5.46638286635925e-07
2.35474277410913e-05 5.22780609912843e-07
2.35954133407934e-05 4.95240357167859e-07
2.36404831829018e-05 4.64466161531618e-07
2.36823262089042e-05 4.30918046134821e-07
2.3720700481733e-05 3.95060165914174e-07
2.37553877111413e-05 3.57357127001023e-07
2.37862387286319e-05 3.18268291721324e-07
2.38131243749107e-05 2.78245167351088e-07
2.38359846123082e-05 2.37725723772897e-07
2.38547812315137e-05 1.97132315804538e-07
2.38695324125682e-05 1.56866690304014e-07
2.38802872584848e-05 1.1730890392414e-07
2.3887138528994e-05 7.88122100914279e-08
2.38902099069932e-05 4.17031991162276e-08
2.38896505422165e-05 6.27808560693666e-09
2.38856423269151e-05 -2.71965063802782e-08
2.38783944388476e-05 -5.84874015885362e-08
2.38681306086175e-05 -8.73928165390225e-08
2.38551109473933e-05 -1.13745471708171e-07
2.38395828341814e-05 -1.37410808065397e-07
2.38218263905882e-05 -1.58286802331986e-07
2.38021344721173e-05 -1.76304862264942e-07
2.3780781745128e-05 -1.91427318441129e-07
2.37580556093908e-05 -2.03645871721392e-07
2.37342507417443e-05 -2.12981465352868e-07
2.37096527243158e-05 -2.19482629404411e-07
2.36845435024891e-05 -2.23223132422845e-07
2.36592050215922e-05 -2.24301174966968e-07
2.3633890124039e-05 -2.22836472829613e-07
2.36088316440536e-05 -2.18966281551047e-07
2.35842696915678e-05 -2.1284491324991e-07
2.35604298255976e-05 -2.04642205403616e-07
2.35375085014256e-05 -1.94539943265681e-07
2.35156858035407e-05 -1.82730069298032e-07
2.34951218080343e-05 -1.69411418227128e-07
2.34759602199125e-05 -1.54788438067044e-07
2.34583174597014e-05 -1.39068472293502e-07
2.3442286301037e-05 -1.22458544637993e-07
2.3427954060351e-05 -1.05164815522585e-07
2.3415380769401e-05 -8.73907879395119e-08
2.34046100890672e-05 -6.93348809477357e-08
2.33956365667809e-05 -5.11874809205892e-08
2.33884711212523e-05 -3.31308953605003e-08
2.33831101186938e-05 -1.53380312895024e-08
2.33795117266372e-05 2.02859595788141e-09
2.3377610464892e-05 1.88197617490005e-08
2.33773572243523e-05 3.48988500320502e-08
2.3378671972718e-05 5.01424857191068e-08
2.33814692200823e-05 6.444141575912e-08
2.33856452866998e-05 7.77006583518869e-08
2.33910801209353e-05 8.98418583972216e-08
2.33976754994286e-05 1.00800050972794e-07
2.34053059128964e-05 1.10524926100197e-07
2.34138476712109e-05 1.1898094243179e-07
2.34231752648251e-05 1.261464461777e-07
2.34331577266128e-05 1.32013571629841e-07
2.34436586322856e-05 1.36587708254865e-07
2.34545561091232e-05 1.3988701041967e-07
2.34657246463849e-05 1.41940844855526e-07
2.34770350947267e-05 1.42789374990571e-07
2.3488374675848e-05 1.42482857512505e-07
2.34996287916955e-05 1.41080537474636e-07
2.35106883016284e-05 1.38649426162374e-07
2.35214531591338e-05 1.3526361541949e-07
2.35318342319685e-05 1.31003215386727e-07
2.35417478444688e-05 1.25952539065111e-07
2.35511194159321e-05 1.20199864284132e-07
2.35598834605749e-05 1.13835668003048e-07
2.35679835873942e-05 1.06952406042637e-07
2.35753688624801e-05 9.96431097632922e-08
2.35820065417197e-05 9.20003806470504e-08
2.35878656997812e-05 8.41155483044531e-08
2.35929263258383e-05 7.60780167752273e-08
2.35971793228623e-05 6.79742129250371e-08
2.36006356024443e-05 5.98858989064865e-08
2.36032842488992e-05 5.18915221903171e-08
2.3605137993335e-05 4.40652634381422e-08
2.36062204806708e-05 3.64758534487919e-08
2.36065517184303e-05 2.91865021040394e-08
2.36061753606659e-05 2.22544507266775e-08
2.36051223292261e-05 1.57305315440226e-08
2.36034399164475e-05 9.65887636539264e-09
2.36011754150833e-05 4.07712974492824e-09
2.35983742993134e-05 -9.83757075800895e-10
2.35951020519237e-05 -5.49925616155633e-09
2.35914150611832e-05 -9.45289357900947e-09
2.35873624394312e-05 -1.2833446305649e-08
2.35829969373463e-05 -1.56354218461274e-08
2.35783785814125e-05 -1.78592252098042e-08
2.35735692173944e-05 -1.95112548340148e-08
2.35686179582278e-05 -2.06028900606725e-08
2.35635848311044e-05 -2.11504520564176e-08
2.35585280441708e-05 -2.11751931544768e-08
2.35534894346412e-05 -2.07024122289567e-08
2.35485235730026e-05 -1.97608933660831e-08
2.35436722966637e-05 -1.83824653277043e-08
2.35389829002369e-05 -1.6602104579988e-08
2.35344881264893e-05 -1.44569796134419e-08
2.35302261751974e-05 -1.19858647451565e-08
2.35262243319934e-05 -9.22887366527902e-09
2.3522511701915e-05 -6.22692297724825e-09
2.35191101136956e-05 -3.0213520574307e-09
2.35160341203605e-05 3.46410899965122e-10
2.35132891799605e-05 3.83660747615977e-09
2.351090439702e-05 7.40892147632621e-09
2.3508867039862e-05 1.10246460849339e-08
2.35071934803349e-05 1.4646637680471e-08
2.35058837190494e-05 1.82388859570892e-08
2.35049377571017e-05 2.17671178859291e-08
2.35043392243228e-05 2.51994514144371e-08
2.35040772074424e-05 2.8506811133866e-08
2.35041407933012e-05 3.16627897234412e-08
2.35045136115081e-05 3.46435093945274e-08
2.35051756539012e-05 3.74282045356722e-08
2.35061050928298e-05 3.9998973022648e-08
2.35072801008512e-05 4.23410746464015e-08
2.350868066954e-05 4.44424479439931e-08
2.35102722381114e-05 4.62943248180636e-08
2.35120420739171e-05 4.78907757894831e-08
2.35139610733209e-05 4.92280811670298e-08
2.35160001324092e-05 5.0305629883951e-08
2.3518133785233e-05 5.11255251467446e-08
2.35203365659825e-05 5.16922433746458e-08
2.35225830086255e-05 5.20126235414864e-08
2.35248531040566e-05 5.20955083516128e-08
2.35271177480706e-05 5.19510940932832e-08
2.35293569317424e-05 5.15924085675579e-08
2.35315488266996e-05 5.10333286740661e-08
2.35336752426318e-05 5.02891772669045e-08
2.35357216272492e-05 4.93761191933118e-08
2.35376661523734e-05 4.83112998495017e-08
2.35394979035131e-05 4.71127385992531e-08
2.35412023283782e-05 4.5798653758311e-08
2.35427703316193e-05 4.43877468114806e-08
2.354419099862e-05 4.28985487133104e-08
2.35454625100578e-05 4.13496685780501e-08
2.35465739516771e-05 3.97590724787733e-08
2.35475253228395e-05 3.81444991148783e-08
2.35483148042087e-05 3.6522916246895e-08
2.35489423954516e-05 3.4910719648451e-08
2.35494099150441e-05 3.33231966465064e-08
2.35497191816841e-05 3.17748423128705e-08
2.35498774710102e-05 3.02789651129842e-08
2.35498884206126e-05 2.88476442733554e-08
2.35497574873206e-05 2.74919429443798e-08
2.35494974036993e-05 2.62215813506828e-08
2.35491136265087e-05 2.50446738903065e-08
2.35486170694355e-05 2.3968411255737e-08
2.35480168275098e-05 2.29985417377065e-08
2.35473256333801e-05 2.21392753019245e-08
2.35465544009134e-05 2.13939266302532e-08
2.35457140440321e-05 2.07640269422882e-08
2.35448154765894e-05 2.02502938861926e-08
2.35438714314834e-05 1.98522265293377e-08
2.3542894641973e-05 1.95680271986021e-08
2.35418942026167e-05 1.93949887261624e-08
2.35408773897605e-05 1.93292848393867e-08
2.35398587553615e-05 1.93668014958348e-08
2.35388546704907e-05 1.95021065962919e-08
2.35378669540959e-05 1.97287199910079e-08
2.35369065204466e-05 2.00401188976684e-08
2.35359806457919e-05 2.04290664385098e-08
2.35350984249261e-05 2.08879527008321e-08
2.35342634963692e-05 2.14089013184093e-08
2.35334849548324e-05 2.19838049986265e-08
2.35327664390023e-05 2.26043219697658e-08
2.35321115867881e-05 2.32621886198103e-08
2.35315240365019e-05 2.3948988570055e-08
2.35310074260808e-05 2.4656579000748e-08
2.35305635749722e-05 2.53770089386762e-08
2.35301924831205e-05 2.61022954362033e-08
2.35298941511086e-05 2.68252300372751e-08
2.35296649407496e-05 2.75388458703674e-08
2.35295084903553e-05 2.82366769965847e-08
2.35294193430546e-05 2.89126624863911e-08
2.35293974989864e-05 2.95611108924732e-08
2.35294375013906e-05 3.01770839428173e-08
2.35295375312916e-05 3.07562544321627e-08
2.35296957699777e-05 3.12944514746505e-08
2.35299049412552e-05 3.17883710465594e-08
2.35301595884752e-05 3.22354267723313e-08
2.35304578926621e-05 3.26335438671777e-08
2.35307943967644e-05 3.29809068944087e-08
2.35311654630671e-05 3.32766560973141e-08
2.35315601775504e-05 3.3520336728543e-08
2.35319767210168e-05 3.37122223470487e-08
2.35324114557789e-05 3.38529062560156e-08
2.35328571055737e-05 3.39436851959363e-08
2.35333118516062e-05 3.39855965592051e-08
2.35337665987767e-05 3.39808288174481e-08
2.35342213471684e-05 3.39315846531463e-08
2.35346651825674e-05 3.38403687294431e-08
2.35350999240741e-05 3.37105596770471e-08
2.35355182954949e-05 3.35452590149998e-08
2.3535918477785e-05 3.3347756556168e-08
2.35362968330211e-05 3.3121452247542e-08
2.35366515420748e-05 3.28701119656216e-08
2.35369807857766e-05 3.25973665837864e-08
2.35372809260365e-05 3.23070175056728e-08
2.35375501439206e-05 3.20027808697887e-08
2.35377902582934e-05 3.16883621565012e-08
2.35379994499157e-05 3.13671826290829e-08
2.35381740809476e-05 3.10428056593537e-08
2.35383159700314e-05 3.07186240888768e-08
2.35384269363786e-05 3.03977749638307e-08
2.35385069796701e-05 3.00832319055644e-08
2.35385542810829e-05 2.97777411617517e-08
2.35385724782489e-05 2.94838393699592e-08
2.35385615712791e-05 2.92039068483518e-08
2.35385233791074e-05 2.89400077235769e-08
2.35384597206678e-05 2.86940249338841e-08
2.35383724148386e-05 2.84674541717322e-08
2.35382614616614e-05 2.82617307334476e-08
2.35381323181044e-05 2.80777960881551e-08
2.35379868031571e-05 2.79163963057272e-08
2.35378230975386e-05 2.77779861335148e-08
2.35376484775812e-05 2.76627680761976e-08
2.3537466581125e-05 2.75709837183058e-08
2.35372701320319e-05 2.75019793605225e-08
2.35370700443771e-05 2.74559859292367e-08
2.35368699563476e-05 2.74319091886355e-08
2.35366698677492e-05 2.74286442447647e-08
2.35364697785401e-05 2.74451856796532e-08
2.35362696888453e-05 2.74805955768898e-08
2.35360695988868e-05 2.75339111510675e-08
2.35358822412435e-05 2.76039529012451e-08
2.35357003404435e-05 2.76885181449416e-08
2.35355275340632e-05 2.77866156750406e-08
2.35353638223801e-05 2.78962488664547e-08
2.35352146623347e-05 2.80159220267251e-08
2.35350764159759e-05 2.81440826199741e-08
2.35349490835118e-05 2.8278837049811e-08
2.35348399406921e-05 2.84186043586487e-08
2.3534743530701e-05 2.85618746431737e-08
2.35346616725973e-05 2.87069497062475e-08
2.35345925474473e-05 2.88523231972704e-08
2.35345379742263e-05 2.89965633726297e-08
2.35345015908717e-05 2.91382100670035e-08
2.35344779405677e-05 2.92761406228692e-08
2.35344652043668e-05 2.94091009322983e-08
2.35344652011471e-05 2.95360642610376e-08
2.35344815690958e-05 2.96560997981032e-08
2.35345070321441e-05 2.97682838379387e-08
2.35345434092676e-05 2.98718632052442e-08
2.35345907006745e-05 2.99665181557884e-08
2.35346452682195e-05 3.0051303667733e-08
2.35347089309196e-05 3.0126461325608e-08
2.35347816888304e-05 3.01909324207372e-08
2.35348544470743e-05 3.02450366973517e-08
2.35349344814284e-05 3.02893674586358e-08
2.3535025430052e-05 3.0322922839332e-08
2.35351163788561e-05 3.03459479766843e-08
2.35352073279654e-05 3.03588656436204e-08
2.35352982773385e-05 3.03622655906111e-08
2.35353892268503e-05 3.03565101944514e-08
2.35354801765841e-05 3.03421323621933e-08
2.35355711266094e-05 3.03195371031961e-08
2.35356620767596e-05 3.02890654779731e-08
2.35357421131954e-05 3.02514671091103e-08
2.35358148738263e-05 3.02083194014813e-08
2.35358876345404e-05 3.01600877605779e-08
2.35359603954349e-05 3.01071452213364e-08
2.35360204234314e-05 3.00501667993558e-08
2.35360749945568e-05 2.99904634459836e-08
2.35361295657655e-05 2.99282376658994e-08
2.35361714040483e-05 2.98641538165612e-08
2.35362077854739e-05 2.97995725873079e-08
2.35362441668441e-05 2.97345366107038e-08
2.35362641773512e-05 2.96697422186298e-08
2.35362823687857e-05 2.96064008864505e-08
2.35362987412585e-05 2.95443243203408e-08
2.35362987427989e-05 2.94845108328445e-08
2.35362987442284e-05 2.94276887302658e-08
2.3536298745519e-05 2.93736626133523e-08
2.35362823758772e-05 2.93229760472968e-08
2.353626418726e-05 2.92764781306687e-08
2.35362459983512e-05 2.9234001885925e-08
2.35362278094842e-05 2.9195465600651e-08
2.35361968875525e-05 2.91609545399751e-08
2.35361605084167e-05 2.91315664924241e-08
2.35361241293502e-05 2.91072090874422e-08
2.35360877499924e-05 2.90875981079353e-08
2.35360513706068e-05 2.9072580787215e-08
2.35360149911101e-05 2.90618480391913e-08
2.35359786115857e-05 2.9055215122753e-08
2.35359422317838e-05 2.90524866386477e-08
2.35359058519957e-05 2.90534707403367e-08
2.35358694721521e-05 2.90579329487173e-08
2.35358330921837e-05 2.90658022095158e-08
2.35357967121042e-05 2.90768298327748e-08
2.35357603320524e-05 2.90909518696481e-08
2.35357239517925e-05 2.91078876557549e-08
2.3535687571602e-05 2.91275625841081e-08
2.35356511912588e-05 2.91499198112888e-08
2.35356148108601e-05 2.91747532799036e-08
2.35355893443701e-05 2.92016650860205e-08
2.35355711537683e-05 2.9229244802309e-08
2.3535552963222e-05 2.92571442628287e-08
2.35355347726479e-05 2.92854984706992e-08
2.35355165819906e-05 2.9314247029788e-08
2.35354983914027e-05 2.93433934928089e-08
2.35354838387519e-05 2.93728774636293e-08
2.3535483838058e-05 2.94015727320129e-08
2.35354838373503e-05 2.94289357327671e-08
2.35354838367674e-05 2.9454962913178e-08
2.35354838361707e-05 2.94795938771131e-08
2.35354838355184e-05 2.95030702091026e-08
2.35354838350049e-05 2.9525342171155e-08
2.35354838344498e-05 2.95465305555354e-08
2.35355002048687e-05 2.95660065319225e-08
2.35355183943464e-05 2.95827220497813e-08
2.35355365838102e-05 2.95968654029366e-08
2.35355547734267e-05 2.96085111983757e-08
2.35355729630571e-05 2.96178122027868e-08
2.35355911528262e-05 2.96249034192897e-08
2.35356093425676e-05 2.96298203750212e-08
2.35356275323922e-05 2.96327691273746e-08
2.35356457222724e-05 2.96337461236362e-08
2.35356639121803e-05 2.96328899196396e-08
2.35356821020882e-05 2.96303106495088e-08
2.3535700292121e-05 2.96260793675174e-08
2.35357184820983e-05 2.96202493643705e-08
2.35357366720756e-05 2.96129343269058e-08
2.35357548623027e-05 2.9604194651256e-08
2.35357730523356e-05 2.95940054684252e-08
2.35357912425488e-05 2.95825657303794e-08
2.35358094327759e-05 2.95698789898324e-08
2.35358276230169e-05 2.95560234064851e-08
2.35358385372864e-05 2.95412156958719e-08
2.35358385376472e-05 2.95268556271822e-08
2.35358385379664e-05 2.95131563632367e-08
2.35358385384382e-05 2.95000752714714e-08
2.35358385386047e-05 2.94876763007323e-08
2.35358385389101e-05 2.94758883967461e-08
2.35358385392292e-05 2.94646831378031e-08
2.35358385394374e-05 2.94540178913394e-08
2.35358385397427e-05 2.94439104209232e-08
2.35358385400064e-05 2.9434389148264e-08
2.35358385402284e-05 2.94252480159685e-08
2.35358385403672e-05 2.94165865000195e-08
2.3535838540617e-05 2.94083264407163e-08
2.35358385408113e-05 2.94004820489135e-08
2.35358385409917e-05 2.93929538486282e-08
2.35358385412276e-05 2.93858519739842e-08
2.35358385413248e-05 2.93790698435714e-08
2.35358385414913e-05 2.93725896938213e-08
2.35358385416717e-05 2.93664470518706e-08
2.35358203518748e-05 2.93614554891519e-08
2.35358021621057e-05 2.93584321298113e-08
2.35357839722949e-05 2.93573982901307e-08
2.35357657822344e-05 2.93581337018622e-08
2.35357475923959e-05 2.93606632340015e-08
2.35357294024463e-05 2.93648589888562e-08
2.35357239453254e-05 2.93702058229428e-08
2.35357239452144e-05 2.93754425229054e-08
2.35357239450062e-05 2.93803950057736e-08
2.3535723944923e-05 2.93850845878296e-08
2.35357239447703e-05 2.93895432434965e-08
2.35357239446593e-05 2.93938207107658e-08
2.35357239447148e-05 2.93979347532058e-08
2.35357239445344e-05 2.94018462909662e-08
2.35357239444234e-05 2.94056334837478e-08
2.35357239442985e-05 2.94092075137087e-08
2.35357239442707e-05 2.94125968025583e-08
2.35357239442152e-05 2.94157977975829e-08
2.35357239441458e-05 2.94188318150646e-08
2.3535723944007e-05 2.94217130658581e-08
2.35357239439793e-05 2.94245197096643e-08
2.35357239438683e-05 2.94271487177866e-08
2.35357239438405e-05 2.94296178537934e-08
2.35357239437572e-05 2.94319981719582e-08
2.35357239436879e-05 2.9434300330422e-08
2.35357239436185e-05 2.94364639330524e-08
2.3535723943563e-05 2.94384996379904e-08
2.35357239434936e-05 2.94404358669453e-08
2.35357239435907e-05 2.94423330160498e-08
2.35357239434242e-05 2.94441484527397e-08
2.35357239434519e-05 2.94458430971645e-08
2.35357239433687e-05 2.94474098438968e-08
2.35357239433687e-05 2.94489304053513e-08
2.35357239432854e-05 2.94503728071049e-08
2.35357239432576e-05 2.94517334964439e-08
2.35357239432438e-05 2.94530728695008e-08
2.35357239432021e-05 2.94543376355705e-08
2.35357239431605e-05 2.94555171365118e-08
2.35357239431605e-05 2.94565296599103e-08
2.3535723943105e-05 2.94574569181805e-08
2.35357239431605e-05 2.94583522020275e-08
2.3535723943105e-05 2.94592297223062e-08
2.35357239431189e-05 2.94600646100207e-08
2.35357239430911e-05 2.94608497597437e-08
2.35357239430495e-05 2.94616029350436e-08
2.3535723943105e-05 2.94623241359204e-08
2.35357239430356e-05 2.94629458608142e-08
2.35357239429662e-05 2.9463478767866e-08
2.35357239430217e-05 2.94640614129094e-08
2.35357239428968e-05 2.94646476106664e-08
2.35357239429107e-05 2.94651769650045e-08
2.35357239429801e-05 2.94656850030606e-08
2.35357239428829e-05 2.94661823829756e-08
2.35357239429385e-05 2.94666797628906e-08
2.35357239429246e-05 2.94671345102415e-08
2.35357239428136e-05 2.94675146506052e-08
2.35357239428691e-05 2.94679232126782e-08
2.35357239428552e-05 2.94683175638966e-08
2.35357239428829e-05 2.94686870461192e-08
2.35357239428968e-05 2.94690174484913e-08
2.35357239428691e-05 2.94693620617181e-08
2.35357239428552e-05 2.94697386493681e-08
2.35357239428136e-05 2.94700477354581e-08
2.35357239427997e-05 2.9470292872702e-08
2.35357239428136e-05 2.94705841952236e-08
2.3535723942758e-05 2.94709003867411e-08
2.35357239427303e-05 2.94711739456943e-08
2.35357239427997e-05 2.94713977666561e-08
2.35357239427442e-05 2.94716357984726e-08
2.35357239428274e-05 2.94718418558659e-08
2.3535723942758e-05 2.94720123861225e-08
2.35357239427858e-05 2.94721544946697e-08
2.35357239426887e-05 2.94723037086442e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
};
\addplot [very thick, learnedWithSideInfo, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131130967030441 0.0250559077740711
0.126954415385522 -0.0387854337854492
0.0959909596281738 -0.0809449603276278
0.0503812628900897 -0.0970377168106555
0.00316271916885161 -0.0880875118528515
-0.03469939238653 -0.0611773146571117
-0.0566952679898909 -0.0263151914150761
-0.0612749820527788 0.00705238800848562
-0.0511259784534823 0.0316363000069835
-0.031761942199843 0.0436166573162033
-0.00960457562654017 0.0431233245649061
0.00978384610990571 0.0332069362135208
0.0227619949645598 0.018247375890077
0.0279291373310218 0.00264443654341662
0.0258931662785029 -0.0100859387020868
0.0186829594563317 -0.0178290667225589
0.00900004124768462 -0.0200002836084217
-0.000507501539022737 -0.0173410445085445
-0.00780568723499855 -0.0114801980385337
-0.0117845089621703 -0.00439395423118327
-0.0123017709765788 0.00209769180047914
-0.0100058964273524 0.00669874361943812
-0.00602103852842832 0.00881470582310939
-0.00159371240002289 0.00853252010690397
0.0022096438162143 0.00644787699847171
0.00469648019858945 0.00341739667362972
0.00561553523699802 0.000311801030164816
0.00511283794299555 -0.00217608016681581
0.00361163997995589 -0.00364112931397997
0.00165921591695453 -0.00398968264241617
-0.000219348990524268 -0.00339138730056732
-0.00163053744599401 -0.00218488068954414
-0.00236933021152091 -0.000767265131614181
-0.00242263262988182 0.000505340418690992
-0.00192999576988896 0.00138681205049451
-0.00111949188836696 0.00177084454872656
-0.000238289741352843 0.00168342198344362
0.000505613310437858 0.00124782931955281
0.000980163413757951 0.000636090728832528
0.00114126652138702 2.05941029776113e-05
0.00102294912556597 -0.000463568540769899
0.000712676699304401 -0.0007397737889967
0.000320487878612399 -0.000793639229122789
-4.99739285566847e-05 -0.000662438977578006
-0.000322658817703977 -0.000415604370697764
-0.000459622137862825 -0.000132503557978225
-0.000460910036814061 0.000117069605966691
-0.000356174982670474 0.000286030351745126
-0.00019167169792797 0.000355282438565752
-1.64946906665991e-05 0.00033171404267307
0.000128767023046414 0.000240956124734737
0.000219012163638607 0.000117645652895959
0.000246686088867659 -4.1232572485228e-06
0.000219555602824884 -9.81183396007168e-05
0.000155633526672944 -0.000149956340877111
7.69868677398533e-05 -0.000157625985934828
4.02745883358591e-06 -0.000129197403261117
-4.8576854990004e-05 -7.88384142360599e-05
-7.38364481969039e-05 -2.23775545400429e-05
-7.22716716766852e-05 2.65163702692917e-05
-5.01424402306466e-05 5.88416259326152e-05
-1.68158260134277e-05 7.11988797164054e-05
1.79641115486823e-05 6.52971436814198e-05
4.628616298058e-05 4.64533492881003e-05
6.33941601827226e-05 2.16356863269596e-05
6.80287568248089e-05 -2.42148050944024e-06
6.19306161658284e-05 -2.06357857130968e-05
4.87986713438582e-05 -3.03213664523128e-05
3.30507518032791e-05 -3.12461686249321e-05
1.87008659687515e-05 -2.5141328496403e-05
8.57229574748042e-06 -1.489012681688e-05
3.94414096889506e-06 -3.64463294033612e-06
4.61286486518053e-06 5.921519072416e-06
9.26382871094256e-06 1.2091093836375e-05
1.60033472853677e-05 1.42670424274627e-05
2.28997475971854e-05 1.28556340399655e-05
2.84133222543115e-05 8.95642772391625e-06
3.16459053790324e-05 3.96930508728133e-06
3.23952760010182e-05 -7.77305540822226e-07
3.10457836701777e-05 -4.30056036293536e-06
2.83550391400184e-05 -6.10146083346308e-06
2.52062045879436e-05 -6.16699580646696e-06
2.23875623630992e-05 -4.86574935010253e-06
2.04414038800782e-05 -2.78327159719538e-06
1.95999513716572e-05 -5.46414614888135e-07
1.98031112140229e-05 1.32258379181849e-06
2.07760678834629e-05 2.49699061072306e-06
2.21366326692979e-05 2.87375436158754e-06
2.35023572939669e-05 2.54663393661758e-06
2.45740270698597e-05 1.74233062821827e-06
2.518264915502e-05 7.41663352954447e-07
2.52975543341277e-05 -1.93654344116112e-07
2.50026077899118e-05 -8.73913528209869e-07
2.44526031316361e-05 -1.20692937599642e-06
2.38238513607103e-05 -1.19664002085074e-06
2.32709520618657e-05 -9.2103739035565e-07
2.2897834276267e-05 -4.98807654736311e-07
2.27462541681767e-05 -5.44513767408716e-08
2.28004163646267e-05 3.10173863482532e-07
2.300311704731e-05 5.33080111608797e-07
2.32773261308883e-05 5.96887488768516e-07
2.35474277410913e-05 5.22780609912843e-07
2.37553877111413e-05 3.57357127001023e-07
2.38695324125682e-05 1.56866690304014e-07
2.38856423269151e-05 -2.71965063802782e-08
2.38218263905882e-05 -1.58286802331986e-07
2.37096527243158e-05 -2.19482629404411e-07
2.35842696915678e-05 -2.1284491324991e-07
2.34759602199125e-05 -1.54788438067044e-07
2.34046100890672e-05 -6.93348809477357e-08
2.3377610464892e-05 1.88197617490005e-08
2.33910801209353e-05 8.98418583972216e-08
2.34331577266128e-05 1.32013571629841e-07
2.3488374675848e-05 1.42482857512505e-07
2.35417478444688e-05 1.25952539065111e-07
2.35820065417197e-05 9.20003806470504e-08
2.36032842488992e-05 5.18915221903171e-08
2.36051223292261e-05 1.57305315440226e-08
2.35914150611832e-05 -9.45289357900947e-09
2.35686179582278e-05 -2.06028900606725e-08
2.35436722966637e-05 -1.83824653277043e-08
2.3522511701915e-05 -6.22692297724825e-09
2.3508867039862e-05 1.10246460849339e-08
2.35040772074424e-05 2.8506811133866e-08
2.35072801008512e-05 4.23410746464015e-08
2.35160001324092e-05 5.0305629883951e-08
2.35271177480706e-05 5.19510940932832e-08
2.35376661523734e-05 4.83112998495017e-08
2.35454625100578e-05 4.13496685780501e-08
2.35494099150441e-05 3.33231966465064e-08
2.35494974036993e-05 2.62215813506828e-08
2.35465544009134e-05 2.13939266302532e-08
2.35418942026167e-05 1.93949887261624e-08
2.35369065204466e-05 2.00401188976684e-08
2.35327664390023e-05 2.26043219697658e-08
2.35301924831205e-05 2.61022954362033e-08
2.35293974989864e-05 2.95611108924732e-08
2.35301595884752e-05 3.22354267723313e-08
2.35319767210168e-05 3.37122223470487e-08
2.35342213471684e-05 3.39315846531463e-08
2.35362968330211e-05 3.3121452247542e-08
2.35377902582934e-05 3.16883621565012e-08
2.35385069796701e-05 3.00832319055644e-08
2.35384597206678e-05 2.86940249338841e-08
2.35378230975386e-05 2.77779861335148e-08
2.35368699563476e-05 2.74319091886355e-08
2.35358822412435e-05 2.76039529012451e-08
2.35350764159759e-05 2.81440826199741e-08
2.35345925474473e-05 2.88523231972704e-08
2.35344652011471e-05 2.95360642610376e-08
2.35346452682195e-05 3.0051303667733e-08
2.3535025430052e-05 3.0322922839332e-08
2.35354801765841e-05 3.03421323621933e-08
2.35358876345404e-05 3.01600877605779e-08
2.35361714040483e-05 2.98641538165612e-08
2.35362987412585e-05 2.95443243203408e-08
2.353626418726e-05 2.92764781306687e-08
2.35361241293502e-05 2.91072090874422e-08
2.35359422317838e-05 2.90524866386477e-08
2.35357603320524e-05 2.90909518696481e-08
2.35355893443701e-05 2.92016650860205e-08
2.35354983914027e-05 2.93433934928089e-08
2.35354838361707e-05 2.94795938771131e-08
2.35355183943464e-05 2.95827220497813e-08
2.35356093425676e-05 2.96298203750212e-08
2.3535700292121e-05 2.96260793675174e-08
2.35357912425488e-05 2.95825657303794e-08
2.35358385379664e-05 2.95131563632367e-08
2.35358385394374e-05 2.94540178913394e-08
2.3535838540617e-05 2.94083264407163e-08
2.35358385414913e-05 2.93725896938213e-08
2.35357657822344e-05 2.93581337018622e-08
2.35357239450062e-05 2.93803950057736e-08
2.35357239445344e-05 2.94018462909662e-08
2.35357239441458e-05 2.94188318150646e-08
2.35357239437572e-05 2.94319981719582e-08
2.35357239435907e-05 2.94423330160498e-08
2.35357239432854e-05 2.94503728071049e-08
2.35357239431605e-05 2.94565296599103e-08
2.35357239430911e-05 2.94608497597437e-08
2.35357239430217e-05 2.94640614129094e-08
2.35357239429385e-05 2.94666797628906e-08
2.35357239428829e-05 2.94686870461192e-08
2.35357239427997e-05 2.9470292872702e-08
2.35357239427442e-05 2.94716357984726e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
2.35357239427997e-05 2.94724351590503e-08
};
\addplot [very thick, learnedWithoutSideInfo]
table {%
0.1 0.1
0.109055686735228 0.0848023914893261
0.116599563650122 0.0696141300385094
0.122731375359578 0.0545466065857809
0.127518374657465 0.0396477853905637
0.130945815911047 0.0249882859606529
0.132898516382125 0.01076790857406
0.133194773514832 -0.00260286764611806
0.131691167303387 -0.0145258706125055
0.128426229610915 -0.0244043073155922
0.123694753124036 -0.0319125519429093
0.117970589006918 -0.0371277075459879
0.111742546955164 -0.0404272647099617
0.105393762062948 -0.0422863412095822
0.0991714484568287 -0.0431316577595382
0.0932119632451851 -0.0432888186678042
0.0875784014548038 -0.0429862567433617
0.0822909370615399 -0.0423779618858653
0.0773466038806552 -0.041566275191613
0.0727309400824279 -0.040619258577884
0.068424474675405 -0.0395825921806789
0.0644062106529426 -0.0384873618218577
0.0606554267397073 -0.0373550741893318
0.0571525546291456 -0.0362008837009746
0.053879552854436 -0.0350356838137316
0.0508200096140734 -0.0338674776437493
0.0479591028781379 -0.0327022875176404
0.0452834890352349 -0.0315447657604366
0.0427811598415928 -0.0303986089242798
0.0404412898657394 -0.0292668406066738
0.0382540866988017 -0.0281520050207966
0.0362106505231422 -0.0270562990811172
0.034302846348043 -0.0259816616220085
0.0325231902987533 -0.0249298324754648
0.0308647502139083 -0.0239023902770228
0.0293210601370346 -0.0229007752971384
0.0278860478933738 -0.0219263018464133
0.0265539747172443 -0.0209801635907674
0.0253193857750538 -0.0200634342474757
0.0241770703745412 -0.0191770655067245
0.0231220306474205 -0.0183218835495396
0.0221494575220009 -0.0174985851761633
0.0212547128550589 -0.0167077342760358
0.0204333166674666 -0.0159497591509918
0.0196809385140486 -0.0152249510235833
0.018993392115733 -0.0145334639269592
0.0183666324810836 -0.0138753160569145
0.0177967548487887 -0.0132503925852028
0.0172799948810902 -0.0126584498688693
0.0168127296337743 -0.0120991209397054
0.0163914789170931 -0.0115719221303294
0.0160129067404471 -0.0110762606746739
0.01567382260659 -0.0106114431053257
0.0153711824797944 -0.0101766842756952
0.0151020893066103 -0.00977111683425846
0.0148637930093798 -0.00939380098890297
0.0146536899088441 -0.00904373440975448
0.0144693215593685 -0.0087198621330522
0.0143083730016145 -0.00842108634175887
0.0141686704551061 -0.00814627591503836
0.0140481784838975 -0.00789427565154099
0.0139449966762744 -0.0076639150865212
0.0138573558874107 -0.0074540168355135
0.0137836140938705 -0.00726340441061879
0.0137222519131717 -0.00709090946684654
0.0136718678398011 -0.00693537844718861
0.0136311732496239 -0.00679567860429486
0.0135989872231068 -0.00667070338697684
0.0135742312341971 -0.00655937718817157
0.0135559237516407 -0.00646065945771923
0.0135431747951824 -0.00637354819124525
0.0135351804868031 -0.00629708281243779
0.0135312176340925 -0.00623034647141552
0.0135306383796698 -0.00617246778582015
0.0135328649471149 -0.00612262205847003
0.0135373845112894 -0.00608003200339624
0.0135437442167488 -0.00604396802013341
0.0135515463649112 -0.00601374805465582
0.0135604437886627 -0.00598873708809933
0.0135701354273021 -0.00596834629328669
0.0135803621150286 -0.0059520319023143
0.0135909025902756 -0.00593929382418779
0.0136015697321392 -0.00592967405300371
0.0136122070272411 -0.0059227549037324
0.0136226852678725 -0.00591815711263521
0.0136328994803485 -0.00591553783608134
0.0136427660797633 -0.00591458857818949
0.0136522202471641 -0.00591503307767027
0.0136612135223173 -0.00591662517771141
0.0136697116044062 -0.00591914670436111
0.0136776923521016 -0.00592240537164912
0.01368514397402 -0.0059262327321683
0.0136920633990119 -0.00593048218772552
0.0136984548158003 -0.00593502707229732
0.0137043283721134 -0.00593975881641384
0.0137096990209644 -0.0059445852022435
0.0137145855049181 -0.00594942871311233
0.0137190094666222 -0.00595422498204456
0.0137229946751964 -0.00595892134266052
0.01372656635878 -0.00596347547978127
0.0137297506338177 -0.00596785418274237
0.0137325740204086 -0.00597203219691878
0.0137350630369928 -0.00597599117285341
0.0137372438639496 -0.00597971870796954
0.0137391420698976 -0.00598320747857883
0.0137407823930924 -0.00598645445624868
0.0137421885708311 -0.00598946020496527
0.0137433832107909 -0.00599222825398016
0.0137443876993655 -0.00599476454076608
0.0137452221411585 -0.00599707691964824
0.0137459053251061 -0.00599917473090983
0.0137464547133133 -0.0060010684252596
0.0137468864485495 -0.00600276923931276
0.0137472153774465 -0.00600428891686988
0.0137474550858843 -0.00600563947189059
0.0137476179443485 -0.00600683298929283
0.01374771516113 -0.00600788145913711
0.0137477568406528 -0.00600879664040121
0.0137477520462581 -0.00600958995164902
0.013747708864926 -0.00601027238516139
0.0137476344732999 -0.00601085444065319
0.0137475352042449 -0.00601134607685339
0.0137474166119405 -0.00601175667927478
0.0137472835362997 -0.00601209503954081
0.0137471401647149 -0.00601236934653215
0.013746990091869 -0.00601258718676689
0.0137468363765114 -0.0060127555521845
0.0137466815953058 -0.00601288085402274
0.0137465278931934 -0.00601296894216929
0.0137463770311692 -0.00601302512748347
0.0137462304300771 -0.00601305420808274
0.0137460892113015 -0.0060130604967128
0.0137459542343503 -0.0060130478500362
0.0137458261313044 -0.00601301969843604
0.0137457053378376 -0.00601297907658349
0.0137455921218994 -0.00601292865277969
0.0137454866090156 -0.00601287075865642
0.013745388805654 -0.00601280741794596
0.0137452986192801 -0.0060127403737269
0.0137452158769267 -0.0060126711150339
0.0137451403412461 -0.00601260090167344
0.0137450717245713 -0.00601253078813713
0.0137450097011613 -0.00601246164536207
0.0137449539180821 -0.00601239418150357
0.0137449040042474 -0.00601232896142534
0.0137448595783436 -0.00601226642386266
0.0137448202554336 -0.00601220689781456
0.0137447856523301 -0.00601215061724858
0.0137447553922403 -0.00601209773460809
0.013744729108482 -0.00601204833298752
0.0137447064473195 -0.00601200243707822
0.0137446870701374 -0.00601196002279636
0.0137446706553017 -0.00601192102637427
0.0137446568991266 -0.00601188535117103
0.0137446455167685 -0.00601185287577621
0.0137446362423939 -0.00601182345906892
0.0137446288294905 -0.00601179694534082
0.0137446230504001 -0.00601177316911361
0.0137446186962218 -0.00601175195897952
0.0137446155759553 -0.00601173314026582
0.0137446135160877 -0.00601171653851651
0.0137446123596305 -0.00601170198098799
0.0137446119651741 -0.00601168929916085
0.0137446122060176 -0.00601167832972394
0.0137446129694754 -0.00601166891591021
0.0137446141556632 -0.00601166090839556
0.0137446156764431 -0.00601165416557592
0.013744617454845 -0.00601164855466152
0.0137446194237587 -0.00601164395116172
0.01374462152545 -0.0060116402392687
0.013744623710229 -0.00601163731219145
0.0137446259361114 -0.00601163507141322
0.0137446281678786 -0.00601163342688693
0.0137446303761435 -0.00601163229634594
0.0137446325370512 -0.00601163160539642
0.0137446346313823 -0.00601163128677129
0.0137446366440868 -0.00601163128033733
0.0137446385638664 -0.00601163153224249
0.0137446403823256 -0.00601163199468502
0.0137446420939387 -0.00601163262534854
0.0137446436954418 -0.00601163338728483
0.0137446451856629 -0.00601163424815354
0.0137446465649202 -0.00601163517997705
0.0137446478349028 -0.00601163615859335
0.0137446489983737 -0.00601163716362052
0.01374465005893 -0.00601163817786698
0.0137446510209271 -0.00601163918662095
0.0137446518893372 -0.00601164017813716
0.0137446526692042 -0.00601164114298314
0.0137446533659118 -0.00601164207342819
0.0137446539851536 -0.00601164296365653
0.0137446545322759 -0.00601164380938712
0.0137446550129241 -0.0060116446075007
0.0137446554324383 -0.00601164535618892
0.0137446557960565 -0.00601164605443572
0.0137446561087946 -0.00601164670200305
0.0137446563755783 -0.00601164729966897
0.0137446566008741 -0.00601164784831454
0.0137446567890813 -0.00601164834956336
0.0137446569441428 -0.00601164880528771
0.0137446570698172 -0.0060116492173421
0.0137446571695858 -0.0060116495882987
0.0137446572467854 -0.00601164992038861
0.0137446573041431 -0.00601165021615202
0.0137446573444895 -0.00601165047817886
0.0137446573702176 -0.00601165070896315
0.0137446573834414 -0.00601165091091005
0.013744657386332 -0.00601165108654556
0.0137446573805442 -0.00601165123811498
0.0137446573676232 -0.00601165136789916
0.0137446573489692 -0.00601165147790539
0.0137446573258415 -0.00601165157029726
0.0137446572992326 -0.00601165164674455
0.0137446572701996 -0.00601165170922968
0.0137446572394488 -0.00601165175936558
0.0137446572077282 -0.00601165179864438
0.0137446571755553 -0.00601165182830599
0.0137446571434274 -0.00601165184978925
0.0137446571117454 -0.00601165186407826
0.0137446570808117 -0.00601165187240227
0.0137446570509077 -0.00601165187556063
0.0137446570223112 -0.00601165187454455
0.0137446569950475 -0.00601165187000419
0.0137446569692279 -0.00601165186253638
0.0137446569449842 -0.00601165185280195
0.0137446569223283 -0.00601165184131247
0.0137446569012853 -0.00601165182852981
0.0137446568818389 -0.00601165181491226
0.0137446568640109 -0.00601165180073693
0.0137446568476498 -0.00601165178622765
0.0137446568327499 -0.00601165177165086
0.0137446568192647 -0.00601165175716645
0.0137446568070594 -0.00601165174303731
0.0137446567961594 -0.00601165172912133
0.0137446567864414 -0.00601165171591234
0.0137446567778012 -0.00601165170326468
0.0137446567701776 -0.00601165169126361
0.0137446567635378 -0.00601165168000506
0.0137446567577493 -0.00601165166933271
0.0137446567526884 -0.00601165165951656
0.0137446567483153 -0.00601165165042872
0.0137446567446211 -0.00601165164187023
0.0137446567415349 -0.00601165163409334
0.0137446567389634 -0.00601165162702344
0.0137446567368804 -0.00601165162064632
0.0137446567351682 -0.00601165161497619
0.0137446567337629 -0.00601165160975015
0.0137446567327484 -0.00601165160509254
0.0137446567319524 -0.00601165160093231
0.0137446567313784 -0.00601165159727657
0.013744656730988 -0.00601165159401518
0.013744656730871 -0.0060116515911659
0.013744656730905 -0.00601165158865413
0.0137446567310511 -0.00601165158659356
0.0137446567312827 -0.0060116515848172
0.0137446567316146 -0.00601165158325756
0.0137446567320143 -0.00601165158201766
0.0137446567324186 -0.0060116515809483
0.0137446567329018 -0.00601165158009564
0.0137446567333548 -0.00601165157950589
0.0137446567337949 -0.00601165157894101
0.0137446567342803 -0.00601165157851824
0.0137446567347415 -0.00601165157823047
0.013744656735168 -0.00601165157805994
0.0137446567356143 -0.00601165157797823
0.0137446567360642 -0.00601165157803152
0.0137446567365442 -0.00601165157812034
0.0137446567369275 -0.00601165157821271
0.0137446567372963 -0.00601165157834416
0.0137446567376514 -0.00601165157850048
0.01374465673794 -0.00601165157861772
0.0137446567382769 -0.00601165157880601
0.0137446567385384 -0.0060116515789268
0.013744656738738 -0.00601165157922523
0.0137446567389707 -0.00601165157944195
0.0137446567391681 -0.00601165157968353
0.0137446567394488 -0.00601165157987538
0.0137446567395849 -0.00601165158013472
0.0137446567398283 -0.00601165158032302
0.0137446567399304 -0.00601165158062145
0.0137446567400143 -0.0060116515808204
0.0137446567400428 -0.00601165158099448
0.0137446567401447 -0.0060116515812183
0.0137446567402222 -0.00601165158133909
0.0137446567402983 -0.00601165158140304
0.0137446567403103 -0.00601165158157713
0.013744656740341 -0.00601165158169437
0.0137446567403745 -0.00601165158182937
0.0137446567403738 -0.00601165158183647
0.0137446567404158 -0.00601165158201056
0.0137446567404906 -0.00601165158212424
0.0137446567404975 -0.00601165158223438
0.01374465674049 -0.00601165158235517
0.0137446567404997 -0.00601165158233741
0.0137446567404755 -0.00601165158237649
0.0137446567404564 -0.00601165158245109
0.0137446567404611 -0.00601165158241201
0.0137446567404271 -0.00601165158244754
0.0137446567404407 -0.00601165158245109
0.0137446567403974 -0.00601165158247241
0.0137446567404413 -0.00601165158243688
0.01374465674041 -0.00601165158232675
0.013744656740422 -0.00601165158232675
0.0137446567404698 -0.00601165158232675
0.0137446567404467 -0.00601165158228412
0.0137446567404349 -0.00601165158230543
0.0137446567404518 -0.00601165158227346
0.0137446567404733 -0.00601165158229833
0.0137446567404158 -0.00601165158227346
0.0137446567404917 -0.00601165158228056
0.0137446567404909 -0.00601165158227701
0.0137446567405104 -0.00601165158222017
0.0137446567405677 -0.00601165158227346
0.0137446567406254 -0.00601165158230899
0.0137446567406247 -0.00601165158232675
0.0137446567405852 -0.00601165158241912
0.0137446567405941 -0.00601165158244754
0.0137446567405888 -0.00601165158250794
0.0137446567405628 -0.00601165158248307
0.0137446567405244 -0.00601165158241201
0.0137446567405184 -0.00601165158241912
0.0137446567405195 -0.00601165158233741
0.0137446567405177 -0.00601165158230188
0.0137446567405284 -0.00601165158230543
0.0137446567405426 -0.00601165158233741
0.0137446567404966 -0.0060116515823232
0.0137446567404831 -0.00601165158238359
0.013744656740502 -0.00601165158236938
0.0137446567404618 -0.00601165158240136
0.0137446567404318 -0.00601165158246886
0.0137446567404222 -0.0060116515825257
0.0137446567404 -0.00601165158256478
0.0137446567404231 -0.00601165158253636
0.0137446567404269 -0.00601165158246886
0.0137446567404087 -0.00601165158246175
0.0137446567404451 -0.00601165158243333
0.0137446567404143 -0.00601165158235872
0.0137446567404316 -0.00601165158230188
0.0137446567404582 -0.00601165158231964
0.0137446567404378 -0.00601165158228056
0.0137446567404316 -0.00601165158226991
0.0137446567404766 -0.00601165158233385
0.0137446567404336 -0.00601165158230899
0.0137446567404105 -0.00601165158226991
0.0137446567404889 -0.00601165158228056
0.0137446567405224 -0.00601165158225569
0.0137446567405364 -0.00601165158222017
0.0137446567405752 -0.00601165158224148
0.0137446567406467 -0.00601165158230899
0.0137446567405943 -0.00601165158236583
0.0137446567405883 -0.00601165158242978
0.0137446567405675 -0.00601165158246175
0.0137446567405766 -0.00601165158246886
0.0137446567405579 -0.00601165158249017
0.0137446567405166 -0.00601165158240491
0.0137446567405037 -0.0060116515823907
0.0137446567405328 -0.00601165158231964
0.01374465674051 -0.00601165158231964
0.0137446567405117 -0.00601165158226635
0.0137446567405153 -0.00601165158232675
0.0137446567404953 -0.00601165158233741
0.0137446567405048 -0.00601165158233741
0.0137446567405035 -0.0060116515823978
0.0137446567404498 -0.00601165158240491
0.0137446567404511 -0.0060116515824653
0.0137446567404238 -0.00601165158253991
0.0137446567404247 -0.00601165158257544
0.0137446567404238 -0.00601165158250438
0.0137446567404362 -0.00601165158248307
0.0137446567404262 -0.00601165158244754
0.0137446567404138 -0.00601165158240136
0.0137446567404058 -0.00601165158231254
0.0137446567404351 -0.00601165158229122
0.0137446567404624 -0.00601165158231254
0.0137446567404436 -0.00601165158227701
0.0137446567404373 -0.00601165158226635
0.0137446567404576 -0.00601165158228767
0.0137446567404433 -0.00601165158233385
0.0137446567404469 -0.00601165158225569
0.0137446567404624 -0.00601165158229477
0.0137446567404946 -0.00601165158222727
0.0137446567405497 -0.00601165158227346
0.0137446567406028 -0.00601165158226635
0.0137446567406392 -0.00601165158230188
0.0137446567405977 -0.00601165158239425
0.0137446567405968 -0.00601165158245465
0.0137446567405908 -0.00601165158250083
0.0137446567405657 -0.00601165158250438
0.0137446567405695 -0.00601165158243333
0.0137446567405095 -0.00601165158240846
0.0137446567405175 -0.00601165158241201
0.0137446567405288 -0.00601165158231609
0.0137446567405126 -0.00601165158233385
0.0137446567405037 -0.00601165158234096
0.0137446567405173 -0.00601165158235162
0.0137446567404831 -0.00601165158232675
0.0137446567404993 -0.00601165158233385
0.01374465674048 -0.00601165158241201
0.0137446567404407 -0.00601165158240136
0.0137446567404336 -0.0060116515824582
0.0137446567404269 -0.0060116515825257
0.0137446567404131 -0.00601165158253281
0.0137446567404305 -0.00601165158250794
0.0137446567404229 -0.0060116515824653
0.0137446567404484 -0.0060116515824582
0.01374465674041 -0.00601165158234096
0.0137446567404127 -0.00601165158231609
0.0137446567404655 -0.00601165158234451
0.0137446567404551 -0.00601165158230543
0.0137446567404411 -0.00601165158228767
0.0137446567404458 -0.00601165158226991
0.013744656740478 -0.00601165158228767
0.0137446567404316 -0.00601165158230899
0.0137446567404844 -0.00601165158227346
0.0137446567404842 -0.00601165158227346
0.0137446567404966 -0.00601165158222727
0.0137446567405541 -0.00601165158229122
0.0137446567406188 -0.00601165158229122
0.0137446567406267 -0.00601165158232675
0.0137446567405923 -0.00601165158242623
0.0137446567405943 -0.00601165158246175
0.0137446567405877 -0.00601165158250438
0.0137446567405435 -0.00601165158248662
0.0137446567405357 -0.00601165158241201
0.0137446567405188 -0.00601165158242623
0.0137446567405204 -0.00601165158236583
0.0137446567405197 -0.00601165158229122
0.0137446567405271 -0.00601165158231609
0.0137446567405186 -0.00601165158234096
0.0137446567405055 -0.00601165158231964
0.0137446567404877 -0.00601165158235872
0.0137446567405108 -0.00601165158236938
0.0137446567404695 -0.00601165158241201
0.0137446567404456 -0.00601165158244754
0.0137446567404509 -0.00601165158251149
0.0137446567404076 -0.00601165158254346
0.0137446567404282 -0.0060116515825257
0.0137446567404351 -0.00601165158247596
0.0137446567404163 -0.0060116515824653
0.0137446567404416 -0.00601165158241557
0.0137446567404222 -0.00601165158237293
0.0137446567404234 -0.00601165158234096
0.0137446567404453 -0.00601165158231964
0.0137446567404511 -0.00601165158230188
0.0137446567404242 -0.00601165158228056
0.0137446567404684 -0.00601165158233385
0.0137446567404411 -0.00601165158230188
0.0137446567404169 -0.00601165158227346
0.0137446567404862 -0.00601165158226635
0.0137446567405171 -0.00601165158226635
0.0137446567405328 -0.00601165158218819
0.0137446567405644 -0.0060116515822628
0.0137446567406339 -0.00601165158229833
0.0137446567406001 -0.00601165158236583
0.0137446567405886 -0.00601165158243333
0.0137446567405646 -0.00601165158246175
0.0137446567405852 -0.00601165158247596
0.0137446567405701 -0.00601165158251504
0.0137446567405144 -0.00601165158240491
0.0137446567404951 -0.00601165158240491
0.0137446567405264 -0.00601165158234451
0.0137446567405159 -0.00601165158230188
0.0137446567405135 -0.00601165158224504
0.0137446567405275 -0.00601165158230543
0.0137446567404997 -0.0060116515823303
0.0137446567404971 -0.00601165158236583
0.0137446567404966 -0.00601165158240491
0.0137446567404582 -0.00601165158241557
0.0137446567404473 -0.00601165158247952
0.0137446567404225 -0.00601165158253636
0.0137446567404087 -0.00601165158258254
0.0137446567404158 -0.0060116515825186
0.0137446567404416 -0.00601165158247952
0.013744656740418 -0.00601165158245109
0.0137446567404225 -0.00601165158238715
0.0137446567404034 -0.0060116515823232
0.0137446567404327 -0.00601165158231609
0.0137446567404669 -0.00601165158230188
0.0137446567404509 -0.00601165158226991
0.0137446567404245 -0.00601165158228767
0.0137446567404564 -0.00601165158229833
0.0137446567404353 -0.0060116515823303
0.0137446567404342 -0.00601165158225925
0.0137446567404658 -0.00601165158229122
0.0137446567405017 -0.00601165158222372
0.0137446567405424 -0.0060116515822628
0.0137446567405866 -0.0060116515822628
0.0137446567406441 -0.00601165158229122
0.0137446567405897 -0.00601165158236938
0.0137446567405817 -0.00601165158244754
0.0137446567405848 -0.00601165158249017
0.0137446567405728 -0.00601165158251504
0.0137446567405568 -0.00601165158243333
0.0137446567405097 -0.0060116515823978
0.0137446567405257 -0.0060116515823978
0.0137446567405248 -0.0060116515823303
0.0137446567405042 -0.00601165158232675
0.0137446567405091 -0.00601165158230543
0.0137446567405206 -0.00601165158236228
0.0137446567405004 -0.00601165158234096
0.0137446567405037 -0.00601165158235872
0.0137446567404809 -0.0060116515823907
0.0137446567404504 -0.0060116515823907
0.013744656740442 -0.00601165158248662
0.0137446567404274 -0.00601165158253281
0.0137446567404265 -0.00601165158253991
0.01374465674042 -0.0060116515825186
0.0137446567404211 -0.00601165158245465
0.0137446567404365 -0.00601165158248307
0.013744656740422 -0.00601165158236938
0.013744656740412 -0.00601165158232675
0.0137446567404524 -0.00601165158230899
0.0137446567404471 -0.00601165158229833
0.0137446567404356 -0.00601165158229122
0.0137446567404313 -0.00601165158228412
0.0137446567404764 -0.00601165158227701
0.0137446567404433 -0.00601165158231609
0.0137446567404671 -0.00601165158225214
0.0137446567404695 -0.00601165158229122
0.0137446567405224 -0.0060116515822024
0.0137446567405575 -0.00601165158228767
0.0137446567406081 -0.00601165158226635
0.0137446567406234 -0.00601165158229833
0.0137446567405892 -0.00601165158240136
0.0137446567405985 -0.00601165158244754
0.0137446567405786 -0.00601165158247952
0.0137446567405437 -0.00601165158249373
0.0137446567405541 -0.00601165158242978
0.0137446567405313 -0.00601165158239425
0.0137446567405324 -0.00601165158236583
0.0137446567405302 -0.00601165158229833
0.0137446567405199 -0.00601165158233741
0.0137446567405195 -0.00601165158231609
0.0137446567405215 -0.00601165158233385
0.0137446567404835 -0.00601165158234096
0.0137446567405117 -0.00601165158235162
0.0137446567404587 -0.00601165158242978
0.0137446567404618 -0.00601165158244044
0.0137446567404556 -0.00601165158250438
0.0137446567404085 -0.00601165158253281
0.0137446567404231 -0.0060116515825186
0.0137446567404347 -0.00601165158247596
0.0137446567404025 -0.0060116515824582
0.013744656740452 -0.00601165158243333
0.0137446567404163 -0.00601165158235872
0.0137446567404178 -0.00601165158233741
0.0137446567404793 -0.00601165158231254
0.0137446567404473 -0.00601165158226991
0.0137446567404373 -0.00601165158229477
0.0137446567404678 -0.00601165158230899
0.0137446567404522 -0.00601165158231964
0.0137446567404167 -0.00601165158227701
0.0137446567405124 -0.00601165158228767
0.0137446567404906 -0.00601165158226991
0.0137446567405202 -0.00601165158220951
0.0137446567405526 -0.00601165158226635
0.0137446567406316 -0.00601165158229833
0.0137446567406172 -0.00601165158234451
0.0137446567405741 -0.00601165158242267
0.0137446567405832 -0.00601165158245109
0.0137446567405921 -0.00601165158247596
0.0137446567405581 -0.00601165158249728
0.0137446567405068 -0.00601165158240491
0.013744656740502 -0.00601165158240491
0.0137446567405299 -0.00601165158234807
0.0137446567405093 -0.00601165158229833
0.0137446567405188 -0.00601165158228056
0.0137446567405357 -0.00601165158231609
0.0137446567404977 -0.0060116515823232
0.0137446567404846 -0.00601165158236938
0.0137446567405062 -0.00601165158238715
0.0137446567404622 -0.0060116515823978
0.0137446567404469 -0.00601165158246886
0.0137446567404167 -0.00601165158252925
0.0137446567404074 -0.00601165158256478
0.0137446567404329 -0.00601165158252925
0.0137446567404369 -0.00601165158248662
0.0137446567404207 -0.00601165158244754
0.0137446567404316 -0.00601165158242267
0.0137446567404058 -0.00601165158234807
0.0137446567404398 -0.00601165158230543
0.01374465674046 -0.00601165158231609
0.013744656740442 -0.00601165158227701
0.0137446567404218 -0.00601165158225925
0.0137446567404762 -0.00601165158233385
0.0137446567404302 -0.00601165158231254
0.0137446567404163 -0.0060116515822628
0.0137446567404833 -0.00601165158230188
0.0137446567405051 -0.00601165158222372
0.0137446567405413 -0.00601165158223438
0.0137446567405772 -0.00601165158226635
0.0137446567406414 -0.00601165158229833
0.0137446567405977 -0.00601165158236228
0.0137446567405672 -0.00601165158242978
0.0137446567405681 -0.00601165158248307
0.013744656740571 -0.00601165158250794
0.0137446567405537 -0.0060116515824653
0.0137446567405171 -0.00601165158239425
0.0137446567405188 -0.0060116515823978
0.0137446567405295 -0.00601165158229833
0.0137446567405073 -0.00601165158235162
0.0137446567405091 -0.00601165158228412
0.0137446567405137 -0.00601165158233741
0.0137446567404982 -0.00601165158234096
0.0137446567404871 -0.00601165158234807
0.0137446567404891 -0.00601165158240491
0.0137446567404458 -0.00601165158239425
0.01374465674045 -0.00601165158247952
0.0137446567404205 -0.00601165158253991
0.0137446567404242 -0.00601165158255412
0.0137446567404191 -0.00601165158250794
0.0137446567404178 -0.00601165158246886
0.0137446567404349 -0.00601165158247596
0.0137446567404049 -0.00601165158238359
0.0137446567404038 -0.00601165158231609
0.0137446567404507 -0.00601165158230899
0.0137446567404691 -0.00601165158229477
0.013744656740448 -0.00601165158227701
0.013744656740436 -0.00601165158228412
0.0137446567404689 -0.00601165158228056
0.0137446567404438 -0.00601165158231964
0.013744656740458 -0.00601165158225925
0.0137446567404684 -0.00601165158228412
0.0137446567404953 -0.00601165158220596
0.0137446567405499 -0.00601165158227701
0.0137446567406037 -0.00601165158226635
0.0137446567406334 -0.00601165158228767
0.0137446567405992 -0.0060116515823978
0.0137446567406063 -0.00601165158246175
0.0137446567405939 -0.00601165158249373
0.0137446567405681 -0.00601165158251504
0.0137446567405632 -0.00601165158242623
0.0137446567405237 -0.00601165158238359
0.0137446567405124 -0.00601165158238715
0.0137446567405193 -0.00601165158231964
0.0137446567405173 -0.00601165158234096
0.0137446567405086 -0.00601165158231964
0.0137446567405124 -0.00601165158234096
0.0137446567404906 -0.00601165158235162
0.0137446567405135 -0.00601165158235162
0.0137446567404644 -0.00601165158240846
0.0137446567404664 -0.00601165158242267
0.0137446567404504 -0.00601165158249373
0.0137446567404127 -0.00601165158252215
0.0137446567404265 -0.00601165158252215
0.0137446567404509 -0.00601165158250083
0.0137446567403974 -0.00601165158247241
0.0137446567404413 -0.00601165158243688
0.01374465674041 -0.00601165158232675
0.013744656740422 -0.00601165158232675
0.0137446567404698 -0.00601165158232675
0.0137446567404467 -0.00601165158228412
0.0137446567404349 -0.00601165158230543
0.0137446567404518 -0.00601165158227346
0.0137446567404733 -0.00601165158229833
0.0137446567404158 -0.00601165158227346
0.0137446567404917 -0.00601165158228056
0.0137446567404909 -0.00601165158227701
0.0137446567405104 -0.00601165158222017
0.0137446567405677 -0.00601165158227346
0.0137446567406254 -0.00601165158230899
0.0137446567406247 -0.00601165158232675
0.0137446567405852 -0.00601165158241912
0.0137446567405941 -0.00601165158244754
0.0137446567405888 -0.00601165158250794
0.0137446567405628 -0.00601165158248307
0.0137446567405244 -0.00601165158241201
0.0137446567405184 -0.00601165158241912
0.0137446567405195 -0.00601165158233741
0.0137446567405177 -0.00601165158230188
0.0137446567405284 -0.00601165158230543
0.0137446567405426 -0.00601165158233741
0.0137446567404966 -0.0060116515823232
0.0137446567404831 -0.00601165158238359
0.013744656740502 -0.00601165158236938
0.0137446567404618 -0.00601165158240136
0.0137446567404318 -0.00601165158246886
0.0137446567404222 -0.0060116515825257
0.0137446567404 -0.00601165158256478
0.0137446567404231 -0.00601165158253636
0.0137446567404269 -0.00601165158246886
0.0137446567404087 -0.00601165158246175
0.0137446567404451 -0.00601165158243333
0.0137446567404143 -0.00601165158235872
0.0137446567404316 -0.00601165158230188
0.0137446567404582 -0.00601165158231964
0.0137446567404378 -0.00601165158228056
0.0137446567404316 -0.00601165158226991
0.0137446567404766 -0.00601165158233385
0.0137446567404336 -0.00601165158230899
0.0137446567404105 -0.00601165158226991
0.0137446567404889 -0.00601165158228056
0.0137446567405224 -0.00601165158225569
0.0137446567405364 -0.00601165158222017
0.0137446567405752 -0.00601165158224148
0.0137446567406467 -0.00601165158230899
0.0137446567405943 -0.00601165158236583
0.0137446567405883 -0.00601165158242978
0.0137446567405675 -0.00601165158246175
0.0137446567405766 -0.00601165158246886
0.0137446567405579 -0.00601165158249017
0.0137446567405166 -0.00601165158240491
0.0137446567405037 -0.0060116515823907
0.0137446567405328 -0.00601165158231964
0.01374465674051 -0.00601165158231964
0.0137446567405117 -0.00601165158226635
0.0137446567405153 -0.00601165158232675
0.0137446567404953 -0.00601165158233741
0.0137446567405048 -0.00601165158233741
0.0137446567405035 -0.0060116515823978
0.0137446567404498 -0.00601165158240491
0.0137446567404511 -0.0060116515824653
0.0137446567404238 -0.00601165158253991
0.0137446567404247 -0.00601165158257544
0.0137446567404238 -0.00601165158250438
0.0137446567404362 -0.00601165158248307
0.0137446567404262 -0.00601165158244754
0.0137446567404138 -0.00601165158240136
0.0137446567404058 -0.00601165158231254
0.0137446567404351 -0.00601165158229122
0.0137446567404624 -0.00601165158231254
0.0137446567404436 -0.00601165158227701
0.0137446567404373 -0.00601165158226635
0.0137446567404576 -0.00601165158228767
0.0137446567404433 -0.00601165158233385
0.0137446567404469 -0.00601165158225569
0.0137446567404624 -0.00601165158229477
0.0137446567404946 -0.00601165158222727
0.0137446567405497 -0.00601165158227346
0.0137446567406028 -0.00601165158226635
0.0137446567406392 -0.00601165158230188
0.0137446567405977 -0.00601165158239425
0.0137446567405968 -0.00601165158245465
0.0137446567405908 -0.00601165158250083
0.0137446567405657 -0.00601165158250438
0.0137446567405695 -0.00601165158243333
0.0137446567405095 -0.00601165158240846
0.0137446567405175 -0.00601165158241201
0.0137446567405288 -0.00601165158231609
0.0137446567405126 -0.00601165158233385
0.0137446567405037 -0.00601165158234096
0.0137446567405173 -0.00601165158235162
0.0137446567404831 -0.00601165158232675
0.0137446567404993 -0.00601165158233385
0.01374465674048 -0.00601165158241201
0.0137446567404407 -0.00601165158240136
0.0137446567404336 -0.0060116515824582
0.0137446567404269 -0.0060116515825257
0.0137446567404131 -0.00601165158253281
0.0137446567404305 -0.00601165158250794
0.0137446567404229 -0.0060116515824653
0.0137446567404484 -0.0060116515824582
0.01374465674041 -0.00601165158234096
0.0137446567404127 -0.00601165158231609
0.0137446567404655 -0.00601165158234451
0.0137446567404551 -0.00601165158230543
0.0137446567404411 -0.00601165158228767
0.0137446567404458 -0.00601165158226991
0.013744656740478 -0.00601165158228767
0.0137446567404316 -0.00601165158230899
0.0137446567404844 -0.00601165158227346
0.0137446567404842 -0.00601165158227346
0.0137446567404966 -0.00601165158222727
0.0137446567405541 -0.00601165158229122
0.0137446567406188 -0.00601165158229122
0.0137446567406267 -0.00601165158232675
0.0137446567405923 -0.00601165158242623
0.0137446567405943 -0.00601165158246175
0.0137446567405877 -0.00601165158250438
0.0137446567405435 -0.00601165158248662
0.0137446567405357 -0.00601165158241201
0.0137446567405188 -0.00601165158242623
0.0137446567405204 -0.00601165158236583
0.0137446567405197 -0.00601165158229122
0.0137446567405271 -0.00601165158231609
0.0137446567405186 -0.00601165158234096
0.0137446567405055 -0.00601165158231964
0.0137446567404877 -0.00601165158235872
0.0137446567405108 -0.00601165158236938
0.0137446567404695 -0.00601165158241201
0.0137446567404456 -0.00601165158244754
0.0137446567404509 -0.00601165158251149
0.0137446567404076 -0.00601165158254346
0.0137446567404282 -0.0060116515825257
0.0137446567404351 -0.00601165158247596
0.0137446567404163 -0.0060116515824653
0.0137446567404416 -0.00601165158241557
0.0137446567404222 -0.00601165158237293
0.0137446567404234 -0.00601165158234096
0.0137446567404453 -0.00601165158231964
0.0137446567404511 -0.00601165158230188
0.0137446567404242 -0.00601165158228056
0.0137446567404684 -0.00601165158233385
0.0137446567404411 -0.00601165158230188
0.0137446567404169 -0.00601165158227346
0.0137446567404862 -0.00601165158226635
0.0137446567405171 -0.00601165158226635
0.0137446567405328 -0.00601165158218819
0.0137446567405644 -0.0060116515822628
0.0137446567406339 -0.00601165158229833
0.0137446567406001 -0.00601165158236583
0.0137446567405886 -0.00601165158243333
0.0137446567405646 -0.00601165158246175
0.0137446567405852 -0.00601165158247596
0.0137446567405701 -0.00601165158251504
0.0137446567405144 -0.00601165158240491
0.0137446567404951 -0.00601165158240491
0.0137446567405264 -0.00601165158234451
0.0137446567405159 -0.00601165158230188
0.0137446567405135 -0.00601165158224504
0.0137446567405275 -0.00601165158230543
0.0137446567404997 -0.0060116515823303
0.0137446567404971 -0.00601165158236583
0.0137446567404966 -0.00601165158240491
0.0137446567404582 -0.00601165158241557
0.0137446567404473 -0.00601165158247952
0.0137446567404225 -0.00601165158253636
0.0137446567404087 -0.00601165158258254
0.0137446567404158 -0.0060116515825186
0.0137446567404416 -0.00601165158247952
0.013744656740418 -0.00601165158245109
0.0137446567404225 -0.00601165158238715
0.0137446567404034 -0.0060116515823232
0.0137446567404327 -0.00601165158231609
0.0137446567404669 -0.00601165158230188
0.0137446567404509 -0.00601165158226991
0.0137446567404245 -0.00601165158228767
0.0137446567404564 -0.00601165158229833
0.0137446567404353 -0.0060116515823303
0.0137446567404342 -0.00601165158225925
0.0137446567404658 -0.00601165158229122
0.0137446567405017 -0.00601165158222372
0.0137446567405424 -0.0060116515822628
0.0137446567405866 -0.0060116515822628
0.0137446567406441 -0.00601165158229122
0.0137446567405897 -0.00601165158236938
0.0137446567405817 -0.00601165158244754
0.0137446567405848 -0.00601165158249017
0.0137446567405728 -0.00601165158251504
0.0137446567405568 -0.00601165158243333
0.0137446567405097 -0.0060116515823978
0.0137446567405257 -0.0060116515823978
0.0137446567405248 -0.0060116515823303
0.0137446567405042 -0.00601165158232675
0.0137446567405091 -0.00601165158230543
0.0137446567405206 -0.00601165158236228
0.0137446567405004 -0.00601165158234096
0.0137446567405037 -0.00601165158235872
0.0137446567404809 -0.0060116515823907
0.0137446567404504 -0.0060116515823907
0.013744656740442 -0.00601165158248662
0.0137446567404274 -0.00601165158253281
0.0137446567404265 -0.00601165158253991
0.01374465674042 -0.0060116515825186
0.0137446567404211 -0.00601165158245465
0.0137446567404365 -0.00601165158248307
0.013744656740422 -0.00601165158236938
0.013744656740412 -0.00601165158232675
0.0137446567404524 -0.00601165158230899
0.0137446567404471 -0.00601165158229833
0.0137446567404356 -0.00601165158229122
0.0137446567404313 -0.00601165158228412
0.0137446567404764 -0.00601165158227701
0.0137446567404433 -0.00601165158231609
0.0137446567404671 -0.00601165158225214
0.0137446567404695 -0.00601165158229122
0.0137446567405224 -0.0060116515822024
0.0137446567405575 -0.00601165158228767
0.0137446567406081 -0.00601165158226635
0.0137446567406234 -0.00601165158229833
0.0137446567405892 -0.00601165158240136
0.0137446567405985 -0.00601165158244754
0.0137446567405786 -0.00601165158247952
0.0137446567405437 -0.00601165158249373
0.0137446567405541 -0.00601165158242978
0.0137446567405313 -0.00601165158239425
0.0137446567405324 -0.00601165158236583
0.0137446567405302 -0.00601165158229833
0.0137446567405199 -0.00601165158233741
0.0137446567405195 -0.00601165158231609
0.0137446567405215 -0.00601165158233385
0.0137446567404835 -0.00601165158234096
0.0137446567405117 -0.00601165158235162
0.0137446567404587 -0.00601165158242978
0.0137446567404618 -0.00601165158244044
0.0137446567404556 -0.00601165158250438
0.0137446567404085 -0.00601165158253281
0.0137446567404231 -0.0060116515825186
0.0137446567404347 -0.00601165158247596
0.0137446567404025 -0.0060116515824582
0.013744656740452 -0.00601165158243333
0.0137446567404163 -0.00601165158235872
0.0137446567404178 -0.00601165158233741
0.0137446567404793 -0.00601165158231254
0.0137446567404473 -0.00601165158226991
0.0137446567404373 -0.00601165158229477
0.0137446567404678 -0.00601165158230899
0.0137446567404522 -0.00601165158231964
0.0137446567404167 -0.00601165158227701
0.0137446567405124 -0.00601165158228767
0.0137446567404906 -0.00601165158226991
0.0137446567405202 -0.00601165158220951
0.0137446567405526 -0.00601165158226635
0.0137446567406316 -0.00601165158229833
0.0137446567406172 -0.00601165158234451
0.0137446567405741 -0.00601165158242267
0.0137446567405832 -0.00601165158245109
0.0137446567405921 -0.00601165158247596
0.0137446567405581 -0.00601165158249728
0.0137446567405068 -0.00601165158240491
0.013744656740502 -0.00601165158240491
0.0137446567405299 -0.00601165158234807
0.0137446567405093 -0.00601165158229833
0.0137446567405188 -0.00601165158228056
0.0137446567405357 -0.00601165158231609
0.0137446567404977 -0.0060116515823232
0.0137446567404846 -0.00601165158236938
0.0137446567405062 -0.00601165158238715
0.0137446567404622 -0.0060116515823978
0.0137446567404469 -0.00601165158246886
0.0137446567404167 -0.00601165158252925
0.0137446567404074 -0.00601165158256478
0.0137446567404329 -0.00601165158252925
0.0137446567404369 -0.00601165158248662
0.0137446567404207 -0.00601165158244754
0.0137446567404316 -0.00601165158242267
0.0137446567404058 -0.00601165158234807
0.0137446567404398 -0.00601165158230543
0.01374465674046 -0.00601165158231609
0.013744656740442 -0.00601165158227701
0.0137446567404218 -0.00601165158225925
0.0137446567404762 -0.00601165158233385
0.0137446567404302 -0.00601165158231254
0.0137446567404163 -0.0060116515822628
0.0137446567404833 -0.00601165158230188
0.0137446567405051 -0.00601165158222372
0.0137446567405413 -0.00601165158223438
0.0137446567405772 -0.00601165158226635
0.0137446567406414 -0.00601165158229833
0.0137446567405977 -0.00601165158236228
0.0137446567405672 -0.00601165158242978
0.0137446567405681 -0.00601165158248307
0.013744656740571 -0.00601165158250794
0.0137446567405537 -0.0060116515824653
0.0137446567405171 -0.00601165158239425
0.0137446567405188 -0.0060116515823978
0.0137446567405295 -0.00601165158229833
0.0137446567405073 -0.00601165158235162
0.0137446567405091 -0.00601165158228412
0.0137446567405137 -0.00601165158233741
0.0137446567404982 -0.00601165158234096
0.0137446567404871 -0.00601165158234807
0.0137446567404891 -0.00601165158240491
0.0137446567404458 -0.00601165158239425
0.01374465674045 -0.00601165158247952
0.0137446567404205 -0.00601165158253991
0.0137446567404242 -0.00601165158255412
0.0137446567404191 -0.00601165158250794
0.0137446567404178 -0.00601165158246886
0.0137446567404349 -0.00601165158247596
0.0137446567404049 -0.00601165158238359
0.0137446567404038 -0.00601165158231609
0.0137446567404507 -0.00601165158230899
0.0137446567404691 -0.00601165158229477
0.013744656740448 -0.00601165158227701
0.013744656740436 -0.00601165158228412
0.0137446567404689 -0.00601165158228056
0.0137446567404438 -0.00601165158231964
0.013744656740458 -0.00601165158225925
0.0137446567404684 -0.00601165158228412
0.0137446567404953 -0.00601165158220596
0.0137446567405499 -0.00601165158227701
0.0137446567406037 -0.00601165158226635
0.0137446567406334 -0.00601165158228767
0.0137446567405992 -0.0060116515823978
0.0137446567406063 -0.00601165158246175
0.0137446567405939 -0.00601165158249373
0.0137446567405681 -0.00601165158251504
0.0137446567405632 -0.00601165158242623
0.0137446567405237 -0.00601165158238359
0.0137446567405124 -0.00601165158238715
0.0137446567405193 -0.00601165158231964
0.0137446567405173 -0.00601165158234096
0.0137446567405086 -0.00601165158231964
0.0137446567405124 -0.00601165158234096
0.0137446567404906 -0.00601165158235162
0.0137446567405135 -0.00601165158235162
0.0137446567404644 -0.00601165158240846
0.0137446567404664 -0.00601165158242267
0.0137446567404504 -0.00601165158249373
0.0137446567404127 -0.00601165158252215
0.0137446567404265 -0.00601165158252215
0.0137446567404509 -0.00601165158250083
0.0137446567403974 -0.00601165158247241
0.0137446567404413 -0.00601165158243688
0.01374465674041 -0.00601165158232675
0.013744656740422 -0.00601165158232675
0.0137446567404698 -0.00601165158232675
0.0137446567404467 -0.00601165158228412
0.0137446567404349 -0.00601165158230543
0.0137446567404518 -0.00601165158227346
};
\addplot [very thick, learnedWithoutSideInfo, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.130945815911047 0.0249882859606529
0.123694753124036 -0.0319125519429093
0.0932119632451851 -0.0432888186678042
0.068424474675405 -0.0395825921806789
0.0508200096140734 -0.0338674776437493
0.0382540866988017 -0.0281520050207966
0.0293210601370346 -0.0229007752971384
0.0231220306474205 -0.0183218835495396
0.018993392115733 -0.0145334639269592
0.0163914789170931 -0.0115719221303294
0.0148637930093798 -0.00939380098890297
0.0140481784838975 -0.00789427565154099
0.0136718678398011 -0.00693537844718861
0.0135431747951824 -0.00637354819124525
0.0135373845112894 -0.00608003200339624
0.0135803621150286 -0.0059520319023143
0.0136328994803485 -0.00591553783608134
0.0136776923521016 -0.00592240537164912
0.0137096990209644 -0.0059445852022435
0.0137297506338177 -0.00596785418274237
0.0137407823930924 -0.00598645445624868
0.0137459053251061 -0.00599917473090983
0.0137476179443485 -0.00600683298929283
0.0137476344732999 -0.00601085444065319
0.013746990091869 -0.00601258718676689
0.0137462304300771 -0.00601305420808274
0.0137455921218994 -0.00601292865277969
0.0137451403412461 -0.00601260090167344
0.0137448595783436 -0.00601226642386266
0.0137447064473195 -0.00601200243707822
0.0137446362423939 -0.00601182345906892
0.0137446135160877 -0.00601171653851651
0.0137446141556632 -0.00601166090839556
0.013744623710229 -0.00601163731219145
0.0137446346313823 -0.00601163128677129
0.0137446436954418 -0.00601163338728483
0.01374465005893 -0.00601163817786698
0.0137446539851536 -0.00601164296365653
0.0137446561087946 -0.00601164670200305
0.0137446570698172 -0.0060116492173421
0.0137446573702176 -0.00601165070896315
0.0137446573489692 -0.00601165147790539
0.0137446572077282 -0.00601165179864438
0.0137446570509077 -0.00601165187556063
0.0137446569223283 -0.00601165184131247
0.0137446568327499 -0.00601165177165086
0.0137446567778012 -0.00601165170326468
0.0137446567483153 -0.00601165165042872
0.0137446567351682 -0.00601165161497619
0.013744656730988 -0.00601165159401518
0.0137446567316146 -0.00601165158325756
0.0137446567337949 -0.00601165157894101
0.0137446567360642 -0.00601165157803152
0.01374465673794 -0.00601165157861772
0.0137446567391681 -0.00601165157968353
0.0137446567400143 -0.0060116515808204
0.0137446567403103 -0.00601165158157713
0.0137446567404906 -0.00601165158212424
0.0137446567404564 -0.00601165158245109
0.0137446567404413 -0.00601165158243688
0.0137446567404349 -0.00601165158230543
0.0137446567404909 -0.00601165158227701
0.0137446567405852 -0.00601165158241912
0.0137446567405184 -0.00601165158241912
0.0137446567404966 -0.0060116515823232
0.0137446567404222 -0.0060116515825257
0.0137446567404451 -0.00601165158243333
0.0137446567404316 -0.00601165158226991
0.0137446567405224 -0.00601165158225569
0.0137446567405883 -0.00601165158242978
0.0137446567405037 -0.0060116515823907
0.0137446567404953 -0.00601165158233741
0.0137446567404238 -0.00601165158253991
0.0137446567404138 -0.00601165158240136
0.0137446567404373 -0.00601165158226635
0.0137446567404946 -0.00601165158222727
0.0137446567405968 -0.00601165158245465
0.0137446567405175 -0.00601165158241201
0.0137446567404831 -0.00601165158232675
0.0137446567404269 -0.0060116515825257
0.01374465674041 -0.00601165158234096
0.0137446567404458 -0.00601165158226991
0.0137446567404966 -0.00601165158222727
0.0137446567405943 -0.00601165158246175
0.0137446567405204 -0.00601165158236583
0.0137446567404877 -0.00601165158235872
0.0137446567404076 -0.00601165158254346
0.0137446567404222 -0.00601165158237293
0.0137446567404684 -0.00601165158233385
0.0137446567405328 -0.00601165158218819
0.0137446567405646 -0.00601165158246175
0.0137446567405264 -0.00601165158234451
0.0137446567404971 -0.00601165158236583
0.0137446567404087 -0.00601165158258254
0.0137446567404034 -0.0060116515823232
0.0137446567404564 -0.00601165158229833
0.0137446567405424 -0.0060116515822628
0.0137446567405848 -0.00601165158249017
0.0137446567405248 -0.0060116515823303
0.0137446567405037 -0.00601165158235872
0.0137446567404265 -0.00601165158253991
0.013744656740412 -0.00601165158232675
0.0137446567404764 -0.00601165158227701
0.0137446567405575 -0.00601165158228767
0.0137446567405786 -0.00601165158247952
0.0137446567405302 -0.00601165158229833
0.0137446567405117 -0.00601165158235162
0.0137446567404231 -0.0060116515825186
0.0137446567404178 -0.00601165158233741
0.0137446567404522 -0.00601165158231964
0.0137446567405526 -0.00601165158226635
0.0137446567405921 -0.00601165158247596
0.0137446567405093 -0.00601165158229833
0.0137446567405062 -0.00601165158238715
0.0137446567404329 -0.00601165158252925
0.0137446567404398 -0.00601165158230543
0.0137446567404302 -0.00601165158231254
0.0137446567405772 -0.00601165158226635
0.013744656740571 -0.00601165158250794
0.0137446567405073 -0.00601165158235162
0.0137446567404891 -0.00601165158240491
0.0137446567404191 -0.00601165158250794
0.0137446567404507 -0.00601165158230899
0.0137446567404438 -0.00601165158231964
0.0137446567406037 -0.00601165158226635
0.0137446567405681 -0.00601165158251504
0.0137446567405173 -0.00601165158234096
0.0137446567404644 -0.00601165158240846
0.0137446567404509 -0.00601165158250083
0.0137446567404698 -0.00601165158232675
0.0137446567404158 -0.00601165158227346
0.0137446567406254 -0.00601165158230899
0.0137446567405628 -0.00601165158248307
0.0137446567405284 -0.00601165158230543
0.0137446567404618 -0.00601165158240136
0.0137446567404269 -0.00601165158246886
0.0137446567404582 -0.00601165158231964
0.0137446567404105 -0.00601165158226991
0.0137446567406467 -0.00601165158230899
0.0137446567405579 -0.00601165158249017
0.0137446567405117 -0.00601165158226635
0.0137446567404498 -0.00601165158240491
0.0137446567404362 -0.00601165158248307
0.0137446567404624 -0.00601165158231254
0.0137446567404469 -0.00601165158225569
0.0137446567406392 -0.00601165158230188
0.0137446567405695 -0.00601165158243333
0.0137446567405037 -0.00601165158234096
0.0137446567404407 -0.00601165158240136
0.0137446567404229 -0.0060116515824653
0.0137446567404551 -0.00601165158230543
0.0137446567404844 -0.00601165158227346
0.0137446567406267 -0.00601165158232675
0.0137446567405357 -0.00601165158241201
0.0137446567405186 -0.00601165158234096
0.0137446567404456 -0.00601165158244754
0.0137446567404163 -0.0060116515824653
0.0137446567404511 -0.00601165158230188
0.0137446567404862 -0.00601165158226635
0.0137446567406001 -0.00601165158236583
0.0137446567405144 -0.00601165158240491
0.0137446567405275 -0.00601165158230543
0.0137446567404473 -0.00601165158247952
0.013744656740418 -0.00601165158245109
0.0137446567404509 -0.00601165158226991
0.0137446567404658 -0.00601165158229122
0.0137446567405897 -0.00601165158236938
0.0137446567405097 -0.0060116515823978
0.0137446567405206 -0.00601165158236228
0.013744656740442 -0.00601165158248662
0.0137446567404365 -0.00601165158248307
0.0137446567404356 -0.00601165158229122
0.0137446567404695 -0.00601165158229122
0.0137446567405892 -0.00601165158240136
0.0137446567405313 -0.00601165158239425
0.0137446567405215 -0.00601165158233385
0.0137446567404556 -0.00601165158250438
0.013744656740452 -0.00601165158243333
0.0137446567404373 -0.00601165158229477
0.0137446567404906 -0.00601165158226991
0.0137446567405741 -0.00601165158242267
0.013744656740502 -0.00601165158240491
0.0137446567404977 -0.0060116515823232
0.0137446567404167 -0.00601165158252925
0.0137446567404316 -0.00601165158242267
0.0137446567404218 -0.00601165158225925
0.0137446567405051 -0.00601165158222372
0.0137446567405672 -0.00601165158242978
0.0137446567405188 -0.0060116515823978
0.0137446567404982 -0.00601165158234096
0.0137446567404205 -0.00601165158253991
0.0137446567404049 -0.00601165158238359
0.013744656740436 -0.00601165158228412
0.0137446567404953 -0.00601165158220596
0.0137446567406063 -0.00601165158246175
0.0137446567405124 -0.00601165158238715
0.0137446567404906 -0.00601165158235162
0.0137446567404127 -0.00601165158252215
0.01374465674041 -0.00601165158232675
0.0137446567404518 -0.00601165158227346
};

==> figures/smd_phase_plots/phase_plot_50_full_space_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.0926769152283669 0.104911841452122
0.0650544390082359 0.080585777759552
-0.0677666291594505 -0.0820656418800354
-0.127343222498894 -0.0687435939908028
-0.108778446912766 -0.0255548115819693
-0.135148167610168 -0.134661048650742
-0.0734996572136879 0.034317173063755
0.0901187360286713 -0.0988252535462379
0.122649542987347 -0.0557215809822083
0.0569019317626953 0.132267102599144
-0.10691375285387 -0.102424830198288
0.0245587918907404 -0.0548642538487911
-0.145891472697258 0.000418173498474061
-0.0587299391627312 0.013023667037487
0.134766399860382 -0.067163847386837
-0.0560438372194767 -0.0206446889787912
-0.136450439691544 0.0200800690799952
0.0608698315918446 -0.00766637874767184
0.116106569766998 -0.0241063330322504
-0.0465967915952206 0.0426911897957325
0.0794783309102058 0.0739545151591301
0.0126688983291388 -0.0810919925570488
0.051988422870636 0.0674897953867912
0.0469152852892876 0.119893714785576
0.0701540857553482 0.0501166842877865
0.121553391218185 0.0386670231819153
-0.0853148624300957 0.0287881884723902
0.147940069437027 -0.118771478533745
-0.0500022023916245 -0.0790142044425011
-0.045499712228775 0.0447170473635197
0.138355076313019 -0.0975632593035698
0.0749749392271042 -0.0526592321693897
0.0465032085776329 0.0545745156705379
0.0193955451250076 0.110306151211262
-0.0649936199188232 0.10236569494009
0.0265224147588015 0.0556329190731049
0.102513208985329 0.0422969870269299
0.123559042811394 0.101078897714615
0.00808075629174709 0.114377178251743
0.109717488288879 0.0455804765224457
-0.129514262080193 0.0168509129434824
-0.116119004786015 -0.0365315638482571
0.0808051452040672 0.0599738247692585
-0.131533429026604 0.0490952730178833
0.0576809234917164 0.0222184956073761
-0.144087761640549 0.140230670571327
-0.0229435581713915 -0.0271971914917231
-0.143589228391647 -0.0451608709990978
0.0175557099282742 -0.124941639602184
0.120490409433842 -0.071074940264225
};
\addplot [very thick, trueDynamics]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, approxDynamics, dashed]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, learnedWithSideInfo]
table {%
0.1 0.1
0.109246441199181 0.0849018149662462
0.116977675526147 0.069722431484091
0.123193363508238 0.0546156064312795
0.127907976823245 0.0397241239173454
0.131149793862819 0.0251798894630877
0.132959625606996 0.0111040857207835
0.133389951247342 -0.00239276626287717
0.13250369617775 -0.0152108546170135
0.130373382528753 -0.0272611840957376
0.127079713480388 -0.0384657560357822
0.122710664238678 -0.0487577619534498
0.11736041656728 -0.0580817073303147
0.111128054917482 -0.0663935334946381
0.104116553140141 -0.0736606485552987
0.0964314929822816 -0.0798618436888623
0.0881800880629998 -0.0849871225265016
0.0794699470810813 -0.0890374032013219
0.0704080903452737 -0.0920241821933921
0.0610998880753585 -0.0939690036884561
0.0516480359499422 -0.0949027658981009
0.0421517430001258 -0.0948651156397533
0.0327058375340427 -0.0939034876652142
0.0234000462870468 -0.0920723228232087
0.0143183527222821 -0.0894320726253525
0.00553842703636739 -0.0860481978599116
-0.00286881788031084 -0.0819902581744622
-0.0108395815462289 -0.0773308760684161
-0.0183174501974898 -0.0721449391812005
-0.0252535686535966 -0.0665087063762985
-0.031606746285347 -0.0604989647114421
-0.0373434703107504 -0.0541923455467279
-0.0424378555221606 -0.0476645984418564
-0.0468715046016617 -0.0409899310821339
-0.0506333591166202 -0.0342404334726763
-0.053719416406673 -0.0274854390831402
-0.056132476267334 -0.0207910375045603
-0.0578817311761314 -0.014219552592574
-0.0589824310232399 -0.00782911251000801
-0.0594553951080849 -0.00167325780994927
-0.0593265464883014 0.00419938283610803
-0.0586264239770089 0.00974533795222151
-0.0573896568865985 0.0149264827867142
-0.0556543950670124 0.0197101391122643
-0.0534617948213336 0.0240691348958746
-0.0508554526640069 0.0279817796244583
-0.0478808763288496 0.0314317824933953
-0.044584896170065 0.0344081477727456
-0.0410152292972088 0.0369049990447127
-0.0372199244988942 0.038921346094104
-0.033246874221362 0.040460890989935
-0.0291433880133247 0.0415317542820609
-0.0249557529312265 0.0421461678911054
-0.0207288423744912 0.0423201752135219
-0.0165057584478735 0.0420732754554398
-0.0123274789815528 0.0414281310754381
-0.00823257626281201 0.0404101337191771
-0.00425696557053178 0.0390471078916626
-0.000433673122604346 0.0373689027365003
0.00320734411608624 0.0354069656766065
0.0066393416889148 0.0331940344594058
0.00983889516662864 0.03076374046307
0.0127859702666736 0.0281502024125516
0.0154639583395913 0.0253877003116485
0.0178596710212752 0.0225103434916055
0.0199633071796267 0.0195517184185674
0.0217683942484154 0.0165446051339843
0.023271673681831 0.0135206778724004
0.0244729938585863 0.0105102688047723
0.0253751461748889 0.00754212517333476
0.0259837328018577 0.00464320450771843
0.0263069338592405 0.00183849795886065
0.0263553341930261 -0.000849120613281436
0.0261416998610622 -0.00339901632987824
0.0256807359915473 -0.00579289003048337
0.0249888576792304 -0.00801484152737757
0.0240839515681782 -0.010051421084653
0.0229851243947942 -0.0118916310850101
0.0217124589813097 -0.0135269234682598
0.0202867795419775 -0.0149511709638581
0.0187293909113336 -0.0161606021812968
0.0170618717891348 -0.0171537329803947
0.0153058297999331 -0.0179312701292149
0.0134827124323591 -0.0184959841561659
0.011613575136646 -0.0188526103261736
0.00971891275217588 -0.019007690925516
0.00781848348351174 -0.0189694270468819
0.00593114870929859 -0.0187475153967328
0.00407473374503789 -0.0183529834175494
0.00226589931664301 -0.0177980093955985
0.000520039343851662 -0.0170957723730465
-0.00114881277947694 -0.0162602352922463
-0.00272805275758953 -0.0153060013623834
-0.0042065605780408 -0.0142481333209699
-0.00557474009746925 -0.013101972741046
-0.0068245326659511 -0.0118829908425522
-0.00794942842332221 -0.0106066216633855
-0.00894445512711266 -0.00928811101660096
-0.0098061478878442 -0.00794238769421274
-0.0105325133166125 -0.006583919813325
-0.0111229755111629 -0.00522660268350669
-0.0115783164540572 -0.00388365110281899
-0.0119006052346318 -0.00256749833785109
-0.0120931039874799 -0.00128971620863156
-0.0121601896631823 -6.09427915073046e-05
-0.0121072515843716 0.00110917678656049
-0.0119405973833196 0.00221203616563202
-0.0116673421754658 0.00324010277976272
-0.0112952940072963 0.0041869376292516
-0.0108328486171603 0.00504720615353931
-0.010288884195878 0.00581667798816187
-0.00967264962761102 0.00649221051920575
-0.00899364993682872 0.00707173289086311
-0.00826154663591565 0.00755421265429545
-0.00748605248470392 0.00793960987155778
-0.00667683742574954 0.00822883776394565
-0.00584343638208378 0.00842370243954713
-0.00499516078013081 0.00852685009601926
-0.00414101752267259 0.00854168592446858
-0.00328963657715782 0.00847231850268121
-0.00244920834228438 0.00832348102766172
-0.00162741938497879 0.00810045529989818
-0.000831404882612105 0.00780899112314304
-6.7703874047593e-05 0.00745523262669624
0.000657774575439593 0.00704563528718932
0.00133977928677175 0.00658688903553811
0.00197373696320572 0.00608584364608839
0.00255576381919763 0.00554943134745645
0.00308267036963874 0.00498459776951511
0.00355196050038306 0.00439823153218739
0.00396182006094005 0.00379710165932729
0.00431110382762168 0.0031877950463061
0.00459931431727087 0.00257666107616765
0.00482657384877037 0.00196976272889376
0.00499359613893014 0.00137282991052066
0.00510164858488995 0.000791218260223542
0.00515251408070463 0.00022987764693068
0.00514844771163341 -0.000306679134649496
0.00509213577650478 -0.000814398750135701
0.00498664549674253 -0.00128970469916111
0.00483537612227606 -0.00172951045983905
0.00464201096855936 -0.00213122368274857
0.00441046945355263 -0.00249275050882417
0.00414485214962842 -0.00281249092538931
0.00384939770968305 -0.00308933007897556
0.00352843350678454 -0.00332262668509965
0.00318632650651357 -0.00351219680881132
0.00282744019279273 -0.00365829231184394
0.00245609289065316 -0.00376157884336044
0.00207651469189177 -0.003823107802198
0.00169281404325028 -0.00384428945323493
0.00130894130757872 -0.00382686026640522
0.000928658436899444 -0.0037728514006402
0.000555510915426523 -0.00368455209421309
0.000192804010048397 -0.00356447839090907
-0.000156418956593954 -0.00341533560390299
-0.000489392832325502 -0.00323998379055331
-0.000803644635350474 -0.00304139929661123
-0.00109700347943558 -0.00282264371227581
-0.00136760803987137 -0.00258682841480954
-0.00161390869350208 -0.00233708075480329
-0.00183466751942377 -0.00207651416056871
-0.00202895731021271 -0.00180819837101463
-0.00219615295794203 -0.00153512955041774
-0.00233592586680509 -0.00126020711701476
-0.00244822986750354 -0.000986208376250961
-0.00253329050756823 -0.000715767671960549
-0.00259158898649955 -0.000451357850679747
-0.00262384422823538 -0.000195273423067317
-0.00263099541919512 5.03830430035944e-05
-0.00261418268362241 0.000283712219537526
-0.00257472473207537 0.000503027016258511
-0.00251409837247263 0.000706858191137196
-0.00243391522716167 0.000893959369937448
-0.00233590240798044 0.00106330712178134
-0.00222187690491308 0.00121410153612611
-0.00209372463122743 0.00134576205288291
-0.00195337946862614 0.00145792305700012
-0.00180279986759157 0.00155042745261964
-0.00164395208339122 0.00162331785329208
-0.00147878700916618 0.00167682662287149
-0.00130922399393878 0.00171136451941418
-0.0011371322158273 0.00172750714142323
-0.000964316304459746 0.00172598311232698
-0.000792500391692391 0.00170765832449774
-0.000623316353285681 0.00167352064775666
-0.000458291323015904 0.00162466579572196
-0.000298838611846293 0.00156227983381876
-0.000146248714498525 0.00148762481273297
-1.68291628877063e-06 0.00140202174317305
0.00013383185101254 0.00130683402426651
0.000259406604533744 0.00120345424171684
0.00037429224543542 0.00109328771890642
0.00047788049816064 0.000977738492695709
0.000569702611283201 0.000858195307547761
0.000649427640636766 0.000736019151823982
0.000716858724351399 0.000612531623298387
0.000771928601136231 0.000489003109198382
0.000814694400934419 0.000366643462792444
0.00084533048561293 0.000246592649157203
0.000864121347817304 0.000129913288718758
0.000871454160557083 1.75838018516058e-05
0.000867808823837431 -8.95070216872622e-05
0.000853750048526858 -0.000190564362853896
0.000829916762649191 -0.00028489079404902
0.00079701250717097 -0.000371888144283653
0.000755796181015914 -0.000451058753297344
0.000707071098028623 -0.000522005529048648
0.000651675382687974 -0.000584430889991502
0.000590471841937042 -0.000638135055422676
0.00052433882650533 -0.000683012829999892
0.000454160248212135 -0.000719050535336635
0.00038081719796979 -0.000746321663179544
0.000305179214506632 -0.000764981836946447
0.000228096382549156 -0.000775263424011319
0.000150391925739179 -0.000777469280886314
7.28556144825265e-05 -0.000771966901004436
-3.76253475640688e-06 -0.000759181524187686
-7.875761699852e-05 -0.000739588777336786
-0.000151474563744572 -0.000713708363709108
-0.000221312105831801 -0.000682096126094751
-0.000287726161919109 -0.000645337443665787
-0.000350232298408074 -0.000604039412434818
-0.000408407446725993 -0.000558824590216483
-0.000461891606081234 -0.000510323582270425
-0.000510387727195085 -0.000459169162630055
-0.00055366188709686 -0.000405989236256174
-0.000591542736289683 -0.00035140136609573
-0.000623919374309615 -0.000296007067331671
-0.000650740622259197 -0.000240386769142128
-0.000672011763291136 -0.000185095195134658
-0.000687792156199332 -0.000130657106067838
-0.000698192208715712 -7.75636444879275e-05
-0.000703368953805078 -2.62691523172372e-05
-0.00070352377963454 2.28114985517673e-05
-0.000698897074524392 6.93050979605619e-05
-0.000689764152452631 0.000112881671892243
-0.000676431586002037 0.000153255698919543
-0.000659231967689374 0.000190186715874903
-0.000638519719018193 0.000223479497082269
-0.000614666666690934 0.000252983786311476
-0.000588057036734993 0.000278593594064399
-0.000559084078432477 0.000300246111380784
-0.000528144709182128 0.000317920304990886
-0.000495636138406203 0.000331634962574922
-0.000461951996699116 0.000341446809417116
-0.000427477999285491 0.000347447786900229
-0.000392589413937083 0.000349762792381655
-0.000357647335606245 0.000348546813169817
-0.000322995921490086 0.000343981739495307
-0.000288959917135747 0.000336273613475838
-0.000255842531772356 0.000325649154335818
-0.000223923240900568 0.000312352745859179
-0.000193456520191771 0.000296643048063546
-0.000164670186494155 0.000278789869099914
-0.000137764801122169 0.000259070980219505
-0.00011291281850024 0.000237769161020907
-9.0258316867095e-05 0.000215168869539689
-6.99169400045646e-05 0.000191553635596469
-5.19761518275745e-05 0.000167203222308039
-3.64957419971436e-05 0.000142391092693976
-2.35085407275173e-05 0.000117382128871972
-1.30214410028304e-05 9.24303075312211e-05
-5.01655904180385e-06 6.77768328237894e-05
5.47405139047612e-07 4.36483873744271e-05
3.73362503466855e-06 2.02555995046263e-05
4.62547989806423e-06 -2.2082590121859e-06
3.32476328870312e-06 -2.35682893912179e-05
-5.01949126878858e-08 -4.36688178676436e-05
-5.36648440018909e-06 -6.23739787992115e-05
-1.24786168268952e-05 -7.95681153136682e-05
-2.12305492857456e-05 -9.51558470166816e-05
-3.14577278991838e-05 -0.000109062175047423
-4.29890844943419e-05 -0.000121232134337805
-5.56490729716465e-05 -0.000131630337232468
-6.92595456052979e-05 -0.0001402404958678
-8.36416266217079e-05 -0.00014706454565989
-9.86175639520112e-05 -0.000152121812837116
-0.000114012297227435 -0.000155447928351897
-0.000129655131274082 -0.000157093741399977
-0.00014538117678386 -0.000157124146981403
-0.000161032681848919 -0.000155616622998432
-0.000176460196144425 -0.000152659984702362
-0.000191523698740487 -0.000148352951752804
-0.00020609341304147 -0.00014280267033302
-0.000220050650834887 -0.000136123338275941
-0.00023328848171551 -0.000128434611552964
-0.000245712096918563 -0.000119860287106421
-0.000257239245909471 -0.00011052689776768
-0.000267800454700593 -0.000100562206451608
-0.000277338909465173 -9.00940842311539e-05
-0.000285810718503584 -7.92491415280159e-05
-0.000293184359301622 -6.81515265101799e-05
-0.000299440736762367 -5.69219331173782e-05
-0.000304572310118178 -4.56765332282768e-05
-0.000308583238473477 -3.4526020956928e-05
-0.000311488187566571 -2.3574848798523e-05
-0.000313312067854206 -1.29204911025887e-05
-0.000314089277827191 -2.65281574498774e-06
-0.000313862394351046 7.14641446766589e-06
-0.000312682114468445 1.64039507583483e-05
-0.000310605916631219 2.50553751868e-05
-0.00030769724579838 3.30453023624422e-05
-0.000304024582116077 4.032746608456e-05
-0.000299660713322914 4.68647646085368e-05
-0.000294681570595058 5.26291609443388e-05
-0.000289165442738692 5.76015308886568e-05
-0.000283192132173194 6.1771394969325e-05
-0.000276842081808943 6.51366434175661e-05
-0.000270195531027363 6.77031377706318e-05
-0.000263331671658189 6.94842402658592e-05
-0.000256328124099847 7.05003866973597e-05
-0.000249260209708909 7.07784781916973e-05
-0.000242200106776566 7.03513671082559e-05
-0.000235216326643469 6.92571690646508e-05
-0.000228373539062655 6.75387491605641e-05
-0.000221731888241719 6.52429324613703e-05
-0.000215346614479653 6.24200191805717e-05
-0.000209267777662092 5.91229734445259e-05
-0.000203540082623081 5.54068733673004e-05
-0.000198202588091343 5.13282374689297e-05
-0.000193288677570756 4.69444129947345e-05
-0.000188826015669871 4.23129640381055e-05
-0.000184836489879367 3.74910960782224e-05
-0.000181336326974862 3.25351200555195e-05
-0.000178336165763999 2.749997465458e-05
-0.00017584124624808 2.24386777980846e-05
-0.000173851671547824 1.74019900537679e-05
-0.000172362495203968 1.24379647909807e-05
-0.000171364245038159 7.59163601113605e-06
-0.000170842923145647 2.90472376487678e-06
-0.000170780718932471 -1.58463111530867e-06
-0.000171156140077998 -5.84205059321607e-06
-0.000171944419984496 -9.83707982956175e-06
-0.000173117968883659 -1.35432932549264e-05
-0.000174646766736495 -1.69383711729029e-05
-0.000176498727030782 -2.00041009303337e-05
-0.000178640176994496 -2.27263760553338e-05
-0.000181036250498891 -2.50951219542433e-05
-0.000183651251858803 -2.71042045406522e-05
-0.000186449063288958 -2.87513089009964e-05
-0.000189393523258029 -3.00377655256577e-05
-0.000192448790291139 -3.09683675164744e-05
-0.000195579634012828 -3.15511641565134e-05
-0.000198751857158962 -3.17972002488428e-05
-0.000201932441101887 -3.17202972210393e-05
-0.000205089822343104 -3.13367560666657e-05
-0.000208194241766309 -3.0665095008315e-05
-0.000211217933819058 -2.972576890723e-05
-0.000214135228383708 -2.85408579038427e-05
-0.000216922725407938 -2.71337706090153e-05
-0.000219559396774569 -2.55289670818108e-05
-0.000222026790036132 -2.37516657033421e-05
-0.000224308882902591 -2.18275498736534e-05
-0.000226392316078497 -1.97825055591279e-05
-0.000228266262302799 -1.76423498525506e-05
-0.000229922499114001 -1.5432588342538e-05
-0.000231355321544784 -1.31781816857046e-05
-0.000232561483919681 -1.09033256645522e-05
-0.000233540127100571 -8.63124438021771e-06
-0.000234292603868267 -6.3840174507699e-06
-0.000234822493478141 -4.18242068160298e-06
-0.000235135281521761 -2.04578176655514e-06
-0.000235238447241326 8.13879393957509e-09
-0.000235141026974648 1.96324256225957e-06
-0.000234853628709088 3.80517475729496e-06
-0.000234388213804158 5.52137439570853e-06
-0.000233757951473586 7.1011222678107e-06
-0.000232976884091451 8.53554272081712e-06
-0.000232059941744161 9.81761183300664e-06
-0.000231022651191858 1.09421320070267e-05
-0.000229880932140546 1.19056994411703e-05
-0.000228651024481473 1.27066479498426e-05
-0.000227349153595221 1.33449811245412e-05
-0.000225991472142158 1.3822288129438e-05
-0.000224594001852564 1.41416586497984e-05
-0.000223172298830041 1.43075697164358e-05
-0.000221741511756843 1.43258015866433e-05
-0.000220315988988939 1.42032910545602e-05
-0.000218909351312272 1.39480120585163e-05
-0.000217534550147661 1.35688525419379e-05
-0.000216203416438145 1.30754823254443e-05
-0.000214926922580366 1.24782345788605e-05
-0.000213714935038411 1.17879482901787e-05
-0.00021257614158129 1.10158578953633e-05
-0.000211518167694891 1.01734529797076e-05
-0.000210547460163512 9.27235339600284e-06
-0.000209669316170972 8.32419521155578e-06
-0.000208887839641917 7.34051760999501e-06
-0.00020820605765456 6.33265335923386e-06
-0.000207625789470555 5.311615699674e-06
-0.000207147850259999 4.28802503865547e-06
-0.000206771963787534 3.27201165872164e-06
-0.000206496907929647 2.27314287392895e-06
-0.000206320485569293 1.30035944603552e-06
-0.000206239728321189 3.61917678971379e-07
-0.000206250780115325 -5.34660368402707e-07
-0.000206349115474639 -1.38262476018485e-06
-0.000206529554066247 -2.17602698287947e-06
-0.000206786406220116 -2.90973728101288e-06
-0.000207113443824903 -3.57945668460818e-06
-0.000207504089502696 -4.18172352945143e-06
-0.000207951489368936 -4.71389655274431e-06
-0.000208448513032669 -5.17414574135967e-06
-0.000208987913667872 -5.56143931106567e-06
-0.000209562415325938 -5.87550411473067e-06
-0.000210164625624855 -6.11679667222517e-06
-0.000210787414099949 -6.28646288958895e-06
-0.000211423708478265 -6.38629236636868e-06
-0.000212066611095096 -6.41866566084091e-06
-0.000212709486206425 -6.38651718923083e-06
-0.000213346047301997 -6.29327051469711e-06
-0.000213970386210568 -6.14277996790038e-06
-0.000214576885789589 -5.9392817687849e-06
-0.000215160627380633 -5.68732185690472e-06
-0.000215716939701654 -5.39169095783044e-06
-0.000216241718989929 -5.05738973038527e-06
-0.000216731312588836 -4.68954528591321e-06
-0.000217182722675604 -4.29337112994952e-06
-0.000217593286120845 -3.87410394356389e-06
-0.000217960980079845 -3.43695582264575e-06
-0.000218284305578554 -2.987062698617e-06
-0.000218562200203314 -2.52943748586809e-06
-0.00021879413996528 -2.06892616152381e-06
-0.000218980095645671 -1.61017009102718e-06
-0.000219120430933258 -1.15756871900538e-06
-0.000219216004288445 -7.15253499245557e-07
-0.000219268008873042 -2.87054338960705e-07
-0.000219278016206592 1.23524171906277e-07
-0.000219248048926263 5.13315716443169e-07
-0.000219180216989507 8.7951010586864e-07
-0.000219077037816366 1.21966438546093e-06
-0.000218941276218556 1.53170576186034e-06
-0.000218775755224781 1.81393951844333e-06
-0.000218583603463079 2.06504223688097e-06
-0.000218367891362984 2.28405906108758e-06
-0.000218131907641414 2.47038878928079e-06
-0.000217878970128086 2.62378995254716e-06
-0.000217612323901176 2.74434734983103e-06
-0.000217335214046745 2.83246252789481e-06
-0.000217050885658263 2.88883614177338e-06
-0.00021676243831687 2.91444260657001e-06
-0.000216472927954266 2.91051064613178e-06
-0.000216185221333164 2.87850518295666e-06
-0.000215902068805937 2.82009114343975e-06
-0.000215626002450794 2.73711353333079e-06
-0.000215359437934329 2.63156759436637e-06
-0.000215104514440078 2.50557841768688e-06
-0.000214863109219525 2.36136610905647e-06
-0.00021463682303932 2.20120958272299e-06
-0.000214427314875068 2.02744115476629e-06
-0.000214235807145706 1.84241981610912e-06
-0.000214063202127965 1.6484972981002e-06
-0.000213910343890125 1.44799297660276e-06
-0.000213777814565128 1.24318820278902e-06
-0.000213665817934439 1.03629167916329e-06
-0.000213574572329265 8.29424321640258e-07
-0.000213503961384525 6.24612907684091e-07
-0.000213453577693785 4.23757497074011e-07
-0.000213423028399349 2.28630317456336e-07
-0.000213411716913433 4.08682835190653e-08
-0.000213418653742742 -1.38049181441259e-07
-0.000213442980357207 -3.06803742672942e-07
-0.000213483692703808 -4.64231488713981e-07
-0.000213539495687166 -6.09336066466695e-07
-0.000213609094207463 -7.41300769895818e-07
-0.000213691251368559 -8.59468169519834e-07
-0.000213784541095464 -9.63342958491126e-07
-0.000213887508205252 -1.05259601477191e-06
-0.000213998697511088 -1.12705625640759e-06
-0.0002141164937512 -1.18671019335532e-06
-0.000214239499938731 -1.23169636941523e-06
-0.000214366304531752 -1.26228002806251e-06
-0.000214495466881375 -1.278853741544e-06
-0.000214625619095286 -1.28193038870933e-06
-0.0002147553932785 -1.27213003384228e-06
-0.000214883596156532 -1.25017160775096e-06
-0.000215009034452947 -1.21685198284155e-06
-0.000215130587648952 -1.17304614569201e-06
-0.000215247251639525 -1.11968919928049e-06
-0.00021535828425309 -1.05775526386973e-06
-0.000215462725038375 -9.8826015982505e-07
-0.00021555986092591 -9.1224672828065e-07
-0.0002156490952611 -8.3077511605148e-07
-0.000215729947804595 -7.44906365579383e-07
-0.000215801996524917 -6.55692807475464e-07
-0.000215864979461992 -5.64171265289917e-07
-0.000215918780175585 -4.71348915741937e-07
-0.000215963325882314 -3.78187226957125e-07
-0.000215998558351556 -2.85614184685357e-07
-0.000216024579424923 -1.94508441041241e-07
-0.000216041563704957 -1.05692645171497e-07
-0.000216049787659109 -1.99281275036454e-08
-0.000216049615068002 6.20927928978235e-08
-0.000216041569785158 1.39754055905519e-07
-0.00021602597193915 2.12512216555064e-07
-0.000216003359938815 2.79888323601908e-07
-0.000215974257643016 3.41481709209036e-07
-0.000215939305327746 3.96965695126025e-07
-0.000215899114167127 4.46093473755078e-07
-0.000215854324440911 4.88689956326758e-07
-0.000215805605534439 5.24652461539668e-07
-0.000215753612282896 5.53948215614893e-07
-0.000215698999523082 5.76610514832227e-07
-0.000215642480301046 5.92736912155643e-07
-0.000215584636697145 6.02485588750354e-07
-0.000215526109000624 6.06065639947688e-07
-0.000215467522950137 6.03738873874039e-07
-0.000215409475181657 5.95813254321027e-07
-0.000215352504124493 5.82636563284129e-07
-0.000215297075449333 5.64593909698971e-07
-0.000215243683931216 5.4209167092787e-07
-0.000215192751586394 5.15567900373839e-07
-0.000215144642223796 4.85472406708959e-07
-0.000215099719652812 4.52274688737646e-07
-0.000215058260371489 4.16448990887483e-07
-0.000215020497222233 3.78472493011393e-07
-0.0002149866484955 3.38821699569832e-07
-0.000214956816066291 2.97965411796743e-07
-0.00021493114546509 2.5636361579125e-07
-0.000214909651254794 2.14458860599374e-07
-0.00021489236254975 1.72676962280609e-07
-0.000214879250256169 1.31422231893115e-07
-0.000214870212520042 9.1073189002408e-08
-0.000214865162038628 5.19818794913855e-08
-0.000214863822333423 1.44632344304188e-08
-0.000214866149755762 -2.11976696334881e-08
-0.000214871940585334 -5.47404232077546e-08
-0.000214880976549097 -8.59387867149612e-08
-0.000214893053925105 -1.14598189975695e-07
-0.000214907823471428 -1.4056004768578e-07
-0.000214925066912454 -1.63701743845831e-07
-0.00021494447866029 -1.83932792420082e-07
-0.000214965767678185 -2.01193929165282e-07
-0.00021498867203243 -2.15457565896221e-07
-0.00021501281337319 -2.26730058491831e-07
-0.000215037958869071 -2.35044679086725e-07
-0.000215063788376528 -2.40462079884648e-07
-0.000215090025407099 -2.43069156817891e-07
-0.000215116364367962 -2.42975208912012e-07
-0.000215142572425255 -2.40312605565875e-07
-0.000215168402192787 -2.35231367918219e-07
-0.000215193577180129 -2.27897579259395e-07
-0.000215217922759878 -2.18492027211255e-07
-0.000215241235200516 -2.07207037717164e-07
-0.000215263339874149 -1.94243309068441e-07
-0.000215284076704638 -1.79807191750831e-07
-0.000215303300167646 -1.64109788651674e-07
-0.000215320893842526 -1.47367859126661e-07
-0.000215336755860583 -1.29795896365061e-07
-0.000215350828008923 -1.11605676150414e-07
-0.000215363052074757 -9.3005130098224e-08
-0.000215373398949242 -7.41972108492944e-08
-0.000215381854075657 -5.53755899147454e-08
-0.000215388432001324 -3.67260240118766e-08
-0.00021539316182574 -1.84227250624863e-08
-0.000215396087200626 -6.27689092109335e-10
-0.000215397251777999 1.65088523121013e-08
-0.000215396742865938 3.28507012638431e-08
-0.000215394633220977 4.82754560545556e-08
-0.000215391126567295 6.2679731478027e-08
-0.000215386266558628 7.59823017035081e-08
-0.00021538014050448 8.81048913378875e-08
-0.000215372864818631 9.89859626427184e-08
-0.000215364570467131 1.08579594489122e-07
-0.000215355359312562 1.16853663938675e-07
-0.000215345391425481 1.23789399915971e-07
-0.000215334812324921 1.29383642020683e-07
-0.000215323738426435 1.33647711582537e-07
-0.000215312286145859 1.36603333341159e-07
-0.000215300601003123 1.38284001944145e-07
-0.000215288813966511 1.38733163184031e-07
-0.000215277026900796 1.3800761419205e-07
-0.000215265385326617 1.36168902490491e-07
-0.000215253991109182 1.3329124618237e-07
-0.000215242931561895 1.29452933607041e-07
-0.000215232279446371 1.24737003341386e-07
-0.000215222151180062 1.1923079535096e-07
-0.000215212619524819 1.13027304894826e-07
-0.000215203742690644 1.06221561086469e-07
-0.000215195593439501 9.89108569701691e-08
-0.000215188171773766 9.11911243778492e-08
-0.000215181550455304 8.31558108799375e-08
-0.000215175744038366 7.48990372227872e-08
-0.00021517076707713 6.65128922459901e-08
-0.000215166634125704 5.80856137355479e-08
-0.000215163286978498 4.97002343212774e-08
-0.000215160696533402 4.14257596199376e-08
-0.000215158906447977 3.33359504774838e-08
-0.000215157931275874 2.55011735153e-08
-0.000215157712811055 1.79865880288801e-08
-0.000215158221951098 1.08480743702191e-08
-0.000215159444145411 4.13902863805743e-09
-0.000215161306635561 -2.09507478726723e-09
-0.000215163780318676 -7.81600134744029e-09
-0.000215166792435976 -1.29925320272416e-08
-0.00021517029933236 -1.75993292959864e-08
-0.000215174228248658 -2.16205575604214e-08
-0.000215178550081382 -2.50430972192212e-08
-0.00021518316296724 -2.78633329213115e-08
-0.00021518803780236 -3.00833022334225e-08
-0.000215193101827053 -3.17086664555419e-08
-0.000215198311385231 -3.27536812411849e-08
-0.000215203550061174 -3.32357745136055e-08
-0.000215208788750393 -3.31818713686372e-08
-0.000215214027452233 -3.26186715112267e-08
-0.000215219222510354 -3.15701574526636e-08
-0.000215224286612462 -3.00705014682004e-08
-0.000215229176101922 -2.81556778963625e-08
-0.000215233861873954 -2.58643782728024e-08
-0.00021523830027182 -2.32375580535606e-08
-0.000215242447638742 -2.03170753458951e-08
-0.000215246289421746 -1.71459194689416e-08
-0.00021524981106786 -1.37670799465334e-08
-0.000215252983472195 -1.02235460726526e-08
-0.00021525577752985 -6.55875979395371e-09
-0.000215258222343623 -2.81435167531763e-09
-0.000215260274256788 9.70083883881923e-10
-0.000215261947820267 4.75427271596357e-09
-0.000215263257585061 8.50133562808539e-09
-0.000215264188998446 1.2178692462058e-08
-0.000215264756611466 1.57510466284455e-08
-0.00021526497497531 1.91898941260052e-08
-0.000215264844089294 2.24669501236625e-08
-0.000215264393056615 2.55573296310818e-08
-0.000215263650980571 2.84399928641987e-08
-0.000215262632412649 3.10975178784839e-08
-0.000215261366456287 3.35145213322015e-08
-0.000215259853111182 3.56790127060969e-08
-0.000215258150584749 3.75814914301345e-08
-0.000215256273428761 3.92165285323723e-08
-0.000215254236195044 4.05807312879071e-08
-0.000215252067987404 4.1673422137168e-08
-0.000215249812461673 4.2498676168512e-08
-0.000215247484169801 4.3058078302502e-08
-0.000215245155871621 4.33627178556689e-08
-0.000215242827567422 4.34243602929173e-08
-0.000215240499257512 4.32554498937948e-08
-0.00021523817094217 4.2867299644006e-08
-0.000215235842621629 4.22694124355139e-08
-0.00021523363071158 4.14776301750977e-08
-0.000215231462452896 4.05095986425602e-08
-0.00021522942515748 3.93834245953142e-08
-0.000215227518825804 3.81174315626856e-08
-0.000215225728906442 3.67313030213111e-08
-0.000215224084503681 3.52440471286519e-08
-0.000215222585617978 3.36739897624158e-08
-0.000215221246801755 3.2042175347486e-08
-0.000215220082607369 3.03657962598576e-08
-0.000215219093035302 2.86649919326205e-08
-0.000215218278086007 2.69578619861016e-08
-0.000215217623207977 2.52604684999186e-08
-0.000215217142953528 2.35895570134884e-08
-0.000215216822771147 2.19609633655277e-08
-0.000215216662661152 2.03875843676933e-08
-0.000215216662623878 1.88829955712587e-08
-0.000215216808107689 1.74580551720767e-08
-0.000215217099112837 1.61231721827748e-08
-0.000215217521087618 1.48864896807113e-08
-0.000215218059480307 1.37559278126295e-08
-0.000215218685187239 1.27371384676424e-08
-0.000215219412760427 1.1834876577875e-08
-0.000215220242199905 1.10502721569448e-08
-0.000215221115298166 1.03887520348442e-08
-0.000215222075710859 9.84692458518358e-09
-0.000215223094334265 9.42931500805613e-09
-0.000215224112960678 9.13297713411171e-09
-0.000215225131589912 8.95044445243381e-09
-0.000215226150221836 8.87651408930032e-09
-0.000215227168856313 8.90575581335984e-09
-0.000215228187493228 9.03319081644802e-09
-0.000215229206132469 9.25474863801637e-09
-0.000215230224773902 9.5643169321924e-09
-0.000215231243417399 9.95760125136608e-09
-0.000215232189303303 1.04302979369794e-08
-0.00021523306243127 1.09679240585525e-08
-0.000215233935560698 1.15643754099691e-08
-0.000215234677724195 1.22124078753318e-08
-0.000215235405336782 1.29004848262171e-08
-0.000215236016534907 1.36220421756775e-08
-0.000215236598629767 1.43657694533575e-08
-0.000215237064309751 1.51262339411797e-08
-0.000215237500886064 1.58928061288512e-08
-0.000215237806495185 1.66595974376849e-08
-0.00021523809755218 1.74175633967794e-08
-0.000215238243089696 1.81608163919537e-08
-0.000215238388626689 1.88828009283458e-08
-0.000215238388643878 1.95767220784876e-08
-0.000215238388660231 2.02369316373852e-08
-0.00021523827226041 2.08611599310064e-08
-0.000215238126755661 2.14408149381597e-08
-0.000215237923042211 2.19779318849991e-08
-0.000215237632016009 2.24627780156909e-08
-0.000215237340988514 2.28953593375825e-08
-0.000215237035407881 2.32788445720354e-08
-0.000215236598858703 2.36077951042135e-08
-0.000215236162308081 2.38781444382788e-08
-0.000215235725756059 2.40919300260357e-08
-0.000215235289202698 2.4252095466408e-08
-0.000215234852648088 2.43615787811832e-08
-0.000215234416092284 2.44228699321572e-08
-0.000215233979535353 2.44386840408603e-08
-0.000215233542977346 2.44110574549455e-08
-0.000215233106418313 2.43422538679858e-08
-0.000215232669858309 2.42340811263883e-08
-0.000215232233297374 2.40881230617433e-08
-0.000215231796735569 2.39075506345068e-08
-0.000215231360172949 2.36937169636846e-08
-0.00021523092360952 2.34473030258191e-08
-0.000215230516149152 2.31698927249252e-08
-0.000215230225103563 2.28723536703328e-08
-0.000215229934057627 2.25605591369984e-08
-0.000215229643011352 2.22354175276156e-08
-0.000215229351964781 2.1898284163855e-08
-0.000215229162781372 2.15521041247932e-08
-0.000215229017253716 2.12070589405283e-08
-0.000215228871726122 2.08645026303876e-08
-0.000215228726198584 2.0524208911403e-08
-0.000215228638878771 2.01870852195932e-08
-0.000215228638870773 1.98642207613342e-08
-0.000215228638863148 1.95565156716274e-08
-0.000215228638855892 1.92635163411004e-08
-0.000215228638848986 1.89849987146037e-08
-0.000215228726153954 1.87225480509715e-08
-0.000215228871667202 1.84861208554418e-08
-0.000215229017181098 1.82757123948218e-08
-0.000215229162695585 1.80890600684144e-08
-0.00021522930821063 1.79250336696142e-08
-0.000215229453726232 1.77836332361514e-08
-0.000215229599242364 1.76635000510676e-08
-0.000215229744758993 1.75635040088051e-08
-0.00021522989027609 1.74822863447006e-08
-0.000215230064897469 1.74193957739113e-08
-0.000215230355934787 1.73832110307755e-08
-0.000215230646972852 1.73771176870639e-08
-0.000215230938011631 1.73999855587227e-08
-0.000215231185395347 1.74497748360244e-08
-0.000215231330916081 1.75153962427704e-08
-0.000215231476437088 1.7592104357457e-08
-0.000215231621958351 1.76792204166151e-08
-0.000215231767479866 1.77762907796475e-08
-0.00021523191300162 1.78830902881205e-08
-0.000215232058523598 1.79989401933103e-08
-0.000215232204045787 1.81233879500975e-08
-0.000215232349568183 1.82559799265583e-08
-0.000215232495090774 1.83967183787007e-08
-0.000215232640613555 1.85449222358733e-08
-0.000215232786136492 1.86994613964216e-08
-0.000215232931659596 1.88607883555916e-08
-0.000215232946215531 1.90232394138394e-08
-0.000215232946219363 1.91779975572057e-08
-0.000215232946223 1.93246092279262e-08
-0.000215232946226458 1.94642079836584e-08
-0.000215232946229749 1.9597018958116e-08
-0.000215232946232883 1.97237220340984e-08
-0.000215232946235867 1.98440887298756e-08
-0.000215232946238712 1.99590263153665e-08
-0.000215232946241434 2.00687588153628e-08
-0.000215232946244016 2.01730621959655e-08
-0.000215232946246476 2.0272387885132e-08
-0.000215232902593063 2.03660547289444e-08
-0.000215232757075893 2.0444331015005e-08
-0.000215232611558277 2.05045065310508e-08
-0.000215232466040232 2.05474874411145e-08
-0.000215232320521785 2.05741776740376e-08
-0.000215232175002959 2.05854822524047e-08
-0.000215232029483759 2.05818548358952e-08
-0.000215231883964213 2.05639719380417e-08
-0.000215231738444333 2.05329682432046e-08
-0.00021523159292414 2.04890666351612e-08
-0.000215231447403646 2.04331743781927e-08
-0.000215231301882856 2.03652903768212e-08
-0.000215231243673348 2.02899445617306e-08
-0.000215231243671541 2.0216863875263e-08
-0.000215231243669823 2.01476307018153e-08
-0.000215231243668183 2.00813377983569e-08
-0.000215231243666627 2.00186661453335e-08
-0.000215231243665143 1.9958708483668e-08
-0.000215231243663727 1.99014659608802e-08
-0.000215231243662371 1.98467122892315e-08
-0.000215231243661077 1.97944474648187e-08
-0.000215231243659845 1.97448988643531e-08
-0.000215231243658679 1.96978379917931e-08
-0.000215231243657563 1.96528134790291e-08
-0.000215231243656504 1.96100515669623e-08
-0.0002152312436555 1.95693248532941e-08
-0.000215231243654546 1.95308618657249e-08
-0.000215231243653637 1.94942089458763e-08
-0.000215231243652767 1.94591398355003e-08
-0.00021523124365193 1.94254282772158e-08
-0.000215231243651149 1.9393751968938e-08
-0.000215231243650402 1.93636605530338e-08
-0.000215231243649677 1.93344742078529e-08
-0.000215231243649007 1.93073230762494e-08
-0.000215231243648355 1.92810780804895e-08
-0.000215231243647741 1.92561895500168e-08
-0.000215231243647156 1.9232659661042e-08
-0.000215231243646598 1.92100337247612e-08
-0.000215231243646068 1.91887664533971e-08
-0.000215231243645566 1.91684030982978e-08
-0.000215231243645075 1.91487196364061e-08
-0.000215231243644629 1.91306188754986e-08
-0.000215231243644205 1.91136505190911e-08
-0.000215231243643815 1.9097812355845e-08
-0.000215231243643424 1.90819742125481e-08
-0.000215231243643067 1.90677209663953e-08
-0.000215231243642733 1.90541454038462e-08
-0.000215231243642398 1.9040569838695e-08
-0.000215231243642074 1.90276741641494e-08
-0.000215231243641796 1.90163611862512e-08
-0.000215231243641517 1.90050482079193e-08
-0.000215231243641238 1.89937352386947e-08
-0.000215231243640964 1.89828759013938e-08
-0.000215231243640741 1.89738255224579e-08
-0.000215231243640518 1.89647751348485e-08
-0.000215231243640295 1.89557247589484e-08
-0.000215231243640072 1.89466743873851e-08
-0.000215231243639855 1.89380776382045e-08
-0.000215231243639687 1.89312898599657e-08
-0.00021523124363952 1.89245020669818e-08
-0.000215231243639353 1.89177142913451e-08
-0.000215231243639185 1.89109264905549e-08
-0.000215231243639018 1.89041387214234e-08
-0.000215231243638851 1.88973509371131e-08
-0.0002152312436387 1.88914692899472e-08
-0.000215231243638588 1.88869441067677e-08
-0.000215231316398067 1.88835526842082e-08
-0.000215231345501989 1.88878540134663e-08
-0.000215231345502101 1.88923792161615e-08
-0.000215231345502212 1.88969043837285e-08
-0.000215231345502324 1.89014295760154e-08
-0.000215231345502436 1.89059547683022e-08
-0.000215231345502547 1.89104799623238e-08
-0.000215231345502659 1.89150051576464e-08
-0.000215231345502742 1.89181716637662e-08
-0.000215231345502798 1.89204342605602e-08
-0.000215231345502854 1.89226968655941e-08
-0.00021523134550291 1.89249594545818e-08
-0.000215231345502966 1.892722204834e-08
-0.000215231345503021 1.89294846525065e-08
-0.000215231345503077 1.89317472367237e-08
-0.000215231345503133 1.89340098322166e-08
-0.000215231345503189 1.893627243248e-08
-0.000215231345503244 1.89385350232024e-08
-0.0002152313455033 1.8940797619129e-08
-0.000215231345503356 1.89430602167903e-08
-0.000215231345503412 1.89453228096811e-08
-0.000215231345503467 1.89475853921636e-08
-0.000215231345503523 1.89498479837534e-08
-0.000215231345503579 1.89521105870526e-08
-0.000215231345503635 1.89543731968569e-08
-0.000215231345503691 1.89566357810741e-08
-0.000215231345503746 1.89588983687608e-08
-0.000215231345503802 1.89611609737947e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
};
\addplot [very thick, learnedWithSideInfo, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131149793862819 0.0251798894630877
0.127079713480388 -0.0384657560357822
0.0964314929822816 -0.0798618436888623
0.0516480359499422 -0.0949027658981009
0.00553842703636739 -0.0860481978599116
-0.031606746285347 -0.0604989647114421
-0.053719416406673 -0.0274854390831402
-0.0593265464883014 0.00419938283610803
-0.0508554526640069 0.0279817796244583
-0.033246874221362 0.040460890989935
-0.0123274789815528 0.0414281310754381
0.0066393416889148 0.0331940344594058
0.0199633071796267 0.0195517184185674
0.0259837328018577 0.00464320450771843
0.0249888576792304 -0.00801484152737757
0.0187293909113336 -0.0161606021812968
0.00971891275217588 -0.019007690925516
0.000520039343851662 -0.0170957723730465
-0.0068245326659511 -0.0118829908425522
-0.0111229755111629 -0.00522660268350669
-0.0121072515843716 0.00110917678656049
-0.010288884195878 0.00581667798816187
-0.00667683742574954 0.00822883776394565
-0.00244920834228438 0.00832348102766172
0.00133977928677175 0.00658688903553811
0.00396182006094005 0.00379710165932729
0.00510164858488995 0.000791218260223542
0.00483537612227606 -0.00172951045983905
0.00352843350678454 -0.00332262668509965
0.00169281404325028 -0.00384428945323493
-0.000156418956593954 -0.00341533560390299
-0.00161390869350208 -0.00233708075480329
-0.00244822986750354 -0.000986208376250961
-0.00261418268362241 0.000283712219537526
-0.00222187690491308 0.00121410153612611
-0.00147878700916618 0.00167682662287149
-0.000623316353285681 0.00167352064775666
0.00013383185101254 0.00130683402426651
0.000649427640636766 0.000736019151823982
0.000864121347817304 0.000129913288718758
0.00079701250717097 -0.000371888144283653
0.00052433882650533 -0.000683012829999892
0.000150391925739179 -0.000777469280886314
-0.000221312105831801 -0.000682096126094751
-0.000510387727195085 -0.000459169162630055
-0.000672011763291136 -0.000185095195134658
-0.000698897074524392 6.93050979605619e-05
-0.000614666666690934 0.000252983786311476
-0.000461951996699116 0.000341446809417116
-0.000288959917135747 0.000336273613475838
-0.000137764801122169 0.000259070980219505
-3.64957419971436e-05 0.000142391092693976
3.73362503466855e-06 2.02555995046263e-05
-1.24786168268952e-05 -7.95681153136682e-05
-6.92595456052979e-05 -0.0001402404958678
-0.00014538117678386 -0.000157124146981403
-0.000220050650834887 -0.000136123338275941
-0.000277338909465173 -9.00940842311539e-05
-0.000308583238473477 -3.4526020956928e-05
-0.000312682114468445 1.64039507583483e-05
-0.000294681570595058 5.26291609443388e-05
-0.000263331671658189 6.94842402658592e-05
-0.000228373539062655 6.75387491605641e-05
-0.000198202588091343 5.13282374689297e-05
-0.000178336165763999 2.749997465458e-05
-0.000170842923145647 2.90472376487678e-06
-0.000174646766736495 -1.69383711729029e-05
-0.000186449063288958 -2.87513089009964e-05
-0.000201932441101887 -3.17202972210393e-05
-0.000216922725407938 -2.71337706090153e-05
-0.000228266262302799 -1.76423498525506e-05
-0.000234292603868267 -6.3840174507699e-06
-0.000234853628709088 3.80517475729496e-06
-0.000231022651191858 1.09421320070267e-05
-0.000224594001852564 1.41416586497984e-05
-0.000217534550147661 1.35688525419379e-05
-0.000211518167694891 1.01734529797076e-05
-0.000207625789470555 5.311615699674e-06
-0.000206239728321189 3.61917678971379e-07
-0.000207113443824903 -3.57945668460818e-06
-0.000209562415325938 -5.87550411473067e-06
-0.000212709486206425 -6.38651718923083e-06
-0.000215716939701654 -5.39169095783044e-06
-0.000217960980079845 -3.43695582264575e-06
-0.000219120430933258 -1.15756871900538e-06
-0.000219180216989507 8.7951010586864e-07
-0.000218367891362984 2.28405906108758e-06
-0.000217050885658263 2.88883614177338e-06
-0.000215626002450794 2.73711353333079e-06
-0.000214427314875068 2.02744115476629e-06
-0.000213665817934439 1.03629167916329e-06
-0.000213411716913433 4.08682835190653e-08
-0.000213609094207463 -7.41300769895818e-07
-0.0002141164937512 -1.18671019335532e-06
-0.0002147553932785 -1.27213003384228e-06
-0.00021535828425309 -1.05775526386973e-06
-0.000215801996524917 -6.55692807475464e-07
-0.000216024579424923 -1.94508441041241e-07
-0.00021602597193915 2.12512216555064e-07
-0.000215854324440911 4.88689956326758e-07
-0.000215584636697145 6.02485588750354e-07
-0.000215297075449333 5.64593909698971e-07
-0.000215058260371489 4.16448990887483e-07
-0.000214909651254794 2.14458860599374e-07
-0.000214863822333423 1.44632344304188e-08
-0.000214907823471428 -1.4056004768578e-07
-0.00021501281337319 -2.26730058491831e-07
-0.000215142572425255 -2.40312605565875e-07
-0.000215263339874149 -1.94243309068441e-07
-0.000215350828008923 -1.11605676150414e-07
-0.00021539316182574 -1.84227250624863e-08
-0.000215391126567295 6.2679731478027e-08
-0.000215355359312562 1.16853663938675e-07
-0.000215300601003123 1.38284001944145e-07
-0.000215242931561895 1.29452933607041e-07
-0.000215195593439501 9.89108569701691e-08
-0.000215166634125704 5.80856137355479e-08
-0.000215157712811055 1.79865880288801e-08
-0.000215166792435976 -1.29925320272416e-08
-0.00021518803780236 -3.00833022334225e-08
-0.000215214027452233 -3.26186715112267e-08
-0.00021523830027182 -2.32375580535606e-08
-0.00021525577752985 -6.55875979395371e-09
-0.000215264188998446 1.2178692462058e-08
-0.000215263650980571 2.84399928641987e-08
-0.000215256273428761 3.92165285323723e-08
-0.000215245155871621 4.33627178556689e-08
-0.00021523363071158 4.14776301750977e-08
-0.000215224084503681 3.52440471286519e-08
-0.000215218278086007 2.69578619861016e-08
-0.000215216662623878 1.88829955712587e-08
-0.000215218685187239 1.27371384676424e-08
-0.000215223094334265 9.42931500805613e-09
-0.000215228187493228 9.03319081644802e-09
-0.00021523306243127 1.09679240585525e-08
-0.000215236598629767 1.43657694533575e-08
-0.000215238243089696 1.81608163919537e-08
-0.000215238126755661 2.14408149381597e-08
-0.000215236598858703 2.36077951042135e-08
-0.000215234416092284 2.44228699321572e-08
-0.000215232233297374 2.40881230617433e-08
-0.000215230225103563 2.28723536703328e-08
-0.000215229017253716 2.12070589405283e-08
-0.000215228638863148 1.95565156716274e-08
-0.000215229017181098 1.82757123948218e-08
-0.000215229744758993 1.75635040088051e-08
-0.000215230938011631 1.73999855587227e-08
-0.000215231767479866 1.77762907796475e-08
-0.000215232495090774 1.83967183787007e-08
-0.000215232946219363 1.91779975572057e-08
-0.000215232946235867 1.98440887298756e-08
-0.000215232902593063 2.03660547289444e-08
-0.000215232175002959 2.05854822524047e-08
-0.000215231447403646 2.04331743781927e-08
-0.000215231243668183 2.00813377983569e-08
-0.000215231243661077 1.97944474648187e-08
-0.0002152312436555 1.95693248532941e-08
-0.000215231243651149 1.9393751968938e-08
-0.000215231243647741 1.92561895500168e-08
-0.000215231243645075 1.91487196364061e-08
-0.000215231243643067 1.90677209663953e-08
-0.000215231243641517 1.90050482079193e-08
-0.000215231243640295 1.89557247589484e-08
-0.000215231243639353 1.89177142913451e-08
-0.000215231243638588 1.88869441067677e-08
-0.000215231345502324 1.89014295760154e-08
-0.000215231345502798 1.89204342605602e-08
-0.000215231345503077 1.89317472367237e-08
-0.000215231345503356 1.89430602167903e-08
-0.000215231345503635 1.89543731968569e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
-0.000215231345503847 1.89627436778146e-08
};
\addplot [very thick, learnedWithoutSideInfo]
table {%
0.1 0.1
0.110528937592068 0.085814668633768
0.118757063755375 0.0719702195829355
0.124373557393049 0.0583896530283852
0.127540635484157 0.0451906863007243
0.12866906678805 0.0324749159339917
0.128216429950769 0.0202642315567612
0.126583025719139 0.00851683978964457
0.124089396717833 -0.00283744782748729
0.120992018291295 -0.0138706682529138
0.117506764712516 -0.0246438766936462
0.113826251888789 -0.0352043371740958
0.110126685141525 -0.0455869215273143
0.106564141479216 -0.0558132686788033
0.103261922043203 -0.0658821986151366
0.100291422784458 -0.075746916287969
0.0976509053414063 -0.0852817769680503
0.0952516512735273 -0.0942564276434542
0.0929267887565224 -0.102351432058039
0.0904728494030635 -0.109241066874457
0.0877090445904045 -0.11471441502327
0.0845164256254687 -0.118751311330082
0.0808340286523173 -0.121498939084112
0.0766270176472754 -0.123182568146336
0.0718556902326595 -0.124019763577484
0.0664598328270563 -0.124173181961695
0.060358089175683 -0.123737530138009
0.0534585525095248 -0.122744255532808
0.0456791246437254 -0.121172622017855
0.0369774935891158 -0.118963230621843
0.0273876060958682 -0.116034079061366
0.0170523393624147 -0.112299218255718
0.00623579865050772 -0.10768715698664
-0.00469743973984471 -0.102153823281922
-0.0153316358411657 -0.0956874480608353
-0.0252561472797512 -0.0883099127314873
-0.0341079591010716 -0.0800836775961026
-0.0415967488661586 -0.0711287034321736
-0.0475218716000279 -0.0616418277865352
-0.0517877495497951 -0.0519014687201991
-0.0544123972229404 -0.0422434756133916
-0.0555185762818224 -0.0330110054247912
-0.0553049930247296 -0.0244994868414431
-0.0540074816636631 -0.0169200821837051
-0.0518645825136002 -0.0103906993483485
-0.0490961249932824 -0.00494777411829755
-0.045894866540785 -0.000566417278452913
-0.0424263999347447 0.00282015929755774
-0.0388321673588194 0.0053054681539797
-0.0352322782951453 0.00699870248006462
-0.0317269259476762 0.00801648582528469
-0.0283966332120755 0.00847629513875858
-0.0253021733317591 0.00849106838846297
-0.0224849793842794 0.00816498007702315
-0.0199684803162072 0.00759051808762123
-0.017760369436258 0.00684690462667892
-0.0158555121890718 0.00599972976946833
-0.0142390905651264 0.00510152958406485
-0.0128896221906083 0.00419298957379777
-0.0117816077356618 0.00330447821408819
-0.0108876861190073 0.0024576809218842
-0.0101802769042187 0.00166718008423083
-0.00963275262965002 0.000941892339297312
-0.00922021484608893 0.000286322735483457
-0.00891995599520712 -0.000298373092956605
-0.00871168438647496 -0.000813509448417071
-0.00857757847105489 -0.00126215556734327
-0.00850222380744636 -0.00164856364069255
-0.00847247396090278 -0.00197771838153948
-0.00847726612699651 -0.0022549882348204
-0.00850741379585029 -0.00248586054307309
-0.00855539216467349 -0.00267574533687609
-0.0086151269921344 -0.00282983465986586
-0.0086817938627215 -0.00295300636274604
-0.00875163211010088 -0.00304976308079602
-0.00882177569679232 -0.00312419865284319
-0.00889010197227957 -0.00317998556797933
-0.00895509828459051 -0.00322037816419601
-0.00901574578836684 -0.00324822727475838
-0.00907141939045486 -0.00326600284476197
-0.00912180253841477 -0.00327582174048013
-0.00916681544090325 -0.00327947856419475
-0.00920655527632697 -0.00327847778125501
-0.00924124697158435 -0.00327406587651591
-0.00927120319699792 -0.00326726259550136
-0.00929679231229796 -0.00325889060116391
-0.00931841310177983 -0.0032496030992516
-0.00933647524672043 -0.00323990916151407
-0.00935138459449902 -0.0032301966138869
-0.00936353239308163 -0.00322075246215703
-0.00937328776354862 -0.00321178090618146
-0.00938099278094828 -0.00320341905029076
-0.00938695962366021 -0.00319575045611764
-0.00939146933307144 -0.00318881670835369
-0.00939477179883452 -0.00318262717706153
-0.00939708665019934 -0.00317716716440641
-0.00939860479109988 -0.00317240462145552
-0.00939949036664256 -0.00316829561366494
-0.00939988299153649 -0.00316478870335135
-0.00939990010763436 -0.00316182840483947
-0.0093996393686826 -0.00315935785425603
-0.00939918097606851 -0.00315732082168391
-0.00939858991079134 -0.00315566317901561
-0.00939791802396872 -0.00315433392316622
-0.00939720596230176 -0.00315328584107155
-0.00939648491570422 -0.00315247589079481
-0.00939577818285775 -0.00315186536183609
-0.00939510255684173 -0.00315141986770817
-0.00939446953758516 -0.00315110921482786
-0.00939388638124417 -0.00315090718384803
-0.0093933569985607 -0.00315079125267381
-0.0093928827156593 -0.00315074228446344
-0.00939246291106155 -0.00315074419880973
-0.00939209554281906 -0.00315078364006116
-0.00939177757912102 -0.00315084965317014
-0.0093915053451088 -0.00315093337452443
-0.00939127479775159 -0.00315102774280668
-0.00939108173954573 -0.00315112723308458
-0.00939092198086389 -0.00315122761573944
-0.00939079145963051 -0.00315132574080079
-0.00939068632600604 -0.00315141934725438
-0.00939060299877914 -0.00315150689637411
-0.00939053819921565 -0.00315158742763783
-0.0093904889672447 -0.00315166043551207
-0.00939045266419303 -0.00315172576519362
-0.00939042696543035 -0.00315178352544848
-0.00939040984584194 -0.0031518340165424
-0.00939039956037258 -0.00315187767147024
-0.00939039462152991 -0.00315191500868472
-0.00939039377527262 -0.00315194659468176
-0.00939039597644431 -0.00315197301499293
-0.00939040036452488 -0.00315199485219225
-0.00939040624039311 -0.00315201266974741
-0.00939041304442867 -0.00315202700063166
-0.00939042033632242 -0.00315203833982036
-0.00939042777668186 -0.00315204713983142
-0.00939043511051718 -0.00315205380867772
-0.00939044215257478 -0.00315205870965163
-0.00939044877451067 -0.00315206216244551
-0.00939045489373314 -0.00315206444527455
-0.00939046046384728 -0.00315206579762084
-0.00939046546653444 -0.00315206642340415
-0.00939046990475534 -0.00315206649435906
-0.00939047379709779 -0.00315206615344654
-0.00939047717314967 -0.00315206551822939
-0.00939048006977261 -0.00315206468409346
-0.00939048252811547 -0.00315206372726662
-0.00939048459130909 -0.00315206270761925
-0.00939048630269435 -0.00315206167120519
-0.00939048770450368 -0.00315206065251594
-0.00939048883692228 -0.00315205967651977
-0.00939048973746459 -0.00315205876041519
-0.00939049044057283 -0.00315205791516293
-0.00939049097742473 -0.00315205714680616
-0.00939049137587755 -0.00315205645757
-0.00939049166052808 -0.00315205584679734
-0.00939049185285734 -0.00315205531173068
-0.00939049197140696 -0.00315205484812264
-0.00939049203201359 -0.00315205445076838
-0.00939049204806386 -0.00315205411389563
-0.00939049203073905 -0.00315205383148132
-0.00939049198926556 -0.00315205359750015
-0.00939049193116226 -0.00315205340608904
-0.00939049186245855 -0.00315205325168127
-0.00939049178792661 -0.00315205312908962
-0.00939049171125372 -0.00315205303356481
-0.00939049163523009 -0.00315205296080523
-0.00939049156189276 -0.00315205290697385
-0.00939049149266857 -0.00315205286868714
-0.00939049142850035 -0.00315205284299336
-0.00939049136992542 -0.00315205282734887
-0.00939049131718228 -0.00315205281958192
-0.00939049127028113 -0.00315205281785769
-0.00939049122906122 -0.00315205282064868
-0.00939049119322855 -0.00315205282669151
-0.00939049116242163 -0.00315205283496306
-0.00939049113621948 -0.0031520528446366
-0.00939049111418067 -0.00315205285506831
-0.00939049109585666 -0.00315205286575293
-0.00939049108080914 -0.00315205287631881
-0.00939049106861711 -0.00315205288648718
-0.009390491058892 -0.00315205289606568
-0.00939049105126921 -0.00315205290493414
-0.00939049104542189 -0.00315205291301601
-0.00939049104105427 -0.00315205292028597
-0.00939049103790524 -0.00315205292674225
-0.00939049103575185 -0.0031520529324095
-0.00939049103439338 -0.0031520529373294
-0.00939049103366596 -0.00315205294155518
-0.00939049103341905 -0.00315205294514526
-0.00939049103353717 -0.00315205294816268
-0.00939049103392398 -0.00315205295066789
-0.00939049103449374 -0.00315205295272536
-0.00939049103518474 -0.00315205295438636
-0.00939049103594414 -0.00315205295571203
-0.00939049103673373 -0.0031520529567497
-0.00939049103751932 -0.00315205295754317
-0.00939049103828404 -0.00315205295813181
-0.00939049103900658 -0.00315205295855514
-0.00939049103967449 -0.00315205295884369
-0.00939049104028866 -0.00315205295902521
-0.00939049104084422 -0.00315205295912235
-0.0093904910413416 -0.00315205295915244
-0.00939049104177858 -0.00315205295912979
-0.00939049104215961 -0.00315205295907212
-0.00939049104248735 -0.00315205295899079
-0.00939049104276757 -0.00315205295889337
-0.00939049104300338 -0.00315205295878696
-0.00939049104320144 -0.00315205295867577
-0.00939049104336398 -0.00315205295856824
-0.00939049104349721 -0.00315205295846288
-0.00939049104360068 -0.00315205295836196
-0.00939049104368639 -0.00315205295826815
-0.00939049104374723 -0.00315205295818255
-0.00939049104379164 -0.00315205295810617
-0.0093904910438285 -0.003152052958038
-0.00939049104385292 -0.00315205295797849
-0.00939049104386891 -0.00315205295792675
-0.00939049104387735 -0.00315205295787974
-0.00939049104387912 -0.00315205295784188
-0.00939049104387912 -0.00315205295781096
-0.00939049104387379 -0.0031520529577862
-0.00939049104386891 -0.003152052957763
-0.00939049104386314 -0.00315205295774357
-0.00939049104385292 -0.00315205295772691
-0.00939049104384315 -0.00315205295771465
-0.00939049104383471 -0.0031520529577086
-0.0093904910438245 -0.00315205295770093
-0.00939049104381517 -0.00315205295770044
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
-0.00939049104381251 -0.00315205295770027
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295769994
};
\addplot [very thick, learnedWithoutSideInfo, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.12866906678805 0.0324749159339917
0.117506764712516 -0.0246438766936462
0.100291422784458 -0.075746916287969
0.0877090445904045 -0.11471441502327
0.0664598328270563 -0.124173181961695
0.0273876060958682 -0.116034079061366
-0.0252561472797512 -0.0883099127314873
-0.0544123972229404 -0.0422434756133916
-0.0490961249932824 -0.00494777411829755
-0.0317269259476762 0.00801648582528469
-0.017760369436258 0.00684690462667892
-0.0108876861190073 0.0024576809218842
-0.00871168438647496 -0.000813509448417071
-0.00850741379585029 -0.00248586054307309
-0.00882177569679232 -0.00312419865284319
-0.00912180253841477 -0.00327582174048013
-0.00929679231229796 -0.00325889060116391
-0.00937328776354862 -0.00321178090618146
-0.00939708665019934 -0.00317716716440641
-0.0093996393686826 -0.00315935785425603
-0.00939648491570422 -0.00315247589079481
-0.0093933569985607 -0.00315079125267381
-0.0093915053451088 -0.00315093337452443
-0.00939068632600604 -0.00315141934725438
-0.00939042696543035 -0.00315178352544848
-0.00939039597644431 -0.00315197301499293
-0.00939042777668186 -0.00315204713983142
-0.00939046046384728 -0.00315206579762084
-0.00939048006977261 -0.00315206468409346
-0.00939048883692228 -0.00315205967651977
-0.00939049166052808 -0.00315205584679734
-0.00939049203073905 -0.00315205383148132
-0.00939049171125372 -0.00315205303356481
-0.00939049136992542 -0.00315205282734887
-0.00939049116242163 -0.00315205283496306
-0.00939049106861711 -0.00315205288648718
-0.00939049103790524 -0.00315205292674225
-0.00939049103353717 -0.00315205294816268
-0.00939049103673373 -0.0031520529567497
-0.00939049104028866 -0.00315205295902521
-0.00939049104248735 -0.00315205295899079
-0.00939049104349721 -0.00315205295846288
-0.0093904910438285 -0.003152052958038
-0.00939049104387912 -0.00315205295781096
-0.00939049104384315 -0.00315205295771465
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
-0.00939049104381295 -0.0031520529576996
-0.00939049104381251 -0.00315205295770027
-0.00939049104381251 -0.00315205295769994
};

==> figures/smd_phase_plots/phase_plot_50_quarter_space_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.0839808732271194 0.0994482040405273
0.0931303426623344 0.0318382531404495
0.0737497732043266 0.135778144001961
0.0458933636546135 0.0842315405607224
0.00452368799597025 0.141100496053696
0.11861914396286 0.0279434863477945
0.143821910023689 0.0297047011554241
0.128507524728775 0.0073636188171804
0.0141577236354351 0.0699533894658089
0.111160345375538 0.0721027925610542
0.0128282625228167 0.116179049015045
0.113642059266567 0.0935259386897087
0.114054314792156 0.00375913036987185
0.0925949066877365 0.0140911275520921
0.107372470200062 0.102853260934353
0.027069415897131 0.121641263365746
0.0358744785189629 0.105421125888824
0.143693581223488 0.07585559040308
0.094265453517437 0.0191213749349117
0.0937533229589462 0.134498134255409
0.133748769760132 0.0891022905707359
0.0770444869995117 0.100217506289482
0.12509161233902 0.134705662727356
0.11181528866291 0.0236758980900049
0.130204707384109 0.0313761942088604
0.0149289695546031 0.0569891221821308
0.0771197602152824 0.0575646832585335
0.127108171582222 0.0588883496820927
0.0504734292626381 0.0226166192442179
0.0276358257979155 0.0366135202348232
0.0565454661846161 0.114331558346748
0.0376495867967606 0.0898406207561493
0.0801086500287056 0.024379700422287
0.0171181075274944 0.117518477141857
0.00829808600246906 0.10522399097681
0.109610736370087 0.144716173410416
0.0895901098847389 0.0249913204461336
0.148184910416603 0.0565091483294964
0.0753039568662643 0.0375259220600128
0.132507354021072 0.0936597362160683
0.0445524007081985 0.00343917869031429
0.0750662982463837 0.0588645227253437
0.0656018257141113 0.102072231471539
0.0221610851585865 0.109879910945892
0.0265114456415176 0.131856635212898
0.126123011112213 0.0447592101991177
0.0665029287338257 0.0892286002635956
0.0387716293334961 0.0300013031810522
0.107425525784492 0.0961355566978455
0.0143502093851566 0.13919261097908
};
\addplot [very thick, trueDynamics]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, dashed, approxDynamics]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, learnedWithSideInfo]
table {%
0.1 0.1
0.109246748678297 0.0849078796512185
0.116978784410934 0.0697313504910003
0.123195182789942 0.0546198145258256
0.127909574276365 0.039713058140546
0.131148956024502 0.0251408339982642
0.132952864801913 0.0110222723172743
0.133372140206764 -0.00253461612184543
0.132467889092112 -0.0154332445393096
0.130310323340097 -0.0275885691132225
0.12697753801571 -0.0389269776754077
0.122554386351484 -0.0493860548060394
0.117131511164947 -0.0589142372985831
0.110804130382256 -0.0674704014762624
0.103671060966292 -0.0750235178247852
0.0958337800877768 -0.08155220449639
0.0873953894411869 -0.0870444325276335
0.0784597807270962 -0.0914970851659502
0.0691306819348083 -0.0949156751409987
0.0595108787201517 -0.0973139560956825
0.0497013799085425 -0.0987134584539713
0.0398006873144798 -0.0991431130008172
0.0299040487998712 -0.0986387920103444
0.0201027914264482 -0.09724276100017
0.0104837244586616 -0.0950031005852733
0.00112859510261184 -0.0919732105084418
-0.00788644620891766 -0.0882111648722856
-0.016491256319674 -0.0837790831787954
-0.0246220823742289 -0.078742597468423
-0.0322218914088985 -0.0731702155932104
-0.0392406084376555 -0.0671326915839112
-0.0456353185586889 -0.0607024878576318
-0.0513704439139048 -0.0539532148659736
-0.0564177604532252 -0.0469590021614969
-0.0607564985142212 -0.0397939692859427
-0.0643732496817204 -0.0325316285619028
-0.0672619071722384 -0.025244240684806
-0.0694235056319963 -0.0180022756800371
-0.0708660460348033 -0.0108737640778257
-0.0716041305897941 -0.00392369728468368
-0.0716587168623352 0.00278659300004023
-0.0710566409296227 0.00920001066814519
-0.0698302746522874 0.0152642493028765
-0.06801692963125 0.0209323071494184
-0.0656583133242816 0.026162924377978
-0.0628000224201014 0.0309209379467193
-0.0594907791721904 0.0351775724264358
-0.0557818987030552 0.0389105841069027
-0.0517265774961605 0.0421043386479463
-0.0473792601189732 0.0447497601825208
-0.0427949537901539 0.0468441987971195
-0.0380286323495037 0.0483911367723739
-0.0331346364981834 0.0493998658796646
-0.0281660926611607 0.04988507608323
-0.0231744082104142 0.0498663786977297
-0.0182088076607452 0.0493677412298153
-0.0133159293971333 0.048416990140884
-0.00853944940531206 0.0470452177661594
-0.00391979999315509 0.0452862123979901
0.000506077902714682 0.0431759406439026
0.00470492455444584 0.0407519781467863
0.00864729918395481 0.0380530333149882
0.0123076662474562 0.0351184373598169
0.0156644417291663 0.0319877680247789
0.0186999862330156 0.028700378294233
0.0214005756602114 0.0252950676948873
0.0237563239231964 0.0218097274268114
0.0257610684037936 0.0182810426550497
0.0274122526164301 0.0147442132337082
0.0287107511266692 0.0112327157947603
0.0296606870183893 0.00777810665250687
0.030269247496878 0.00440982580842111
0.0305464417484334 0.00115506188373554
0.0305048774255947 -0.00196137590055438
0.0301595240926165 -0.00491715083820646
0.0295274617688885 -0.00769246572178202
0.0286276201580785 -0.0102701074506197
0.0274805216017462 -0.0126354631598988
0.0261080128563475 -0.0147765213572665
0.0245330154957108 -0.0166838394871802
0.022779268863052 -0.0183505217079844
0.0208710879224186 -0.0197721192414158
0.0188330968966116 -0.020946596666382
0.0166900076075219 -0.0218742080817294
0.0144664108550512 -0.0225574123665311
0.0121865305430108 -0.0230007456206017
0.00987404951650589 -0.0232106880864667
0.0075519037347531 -0.0231955272667846
0.00524211928487999 -0.0229652247406028
0.00296565009390448 -0.022531242066954
0.000742233569227232 -0.0219063907966709
-0.00140973303858485 -0.0211046656523853
-0.00347330556306724 -0.0201410796283279
-0.00543308466083492 -0.0190314821906951
-0.00727528938938243 -0.017792405344665
-0.00898782030788926 -0.0164408781169257
-0.0105602978969718 -0.0149942585353814
-0.011984089336714 -0.0134700823369586
-0.0132523154948755 -0.0118858661978962
-0.0143598425465498 -0.0102589758118969
-0.0153032605562925 -0.00860646063712395
-0.0160808387763088 -0.00694491733802859
-0.0166924837390137 -0.00529034445894617
-0.0171396563709385 -0.00365801493130141
-0.017425316115093 -0.00206236443194869
-0.0175538082423517 -0.000516882705595792
-0.0175307800340219 0.000965979478546101
-0.0173630746123605 0.00237488923142629
-0.0170586061446089 0.00369969625415589
-0.0166262369095741 0.0049314875577066
-0.0160756636772411 0.00606262243160363
-0.0154172798738499 0.00708675719927847
-0.0146620489224949 0.00799884792394213
-0.0138213738585263 0.0087951558909148
-0.0129069660129583 0.00947321550473128
-0.0119307183526514 0.0100318203150544
-0.010904589064277 0.0104709598346983
-0.00984047489394302 0.0107917861177686
-0.00875010683768729 0.0109965311517296
-0.00764493698478303 0.0110884483878045
-0.00653604584939902 0.0110717283419152
-0.00543405203053174 0.0109514197897686
-0.00434902978786368 0.0107333277413871
-0.00329043849190414 0.0104239309888223
-0.00226706045599777 0.01003028569063
-0.00128694726617611 0.0095599234629908
-0.000357377694930247 0.00902076797765587
0.000515177400847106 0.00842102097581513
0.00132507766674737 0.00776908449829969
0.00206752896919811 0.00707347100245225
0.0027385903246951 0.00634270700686301
0.003335171981031 0.00558525806866026
0.00385502179873081 0.00480944955904372
0.00429671163241483 0.00402339580618332
0.00465961102262796 0.00323493291067163
0.00494385902487263 0.0024515575843572
0.00515032067154429 0.00168037676082483
0.00528055344559724 0.000928055345940087
0.00533675745564245 0.000200777751867166
0.00532172374831673 -0.00049578773323556
0.00523878588006754 -0.00115651689090926
0.00509175798458166 -0.00177685193659794
0.00488488541289976 -0.00235281729620199
0.00462277814383665 -0.00288102844283948
0.0043103563015593 -0.00335869799015325
0.00395278961932847 -0.00378363214170617
0.00355543480760089 -0.00415422333126679
0.00312378363236416 -0.0044694416939813
0.00266340098158826 -0.00472881632615687
0.00217987271030864 -0.00493241170643152
0.00167875197254428 -0.00508080965807065
0.00116550869613252 -0.00517507600378763
0.000645483597795608 -0.0052167337329541
0.0001238439880331 -0.00520772314232486
-0.00039445661143007 -0.00515037129927004
-0.000904714935681462 -0.00504735125080167
-0.00140251101045655 -0.00490164263960043
-0.00188373564176721 -0.00471649047203322
-0.00234461700310627 -0.00449536710496324
-0.00278173844809603 -0.00424192403778586
-0.00319205818547836 -0.00395995668247939
-0.00357291626505327 -0.00365336009692429
-0.00392204831546562 -0.00332608932694335
-0.00423758507949738 -0.0029821197831879
-0.00451805451023812 -0.002625408963354
-0.00476237851228809 -0.00225986076297363
-0.00496986549180008 -0.00188929218900657
-0.00514020057831013 -0.00151739985954091
-0.00527342839582313 -0.00114773124362203
-0.00536994142184466 -0.000783657765801254
-0.00543045996440582 -0.000428350683829345
-0.00545600981074902 -8.47601392898467e-05
-0.00544790080726603 0.000244403550311922
-0.00540769985144195 0.000556684864167624
-0.00533720760902403 0.000849895502776885
-0.00523842824619986 0.00112212302161417
-0.0051135438183376 0.00137173710295825
-0.00496488586467519 0.00159739202461436
-0.00479490700300087 0.00179802881020972
-0.00460614786757787 0.00197286972472612
-0.00440121755127994 0.00212141643034028
-0.00418275635247226 0.00224344036767778
-0.00395341901095098 0.00233897198031635
-0.0037158432755557 0.0024082920342316
-0.00347262499096553 0.00245191608347761
-0.00322630040212874 0.0024705780277655
-0.00297931891272802 0.00246521388450431
-0.00273402934774566 0.00243694534334937
-0.00249265899824361 0.00238706006818046
-0.00225729871973156 0.00231699176789172
-0.00202988966030194 0.00222829957818128
-0.00181221220070397 0.00212264766652223
-0.00160587547647055 0.00200178577317721
-0.00141231015972017 0.00186752857883419
-0.00123276298706574 0.00172173463107783
-0.00106829349960576 0.00156628860869044
-0.000919772296188879 0.00140307988573593
-0.000787881906118659 0.00123398666451948
-0.00067311772009512 0.00106085858928805
-0.000575792704636061 0.000885499887413754
-0.000496042174759665 0.000709654537137793
-0.000433830545770118 0.000534992998400334
-0.000388959482065318 0.00036310004198415
-0.000361076860856358 0.000195463203480396
-0.000349687016522037 3.34637087195007e-05
-0.000354162061830499 -0.000121631820070124
-0.000373753150986401 -0.000268678089475722
-0.000407603372532195 -0.000406656405557404
-0.000454760496770575 -0.000534678246335872
-0.000514189897829482 -0.000651988125138153
-0.000584788261572234 -0.000757964574152674
-0.000665396653263477 -0.000852119367933321
-0.000754814080001606 -0.000934097125504898
-0.000851810442024023 -0.00100367201273078
-0.000955139571331383 -0.00106074450437569
-0.00106355098979429 -0.00110533553699958
-0.00117580277316583 -0.00113758263298688
-0.00129067197044174 -0.00115773272057928
-0.00140696554710492 -0.00116613460775097
-0.00152352981494478 -0.00116323168371543
-0.00163926021115995 -0.00114955311449614
-0.001753109098408 -0.00112570573850112
-0.00186409263351711 -0.00109236491124279
-0.00197129821831335 -0.00105026407729507
-0.00207388729379368 -0.00100018666226535
-0.00217110442074703 -0.000942956455536594
-0.00226227646508275 -0.00087942700536999
-0.00234681643973251 -0.000810473450883835
-0.00242422746299083 -0.000736982903486301
-0.00249409926624985 -0.000659845754572139
-0.00255611215231593 -0.000579946925303448
-0.00261003373595393 -0.000498158159598322
-0.00265571684857268 -0.000415330460256971
-0.00269310046971677 -0.000332286817716783
-0.00272220134529571 -0.000249815498920426
-0.00274311538468592 -0.000168664803117113
-0.00275600951177668 -8.95373229320511e-05
-0.00276112003524966 -1.30855857428526e-05
-0.00275874403392149 6.0092012036148e-05
-0.00274923609717727 0.00012945428659653
-0.00273300390123962 0.000194519830405421
-0.0027104974989892 0.000254869073551034
-0.00268220722450682 0.000310145250644051
-0.00264865531116978 0.000360055077661149
-0.00261039100220095 0.000404368724360883
-0.00256798170307848 0.000442919164718265
-0.00252201065318999 0.000475600816933681
-0.00247306668123392 0.000502367923779241
-0.00242174187685553 0.00052323229404915
-0.00236862320867833 0.000538260696339801
-0.00231428879892006 0.000547571589113576
-0.00225930256822334 0.000551332223256492
-0.00220420888043947 0.000549754240607993
-0.00214952951573697 0.000543089850891065
-0.00209575901389524 0.000531628066934714
-0.00204336071605884 0.000515689781982326
-0.00199276629899486 0.000495623711424411
-0.00194436925570811 0.000471802052612508
-0.00189852605949422 0.000444615382558696
-0.00185555302061197 0.000414468489795412
-0.00181572523845253 0.000381776027360933
-0.00177927636860263 0.000346958022900755
-0.00174639850632657 0.000310435562726666
-0.0017172402074238 0.000272627257505122
-0.00169190974776185 0.000233944750349699
-0.00167047442471374 0.000194789907848803
-0.0016529621868886 0.000155550922341396
-0.00163936256539293 0.000116599515632585
-0.00162962888565821 7.8288143142982e-05
-0.00162368059569947 4.09476169167923e-05
-0.00162140489587981 4.88482730881751e-06
-0.00162265988209101 -2.96189202679442e-05
-0.00162727640836721 -6.23094743312023e-05
-0.00163506169573897 -9.29610155192967e-05
-0.00164580177694068 -0.000121376923229519
-0.00165926487245135 -0.000147390164204409
-0.00167520336954888 -0.000170863796991085
-0.00169335754761149 -0.000191690723181481
-0.00171345895417909 -0.000209793327038812
-0.00173523180194447 -0.000225123164118629
-0.00175839809106696 -0.000237659761384546
-0.00178267854051204 -0.000247409907587432
-0.00180779608055457 -0.000254406090385192
-0.00183347794828767 -0.000258705091436911
-0.00185945836521762 -0.000260386568831148
-0.00188547970146019 -0.000259551144852351
-0.00191129655032468 -0.000256318552918207
-0.00193667584477847 -0.00025082569745358
-0.00196139918580225 -0.000243224611850377
-0.00198526365734689 -0.000233680300134472
-0.00200808415469323 -0.000222368637629608
-0.00202969256959447 -0.000209474227194346
-0.00204994058429013 -0.000195188312975775
-0.00206869827457335 -0.00017970678249374
-0.00208585667097755 -0.000163227877331517
-0.0021013256633404 -0.000145950483963522
-0.00211503446650776 -0.000128072206859369
-0.0021269337158587 -0.000109787370178617
-0.00213699244053753 -9.12855176953458e-05
-0.00214519759782455 -7.27498221176856e-05
-0.00215155500449561 -5.43556372918372e-05
-0.0021560867757104 -3.62691917670972e-05
-0.00215883202353113 -1.86464222535856e-05
-0.002159843830141 -1.6320078909623e-06
-0.00215919087768036 1.46415230829577e-05
-0.00215695232598285 3.00544834376843e-05
-0.00215322060655721 4.45005939197179e-05
-0.00214809560182027 5.78873286436509e-05
-0.00214168906889488 7.01362302268581e-05
-0.00213411672335455 8.11830180709621e-05
-0.0021255026630144 9.09775538337977e-05
-0.00211597284865633 9.9483619285589e-05
-0.00210565766516493 0.000106678727352804
-0.00209468912754636 0.000112553688266524
-0.0020831985526047 0.000117112067319269
-0.00207131842158108 0.000120369764043498
-0.00205917586086127 0.00012235400780146
-0.00204689729858386 0.000123102849343094
-0.00203460334233794 0.000122664235163816
-0.00202241110745119 0.000121095094388362
-0.00201042839619432 0.000118460442472299
-0.00199875998419337 0.000114832307336125
-0.00198750063548198 0.000110288963843293
-0.00197673789644332 0.000104913687468719
-0.00196655046597898 9.87939354380823e-05
-0.00195700889396966 9.20201960957151e-05
-0.00194817313653087 8.46850984925216e-05
-0.00194009511713483 7.68824040109496e-05
-0.00193281709676738 6.87061099029843e-05
-0.00192637120824745 6.0249485411769e-05
-0.00192078120244159 5.16043326765836e-05
-0.00191606151691945 4.28601034525937e-05
-0.00191221762518513 3.41032108148297e-05
-0.00190924650232442 2.54163625689361e-05
-0.00190713732348249 1.68779128857394e-05
-0.00190587169668238 8.56133723647467e-06
-0.00190542342998448 5.34745038357348e-07
-0.00190576074337227 -7.13949490086787e-06
-0.00190684557025069 -1.44050757600496e-05
-0.00190863460518176 -2.12120419551902e-05
-0.00191107907104776 -2.75169579517171e-05
-0.00191412762943649 -3.32830433607879e-05
-0.00191772486724155 -3.84801550748935e-05
-0.00192181199515121 -4.30848707847252e-05
-0.00192632929237876 -4.70803906851367e-05
-0.00193121505892786 -5.04563107412087e-05
-0.00193640771107254 -5.32085316739734e-05
-0.0019418441515486 -5.53389709240419e-05
-0.00194746256352931 -5.68553514316223e-05
-0.00195320275988419 -5.77707276448996e-05
-0.00195900408770324 -5.81032963086901e-05
-0.00196481206399428 -5.78758520011768e-05
-0.00197057069227106 -5.71152885278699e-05
-0.00197622735200497 -5.5852495086892e-05
-0.00198173407921471 -5.41216765854026e-05
-0.00198704523816327 -5.19598886193203e-05
-0.0019921205481735 -4.94066116679074e-05
-0.00199692345382565 -4.65031186576148e-05
-0.00200141926231197 -4.32922311421934e-05
-0.00200558073139503 -3.98178018763706e-05
-0.00200938387846632 -3.61240419818366e-05
-0.00201280774771399 -3.22553814406444e-05
-0.0020158386010984 -2.82559009641922e-05
-0.00201846433041669 -2.41688781004914e-05
-0.00202067864826343 -2.00366026279894e-05
-0.00202247945823044 -1.58997818790712e-05
-0.00202386745791811 -1.17974788168313e-05
-0.00202484963141841 -7.76656286359794e-06
-0.00202543319570321 -3.84164953736756e-06
-0.00202563049008479 -5.49165630222941e-08
-0.00202545757923806 3.56432331290223e-06
-0.00202493169205632 6.98952918414897e-06
-0.00202407494695429 1.01972149989652e-05
-0.00202290876392787 1.31670396755672e-05
-0.0020214578226732 1.58816583098681e-05
-0.00201974843277906 1.83269336209392e-05
-0.00201780946504811 2.04919325720639e-05
-0.00201566862620154 2.23689019468627e-05
-0.00201335408868844 2.39530074322364e-05
-0.00201089565484302 2.5242383735781e-05
-0.00200832266140343 2.62380265399183e-05
-0.00200566491083031 2.69436368708275e-05
-0.00200295104149114 2.73655376572487e-05
-0.00200020829481773 2.75123705270404e-05
-0.00199746414512458 2.73949786002447e-05
-0.00199474466978389 2.7026190317722e-05
-0.00199207385073225 2.64206851197566e-05
-0.00198947520427696 2.5594664012371e-05
-0.00198696991844808 2.45657373671949e-05
-0.00198457685298863 2.33525776248879e-05
-0.00198231416917043 2.19748062481235e-05
-0.00198019537165735 2.04526331096947e-05
-0.00197823443078342 1.88066337437633e-05
-0.00197644415273604 1.70577752817585e-05
-0.00197483338557642 1.52270914223333e-05
-0.00197340934754432 1.33354317330501e-05
-0.0019721762300666 1.14032630830359e-05
-0.0019711368275677 9.45040669090517e-06
-0.00197029346879819 7.49610785217994e-06
-0.00196964499002454 5.55880368159362e-06
-0.00196918929616493 3.65594146759787e-06
-0.00196892079964691 1.80384875146308e-06
-0.00196883344720431 1.75189726861653e-08
-0.00196892118554495 -1.68922975733081e-06
-0.00196917586586825 -3.30386428601132e-06
-0.00196958701102782 -4.81530330058953e-06
-0.00197014344535224 -6.21396318209932e-06
-0.00197083469162809 -7.49172236727503e-06
-0.00197164678014312 -8.6419357338322e-06
-0.0019725659739766 -9.65964837212809e-06
-0.00197358016599612 -1.05412298335673e-05
-0.0019746763177125 -1.1284429812576e-05
-0.00197583976078842 -1.18883991728925e-05
-0.00197705699100947 -1.23536542439026e-05
-0.00197831380563879 -1.26819908209566e-05
-0.00197959670040658 -1.28764152900352e-05
-0.00198089217101473 -1.29410893368949e-05
-0.00198218787729797 -1.28812024194833e-05
-0.00198347194473338 -1.27028174171737e-05
-0.00198473226594736 -1.24128713338283e-05
-0.00198595836336441 -1.20190741487295e-05
-0.00198714022506015 -1.15297172683395e-05
-0.00198826807192618 -1.09536948934424e-05
-0.00198933445315634 -1.03002732937973e-05
-0.00199033168510655 -9.57903925562524e-06
-0.00199125580942641 -8.79969122082264e-06
-0.00199209960813064 -7.9720219446364e-06
-0.00199285865720144 -7.10594146562495e-06
-0.00199352899828568 -6.21130412263452e-06
-0.00199410876851445 -5.29779315811474e-06
-0.00199459610502158 -4.37488589654506e-06
-0.00199499193892664 -3.4515912685682e-06
-0.00199529464021326 -2.53661099513429e-06
-0.00199550653700224 -1.63822625079456e-06
-0.0019956294917675 -7.64135376480311e-07
-0.0019956665311494 7.85318065793864e-08
-0.00199562301011606 8.83354234918008e-07
-0.0019955010240163 1.64457649769797e-06
-0.00199530499652055 2.35696037409255e-06
-0.00199504028263933 3.01596080501051e-06
-0.00199471247023212 3.61778212374557e-06
-0.00199432738000479 4.15931128490421e-06
-0.00199389129834082 4.63815593239629e-06
-0.00199341051164105 5.05261145320639e-06
-0.00199289130632074 5.40163610885346e-06
-0.00199234020164028 5.68484919939022e-06
-0.0019917641825382 5.90250874777948e-06
-0.00199116976830517 6.05550493271894e-06
-0.00199056301258143 6.145267827125e-06
-0.00198995090034398 6.17377217415919e-06
-0.00198933878676554 6.14353820636892e-06
-0.0019887322598566 6.05740851326083e-06
-0.00198813690763755 5.91867117719948e-06
-0.00198755808530653 5.73096730635894e-06
-0.00198700044957503 5.49824255298512e-06
-0.00198646819149793 5.22469083996191e-06
-0.00198596526930442 4.91471428859958e-06
-0.00198549494273218 4.57283317487501e-06
-0.00198506023869115 4.20367088281711e-06
-0.00198466371843034 3.81191438568722e-06
-0.00198430747753589 3.40226554041692e-06
-0.00198399291310106 2.97936818565098e-06
-0.0019837214222157 2.5477740787077e-06
-0.00198349323781331 2.11193555539699e-06
-0.00198330859282163 1.67612604228462e-06
-0.00198316772016568 1.24444668948235e-06
-0.00198306759312879 8.20679254668472e-07
-0.00198300914311363 4.08320202900138e-07
-0.00198299143887397 1.07521580072593e-08
-0.00198301261783163 -3.68938680040537e-07
-0.00198307081740067 -7.27990157544343e-07
-0.00198316370932703 -1.06395526997156e-06
-0.00198328943101015 -1.37469103466499e-06
-0.00198344472285744 -1.65838025427889e-06
-0.00198362702375941 -1.91358413475021e-06
-0.00198383307410668 -2.13917879412356e-06
-0.00198406054560743 -2.33435768262711e-06
-0.00198430617863691 -2.4986304854261e-06
-0.00198456648073457 -2.63181692132693e-06
-0.00198483865792271 -2.73406411631458e-06
-0.00198511968338918 -2.80577675081627e-06
-0.00198540629748281 -2.84764157768708e-06
-0.00198569500771625 -2.86060982132358e-06
-0.00198598371858106 -2.8459045746344e-06
-0.00198627010173775 -2.80482343063436e-06
-0.00198655113034657 -2.73892424043501e-06
-0.00198682447605687 -2.64992800911527e-06
-0.0019870875776853 -2.5397026684271e-06
-0.00198733880536851 -2.41023387410281e-06
-0.00198757629641082 -2.26356879092122e-06
-0.00198779818811473 -2.1018706359106e-06
-0.00198800308344335 -1.92732977955141e-06
-0.00198819005102252 -1.7421568933966e-06
-0.00198835792664632 -1.54856060974188e-06
-0.00198850647743297 -1.34873168115574e-06
-0.00198863453917884 -1.14481917099386e-06
-0.00198874187900429 -9.38936050016818e-07
-0.00198882849686307 -7.33108525707241e-07
-0.00198889462554225 -5.29265121001522e-07
-0.00198894073066161 -3.2924200172495e-07
-0.00198896657935216 -1.3474135988293e-07
-0.00198897356856295 5.26357629049463e-08
-0.00198896216392337 2.31456914988326e-07
-0.00198893329672886 4.0041782676083e-07
-0.0019888883639387 5.58386537785616e-07
-0.00198882783119365 7.04366691326851e-07
-0.00198875402678388 8.37515692701275e-07
-0.00198866904617788 9.57307467881231e-07
-0.00198857288936394 1.06324777302946e-06
-0.00198846672048956 1.15496848435799e-06
-0.0019883521693669 1.23224267885953e-06
-0.00198823086581106 1.29499565207358e-06
-0.00198810397397948 1.34328838554982e-06
-0.00198797265803206 1.37731416919706e-06
-0.0019878387806239 1.39738022540302e-06
-0.00198770373875123 1.40391335247229e-06
-0.00198756869658267 1.39747980349228e-06
-0.00198743481828697 1.37868219216367e-06
-0.00198730326803672 1.34825695963974e-06
-0.00198717544283609 1.30700403740917e-06
-0.00198705227403004 1.25580660428545e-06
-0.00198693469296344 1.19558788696551e-06
-0.001986823630983 1.12731075381034e-06
-0.00198672001943607 1.05198706205813e-06
-0.00198662409117747 9.70654264027815e-07
-0.00198653468207304 8.84243519536608e-07
-0.00198645365479139 7.93654165639427e-07
-0.00198638194068105 6.99928745598495e-07
-0.00198631953976526 6.04084889823438e-07
-0.00198626668489733 5.07096681131268e-07
-0.00198622384176163 4.09939939825018e-07
-0.00198619077754776 3.13536495862542e-07
-0.00198616702661436 2.18764574927421e-07
-0.00198615258897917 1.26415533682148e-07
-0.00198614746465964 3.72553213968778e-08
-0.00198615095517928 -4.79988247242998e-08
-0.00198616306055153 -1.2872203303e-07
-0.00198618284946566 -2.04356415341861e-07
-0.00198620985627018 -2.74420069655903e-07
-0.00198624361531208 -3.38509014510997e-07
-0.00198628366093751 -3.96280941429572e-07
-0.00198632882899663 -4.47472759406049e-07
-0.00198637888666244 -4.91906931817006e-07
-0.00198643336827565 -5.29458344587959e-07
-0.00198649087685141 -5.60077676166424e-07
-0.00198655117955752 -5.83793712376386e-07
-0.00198661381072995 -6.00689578245973e-07
-0.00198667737337882 -6.10918669897813e-07
-0.00198674256599443 -6.14622551939163e-07
-0.0019868077587534 -6.1204681623241e-07
-0.00198687178749365 -6.034989119383e-07
-0.00198693465220472 -5.89402390571876e-07
-0.00198699565438648 -5.70095760369337e-07
-0.00198705456119746 -5.46018869327682e-07
-0.00198711113979684 -5.1759896271342e-07
-0.00198716445885065 -4.85275773754682e-07
-0.00198721451834687 -4.49543482335113e-07
-0.00198726061978204 -4.10883631495832e-07
-0.0019873027631445 -3.69790473646239e-07
-0.00198734071559145 -3.26778171516953e-07
-0.00198737424428025 -2.82335454761078e-07
-0.00198740334920102 -2.36931468343242e-07
-0.00198742779751171 -1.91029591893252e-07
-0.00198744758920167 -1.45098815840499e-07
-0.0019874627242609 -9.95755204827656e-08
-0.00198747343551115 -5.48653839873257e-08
-0.00198747972294407 -1.1337812547748e-08
-0.00198748158655111 3.06341907834774e-08
-0.00198747949198723 7.07353806422492e-08
-0.00198747343924493 1.08650754983286e-07
-0.00198746366115059 1.44146505798044e-07
-0.00198745062336021 1.76983585420745e-07
-0.00198743432587037 2.06978951969826e-07
-0.00198741500150767 2.33969709133395e-07
-0.00198739334876291 2.57834201423685e-07
-0.00198736960046548 2.78499917078911e-07
-0.00198734398944482 2.95912524279646e-07
-0.00198731628287058 3.10064691322071e-07
-0.0019872881105599 3.20959511164367e-07
-0.00198725784269521 3.28615807006043e-07
-0.00198722757475794 3.33088818666762e-07
-0.00198719730675108 3.34514370937608e-07
-0.00198716703867802 3.33037309374271e-07
-0.00198713677054178 3.28791631244024e-07
-0.00198710650234518 3.21898650267223e-07
-0.00198707809674028 3.12533410281365e-07
-0.00198705015674759 3.00962436933054e-07
-0.00198702384652527 2.87341171471573e-07
-0.00198699846758586 2.71908832121578e-07
-0.00198697518409037 2.54887582452727e-07
-0.001986953763212 2.36511313746364e-07
-0.0019869339721256 2.17013574837707e-07
-0.00198691627649844 1.96620542007152e-07
-0.00198690067633599 1.75574867228735e-07
-0.00198688717164355 1.54106502453163e-07
-0.00198687576242618 1.32436354274238e-07
-0.00198686644868897 1.10768950062259e-07
-0.00198685946326639 8.92945191373687e-08
-0.00198685457333242 6.82122302366264e-08
-0.0019868517788912 4.77013335771319e-08
-0.00198685107994652 2.79338773362392e-08
-0.00198685224367079 9.05840980957445e-09
-0.00198685503723635 -8.77468538454385e-09
-0.00198685969347738 -2.54478863329077e-08
-0.00198686621239499 -4.0874097790005e-08
-0.00198687389549864 -5.49571861361078e-08
-0.00198688320845331 -6.75887561062301e-08
-0.001986893452765 -7.87665673834988e-08
-0.00198690509409906 -8.83895732353007e-08
-0.00198691673546783 -9.64915614458384e-08
-0.00198693023951922 -1.03080376387833e-07
-0.00198694420926989 -1.0806152423706e-07
-0.00198695817905563 -1.11505357468233e-07
-0.00198697214887473 -1.13487928599804e-07
-0.00198698611872582 -1.14067174311096e-07
-0.00198700008860739 -1.13311912075097e-07
-0.00198701405851803 -1.11281889371775e-07
-0.00198702802845659 -1.08027807770375e-07
-0.00198704199842172 -1.03609422902329e-07
-0.00198705596841194 -9.80919226054033e-08
-0.00198706761011404 -9.16012647391926e-08
-0.00198707925183408 -8.43047396493352e-08
-0.00198709089357169 -7.62404709303902e-08
-0.00198710067267602 -6.75255410753639e-08
-0.00198710998612903 -5.83141914162026e-08
-0.00198711860109972 -4.86463721405955e-08
-0.00198712558625867 -3.870623859056e-08
-0.00198713257142255 -2.85506311613337e-08
-0.00198713722827845 -1.82928321630985e-08
-0.00198714188513334 -8.06029501086367e-09
-0.00198714491216967 2.10576359387787e-09
-0.00198714724070727 1.20494539979435e-08
-0.00198714863791514 2.17362829766504e-08
-0.00198714863812738 3.10380338440323e-08
-0.00198714863833021 3.99287553862551e-08
-0.00198714677587426 4.83510958393558e-08
-0.00198714444774227 5.61852187361961e-08
-0.0019871421195974 6.34562071764357e-08
-0.00198713792879069 7.01248254950104e-08
-0.00198713327230443 7.60476724604928e-08
-0.00198712861580222 8.12752149223321e-08
-0.00198712395928471 8.58291492838829e-08
-0.00198711813859702 8.97170929028447e-08
-0.0019871111537354 9.28088315990672e-08
-0.00198710416885572 9.51092783089275e-08
-0.00198709718395878 9.6652837742843e-08
-0.0019870901990453 9.74721038647999e-08
-0.00198708321411604 9.75978515951707e-08
-0.00198707622917163 9.70608723394051e-08
-0.0019870692442128 9.58919492803634e-08
-0.00198706225924023 9.41200464922402e-08
-0.00198705527425445 9.17705231906311e-08
-0.00198704828925606 8.88669110868379e-08
-0.00198704293406384 8.54865534216133e-08
-0.00198703827735852 8.18106988841917e-08
-0.00198703362064707 7.78650390024713e-08
-0.00198702896392961 7.36568250203282e-08
-0.00198702430720644 6.91987324264592e-08
-0.00198701988330881 6.45179227547373e-08
-0.00198701755488891 5.97312024451166e-08
-0.00198701522646873 5.49336260429953e-08
-0.00198701289804841 5.01287983718443e-08
-0.00198701056962781 4.53131142551765e-08
-0.00198700870686898 4.04991511299135e-08
-0.00198700870676264 3.58401353733884e-08
-0.00198700870666094 3.13820992204825e-08
-0.00198700870656368 2.71178077241793e-08
-0.0019870087064709 2.30527095407621e-08
-0.00198700870638228 1.91668616368948e-08
-0.00198701056894696 1.55103808394987e-08
-0.00198701289718291 1.22320677389126e-08
-0.00198701522542738 9.33040386792705e-09
-0.00198701755367986 6.77820307997887e-09
-0.00198701988193999 4.56098735689137e-09
-0.00198702221020736 2.66064893207629e-09
-0.00198702453848164 1.06270159252325e-09
-0.00198702686676254 -2.43711027921034e-10
-0.0019870291950497 -1.27670492884244e-09
-0.00198703152334293 -2.04352327637727e-09
-0.00198703385164189 -2.55864393387817e-09
-0.00198703617994639 -2.83112904647664e-09
-0.00198703850825616 -2.87365402784276e-09
-0.00198704083657099 -2.69345375213462e-09
-0.00198704316489059 -2.30320370111017e-09
-0.00198704549321475 -1.71377659285987e-09
-0.00198704782154344 -9.26983371139778e-10
-0.00198705014987624 4.08873520978126e-11
-0.00198705247821307 1.18439494930372e-09
-0.00198705480655368 2.4944937790719e-09
-0.00198705713489791 3.96394079149251e-09
-0.00198705946324568 5.58729536161845e-09
-0.00198706179159678 7.35732266906805e-09
-0.00198706411995088 9.25953654766845e-09
-0.00198706644830815 1.12993610449155e-08
-0.00198706877666809 1.34550669113331e-08
-0.0019870711050307 1.5730292054171e-08
-0.00198707343339603 1.81232093590146e-08
-0.00198707366628282 2.05457978633833e-08
-0.0019870736663357 2.28635397910189e-08
-0.0019870736663862 2.50780758082568e-08
-0.00198707366643452 2.71948217647235e-08
-0.00198707366648058 2.92137941324856e-08
-0.00198707366652463 3.11458575679401e-08
-0.00198707366656678 3.29928063814468e-08
-0.00198707366660704 3.47564595155718e-08
-0.00198707366664561 3.64495089224051e-08
-0.00198707366668254 3.80683083606517e-08
-0.00198707366671783 3.96146768374961e-08
-0.00198707366675151 4.10886061819569e-08
-0.00198707203696519 4.24363177753233e-08
-0.0019870697086791 4.3516391865818e-08
-0.00198706738038698 4.43321010812694e-08
-0.00198706505208905 4.48924911029824e-08
-0.00198706272378553 4.52084347873916e-08
-0.00198706039547671 4.52907885821821e-08
-0.00198705806716287 4.51540469121117e-08
-0.00198705573884417 4.48036338255436e-08
-0.00198705341052083 4.42522412585217e-08
-0.00198705108219301 4.3501655283204e-08
-0.00198704875386103 4.257000007276e-08
-0.00198704665835559 4.14572674297536e-08
-0.00198704665832935 4.03092688954117e-08
-0.00198704665830451 3.92210181268324e-08
-0.00198704665828074 3.81798475161677e-08
-0.00198704665825804 3.71839380111302e-08
-0.00198704665823633 3.62333061228182e-08
-0.00198704665821564 3.53261245455636e-08
-0.00198704665819578 3.44551585600324e-08
-0.00198704665817674 3.36204079688998e-08
-0.00198704665815852 3.2821872876683e-08
-0.00198704665814113 3.20595532781777e-08
-0.00198704665812447 3.13298276627405e-08
-0.0019870466581086 3.06326877193112e-08
-0.00198704665809338 2.99663391852348e-08
-0.00198704665807882 2.93289630585308e-08
-0.00198704665806501 2.87223618326837e-08
-0.00198704665805172 2.81411196949299e-08
-0.0019870466580391 2.75870309157308e-08
-0.00198704665802701 2.70564822534361e-08
-0.00198704665801541 2.65494818499704e-08
-0.00198704665800439 2.60660132870433e-08
-0.00198704665799386 2.5604274044716e-08
-0.00198704665798379 2.51624533115051e-08
-0.00198704665797416 2.47405510843748e-08
-0.00198704665796495 2.43367566151592e-08
-0.00198704665795615 2.39510698713322e-08
-0.00198704665794772 2.35816801186055e-08
-0.0019870466579397 2.32303981181556e-08
-0.00198704665793201 2.28936022691334e-08
-0.00198704665792465 2.25712926483004e-08
-0.00198704665791766 2.22634610144191e-08
-0.001987046657911 2.19719345599667e-08
-0.00198704665790458 2.1691272729385e-08
-0.00198704665789841 2.14196565844448e-08
-0.00198704665789261 2.1166156377074e-08
-0.00198704665788702 2.09217100423723e-08
-0.00198704665788168 2.06863094188992e-08
-0.00198704665787662 2.04654031230392e-08
-0.00198704665787168 2.02481102145463e-08
-0.00198704665786708 2.00471224481857e-08
-0.00198704665786255 1.98479372828624e-08
-0.00198704665785836 1.96650572618397e-08
-0.00198704665785425 1.94839798336142e-08
-0.00198704665785038 1.93155860316735e-08
-0.00198704665784668 1.91526163427144e-08
-0.00198704665784306 1.89950871559708e-08
-0.00198704665783977 1.88502252292631e-08
-0.00198704665783648 1.87053632921472e-08
-0.00198704665783335 1.85695634103908e-08
-0.00198704665783048 1.84428091873877e-08
-0.00198704735632057 1.83249379654901e-08
-0.00198704945180171 1.83711409214478e-08
-0.001987049451805 1.85160032670911e-08
-0.00198704945180808 1.86499923898395e-08
-0.00198704945181096 1.87767465963627e-08
-0.00198704945181384 1.89035007803345e-08
-0.00198704945181655 1.90211929132836e-08
-0.00198704945181902 1.91298393653616e-08
-0.00198704945182149 1.92384858174396e-08
-0.00198704945182395 1.93471322794923e-08
-0.00198704945182613 1.94412843640586e-08
-0.00198704945182819 1.95318230716661e-08
-0.00198704945183025 1.96223617805746e-08
-0.0019870494518323 1.97129005059631e-08
-0.00198704945183424 1.97961879198211e-08
-0.00198704945183588 1.98686189042084e-08
-0.00198704945183753 1.9941049876019e-08
-0.00198704945183917 2.00134808239771e-08
-0.00198704945184082 2.00859117866804e-08
-0.00198704945184246 2.01583427675983e-08
-0.00198704945184374 2.02126578174519e-08
-0.00198704945184497 2.02669810656086e-08
-0.0019870494518462 2.03213042851424e-08
-0.00198704945184744 2.03756275194214e-08
-0.00198704945184867 2.04299507471951e-08
-0.0019870494518499 2.04842739541522e-08
-0.00198704945185114 2.05385971680482e-08
-0.00198704945185217 2.05820475879595e-08
-0.00198704945185299 2.061826308037e-08
-0.00198704945185381 2.06544785502291e-08
-0.00198704945185463 2.06906940374355e-08
-0.00198704945185546 2.07269095328817e-08
-0.00198704945185628 2.07631250140165e-08
-0.0019870494518571 2.0799340494284e-08
-0.00198704945185792 2.08355559775872e-08
-0.00198704945185875 2.08717714552525e-08
-0.00198704945185957 2.09079869424589e-08
-0.00198704945186039 2.09442024270631e-08
-0.00198704945186101 2.09695450730137e-08
-0.00198704945186142 2.09876528365661e-08
-0.00198704945186183 2.10057605810367e-08
-0.00198704945186224 2.10238683038232e-08
-0.00198704945186265 2.10419760725798e-08
-0.00198704945186306 2.10600837944989e-08
-0.00198704945186347 2.10781915363674e-08
-0.00198704945186389 2.10962992856084e-08
-0.0019870494518643 2.1114407032681e-08
-0.00198704945186471 2.11325147784526e-08
-0.00198704945186512 2.11506225120811e-08
-0.00198704945186553 2.1168730247878e-08
-0.00198704945186594 2.11868380062263e-08
-0.00198704945186635 2.12049457316149e-08
-0.00198704945186676 2.12230534908306e-08
-0.00198704945186718 2.12411612201223e-08
-0.00198704945186759 2.12592689537508e-08
-0.001987049451868 2.12773767086297e-08
-0.00198704945186841 2.12954844444266e-08
-0.00198704945186882 2.13135921988718e-08
-0.00198704945186923 2.13316999359697e-08
-0.00198704945186964 2.13498076513836e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
};
\addplot [very thick, learnedWithSideInfo, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131148956024502 0.0251408339982642
0.12697753801571 -0.0389269776754077
0.0958337800877768 -0.08155220449639
0.0497013799085425 -0.0987134584539713
0.00112859510261184 -0.0919732105084418
-0.0392406084376555 -0.0671326915839112
-0.0643732496817204 -0.0325316285619028
-0.0716587168623352 0.00278659300004023
-0.0628000224201014 0.0309209379467193
-0.0427949537901539 0.0468441987971195
-0.0182088076607452 0.0493677412298153
0.00470492455444584 0.0407519781467863
0.0214005756602114 0.0252950676948873
0.0296606870183893 0.00777810665250687
0.0295274617688885 -0.00769246572178202
0.022779268863052 -0.0183505217079844
0.0121865305430108 -0.0230007456206017
0.000742233569227232 -0.0219063907966709
-0.00898782030788926 -0.0164408781169257
-0.0153032605562925 -0.00860646063712395
-0.0175538082423517 -0.000516882705595792
-0.0160756636772411 0.00606262243160363
-0.0119307183526514 0.0100318203150544
-0.00653604584939902 0.0110717283419152
-0.00128694726617611 0.0095599234629908
0.0027385903246951 0.00634270700686301
0.00494385902487263 0.0024515575843572
0.00523878588006754 -0.00115651689090926
0.00395278961932847 -0.00378363214170617
0.00167875197254428 -0.00508080965807065
-0.000904714935681462 -0.00504735125080167
-0.00319205818547836 -0.00395995668247939
-0.00476237851228809 -0.00225986076297363
-0.00543045996440582 -0.000428350683829345
-0.00523842824619986 0.00112212302161417
-0.00440121755127994 0.00212141643034028
-0.00322630040212874 0.0024705780277655
-0.00202988966030194 0.00222829957818128
-0.00106829349960576 0.00156628860869044
-0.000496042174759665 0.000709654537137793
-0.000354162061830499 -0.000121631820070124
-0.000584788261572234 -0.000757964574152674
-0.00106355098979429 -0.00110533553699958
-0.00163926021115995 -0.00114955311449614
-0.00217110442074703 -0.000942956455536594
-0.00255611215231593 -0.000579946925303448
-0.00274311538468592 -0.000168664803117113
-0.00273300390123962 0.000194519830405421
-0.00256798170307848 0.000442919164718265
-0.00231428879892006 0.000547571589113576
-0.00204336071605884 0.000515689781982326
-0.00181572523845253 0.000381776027360933
-0.00167047442471374 0.000194789907848803
-0.00162140489587981 4.88482730881751e-06
-0.00165926487245135 -0.000147390164204409
-0.00175839809106696 -0.000237659761384546
-0.00188547970146019 -0.000259551144852351
-0.00200808415469323 -0.000222368637629608
-0.0021013256633404 -0.000145950483963522
-0.00215155500449561 -5.43556372918372e-05
-0.00215695232598285 3.00544834376843e-05
-0.0021255026630144 9.09775538337977e-05
-0.00207131842158108 0.000120369764043498
-0.00201042839619432 0.000118460442472299
-0.00195700889396966 9.20201960957151e-05
-0.00192078120244159 5.16043326765836e-05
-0.00190587169668238 8.56133723647467e-06
-0.00191107907104776 -2.75169579517171e-05
-0.00193121505892786 -5.04563107412087e-05
-0.00195900408770324 -5.81032963086901e-05
-0.00198704523816327 -5.19598886193203e-05
-0.00200938387846632 -3.61240419818366e-05
-0.00202247945823044 -1.58997818790712e-05
-0.00202545757923806 3.56432331290223e-06
-0.00201974843277906 1.83269336209392e-05
-0.00200832266140343 2.62380265399183e-05
-0.00199474466978389 2.7026190317722e-05
-0.00198231416917043 2.19748062481235e-05
-0.00197340934754432 1.33354317330501e-05
-0.00196918929616493 3.65594146759787e-06
-0.00196958701102782 -4.81530330058953e-06
-0.00197358016599612 -1.05412298335673e-05
-0.00197959670040658 -1.28764152900352e-05
-0.00198595836336441 -1.20190741487295e-05
-0.00199125580942641 -8.79969122082264e-06
-0.00199459610502158 -4.37488589654506e-06
-0.0019956665311494 7.85318065793864e-08
-0.00199471247023212 3.61778212374557e-06
-0.00199234020164028 5.68484919939022e-06
-0.00198933878676554 6.14353820636892e-06
-0.00198646819149793 5.22469083996191e-06
-0.00198430747753589 3.40226554041692e-06
-0.00198316772016568 1.24444668948235e-06
-0.00198307081740067 -7.27990157544343e-07
-0.00198383307410668 -2.13917879412356e-06
-0.00198511968338918 -2.80577675081627e-06
-0.00198655113034657 -2.73892424043501e-06
-0.00198779818811473 -2.1018706359106e-06
-0.00198863453917884 -1.14481917099386e-06
-0.00198896657935216 -1.3474135988293e-07
-0.00198882783119365 7.04366691326851e-07
-0.0019883521693669 1.23224267885953e-06
-0.00198770373875123 1.40391335247229e-06
-0.00198705227403004 1.25580660428545e-06
-0.00198653468207304 8.84243519536608e-07
-0.00198622384176163 4.09939939825018e-07
-0.00198615095517928 -4.79988247242998e-08
-0.00198628366093751 -3.96280941429572e-07
-0.00198655117955752 -5.83793712376386e-07
-0.00198687178749365 -6.034989119383e-07
-0.00198716445885065 -4.85275773754682e-07
-0.00198737424428025 -2.82335454761078e-07
-0.00198747343551115 -5.48653839873257e-08
-0.00198746366115059 1.44146505798044e-07
-0.00198736960046548 2.78499917078911e-07
-0.00198722757475794 3.33088818666762e-07
-0.00198707809674028 3.12533410281365e-07
-0.001986953763212 2.36511313746364e-07
-0.00198687576242618 1.32436354274238e-07
-0.00198685107994652 2.79338773362392e-08
-0.00198687389549864 -5.49571861361078e-08
-0.00198693023951922 -1.03080376387833e-07
-0.00198700008860739 -1.13311912075097e-07
-0.00198706761011404 -9.16012647391926e-08
-0.00198711860109972 -4.86463721405955e-08
-0.00198714491216967 2.10576359387787e-09
-0.00198714677587426 4.83510958393558e-08
-0.00198712861580222 8.12752149223321e-08
-0.00198709718395878 9.6652837742843e-08
-0.00198706225924023 9.41200464922402e-08
-0.00198703362064707 7.78650390024713e-08
-0.00198701522646873 5.49336260429953e-08
-0.00198700870666094 3.13820992204825e-08
-0.00198701289718291 1.22320677389126e-08
-0.00198702453848164 1.06270159252325e-09
-0.00198703617994639 -2.83112904647664e-09
-0.00198704782154344 -9.26983371139778e-10
-0.00198705946324568 5.58729536161845e-09
-0.0019870711050307 1.5730292054171e-08
-0.00198707366643452 2.71948217647235e-08
-0.00198707366664561 3.64495089224051e-08
-0.0019870697086791 4.3516391865818e-08
-0.00198705806716287 4.51540469121117e-08
-0.00198704665835559 4.14572674297536e-08
-0.00198704665823633 3.62333061228182e-08
-0.00198704665814113 3.20595532781777e-08
-0.00198704665806501 2.87223618326837e-08
-0.00198704665800439 2.60660132870433e-08
-0.00198704665795615 2.39510698713322e-08
-0.00198704665791766 2.22634610144191e-08
-0.00198704665788702 2.09217100423723e-08
-0.00198704665786255 1.98479372828624e-08
-0.00198704665784306 1.89950871559708e-08
-0.00198704735632057 1.83249379654901e-08
-0.00198704945181384 1.89035007803345e-08
-0.00198704945182613 1.94412843640586e-08
-0.00198704945183588 1.98686189042084e-08
-0.00198704945184374 2.02126578174519e-08
-0.0019870494518499 2.04842739541522e-08
-0.00198704945185463 2.06906940374355e-08
-0.00198704945185875 2.08717714552525e-08
-0.00198704945186183 2.10057605810367e-08
-0.00198704945186389 2.10962992856084e-08
-0.00198704945186594 2.11868380062263e-08
-0.001987049451868 2.12773767086297e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
};
\addplot [very thick, learnedWithoutSideInfo]
table {%
0.1 0.1
0.115594826513299 0.0883254418870514
0.129118663882368 0.0737378658119523
0.138001393166779 0.0565968585640342
0.141510552085688 0.0388115850309954
0.140443113950194 0.0233187297218309
0.136431867375503 0.012239018930571
0.131269706827035 0.00555251715416105
0.126158759892613 0.00193111051776373
0.121583686406387 6.33264929668087e-05
0.117614430338323 -0.000889583316934672
0.11416900889511 -0.00137721112636435
0.111136690284376 -0.00162423385168609
0.108419002533943 -0.00174087212090357
0.105937975448418 -0.00178163896118422
0.103634160768573 -0.00177409403385265
0.101462574293361 -0.00173254800506428
0.0993890112683431 -0.00166459497645244
0.0973872417280823 -0.00157427649363973
0.0954370191765097 -0.00146365862451514
0.0935227169754222 -0.00133365223745341
0.0916324195602201 -0.00118446677601503
0.089757334696662 -0.00101588459258251
0.0878914278940472 -0.000827447989046437
0.0860312046452014 -0.00061860573030259
0.0841755814442351 -0.000388843051740695
0.0823257953686545 -0.000137806694374465
0.0804853074548415 0.000134571441806175
0.0786596600447922 0.00042795436841736
0.0768562552873995 0.000741490958685809
0.0750840328869629 0.00107372858040278
0.0733530406404501 0.00142256012333064
0.0716739102404933 0.00178521756838212
0.0700572703938542 0.00215832072610023
0.068513145401389 0.00253798344891676
0.0670503957959028 0.00291997149293266
0.0656762557382429 0.00329989800395025
0.0643960095782381 0.00367343633213957
0.063212830125047 0.00403652715327252
0.0621277785438323 0.00438555834782162
0.0611399455388968 0.00471750125151216
0.0602466994513815 0.00502999430414142
0.0594440007329755 0.0053213729681274
0.0587267433961509 0.0055906514568842
0.058089090435498 0.00583746630860316
0.0575247792919047 0.00606199388671635
0.0570273828957033 0.00626485379123443
0.0565905200946801 0.0064470085600703
0.0562080155576776 0.00660966763540127
0.055874013396207 0.00675420097280699
0.0555830510206077 0.0068820653011521
0.0553301005836317 0.00699474412610845
0.0551105852264087 0.00709370118286268
0.0549203766305988 0.0071803461523563
0.0547557793991755 0.00725601097546158
0.0546135067409779 0.00732193492642974
0.0544906509453815 0.00737925664225725
0.054384651265881 0.00742901146554242
0.0542932611088531 0.00747213268215918
0.0542145158452447 0.00750945547893256
0.0541467021146005 0.00754172268184461
0.0540883291531902 0.00756959154771142
0.0540381024308996 0.0075936410640447
0.0539948997058266 0.00761437936164344
0.0539577494846775 0.00763225096432296
0.0539258117978001 0.00764764369308923
0.0538983611483781 0.00766089511263046
0.0538747714684877 0.00767229845991557
0.0538545029025519 0.00768210803199132
0.053837090237784 0.00769054403590341
0.0538221328063937 0.00769779692089156
0.0538092856945287 0.00770403122376506
0.0537982521048406 0.00770938896436624
0.0537887767331888 0.0077139926308083
0.0537806400333558 0.00771794779452595
0.053773653257152 0.00772134539410474
0.0537676541696772 0.00772426372467838
0.053762503351277 0.00772677016715928
0.053758081008354 0.00772892268854264
0.053754284224854 0.00773077114153375
0.053751024594912 0.00773235838890596
0.053748226184811 0.0077337212750852
0.053745823779102 0.0077348914649249
0.0537437613719058 0.00773589616723425
0.0537419908694572 0.00773675875845425
0.0537404709746028 0.00773749931994749
0.0537391662279987 0.00773813510059562
0.0537380461841055 0.0077386809149842
0.0537370847031546 0.00773914948591647
0.0537362593428954 0.00773955173905616
0.0537355508360626 0.00773989705621148
0.0537349426415545 0.00774019349310118
0.0537344205589907 0.00774044796649065
0.0537339723976649 0.00774066641500504
0.0537335876922693 0.00774085393728874
0.0537332574588154 0.00774101491070955
0.0537329739850305 0.00774115309329382
0.053732730650399 0.00774127171128902
0.0537325217716589 0.00774137353437898
0.0537323424701341 0.00774146094025374
0.0537321885578921 0.00774153597005411
0.0537320564399133 0.00774160037599225
0.0537319430301846 0.00774165566225293
0.0537318456796498 0.00774170312007216
0.0537317621143201 0.00774174385788551
0.053731690382202 0.00774177882719695
0.0537316288076886 0.00774180884479847
0.0537315759524359 0.00774183461183697
0.0537315305817732 0.0077418567301839
0.0537314916358529 0.00774187571649088
0.0537314582049007 0.00774189201425823
0.0537314295079785 0.00774190600418767
0.0537314048747142 0.00774191801307222
0.0537313837296765 0.00774192832143772
0.0537313655789156 0.00774193717008198
0.0537313499984231 0.00774194476570389
0.0537313366242307 0.00774195128574218
0.0537313251439109 0.00774195688250101
0.05373131528928 0.00774196168672625
0.0537313068301364 0.00774196581064612
0.0537312995688684 0.00774196935058447
0.0537312933358409 0.00774197238924623
0.0537312879854568 0.00774197499761398
0.0537312833927261 0.0077419772366194
0.0537312794503571 0.00774197915856556
0.0537312760662543 0.00774198080835053
0.0537312731613619 0.00774198222451572
0.053731270667825 0.00774198344014065
0.0537312685273905 0.00774198448362684
0.0537312666900585 0.00774198537934567
0.0537312651129049 0.00774198614822352
0.053731263759091 0.00774198680822669
0.0537312625969841 0.00774198737476683
0.0537312615994381 0.00774198786108182
0.0537312607431559 0.00774198827852945
0.0537312600081306 0.00774198863686104
0.0537312593771837 0.00774198894445344
0.0537312588355867 0.00774198920848845
0.0537312583706795 0.00774198943513493
0.0537312579716058 0.00774198962968975
0.053731257629047 0.00774198979669061
0.0537312573349951 0.00774198994004172
0.0537312570825854 0.00774199006309839
0.0537312568659196 0.00774199016872568
0.0537312566799351 0.00774199025939626
0.0537312565202877 0.00774199033722334
0.0537312563832462 0.00774199040403323
0.0537312562656105 0.00774199046138158
0.0537312561646326 0.00774199051061042
0.0537312560779544 0.00774199055286529
0.0537312560035517 0.00774199058914027
0.0537312559396819 0.00774199062027603
0.0537312558848582 0.00774199064700332
0.053731255837798 0.00774199066994474
0.0537312557974001 0.00774199068963877
0.0537312557627256 0.0077419907065448
0.0537312557329619 0.00774199072105386
0.0537312557074099 0.00774199073351278
0.0537312556854825 0.00774199074420268
0.0537312556666532 0.00774199075338045
0.0537312556504927 0.00774199076125903
0.0537312556366256 0.00774199076802007
0.0537312556247169 0.00774199077382409
0.0537312556144967 0.007741990778805
0.0537312556057241 0.00774199078308135
0.0537312555981888 0.00774199078675575
0.0537312555917211 0.00774199078990812
0.0537312555861771 0.00774199079261306
0.0537312555814147 0.00774199079493587
0.0537312555773228 0.0077419907969285
0.053731255573811 0.0077419907986398
0.0537312555708001 0.00774199080010973
0.053731255568211 0.00774199080137383
0.0537312555659941 0.00774199080245408
0.0537312555640863 0.00774199080338245
0.0537312555624494 0.00774199080418181
0.053731255561047 0.00774199080486659
0.053731255559839 0.00774199080545235
0.0537312555588079 0.00774199080595572
0.0537312555579206 0.00774199080638693
0.0537312555571594 0.00774199080675886
0.0537312555564995 0.00774199080707727
0.0537312555559417 0.00774199080735305
0.0537312555554594 0.00774199080758797
0.0537312555550429 0.00774199080778915
0.0537312555546894 0.00774199080796212
0.0537312555543838 0.00774199080810978
0.0537312555541201 0.00774199080824056
0.0537312555538936 0.00774199080834892
0.0537312555536982 0.00774199080844529
0.0537312555535321 0.007741990808527
0.0537312555533918 0.00774199080859761
0.0537312555532692 0.00774199080865579
0.0537312555531635 0.00774199080870885
0.053731255553072 0.00774199080875348
0.0537312555529965 0.00774199080878857
0.0537312555529326 0.00774199080882143
0.0537312555528793 0.00774199080884763
0.0537312555528278 0.0077419908088705
0.0537312555527807 0.00774199080889182
0.0537312555527452 0.00774199080890936
0.0537312555527159 0.00774199080892468
0.0537312555526892 0.00774199080893956
0.0537312555526661 0.00774199080895044
0.0537312555526466 0.00774199080896021
0.0537312555526306 0.00774199080896754
0.0537312555526182 0.00774199080897442
0.0537312555526075 0.0077419908089793
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
};
\addplot [very thick, learnedWithoutSideInfo, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.140443113950194 0.0233187297218309
0.117614430338323 -0.000889583316934672
0.103634160768573 -0.00177409403385265
0.0935227169754222 -0.00133365223745341
0.0841755814442351 -0.000388843051740695
0.0750840328869629 0.00107372858040278
0.0670503957959028 0.00291997149293266
0.0611399455388968 0.00471750125151216
0.0575247792919047 0.00606199388671635
0.0555830510206077 0.0068820653011521
0.0546135067409779 0.00732193492642974
0.0541467021146005 0.00754172268184461
0.0539258117978001 0.00764764369308923
0.0538221328063937 0.00769779692089156
0.053773653257152 0.00772134539410474
0.053751024594912 0.00773235838890596
0.0537404709746028 0.00773749931994749
0.0537355508360626 0.00773989705621148
0.0537332574588154 0.00774101491070955
0.0537321885578921 0.00774153597005411
0.053731690382202 0.00774177882719695
0.0537314582049007 0.00774189201425823
0.0537313499984231 0.00774194476570389
0.0537312995688684 0.00774196935058447
0.0537312760662543 0.00774198080835053
0.0537312651129049 0.00774198614822352
0.0537312600081306 0.00774198863686104
0.053731257629047 0.00774198979669061
0.0537312565202877 0.00774199033722334
0.0537312560035517 0.00774199058914027
0.0537312557627256 0.0077419907065448
0.0537312556504927 0.00774199076125903
0.0537312555981888 0.00774199078675575
0.053731255573811 0.0077419907986398
0.0537312555624494 0.00774199080418181
0.0537312555571594 0.00774199080675886
0.0537312555546894 0.00774199080796212
0.0537312555535321 0.007741990808527
0.0537312555529965 0.00774199080878857
0.0537312555527452 0.00774199080890936
0.0537312555526306 0.00774199080896754
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
};

==> figures/smd_phase_plots/test_phase_plot_data.tex <==
\addplot [semithick, gray, opacity=0.2, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.0839808732271194 0.0994482040405273
0.0931303426623344 0.0318382531404495
0.0737497732043266 0.135778144001961
0.0458933636546135 0.0842315405607224
0.00452368799597025 0.141100496053696
0.11861914396286 0.0279434863477945
0.143821910023689 0.0297047011554241
0.128507524728775 0.0073636188171804
0.0141577236354351 0.0699533894658089
0.111160345375538 0.0721027925610542
0.0128282625228167 0.116179049015045
0.113642059266567 0.0935259386897087
0.114054314792156 0.00375913036987185
0.0925949066877365 0.0140911275520921
0.107372470200062 0.102853260934353
0.027069415897131 0.121641263365746
0.0358744785189629 0.105421125888824
0.143693581223488 0.07585559040308
0.094265453517437 0.0191213749349117
0.0937533229589462 0.134498134255409
0.133748769760132 0.0891022905707359
0.0770444869995117 0.100217506289482
0.12509161233902 0.134705662727356
0.11181528866291 0.0236758980900049
0.130204707384109 0.0313761942088604
0.0149289695546031 0.0569891221821308
0.0771197602152824 0.0575646832585335
0.127108171582222 0.0588883496820927
0.0504734292626381 0.0226166192442179
0.0276358257979155 0.0366135202348232
0.0565454661846161 0.114331558346748
0.0376495867967606 0.0898406207561493
0.0801086500287056 0.024379700422287
0.0171181075274944 0.117518477141857
0.00829808600246906 0.10522399097681
0.109610736370087 0.144716173410416
0.0895901098847389 0.0249913204461336
0.148184910416603 0.0565091483294964
0.0753039568662643 0.0375259220600128
0.132507354021072 0.0936597362160683
0.0445524007081985 0.00343917869031429
0.0750662982463837 0.0588645227253437
0.0656018257141113 0.102072231471539
0.0221610851585865 0.109879910945892
0.0265114456415176 0.131856635212898
0.126123011112213 0.0447592101991177
0.0665029287338257 0.0892286002635956
0.0387716293334961 0.0300013031810522
0.107425525784492 0.0961355566978455
0.0143502093851566 0.13919261097908
};
\addplot [very thick, black]
table {%
0.100000001490116 0.100000001490116
0.109246507287025 0.0849018394947052
0.116977341473103 0.0697125717997551
0.123191073536873 0.0545846745371819
0.127901151776314 0.039662592113018
0.13113497197628 0.0250817146152258
0.132933050394058 0.0109675116837025
0.133347868919373 -0.00256522372364998
0.132442861795425 -0.0154129592701793
0.130291193723679 -0.0274838879704475
0.126974642276764 -0.0386982522904873
0.122582353651524 -0.0489885360002518
0.11720959842205 -0.0582995116710663
0.11095654219389 -0.0665882006287575
0.103927075862885 -0.0738236755132675
0.0962275639176369 -0.0799867883324623
0.0879657343029976 -0.0850697755813599
0.0792495235800743 -0.0890757739543915
0.0701860412955284 -0.092018261551857
0.0608805567026138 -0.0939204320311546
0.0514355674386024 -0.0948144868016243
0.0419499240815639 -0.0947408825159073
0.032518059015274 -0.0937475189566612
0.0232292674481869 -0.0918889418244362
0.0141671057790518 -0.0892254561185837
0.00540883745998144 -0.0858222842216492
-0.00297499913722277 -0.0817486569285393
-0.0109209567308426 -0.0770769864320755
-0.0183729510754347 -0.071881964802742
-0.0252824425697327 -0.0662397444248199
-0.0316085517406464 -0.0602271296083927
-0.037318080663681 -0.0539207793772221
-0.0423854477703571 -0.0473964810371399
-0.0467925854027271 -0.0407284535467625
-0.0505287498235703 -0.0339886881411076
-0.0535902418196201 -0.0272463709115982
-0.055980134755373 -0.0205673389136791
-0.057707890868187 -0.0140135977417231
-0.05878896266222 -0.00764290988445282
-0.0592443533241749 -0.00150843616575003
-0.0591001398861408 0.0043415566906333
-0.058386966586113 0.00986392982304096
-0.0571395419538021 0.0150208389386535
-0.0553960688412189 0.0197798497974873
-0.0531977377831936 0.0241139885038137
-0.0505881570279598 0.028001731261611
-0.0476128160953522 0.0314269624650478
-0.0443185493350029 0.0343788601458073
-0.0407530181109905 0.0368517301976681
-0.0369642004370689 0.0388448461890221
-0.0329999141395092 0.0403621718287468
-0.0289073493331671 0.0414121262729168
-0.0247326511889696 0.0420072749257088
-0.0205205120146275 0.0421639941632748
-0.0163138080388308 0.0419021397829056
-0.0121532743796706 0.0412446781992912
-0.00807720609009266 0.0402173101902008
-0.00412120949476957 0.038848090916872
-0.00031798382406123 0.0371670387685299
0.00330285541713238 0.0352057404816151
0.00671491445973516 0.032996978610754
0.00989512167870998 0.0305743552744389
0.0128237912431359 0.0279719065874815
0.0154846468940377 0.0252237655222416
0.0178648177534342 0.0223638229072094
0.0199547968804836 0.0194254033267498
0.0217483658343554 0.0164409726858139
0.0232425034046173 0.0134418616071343
0.0244372505694628 0.0104580139741302
0.0253355614840984 0.00751776667311788
0.0259431432932615 0.00464764889329672
0.0262682493776083 0.00187221250962466
0.0263214912265539 -0.000786110933404416
0.026115607470274 -0.00330712483264506
0.0256652422249317 -0.00567295635119081
0.0249867085367441 -0.00786811672151089
0.0240977462381124 -0.00987953413277864
0.0230172835290432 -0.0116965686902404
0.0217651892453432 -0.0133109902963042
0.0203620363026857 -0.0147169474512339
0.0188288688659668 -0.0159109029918909
0.0171869676560163 -0.0168915633112192
0.015457640402019 -0.0176597684621811
0.0136620020493865 -0.0182183980941772
0.0118207894265652 -0.0185722261667252
0.00995416752994061 -0.0187277924269438
0.00808156933635473 -0.0186932515352964
0.006221535615623 -0.0184782091528177
0.00439158175140619 -0.0180935673415661
0.00260807573795319 -0.0175513457506895
0.000886133871972561 -0.0168645121157169
-0.000760464114136994 -0.01604681648314
-0.0023193450178951 -0.0151126058772206
-0.00377959408797324 -0.0140766715630889
-0.00513179041445255 -0.0129540683701634
-0.00636802474036813 -0.011759964749217
-0.00748190423473716 -0.010509486310184
-0.00846854131668806 -0.00921756867319345
-0.00932452455163002 -0.00789882522076368
-0.010047884657979 -0.00656741484999657
-0.0106380386278033 -0.00523693254217505
-0.0110957333818078 -0.00392029946669936
-0.011422966606915 -0.0026296719443053
-0.0116229122504592 -0.00137636042200029
-0.0116998301818967 -0.00017075969662983
-0.0116589702665806 0.000977707444690168
-0.0115064745768905 0.00206063431687653
-0.0112492740154266 0.00307066342793405
-0.0108949821442366 0.00400150613859296
-0.0104517871513963 0.00484795263037086
-0.00992834381759167 0.00560586946085095
-0.00933366827666759 0.00627218699082732
-0.00867702905088663 0.00684487959370017
-0.00796784833073616 0.00732293119654059
-0.00721559952944517 0.00770629895851016
-0.00642971601337194 0.00799586437642574
-0.00561949610710144 0.00819337926805019
-0.00479402346536517 0.00830140896141529
-0.00396208744496107 0.00832326523959637
-0.00313211092725396 0.00826293602585793
-0.00231208698824048 0.00812501925975084
-0.00150952278636396 0.00791464187204838
-0.00073138828156516 0.00763738946989179
1.59242717927555e-05 0.00729922438040376
0.000726634752936661 0.00690641347318888
0.00139560177922249 0.00646545086055994
0.00201834132894874 0.00598298152908683
0.0025910388212651 0.00546573288738728
0.00311055313795805 0.00492044165730476
0.00357441511005163 0.00435378961265087
0.00398081820458174 0.00377234211191535
0.00432860339060426 0.0031824866309762
0.00461724074557424 0.00259038223885
0.00484680151566863 0.00200190930627286
0.0050179292447865 0.00142262596637011
0.00513180671259761 0.000857729755807668
0.00519011542201042 0.000312024436425418
0.00519499788060784 -0.000210107551538385
0.00514901150017977 -0.00070472713559866
0.00505508575588465 -0.00116835557855666
0.0049164742231369 -0.00159798585809767
0.00473670708015561 -0.00199108873493969
0.00451954314485192 -0.00234561483375728
0.00426892284303904 -0.00265998998656869
0.00398892071098089 -0.00293310871347785
0.00368369836360216 -0.00316432118415833
0.00335746072232723 -0.00335341785103083
0.00301441201008856 -0.00350060989148915
0.00265871570445597 -0.00360650639049709
0.00229445495642722 -0.00367208919487894
0.00192559778224677 -0.00369868520647287
0.00155596307013184 -0.00368793704546988
0.00118919124361128 -0.00364177045412362
0.000828717311378568 -0.00356236263178289
0.000477747147670016 -0.00345210870727897
0.000139237934490666 -0.00331358797848225
-0.000184119024197571 -0.00314952875487506
-0.00048991123912856 -0.0029627752956003
-0.00077601516386494 -0.0027562549803406
-0.001040602568537 -0.00253294431604445
-0.00128214422147721 -0.00229583843611181
-0.00149940990377218 -0.00204792129807174
-0.00169146619737148 -0.00179213611409068
-0.00185767083894461 -0.00153135962318629
-0.00199766480363905 -0.00126837671268731
-0.00211136182770133 -0.00100585806649178
-0.00219893641769886 -0.000746339443139732
-0.00226080929860473 -0.000492203922476619
-0.00229763076640666 -0.000245665753027424
-0.00231026369147003 -8.75710338732461e-06
-0.00229976465925574 0.000216682703467086
-0.00226736417971551 0.000429015897680074
-0.00221444619819522 0.000626812281552702
-0.00214252714067698 0.000808853132184595
-0.00205323472619057 0.000974132679402828
-0.00194828608073294 0.00112185755278915
-0.0018294679466635 0.00125144422054291
-0.00169861468020827 0.00136251421645284
-0.00155758846085519 0.00145488826092333
-0.00140826008282602 0.00152857787907124
-0.00125248951371759 0.00158377608750015
-0.00109210924711078 0.00162084680050611
-0.000928907131310552 0.00164031272288412
-0.000764611351769418 0.00164284289348871
-0.000600876519456506 0.00162923848256469
-0.000439270952483639 0.00160041905473918
-0.000281265849480405 0.00155740755144507
-0.000128225539810956 0.00150131515692919
1.86005854629911e-05 0.00143332662992179
0.000158084629219957 0.00135468482039869
0.000289225281449035 0.00126667565200478
0.000411151326261461 0.00117061380296946
0.000523123890161514 0.00106782803777605
0.000624537118710577 0.000959648168645799
0.000714917667210102 0.000847391609568149
0.000793922692537308 0.000732351210899651
0.000861337059177458 0.00061578385066241
0.000917068973649293 0.000498900189995766
0.000961145095061511 0.000382854690542445
0.000993704306893051 0.000268737523583695
0.00101499096490443 0.000157566799316555
0.00102534727193415 5.02822840644512e-05
0.00102520559448749 -5.2259951189626e-05
0.00101507909130305 -0.000149291809066199
0.000995553564280272 -0.000240136389038526
0.00096727762138471 -0.000324210035614669
0.000930953654460609 -0.000401023629819974
0.000887328118551522 -0.000470182625576854
0.000837182393297553 -0.000531386293005198
0.000781323120463639 -0.000584426103159785
0.000720573356375098 -0.000629183370620012
0.000655763666145504 -0.000665625731926411
0.000587723799981177 -0.000693803653120995
0.000517274253070354 -0.000713845482096076
0.000445219251560047 -0.000725952733773738
0.000372339301975444 -0.000730394385755062
0.000299384933896363 -0.000727500999346375
0.000227070777327754 -0.000717658491339535
0.000156070411321707 -0.000701301731169224
8.70117146405391e-05 -0.000678907847031951
2.04730313271284e-05 -0.000650989473797381
-4.3020052544307e-05 -0.000618088117334992
-0.000102997270005289 -0.00058076751884073
-0.000159045550390147 -0.000539606960956007
-0.000210810263524763 -0.000495194806717336
-0.000257995852734894 -0.000448122475063428
-0.000300365703878924 -0.000398978474549949
-0.000337741832481697 -0.000348342844517902
-0.000370003457646817 -0.000296781799988821
-0.000397085619624704 -0.000244842958636582
-0.000418976967921481 -0.000193050989764743
-0.000435717345681041 -0.000141903467010707
-0.000447394762886688 -9.18674486456439e-05
-0.00045414236956276 -4.33763743785676e-05
-0.000456134817795828 3.17250555781357e-06
-0.000453584623755887 4.74202497571241e-05
-0.000446738151367754 8.90478549990803e-05
-0.000435871683293954 0.000127777399029583
-0.000421287200879306 0.0001633727515582
-0.000403308134991676 0.000195639877347276
-0.000382275262381881 0.000224426607019268
-0.000358542543835938 0.000249622127739713
-0.000332472933223471 0.00027115605189465
-0.000304434477584437 0.000288997078314424
-0.000274796446319669 0.000303151406114921
-0.000243925736867823 0.000313660886604339
-0.000212183294934221 0.00032060089870356
-0.000179921014932916 0.000324077875120565
-0.00014747868408449 0.000324226828524843
-0.000115181253931951 0.000321208586683497
-8.33364319987595e-05 0.000315207056701183
-5.22325026395265e-05 0.000306426227325574
-2.21364753087983e-05 0.000295087200356647
6.70749432174489e-06 0.000281425280263647
3.40793558279984e-05 0.000265686889179051
5.97841390117537e-05 0.000248126685619354
8.36526305647567e-05 0.000229004654102027
0.000105541759694461 0.000208583354833536
0.00012533474364318 0.000187125158845447
0.000142940887599252 0.000164889759616926
0.000158295282744803 0.00014213178656064
0.000171358085935935 0.000119098527648021
0.000182113755727187 9.60278703132644e-05
0.000190569975529797 7.31464970158413e-05
0.000196756504010409 5.06681790284347e-05
0.000200723719899543 2.87923267023871e-05
0.000202541195903905 7.70276528783143e-06
0.000202296068891883 -1.24333182611736e-05
0.000200091322767548 -3.14661774609704e-05
0.000196044013136998 -4.92641265736893e-05
0.000190283462870866 -6.57139316899702e-05
0.000182949341251515 -8.07210162747651e-05
0.000174189903191291 -9.42094993661158e-05
0.000164159995620139 -0.000106121973658446
0.000153019369463436 -0.000116419207188301
0.000140930744237266 -0.000125079619465396
0.000128058178233914 -0.000132098619360477
0.000114565358671825 -0.000137487877509557
0.000100614037364721 -0.000141274344059639
8.63625537022017e-05 -0.00014349928824231
7.19644303899258e-05 -0.000144217177876271
5.75671474507544e-05 -0.000143494515214115
4.33109780715313e-05 -0.00014140858547762
2.93279863399221e-05 -0.000138046234496869
1.57411195687018e-05 -0.000133502471726388
2.66348069999367e-06 -0.00012787920422852
-9.80231288849609e-06 -0.000121283861517441
-2.15646086871857e-05 -0.000113828151370399
-3.2543084671488e-05 -0.000105626691947691
-4.26689657615498e-05 -9.67957894317806e-05
-5.18851520610042e-05 -8.74522011145018e-05
-6.01461870246567e-05 -7.77120003476739e-05
-6.74181428621523e-05 -6.768944876967e-05
-7.36783840693533e-05 -5.74960067751817e-05
-7.89152400102466e-05 -4.72393476229627e-05
-8.31275901873596e-05 -3.70225170627236e-05
-8.63243330968544e-05 -2.69431475317106e-05
-8.85238623595797e-05 -1.70927669387311e-05
-8.9753360953182e-05 -7.55620840209303e-06
-9.00481609278359e-05 1.58888929036038e-06
-8.94509721547365e-05 1.02724898169981e-05
-8.80111256265081e-05 1.84324708243366e-05
-8.57837439980358e-05 2.60148426605156e-05
-8.28289412311278e-05 3.29738759319298e-05
-7.92110004113056e-05 3.9272152207559e-05
-7.49975151848048e-05 4.48805112682749e-05
-7.02586039551534e-05 4.97779401484877e-05
-6.50660731480457e-05 5.39513857802376e-05
-5.94926459598355e-05 5.73954785068054e-05
-5.36112274858169e-05 6.01122264924925e-05
-4.74941552965902e-05 6.21106228209101e-05
-4.12125373259187e-05 6.34062307653949e-05
-3.48356188624166e-05 6.40206926618703e-05
-2.84302004729398e-05 6.39812424196862e-05
-2.20600977627328e-05 6.33201489108615e-05
-1.57856702571735e-05 6.20741848251782e-05
-9.66340394370491e-06 6.02840154897422e-05
-3.74554429072305e-06 5.7993624068331e-05
1.92020183931163e-06 5.52497294847853e-05
7.29091198081733e-06 5.21011970704421e-05
1.23286326925154e-05 4.85984382976312e-05
1.70005059771938e-05 4.4792872358812e-05
2.12788418139098e-05 4.07363550039008e-05
2.51411383942468e-05 3.64806619472802e-05
2.8570042559295e-05 3.20769795507658e-05
3.15532743115909e-05 2.75754464382771e-05
3.4083492209902e-05 2.30247060244437e-05
3.61581369361375e-05 1.84715081559261e-05
3.77791984647047e-05 1.39603489515139e-05
3.8953006878728e-05 9.53314520302229e-06
3.96899340557866e-05 5.22894833920873e-06
4.00040989916306e-05 1.08370852558437e-06
3.99130658479407e-05 -2.86992735709646e-06
3.94374765164685e-05 -6.6027719185513e-06
3.86007268389221e-05 -1.00892129921704e-05
3.74285846191924e-05 -1.33072890093899e-05
3.59488294634502e-05 -1.62387241289252e-05
3.41908853442874e-05 -1.88689300557598e-05
3.21854531648569e-05 -2.11869628401473e-05
2.99641469609924e-05 -2.31854555750033e-05
2.7559146474232e-05 -2.48605156230042e-05
2.50028479058528e-05 -2.62115918303607e-05
2.23275419557467e-05 -2.72413180937292e-05
1.95651100511895e-05 -2.79553278232925e-05
1.67467223946005e-05 -2.83620647678617e-05
1.39025751195732e-05 -2.84725483652437e-05
1.1061644727306e-05 -2.83001500065438e-05
8.25146071292693e-06 -2.78603474725969e-05
5.49791275261668e-06 -2.71704666374717e-05
2.82507426163647e-06 -2.62494286289439e-05
2.55058495213234e-07 -2.51174842560431e-05
-2.19210187424324e-06 -2.37959502555896e-05
-4.49854860562482e-06 -2.2306952814688e-05
-6.64866593069746e-06 -2.06731710932218e-05
-8.62912293086993e-06 -1.89175898412941e-05
-1.04288928923779e-05 -1.70632592926268e-05
-1.20392460303265e-05 -1.51330659718951e-05
-1.34537276608171e-05 -1.31495235109469e-05
-1.46681049955077e-05 -1.11345643745153e-05
-1.56802998390049e-05 -9.10935796127887e-06
-1.64903103723191e-05 -7.09414280208875e-06
-1.71001011040062e-05 -5.10807149112225e-06
-1.75134955497924e-05 -3.16907858177728e-06
-1.77360416273586e-05 -1.29376564927952e-06
-1.77748788701138e-05 5.02696195781027e-07
-1.76385874510743e-05 2.20664423977723e-06
-1.73370390257332e-05 3.80598385163466e-06
-1.68812293850351e-05 5.29022963746684e-06
-1.62831256602658e-05 6.65052948534139e-06
-1.55554971570382e-05 7.87967019277858e-06
-1.47117516462458e-05 8.97207064554095e-06
-1.37657752929954e-05 9.92375225905562e-06
-1.27317744045286e-05 1.07323021438788e-05
-1.16241180876386e-05 1.13968226287398e-05
-1.0457193639013e-05 1.19178603199543e-05
-9.24526557355421e-06 1.22973360703327e-05
-8.0023401096696e-06 1.25384540297091e-05
-6.74204147799173e-06 1.26456134239561e-05
-5.4775009630248e-06 1.26243021441041e-05
-4.22124867327511e-06 1.24809939734405e-05
-2.98512441077037e-06 1.22230349006713e-05
-1.78019388386019e-06 1.18585321615683e-05
-6.16678562437301e-07 1.13962323666783e-05
4.96101563385309e-07 1.08454123619595e-05
1.54977567490278e-06 1.02157564469962e-05
2.53695748142491e-06 9.51724632614059e-06
3.45126863976475e-06 8.76004833116895e-06
4.28735256718937e-06 7.95440428191796e-06
5.04087529407116e-06 7.11052780388854e-06
5.70852034798008e-06 6.23850883130217e-06
6.28796851742663e-06 5.34821856490453e-06
6.77787420499953e-06 4.44922397946357e-06
7.17782995707239e-06 3.55071210833557e-06
7.48832417230005e-06 2.66141614702065e-06
7.71069517213618e-06 1.78955326646246e-06
7.84707208367763e-06 9.42770668643789e-07
7.90032026998233e-06 1.28097980223174e-07
7.87397493695607e-06 -6.48091088351066e-07
7.77217519498663e-06 -1.38010864247917e-06
7.5995922088623e-06 -2.0629747723433e-06
7.36136098566931e-06 -2.69243150796683e-06
7.06300488673151e-06 -3.26494887303852e-06
6.71036332278163e-06 -3.7777238048875e-06
6.30952172286925e-06 -4.22867287852569e-06
5.86673650104785e-06 -4.61641639049049e-06
5.388369118009e-06 -4.94025789521402e-06
4.88081695948495e-06 -5.20015782967675e-06
4.35045012636692e-06 -5.39670145371929e-06
3.80355004381272e-06 -5.53106337974896e-06
3.24625329994888e-06 -5.60496664547827e-06
2.68449821305694e-06 -5.62063996767392e-06
2.12397708310164e-06 -5.58076999368495e-06
1.57009287704568e-06 -5.48845400771825e-06
1.02791966583027e-06 -5.3471503633773e-06
5.02170450999984e-07 -5.16062482347479e-06
-2.83179746318751e-09 -4.93290053782403e-06
-4.83177188925765e-07 -4.66820711153559e-06
-9.35386822220607e-07 -4.37092603533529e-06
-1.35642574150552e-06 -4.04554475608165e-06
-1.74371052708011e-06 -3.696604835568e-06
-2.09511313187249e-06 -3.32865556629258e-06
-2.40895860770252e-06 -2.94621054308664e-06
-2.68401981884381e-06 -2.55370377999498e-06
-2.91950800601626e-06 -2.15545151149854e-06
-3.11505755234975e-06 -1.75561513060529e-06
-3.2707109767216e-06 -1.35816878810147e-06
-3.38689665113634e-06 -9.66869492913247e-07
-3.46440720022656e-06 -5.85230907290679e-07
-3.50437335328024e-06 -2.16501462091401e-07
-3.50823688677337e-06 1.36354870505784e-07
-3.47772061104479e-06 4.70673285235534e-07
-3.41479903909203e-06 7.84099654538295e-07
-3.32166541738843e-06 1.07459811715671e-06
-3.2007010304369e-06 1.34045592403709e-06
-3.05444223158702e-06 1.58028353780537e-06
-2.88554792859941e-06 1.79301321168168e-06
-2.69676820607856e-06 1.97789313460817e-06
-2.49091272053192e-06 2.13447992791771e-06
-2.27082045967109e-06 2.26262727665016e-06
-2.03933086595498e-06 2.3624734240002e-06
-1.79925598331465e-06 2.43442514147318e-06
-1.55335396812006e-06 2.4791418127279e-06
-1.30430589706521e-06 2.49751610681415e-06
-1.05469223399268e-06 2.49065351454192e-06
-8.06973389444465e-07 2.45985165747697e-06
-5.63471132863924e-07 2.4065782326943e-06
-3.26353045920769e-07 2.33244873015792e-06
-9.76187308765475e-08 2.2392023311113e-06
1.20911479939423e-07 2.12868053495185e-06
3.27605448546819e-07 2.00280283024767e-06
5.21025981470302e-07 1.86354486686469e-06
6.99935355896741e-07 1.71291651440697e-06
8.63297714204236e-07 1.55294037540443e-06
1.01027910659468e-06 1.38563143536885e-06
1.14024589947803e-06 1.2129778497183e-06
1.25276130802376e-06 1.03692298125679e-06
1.34757988234924e-06 8.59348631365719e-07
1.42464068630943e-06 6.8205946490707e-07
1.48405854361044e-06 5.06769481489755e-07
1.52611505654932e-06 3.35089481495743e-07
1.55124678258289e-06 1.68516649523553e-07
1.5600345477651e-06 8.42530312183953e-09
1.55318957695272e-06 -1.43940411589938e-07
1.53154110194009e-06 -2.87472317950233e-07
1.49602203691757e-06 -4.21202372535845e-07
1.44765499499044e-06 -5.44305294170044e-07
1.38753807732428e-06 -6.56099643947528e-07
1.31683009385597e-06 -7.56047427330486e-07
1.23673680718639e-06 -8.43752218315785e-07
1.148496494352e-06 -9.18956345685729e-07
1.05336653177801e-06 -9.81536686595064e-07
9.52609923388081e-07 -1.03149886854226e-06
8.47483136112714e-07 -1.06897130081052e-06
7.39223935397604e-07 -1.09419806904043e-06
6.29040130206704e-07 -1.10753046556056e-06
5.18099398050254e-07 -1.10941869024828e-06
4.07519962664082e-07 -1.10040241452225e-06
2.98361840123107e-07 -1.0811013453349e-06
1.9161960551628e-07 -1.05220522073068e-06
8.82157067394473e-08 -1.0144635780307e-06
-1.10048610224567e-08 -9.6867563570413e-07
-1.05279134743341e-07 -9.15680118396267e-07
-1.93929551528527e-07 -8.56345025113114e-07
-2.76366392881755e-07 -7.91557795309927e-07
-3.52089273292222e-07 -7.22215816040261e-07
-4.2068765537806e-07 -6.49216929105023e-07
-4.81840459087834e-07 -5.7345096138306e-07
-5.35314768512762e-07 -4.95791312005167e-07
-5.80963956053893e-07 -4.17087193227417e-07
-6.18724698142614e-07 -3.38156610268925e-07
-6.48613763587491e-07 -2.59779824318684e-07
-6.70723750317848e-07 -1.82693710826243e-07
-6.85218537910259e-07 -1.0758660096144e-07
-6.92328285367694e-07 -3.50939721727173e-08
-6.92343860464462e-07 3.4205175580837e-08
-6.85611041717493e-07 9.97911939748519e-08
-6.72524720357615e-07 1.61205989002156e-07
-6.53522135962703e-07 2.18054438505533e-07
-6.29077135272382e-07 2.70005187985589e-07
-5.99693350977759e-07 3.16790817578294e-07
-5.65898005788767e-07 3.58207245199083e-07
-5.28235659658094e-07 3.94112674939606e-07
-4.87261957005103e-07 4.24425962819441e-07
-4.43537715000275e-07 4.49124399892753e-07
-3.97623210801612e-07 4.68241097451028e-07
-3.50072724586425e-07 4.81862002743583e-07
-3.01429537330478e-07 4.90122431529016e-07
-2.52220957008831e-07 4.93203231144435e-07
-2.0295416902627e-07 4.91327000418096e-07
-1.54112157702002e-07 4.84753854834707e-07
-1.06150224610246e-07 4.73776850640206e-07
-5.94928835084829e-08 4.58717778428763e-07
-1.45312304411505e-08 4.39922473560728e-07
2.83792367383739e-08 4.17756382375956e-07
6.89203503156932e-08 3.92599872611754e-07
1.06812557021385e-07 3.64843970146467e-07
1.41815746701468e-07 3.34886010477931e-07
1.7372967420215e-07 3.03125290201933e-07
2.02393962922542e-07 2.69959315346568e-07
2.27687763754147e-07 2.35779850754625e-07
2.49528909535002e-07 2.00969424213326e-07
2.67872962922411e-07 1.65898072168602e-07
2.8271168162064e-07 1.30920341234741e-07
2.94071384132621e-07 9.63725312885799e-08
3.02011073927133e-07 6.25704004164618e-08
3.06620108858624e-07 2.98070084170377e-08
3.08016069539008e-07 -1.64899549570663e-09
3.06342030853557e-07 -3.15548014384603e-08
3.01764004007055e-07 -5.96945497477464e-08
2.94468293304817e-07 -8.58801243452945e-08
2.84658483451494e-07 -1.09951628246563e-07
2.72552853175512e-07 -1.31777554202017e-07
2.58381305684452e-07 -1.51254724300998e-07
2.42382725446078e-07 -1.68307849435223e-07
2.24802164439097e-07 -1.8288896797003e-07
2.05888085247352e-07 -1.9497650782796e-07
1.85889874160239e-07 -2.04574305939786e-07
1.65055311640572e-07 -2.11710229791606e-07
1.43628227533554e-07 -2.16434798971932e-07
1.21846369438572e-07 -2.18819579345109e-07
9.99392995026938e-08 -2.18955449327041e-07
7.81266464855435e-08 -2.16950738263222e-07
5.66163862458779e-08 -2.12929407439333e-07
3.56034135506889e-08 -2.07028989507307e-07
1.52682630982781e-08 -1.99398641598236e-07
-4.22393453547443e-09 -1.90197084748434e-07
-2.27243202033378e-08 -1.79590642801486e-07
-4.01009607742253e-08 -1.67751196045174e-07
-5.62393047687237e-08 -1.5485424853523e-07
-7.1042471461169e-08 -1.41077094895081e-07
-8.44312921799428e-08 -1.26596930272171e-07
-9.63442730039787e-08 -1.11589152140823e-07
-1.06737275018531e-07 -9.62257686865087e-08
-1.15583148385667e-07 -8.06738498226878e-08
-1.2287112838294e-07 -6.50941629487534e-08
-1.28606174598644e-07 -4.9639893973108e-08
-1.32808111175109e-07 -3.44555530773505e-08
-1.35510788368265e-07 -1.96759550874503e-08
-1.36760959890125e-07 -5.42540501413669e-09
-1.36617288148955e-07 8.18301248983744e-09
-1.35149150537472e-07 2.10479882412073e-08
-1.32435445721057e-07 3.30803970882698e-08
-1.28563385715097e-07 4.4203581239799e-08
-1.23627188486353e-07 5.43534710573113e-08
-1.1772687003031e-07 6.34786161413103e-08
-1.10966936972545e-07 7.15400574335945e-08
-1.03455214173209e-07 7.85111140544359e-08
-9.53015657501055e-08 8.43770209257855e-08
-8.66167724211664e-08 8.91345024456314e-08
-7.75113733197941e-08 9.27912537918019e-08
-6.8094621497039e-08 9.53653227497853e-08
-5.84734820563426e-08 9.68844275917036e-08
-4.87516871316984e-08 9.73852039010126e-08
-3.90289009999378e-08 9.69124442917746e-08
-2.93999224965091e-08 9.55182315465208e-08
-1.99540242107332e-08 9.32611001758232e-08
-1.07743352018019e-08 9.02051269235926e-08
-1.9373391779709e-09 8.64190567995138e-08
6.48755271726031e-09 8.19753935843437e-08
1.44383305311635e-08 7.69495258623465e-08
2.18606288626688e-08 7.14188175265917e-08
2.87078822935882e-08 6.54617977602356e-08
3.49414044364948e-08 5.91573154906655e-08
4.05303772765819e-08 5.2583761345204e-08
4.54517632419993e-08 4.58183215812369e-08
4.96901577662356e-08 3.89362924124725e-08
5.32375672435137e-08 3.20104334150528e-08
5.60931106008411e-08 2.51103742243686e-08
5.82627066592067e-08 1.8302111826074e-08
5.9758662018794e-08 1.16475202815991e-08
6.05992482860529e-08 5.20395992964495e-09
6.0808240220922e-08 -9.76061897972613e-10
6.04144076987723e-08 -6.84516798798995e-09
5.94509792506415e-08 -1.23613208558027e-08
5.79551304724646e-08 -1.74879755121538e-08
5.59674049327441e-08 -2.21941611755483e-08
5.35311670546434e-08 -2.64545203521038e-08
5.06920301290847e-08 -3.02492750847705e-08
4.74973127495559e-08 -3.35641452409163e-08
4.39954987996316e-08 -3.63902330491328e-08
4.02356867823528e-08 -3.87238330290529e-08
3.62671102038803e-08 -4.05662206048873e-08
3.21386224300113e-08 -4.19233927573259e-08
2.78982614787537e-08 -4.28057909118706e-08
2.359280948383e-08 -4.32279705364635e-08
1.92674018961725e-08 -4.32082600809736e-08
1.49651651071281e-08 -4.27684057058286e-08
1.07269020332978e-08 -4.1933180483511e-08
6.59079679721231e-09 -4.07300078109074e-08
2.59217824982727e-09 -3.91885635053768e-08
-1.23668897344942e-09 -3.73403636899639e-08
-4.8667674334979e-09 -3.52183846530352e-08
-8.27237300882189e-09 -3.28566542862063e-08
-1.14312630472568e-08 -3.02898897075465e-08
-1.43246836614708e-08 -2.75530993576467e-08
-1.69373812752838e-08 -2.46812543736041e-08
-1.9257585748278e-08 -2.17089262122272e-08
-2.12769482033082e-08 -1.86699846693728e-08
-2.29904593140873e-08 -1.55972976756402e-08
-2.43963373947054e-08 -1.25224568492399e-08
-2.54958827383689e-08 -9.47553324692763e-09
-2.62933212979988e-08 -6.48486109255941e-09
-2.67956128396918e-08 -3.57684482032994e-09
-2.7012257319825e-08 -7.75794262164453e-10
-2.69550763931647e-08 1.8962083014884e-09
-2.66379789337634e-08 4.41941550022307e-09
-2.60767336612844e-08 6.77649270031111e-09
-2.52887168983307e-08 8.95257024069451e-09
-2.42926674332011e-08 1.09352678023811e-08
-2.31084413826466e-08 1.2714692410043e-08
-2.17567563964849e-08 1.42834171157347e-08
-2.02589518494278e-08 1.56364272640985e-08
-1.86367525856213e-08 1.67710592080539e-08
-1.69120344395424e-08 1.76869026091708e-08
-1.51066075204653e-08 1.83857036262225e-08
-1.32420048259974e-08 1.88712370174926e-08
-1.13392824019343e-08 1.91491729140125e-08
-9.41884525929026e-09 1.92269240528731e-08
-7.50027240314921e-09 1.91134983396068e-08
-5.60217161549303e-09 1.88193265415748e-08
-3.74204356390351e-09 1.83560864286392e-08
-1.93616545018926e-09 1.7736541124691e-08
-1.99490993169071e-10 1.69743508138254e-08
1.45442902166337e-09 1.60839022100845e-08
3.0135114403862e-09 1.50801273690604e-08
4.46718706470506e-09 1.39783358221734e-08
5.80642867120673e-09 1.27940475991295e-08
7.02376556915851e-09 1.15428262503769e-08
8.11327893757152e-09 1.02401322976675e-08
9.07058339549849e-09 8.90117046736805e-09
9.89279858032432e-09 7.54076001641124e-09
1.0578498077507e-08 6.17320550233558e-09
1.11276579062292e-08 4.81218354053681e-09
1.15415845769462e-08 3.47063955352667e-09
1.1822840484399e-08 2.1606989530909e-09
1.19751533134149e-08 8.93586593608831e-10
1.20033281092446e-08 -3.20436788214806e-10
1.19131451370436e-08 -1.47212864121116e-09
1.17112541886399e-08 -2.55330445675384e-09
1.14050724420167e-08 -3.5568661349572e-09
1.10026689981169e-08 -4.47681847148829e-09
1.05126600757899e-08 -5.30827293232505e-09
9.94409177224043e-09 -6.04744254673051e-09
9.30633881068843e-09 -6.6916245877735e-09
8.60898996535298e-09 -7.23917237266392e-09
7.86174769729087e-09 -7.68946328832953e-09
7.0743277902352e-09 -8.04285171795982e-09
6.25636520368289e-09 -8.30061974710361e-09
5.41732037007137e-09 -8.46491854389342e-09
4.56639925872082e-09 -8.53870574246685e-09
3.71247388386564e-09 -8.52567616504984e-09
2.86401324878227e-09 -8.43018987950472e-09
2.02901984103221e-09 -8.25720114505657e-09
1.21497478744459e-09 -8.01217403534338e-09
4.28790059014972e-10 -7.70101049596406e-09
-3.23230997523183e-10 -7.32996863206381e-09
-1.03542530105472e-09 -6.90558454863321e-09
-1.70279434996701e-09 -6.43459685534253e-09
-2.32101982078348e-09 -5.92386761866237e-09
-2.88647372670425e-09 -5.38031308394693e-09
-3.39621841760618e-09 -4.81083128889281e-09
-3.84800280528452e-09 -4.22223722651438e-09
-4.24025126122274e-09 -3.62119956243134e-09
-4.57204407666723e-09 -3.01418245918228e-09
-4.84309570225605e-09 -2.40739383983168e-09
-5.05372721448794e-09 -1.80673620508998e-09
-5.20483300903152e-09 -1.21776455586087e-09
-5.2978426090533e-09 -6.45649089747735e-10
-5.33468336172405e-09 -9.51435388807376e-11
-5.31773602929775e-09 4.29440816240856e-10
-5.24978815974464e-09 9.2425556097453e-10
-5.1339901219194e-09 1.38593014842314e-09
-4.9738035912128e-09 1.81158132939174e-09
-4.7729549201847e-09 2.19881757246299e-09
-4.5353845123941e-09 2.54573850888562e-09
-4.26519841667528e-09 2.85092904839246e-09
-3.96662125368152e-09 3.11345016434927e-09
-3.6439473660721e-09 3.33282446085548e-09
-3.30149640959121e-09 3.50901796508651e-09
-2.94357049845928e-09 3.64241947714561e-09
-2.57441290507643e-09 3.73381592311262e-09
-2.1981692022166e-09 3.78436526560222e-09
-1.81885184691311e-09 3.79556697183148e-09
-1.44030742887935e-09 3.76923070533053e-09
-1.06618758266563e-09 3.70744412947488e-09
-6.99922786395746e-10 3.61253826852703e-09
-3.44699463417086e-10 3.48705309072272e-09
-3.4411653214439e-12 3.33370309135717e-09
3.21207310749472e-10 3.15534176564825e-09
6.26892038280147e-10 2.95492741386738e-09
9.11558606375706e-10 2.73548872442575e-09
1.17345788641643e-09 2.50009213331737e-09
1.41114753215987e-09 2.25181007174058e-09
1.62349200749645e-09 1.9936907680318e-09
1.80965775697928e-09 1.72872949288916e-09
1.96910709959752e-09 1.45984246913144e-09
2.10158912494762e-09 1.18984155861313e-09
2.20712803589151e-09 9.21412557364221e-10
2.28600893770192e-09 6.57094934020108e-10
2.33876340516304e-09 3.99264205031002e-10
2.36615149695751e-09 1.50116780117671e-10
2.36914332596427e-09 -8.83426040654278e-11
2.34889951933326e-09 -3.14311188187588e-10
2.30675079038178e-09 -5.2619592016967e-10
2.24417595617865e-09 -7.22618576087797e-10
2.16278128739589e-09 -9.02418972881236e-10
2.06427785975904e-09 -1.06465547489165e-09
1.95046001572052e-09 -1.20860343955087e-09
1.8231841591998e-09 -1.33375188671181e-09
1.68434666214523e-09 -1.43979805855565e-09
1.53586487972035e-09 -1.52664014763104e-09
1.37965605606638e-09 -1.59436819302528e-09
1.21761944971155e-09 -1.64325442142399e-09
1.05161857000269e-09 -1.6737412567025e-09
8.83464690293323e-10 -1.68642899645022e-09
7.14901471354779e-10 -1.68206204520516e-09
5.47591749722187e-10 -1.66151470359921e-09
3.83104964418735e-10 -1.62577640239192e-09
2.22906595959138e-10 -1.57593627037045e-09
6.83487433317254e-11 -1.51316781327182e-09
-7.93373630680883e-11 -1.43871325963829e-09
-2.19047516236692e-10 -1.35386812871729e-09
-3.49809070598894e-10 -1.25996635347292e-09
-4.70784078387965e-10 -1.15836440439665e-09
-5.81270809263401e-10 -1.05042841092029e-09
-6.80703993172216e-10 -9.37518951360516e-10
-7.68653640736972e-10 -8.2097911802137e-10
-8.44822600765127e-10 -7.02121694118318e-10
-9.09043174068813e-10 -5.82218218081465e-10
-9.61272061950069e-10 -4.62488186636634e-10
-1.00158525917493e-09 -3.4409006199887e-10
-1.03017094854607e-09 -2.28112778666301e-10
-1.0473223399643e-09 -1.15568582481629e-10
-1.05343012091197e-09 -7.38690792562169e-12
-1.04897335262422e-09 9.55906742650114e-11
-1.03451058830473e-09 1.92614368899058e-10
-1.01067088031925e-09 2.83028933623086e-10
-9.7814378818839e-10 3.66275537677652e-10
-9.3767016373647e-10 4.41892411551237e-10
-8.90031937039737e-10 5.09514763713526e-10
-8.36042790552938e-10 5.68873392836622e-10
-7.76538666702464e-10 6.19792828171484e-10
-7.12368442012945e-10 6.62188415212484e-10
-6.44385100834199e-10 6.96062651961427e-10
-5.73437186623948e-10 7.21501025591209e-10
-5.00360752830886e-10 7.38666960931056e-10
-4.25971757866961e-10 7.47796713440607e-10
-3.51059237235773e-10 7.49193151960981e-10
-2.7637883648346e-10 7.43219874532741e-10
-2.02647051916749e-10 7.30294491546601e-10
-1.30536220721567e-10 7.10882075427577e-10
-6.06700592542531e-11 6.85488110718779e-10
6.37997077043706e-12 6.54651943765572e-10
7.00977539902503e-11 6.18939399732454e-10
1.30024810363061e-10 5.78936398820673e-10
1.85761975246557e-10 5.35242017374316e-10
2.36970360001365e-10 4.88462215120222e-10
2.83371798248666e-10 4.39203340363292e-10
3.24748450353241e-10 3.88066384582331e-10
3.60942137289655e-10 3.35641320292623e-10
3.91852911230117e-10 2.82501882997721e-10
4.17437168165335e-10 2.29200824986009e-10
4.37705316436166e-10 1.76265502194184e-10
4.52719084442776e-10 1.24194002304456e-10
4.62588467531333e-10 7.34516475420222e-11
4.67468119769165e-10 2.44681740146913e-11
4.67553828986667e-10 -2.23648148611755e-11
4.63078575485554e-10 -6.66957669648305e-11
4.54308451969254e-10 -1.08214652516647e-10
4.41538361428684e-10 -1.46653980626077e-10
4.2508782605033e-10 -1.81789305830904e-10
4.05296712857606e-10 -2.13439349527889e-10
3.82520792818752e-10 -2.41465625272497e-10
3.57127633021648e-10 -2.65771737950615e-10
3.29492350070737e-10 -2.86302204166589e-10
2.9999364103972e-10 -3.03041092220013e-10
2.69009842179813e-10 -3.16010162482172e-10
2.36915376206071e-10 -3.25266896750165e-10
2.04077213461495e-10 -3.30902139022982e-10
1.70851638392477e-10 -3.33037569744121e-10
1.37581390724506e-10 -3.31823096777484e-10
1.04592869087927e-10 -3.27433885560779e-10
7.21938619996365e-11 -3.20067583547967e-10
4.06713759892874e-11 -3.09941156073634e-10
1.02898757223246e-11 -2.97287916506406e-10
-1.87101879128848e-11 -2.82354417624475e-10
-4.61135504781218e-11 -2.65397426257863e-10
-7.17310169595642e-11 -2.46680870175098e-10
-9.54000073383199e-11 -2.26472965381141e-10
-1.16984893994143e-10 -2.05043426682039e-10
-1.36376923642878e-10 -1.82660650493993e-10
-1.5349407855858e-10 -1.59589300108287e-10
-1.6828045901196e-10 -1.3608779381169e-10
-1.80705644892143e-10 -1.12406160768241e-10
-1.90763682628159e-10 -8.87839871066554e-11
-1.98472016599283e-10 -6.54485909912239e-11
-2.03870087478464e-10 -4.26134093289843e-11
-2.0701798608691e-10 -2.04766065214912e-11
-2.07994774181763e-10 7.80136914270424e-13
-2.06896791365985e-10 2.09925739985684e-11
-2.03835948120457e-10 4.00146443757521e-11
-1.98937810669264e-10 5.77190170658604e-11
-1.92339699722766e-10 7.39974054253523e-11
-1.84188858609602e-10 8.87607140565017e-11
-1.74640413241889e-10 1.01938943397606e-10
-1.63855623513953e-10 1.13480967678381e-10
-1.51999871023101e-10 1.23354090830752e-10
-1.39240952101716e-10 1.31543498316233e-10
-1.2574724594927e-10 1.3805147303092e-10
-1.11686097870045e-10 1.42896611210475e-10
-9.72222372053189e-11 1.46112774657148e-10
-8.25162577156036e-11 1.47748063783482e-10
-6.77232922519089e-11 1.47863665755921e-10
-5.29917602853924e-11 1.46532536104971e-10
-3.84622368676535e-11 1.43838232991023e-10
-2.4266472511969e-11 1.3987347391442e-10
-1.05265431787904e-11 1.34738886714558e-10
2.64587353762669e-12 1.28541538524374e-10
1.51500773731827e-11 1.21393686769444e-10
2.68967903505057e-11 1.13411328939161e-10
3.78084751007091e-11 1.0471297440251e-10
4.781950876942e-11 9.54183121404384e-11
5.68762502373144e-11 8.56470033783197e-11
6.4936972465901e-11 7.55175436073507e-11
7.19716924946212e-11 6.51461037892709e-11
7.79618938850923e-11 5.46455693195558e-11
8.29001312041555e-11 4.41245824600589e-11
8.67895894041126e-11 3.36866680383796e-11
8.96435009556384e-11 2.34295083334501e-11
9.14845629806926e-11 1.3444253522954e-11
9.23442225464477e-11 3.81495703083434e-12
9.22619758370047e-11 -5.38189371540598e-12
9.12845563028064e-11 -1.40777571891459e-11
8.94651436267324e-11 -2.22123153204024e-11
8.68625379957244e-11 -2.97336669174975e-11
8.35403066168361e-11 -3.65984152705945e-11
7.95659163554951e-11 -4.27716750905915e-11
7.50099080071287e-11 -4.82270091917147e-11
6.99450566910009e-11 -5.29462654275115e-11
6.44455391829446e-11 -5.69193477073515e-11
5.85861498203499e-11 -6.01439245628832e-11
5.24415441627291e-11 -6.26250717949972e-11
4.6085520816197e-11 -6.43748734874272e-11
3.95903344829751e-11 -6.54119328147296e-11
3.30260749303868e-11 -6.57609175447327e-11
2.64600875932164e-11 -6.54519702325551e-11
1.99564462177726e-11 -6.45202016813506e-11
1.35754966296142e-11 -6.3005059502963e-11
7.37344300200116e-12 -6.09497660675196e-11
1.40200535642815e-12 -5.84006940029802e-11
-4.29186590780728e-12 -5.54067729197083e-11
-9.66621487713537e-12 -5.20188683794665e-11
-1.46842468740083e-11 -4.82892198450102e-11
-1.9314433732931e-11 -4.42708439352124e-11
-2.35305663842666e-11 -4.00169827829977e-11
-2.73117466143002e-11 -3.55805801488529e-11
-3.06423358908958e-11 -3.1013771412125e-11
-3.35118530148115e-11 -2.63674325429175e-11
-3.59148127904163e-11 -2.16907221350926e-11
-3.78505560227893e-11 -1.70306980323831e-11
-3.93229997175393e-11 -1.24319651795268e-11
-4.0340390750071e-11 -7.93635383106173e-12
-4.09150040237005e-11 -3.58264850078283e-12
-4.10628371583233e-11 5.9364064228587e-13
-4.08032635457189e-11 4.56046441929536e-12
-4.01586784659624e-11 8.28937699731691e-12
-3.91541452038346e-11 1.17556407316921e-11
-3.78170099402109e-11 1.49382832492773e-11
-3.61765201128961e-11 1.78201169098724e-11
-3.42634635941419e-11 2.03877279641995e-11
-3.21097766431411e-11 2.2631415838581e-11
-2.97481830835444e-11 2.45451124702978e-11
-2.72118421545953e-11 2.61262608769464e-11
-2.45339928928168e-11 2.73756694396665e-11
-2.17476366776159e-11 2.82973401655173e-11
-1.88852197768874e-11 2.88982743984478e-11
-1.59783488523635e-11 2.91882594483095e-11
-1.30575246795606e-11 2.91796344031869e-11
-1.0151890612875e-11 2.88870437986644e-11
-7.2890261534897e-12 2.83271895523685e-11
-4.4947470224932e-12 2.75185655512766e-11
-1.79294014530929e-12 2.64811818306843e-11
7.94571873574679e-13 2.52363061004068e-11
3.2481454591976e-12 2.38061913931942e-11
5.55040085073455e-12 2.22138089173152e-11
7.68627956421186e-12 2.04825930522068e-11
9.64307973749801e-12 1.86361863441231e-11
1.14104645870805e-11 1.66982001142957e-11
1.29804457113525e-11 1.46919924143285e-11
1.4347352299271e-11 1.26404390426993e-11
1.55077634761414e-11 1.05657487967092e-11
1.64604423841253e-11 8.48926744873024e-12
1.72062364356407e-11 6.43132205477293e-12
1.77479645563361e-11 4.4110635283312e-12
1.80903018259793e-11 2.44634434237723e-12
1.82396354964087e-11 5.53603549720977e-13
1.82039210094853e-11 -1.25222260945884e-12
1.79925345455967e-11 -2.9577735660008e-12
1.76161030207567e-11 -4.55131722240654e-12
1.7086342757322e-11 -6.02278600256301e-12
1.64158964199856e-11 -7.36379186794256e-12
1.56181578087056e-11 -8.5676292449488e-12
1.47071122641451e-11 -9.62925485875621e-12
1.36971631953253e-11 -1.05452573756493e-11
1.26029776892356e-11 -1.13138118665312e-11
1.14393269162738e-11 -1.19346190916025e-11
1.02209412808363e-11 -1.24088352440599e-11
8.96236383718385e-12 -1.27389860812843e-11
7.677821052543e-12 -1.29288819233908e-11
6.38109747333471e-12 -1.29835118350963e-11
5.08542600391459e-12 -1.29089404096727e-11
3.80338295580263e-12 -1.27121950119213e-11
2.54679784206235e-12 -1.24011521537848e-11
1.32667607368603e-12 -1.19844177984274e-11
1.53130681962779e-13 -1.14712076643153e-11
-9.64672677676581e-13 -1.08712283966583e-11
-2.01855828059483e-12 -1.01945596062136e-11
-3.00137258796296e-12 -9.45153677545107e-12
-3.90700319319315e-12 -8.65263676680383e-12
-4.73038795634206e-12 -7.80837113717459e-12
-5.46751359464803e-12 -6.92918075348437e-12
-6.11540245526454e-12 -6.02533691343443e-12
-6.67209299962113e-12 -5.10685157356638e-12
-7.13660771103908e-12 -4.18338974572663e-12
-7.50891362977235e-12 -3.2641942534356e-12
-7.78988071964415e-12 -2.35801569242744e-12
-7.98122505585308e-12 -1.47305084796656e-12
-8.08545157909846e-12 -6.16889948411997e-13
-8.10579468130124e-12 2.03527746414113e-13
-8.04614708194151e-12 9.81949656135572e-13
-7.91099043911947e-12 1.71283733724215e-12
-7.70532509325461e-12 2.3913859174135e-12
-7.43459373925281e-12 3.01353495109347e-12
-7.10460943548208e-12 3.57597133328336e-12
-6.72147667385437e-12 4.07612615535569e-12
-6.29152199088656e-12 4.5121623451494e-12
-5.82121980827188e-12 4.88295731973509e-12
-5.31712044185562e-12 5.18807869928639e-12
-4.78578591686651e-12 5.42775676834473e-12
-4.2337227473821e-12 5.60284631190289e-12
-3.66732208836873e-12 5.71479148725462e-12
-3.0928035740091e-12 5.76558072118427e-12
-2.51616219179573e-12 5.75770160715638e-12
-1.9431214449972e-12 5.6940923330584e-12
-1.37909041825202e-12 5.57809094053896e-12
-8.2912702311505e-13 5.41338284962278e-12
-2.97905011206398e-13 5.20394881700637e-12
2.10312399006457e-13 4.95401115963023e-12
6.91694043621766e-13 4.66798171297467e-12
1.14285718475632e-12 4.35040805463194e-12
1.56087859651266e-12 4.00592319732551e-12
1.94330055519609e-12 3.63919788401446e-12
2.28813214035728e-12 3.2548900640722e-12
2.59384592797562e-12 2.85760304308269e-12
2.85937029262384e-12 2.45184189791303e-12
3.0840776980845e-12 2.04197422859487e-12
3.26776843431742e-12 1.63219492175376e-12
3.41065283654407e-12 1.22649351612381e-12
3.51332851700192e-12 8.2862503750919e-13
3.57675564513493e-12 4.42085035029169e-13
3.60223049306052e-12 7.0088256216589e-14
3.59135572843006e-12 -2.84449113568952e-13
3.54600983992759e-12 -6.18923261166276e-13
3.46831634592815e-12 -9.31052869350413e-13
3.36060953370909e-12 -1.21888566947947e-12
3.22540345126798e-12 -1.48080148403701e-12
3.06535656233176e-12 -1.71551173874102e-12
2.88324030449372e-12 -1.92205561362624e-12
2.68190591262707e-12 -2.09979386309178e-12
2.46425297702191e-12 -2.24839916650177e-12
2.23319843520309e-12 -2.36784398512102e-12
1.99164794899287e-12 -2.45838635906659e-12
1.74246728157357e-12 -2.52055364427517e-12
1.48845736083758e-12 -2.5551236473853e-12
1.23232901747677e-12 -2.56310554377914e-12
9.76682059880551e-13 -2.54571819353899e-12
7.23984349033924e-13 -2.504368023723e-12
4.76554939173729e-13 -2.44062712748128e-12
2.36548302647022e-13 -2.35620876108678e-12
5.94153929005313e-15 -2.25294370832796e-12
-2.13476317786204e-13 -2.13275794594403e-12
};
\addplot [very thick, dashed, gray]
table {%
0.100000001490116 0.100000001490116
0.109483756124973 0.0895170792937279
0.117873594164848 0.0781397223472595
0.125085666775703 0.0659816265106201
0.131047934293747 0.0531642660498619
0.135700806975365 0.0398157015442848
0.138997808098793 0.0260693151503801
0.140905991196632 0.012062449939549
0.141406282782555 -0.00206493819132447
0.14049369096756 -0.0161716938018799
0.138177335262299 -0.0301168691366911
0.134480357170105 -0.0437611229717731
0.129439681768417 -0.0569681338965893
0.123105704784393 -0.0696059390902519
0.115541689097881 -0.0815482586622238
0.106823220849037 -0.0926757827401161
0.0970374122262001 -0.10287731140852
0.086282029747963 -0.11205093562603
0.0746645554900169 -0.120104975998402
0.0623010508716106 -0.126958966255188
0.049315057694912 -0.132544428110123
0.0358363278210163 -0.136805549263954
0.021999528631568 -0.139699757099152
0.00794291868805885 -0.141198128461838
-0.00619305390864611 -0.141285687685013
-0.0202671475708485 -0.139961570501328
-0.0341387391090393 -0.137239009141922
-0.0476692281663418 -0.133145198225975
-0.0607234202325344 -0.127721056342125
-0.0731708854436874 -0.121020749211311
-0.0848872512578964 -0.11311125010252
-0.0957554504275322 -0.104071579873562
-0.105666890740395 -0.0939920619130135
-0.11452254652977 -0.0829734057188034
-0.122233934700489 -0.0711257085204124
-0.128723993897438 -0.0585673451423645
-0.133927881717682 -0.045423798263073
-0.137793615460396 -0.0318263880908489
-0.140282556414604 -0.0179109815508127
-0.141369849443436 -0.00381661439314485
-0.141044616699219 0.0103158876299858
-0.139310106635094 0.0243453159928322
-0.13618366420269 0.0381314940750599
-0.131696507334709 0.051536675542593
-0.125893503427505 0.0644269213080406
-0.118832595646381 0.0766734331846237
-0.110584355890751 0.0881538465619087
-0.101231195032597 0.098753459751606
-0.0908665657043457 0.10836636275053
-0.0795940235257149 0.116896502673626
-0.0675262063741684 0.124258644878864
-0.0547836944460869 0.130379244685173
-0.0414937995374203 0.135197132825851
-0.0277893114835024 0.138664186000824
-0.0138071617111564 0.140745744109154
0.000312945019686595 0.141421005129814
0.0144299240782857 0.140683248639107
0.0284027252346277 0.138539835810661
0.0420917347073555 0.135012164711952
0.0553601756691933 0.130135506391525
0.0680754780769348 0.123958580195904
0.0801105946302414 0.116543099284172
0.0913452729582787 0.107963152229786
0.101667255163193 0.0983044728636742
0.110973410308361 0.0876635760068893
};
\addplot [very thick, green]
table {%
0.1 0.1
0.109246748678297 0.0849078796512185
0.116978784410934 0.0697313504910003
0.123195182789942 0.0546198145258256
0.127909574276365 0.039713058140546
0.131148956024502 0.0251408339982642
0.132952864801913 0.0110222723172743
0.133372140206764 -0.00253461612184543
0.132467889092112 -0.0154332445393096
0.130310323340097 -0.0275885691132225
0.12697753801571 -0.0389269776754077
0.122554386351484 -0.0493860548060394
0.117131511164947 -0.0589142372985831
0.110804130382256 -0.0674704014762624
0.103671060966292 -0.0750235178247852
0.0958337800877768 -0.08155220449639
0.0873953894411869 -0.0870444325276335
0.0784597807270962 -0.0914970851659502
0.0691306819348083 -0.0949156751409987
0.0595108787201517 -0.0973139560956825
0.0497013799085425 -0.0987134584539713
0.0398006873144798 -0.0991431130008172
0.0299040487998712 -0.0986387920103444
0.0201027914264482 -0.09724276100017
0.0104837244586616 -0.0950031005852733
0.00112859510261184 -0.0919732105084418
-0.00788644620891766 -0.0882111648722856
-0.016491256319674 -0.0837790831787954
-0.0246220823742289 -0.078742597468423
-0.0322218914088985 -0.0731702155932104
-0.0392406084376555 -0.0671326915839112
-0.0456353185586889 -0.0607024878576318
-0.0513704439139048 -0.0539532148659736
-0.0564177604532252 -0.0469590021614969
-0.0607564985142212 -0.0397939692859427
-0.0643732496817204 -0.0325316285619028
-0.0672619071722384 -0.025244240684806
-0.0694235056319963 -0.0180022756800371
-0.0708660460348033 -0.0108737640778257
-0.0716041305897941 -0.00392369728468368
-0.0716587168623352 0.00278659300004023
-0.0710566409296227 0.00920001066814519
-0.0698302746522874 0.0152642493028765
-0.06801692963125 0.0209323071494184
-0.0656583133242816 0.026162924377978
-0.0628000224201014 0.0309209379467193
-0.0594907791721904 0.0351775724264358
-0.0557818987030552 0.0389105841069027
-0.0517265774961605 0.0421043386479463
-0.0473792601189732 0.0447497601825208
-0.0427949537901539 0.0468441987971195
-0.0380286323495037 0.0483911367723739
-0.0331346364981834 0.0493998658796646
-0.0281660926611607 0.04988507608323
-0.0231744082104142 0.0498663786977297
-0.0182088076607452 0.0493677412298153
-0.0133159293971333 0.048416990140884
-0.00853944940531206 0.0470452177661594
-0.00391979999315509 0.0452862123979901
0.000506077902714682 0.0431759406439026
0.00470492455444584 0.0407519781467863
0.00864729918395481 0.0380530333149882
0.0123076662474562 0.0351184373598169
0.0156644417291663 0.0319877680247789
0.0186999862330156 0.028700378294233
0.0214005756602114 0.0252950676948873
0.0237563239231964 0.0218097274268114
0.0257610684037936 0.0182810426550497
0.0274122526164301 0.0147442132337082
0.0287107511266692 0.0112327157947603
0.0296606870183893 0.00777810665250687
0.030269247496878 0.00440982580842111
0.0305464417484334 0.00115506188373554
0.0305048774255947 -0.00196137590055438
0.0301595240926165 -0.00491715083820646
0.0295274617688885 -0.00769246572178202
0.0286276201580785 -0.0102701074506197
0.0274805216017462 -0.0126354631598988
0.0261080128563475 -0.0147765213572665
0.0245330154957108 -0.0166838394871802
0.022779268863052 -0.0183505217079844
0.0208710879224186 -0.0197721192414158
0.0188330968966116 -0.020946596666382
0.0166900076075219 -0.0218742080817294
0.0144664108550512 -0.0225574123665311
0.0121865305430108 -0.0230007456206017
0.00987404951650589 -0.0232106880864667
0.0075519037347531 -0.0231955272667846
0.00524211928487999 -0.0229652247406028
0.00296565009390448 -0.022531242066954
0.000742233569227232 -0.0219063907966709
-0.00140973303858485 -0.0211046656523853
-0.00347330556306724 -0.0201410796283279
-0.00543308466083492 -0.0190314821906951
-0.00727528938938243 -0.017792405344665
-0.00898782030788926 -0.0164408781169257
-0.0105602978969718 -0.0149942585353814
-0.011984089336714 -0.0134700823369586
-0.0132523154948755 -0.0118858661978962
-0.0143598425465498 -0.0102589758118969
-0.0153032605562925 -0.00860646063712395
-0.0160808387763088 -0.00694491733802859
-0.0166924837390137 -0.00529034445894617
-0.0171396563709385 -0.00365801493130141
-0.017425316115093 -0.00206236443194869
-0.0175538082423517 -0.000516882705595792
-0.0175307800340219 0.000965979478546101
-0.0173630746123605 0.00237488923142629
-0.0170586061446089 0.00369969625415589
-0.0166262369095741 0.0049314875577066
-0.0160756636772411 0.00606262243160363
-0.0154172798738499 0.00708675719927847
-0.0146620489224949 0.00799884792394213
-0.0138213738585263 0.0087951558909148
-0.0129069660129583 0.00947321550473128
-0.0119307183526514 0.0100318203150544
-0.010904589064277 0.0104709598346983
-0.00984047489394302 0.0107917861177686
-0.00875010683768729 0.0109965311517296
-0.00764493698478303 0.0110884483878045
-0.00653604584939902 0.0110717283419152
-0.00543405203053174 0.0109514197897686
-0.00434902978786368 0.0107333277413871
-0.00329043849190414 0.0104239309888223
-0.00226706045599777 0.01003028569063
-0.00128694726617611 0.0095599234629908
-0.000357377694930247 0.00902076797765587
0.000515177400847106 0.00842102097581513
0.00132507766674737 0.00776908449829969
0.00206752896919811 0.00707347100245225
0.0027385903246951 0.00634270700686301
0.003335171981031 0.00558525806866026
0.00385502179873081 0.00480944955904372
0.00429671163241483 0.00402339580618332
0.00465961102262796 0.00323493291067163
0.00494385902487263 0.0024515575843572
0.00515032067154429 0.00168037676082483
0.00528055344559724 0.000928055345940087
0.00533675745564245 0.000200777751867166
0.00532172374831673 -0.00049578773323556
0.00523878588006754 -0.00115651689090926
0.00509175798458166 -0.00177685193659794
0.00488488541289976 -0.00235281729620199
0.00462277814383665 -0.00288102844283948
0.0043103563015593 -0.00335869799015325
0.00395278961932847 -0.00378363214170617
0.00355543480760089 -0.00415422333126679
0.00312378363236416 -0.0044694416939813
0.00266340098158826 -0.00472881632615687
0.00217987271030864 -0.00493241170643152
0.00167875197254428 -0.00508080965807065
0.00116550869613252 -0.00517507600378763
0.000645483597795608 -0.0052167337329541
0.0001238439880331 -0.00520772314232486
-0.00039445661143007 -0.00515037129927004
-0.000904714935681462 -0.00504735125080167
-0.00140251101045655 -0.00490164263960043
-0.00188373564176721 -0.00471649047203322
-0.00234461700310627 -0.00449536710496324
-0.00278173844809603 -0.00424192403778586
-0.00319205818547836 -0.00395995668247939
-0.00357291626505327 -0.00365336009692429
-0.00392204831546562 -0.00332608932694335
-0.00423758507949738 -0.0029821197831879
-0.00451805451023812 -0.002625408963354
-0.00476237851228809 -0.00225986076297363
-0.00496986549180008 -0.00188929218900657
-0.00514020057831013 -0.00151739985954091
-0.00527342839582313 -0.00114773124362203
-0.00536994142184466 -0.000783657765801254
-0.00543045996440582 -0.000428350683829345
-0.00545600981074902 -8.47601392898467e-05
-0.00544790080726603 0.000244403550311922
-0.00540769985144195 0.000556684864167624
-0.00533720760902403 0.000849895502776885
-0.00523842824619986 0.00112212302161417
-0.0051135438183376 0.00137173710295825
-0.00496488586467519 0.00159739202461436
-0.00479490700300087 0.00179802881020972
-0.00460614786757787 0.00197286972472612
-0.00440121755127994 0.00212141643034028
-0.00418275635247226 0.00224344036767778
-0.00395341901095098 0.00233897198031635
-0.0037158432755557 0.0024082920342316
-0.00347262499096553 0.00245191608347761
-0.00322630040212874 0.0024705780277655
-0.00297931891272802 0.00246521388450431
-0.00273402934774566 0.00243694534334937
-0.00249265899824361 0.00238706006818046
-0.00225729871973156 0.00231699176789172
-0.00202988966030194 0.00222829957818128
-0.00181221220070397 0.00212264766652223
-0.00160587547647055 0.00200178577317721
-0.00141231015972017 0.00186752857883419
-0.00123276298706574 0.00172173463107783
-0.00106829349960576 0.00156628860869044
-0.000919772296188879 0.00140307988573593
-0.000787881906118659 0.00123398666451948
-0.00067311772009512 0.00106085858928805
-0.000575792704636061 0.000885499887413754
-0.000496042174759665 0.000709654537137793
-0.000433830545770118 0.000534992998400334
-0.000388959482065318 0.00036310004198415
-0.000361076860856358 0.000195463203480396
-0.000349687016522037 3.34637087195007e-05
-0.000354162061830499 -0.000121631820070124
-0.000373753150986401 -0.000268678089475722
-0.000407603372532195 -0.000406656405557404
-0.000454760496770575 -0.000534678246335872
-0.000514189897829482 -0.000651988125138153
-0.000584788261572234 -0.000757964574152674
-0.000665396653263477 -0.000852119367933321
-0.000754814080001606 -0.000934097125504898
-0.000851810442024023 -0.00100367201273078
-0.000955139571331383 -0.00106074450437569
-0.00106355098979429 -0.00110533553699958
-0.00117580277316583 -0.00113758263298688
-0.00129067197044174 -0.00115773272057928
-0.00140696554710492 -0.00116613460775097
-0.00152352981494478 -0.00116323168371543
-0.00163926021115995 -0.00114955311449614
-0.001753109098408 -0.00112570573850112
-0.00186409263351711 -0.00109236491124279
-0.00197129821831335 -0.00105026407729507
-0.00207388729379368 -0.00100018666226535
-0.00217110442074703 -0.000942956455536594
-0.00226227646508275 -0.00087942700536999
-0.00234681643973251 -0.000810473450883835
-0.00242422746299083 -0.000736982903486301
-0.00249409926624985 -0.000659845754572139
-0.00255611215231593 -0.000579946925303448
-0.00261003373595393 -0.000498158159598322
-0.00265571684857268 -0.000415330460256971
-0.00269310046971677 -0.000332286817716783
-0.00272220134529571 -0.000249815498920426
-0.00274311538468592 -0.000168664803117113
-0.00275600951177668 -8.95373229320511e-05
-0.00276112003524966 -1.30855857428526e-05
-0.00275874403392149 6.0092012036148e-05
-0.00274923609717727 0.00012945428659653
-0.00273300390123962 0.000194519830405421
-0.0027104974989892 0.000254869073551034
-0.00268220722450682 0.000310145250644051
-0.00264865531116978 0.000360055077661149
-0.00261039100220095 0.000404368724360883
-0.00256798170307848 0.000442919164718265
-0.00252201065318999 0.000475600816933681
-0.00247306668123392 0.000502367923779241
-0.00242174187685553 0.00052323229404915
-0.00236862320867833 0.000538260696339801
-0.00231428879892006 0.000547571589113576
-0.00225930256822334 0.000551332223256492
-0.00220420888043947 0.000549754240607993
-0.00214952951573697 0.000543089850891065
-0.00209575901389524 0.000531628066934714
-0.00204336071605884 0.000515689781982326
-0.00199276629899486 0.000495623711424411
-0.00194436925570811 0.000471802052612508
-0.00189852605949422 0.000444615382558696
-0.00185555302061197 0.000414468489795412
-0.00181572523845253 0.000381776027360933
-0.00177927636860263 0.000346958022900755
-0.00174639850632657 0.000310435562726666
-0.0017172402074238 0.000272627257505122
-0.00169190974776185 0.000233944750349699
-0.00167047442471374 0.000194789907848803
-0.0016529621868886 0.000155550922341396
-0.00163936256539293 0.000116599515632585
-0.00162962888565821 7.8288143142982e-05
-0.00162368059569947 4.09476169167923e-05
-0.00162140489587981 4.88482730881751e-06
-0.00162265988209101 -2.96189202679442e-05
-0.00162727640836721 -6.23094743312023e-05
-0.00163506169573897 -9.29610155192967e-05
-0.00164580177694068 -0.000121376923229519
-0.00165926487245135 -0.000147390164204409
-0.00167520336954888 -0.000170863796991085
-0.00169335754761149 -0.000191690723181481
-0.00171345895417909 -0.000209793327038812
-0.00173523180194447 -0.000225123164118629
-0.00175839809106696 -0.000237659761384546
-0.00178267854051204 -0.000247409907587432
-0.00180779608055457 -0.000254406090385192
-0.00183347794828767 -0.000258705091436911
-0.00185945836521762 -0.000260386568831148
-0.00188547970146019 -0.000259551144852351
-0.00191129655032468 -0.000256318552918207
-0.00193667584477847 -0.00025082569745358
-0.00196139918580225 -0.000243224611850377
-0.00198526365734689 -0.000233680300134472
-0.00200808415469323 -0.000222368637629608
-0.00202969256959447 -0.000209474227194346
-0.00204994058429013 -0.000195188312975775
-0.00206869827457335 -0.00017970678249374
-0.00208585667097755 -0.000163227877331517
-0.0021013256633404 -0.000145950483963522
-0.00211503446650776 -0.000128072206859369
-0.0021269337158587 -0.000109787370178617
-0.00213699244053753 -9.12855176953458e-05
-0.00214519759782455 -7.27498221176856e-05
-0.00215155500449561 -5.43556372918372e-05
-0.0021560867757104 -3.62691917670972e-05
-0.00215883202353113 -1.86464222535856e-05
-0.002159843830141 -1.6320078909623e-06
-0.00215919087768036 1.46415230829577e-05
-0.00215695232598285 3.00544834376843e-05
-0.00215322060655721 4.45005939197179e-05
-0.00214809560182027 5.78873286436509e-05
-0.00214168906889488 7.01362302268581e-05
-0.00213411672335455 8.11830180709621e-05
-0.0021255026630144 9.09775538337977e-05
-0.00211597284865633 9.9483619285589e-05
-0.00210565766516493 0.000106678727352804
-0.00209468912754636 0.000112553688266524
-0.0020831985526047 0.000117112067319269
-0.00207131842158108 0.000120369764043498
-0.00205917586086127 0.00012235400780146
-0.00204689729858386 0.000123102849343094
-0.00203460334233794 0.000122664235163816
-0.00202241110745119 0.000121095094388362
-0.00201042839619432 0.000118460442472299
-0.00199875998419337 0.000114832307336125
-0.00198750063548198 0.000110288963843293
-0.00197673789644332 0.000104913687468719
-0.00196655046597898 9.87939354380823e-05
-0.00195700889396966 9.20201960957151e-05
-0.00194817313653087 8.46850984925216e-05
-0.00194009511713483 7.68824040109496e-05
-0.00193281709676738 6.87061099029843e-05
-0.00192637120824745 6.0249485411769e-05
-0.00192078120244159 5.16043326765836e-05
-0.00191606151691945 4.28601034525937e-05
-0.00191221762518513 3.41032108148297e-05
-0.00190924650232442 2.54163625689361e-05
-0.00190713732348249 1.68779128857394e-05
-0.00190587169668238 8.56133723647467e-06
-0.00190542342998448 5.34745038357348e-07
-0.00190576074337227 -7.13949490086787e-06
-0.00190684557025069 -1.44050757600496e-05
-0.00190863460518176 -2.12120419551902e-05
-0.00191107907104776 -2.75169579517171e-05
-0.00191412762943649 -3.32830433607879e-05
-0.00191772486724155 -3.84801550748935e-05
-0.00192181199515121 -4.30848707847252e-05
-0.00192632929237876 -4.70803906851367e-05
-0.00193121505892786 -5.04563107412087e-05
-0.00193640771107254 -5.32085316739734e-05
-0.0019418441515486 -5.53389709240419e-05
-0.00194746256352931 -5.68553514316223e-05
-0.00195320275988419 -5.77707276448996e-05
-0.00195900408770324 -5.81032963086901e-05
-0.00196481206399428 -5.78758520011768e-05
-0.00197057069227106 -5.71152885278699e-05
-0.00197622735200497 -5.5852495086892e-05
-0.00198173407921471 -5.41216765854026e-05
-0.00198704523816327 -5.19598886193203e-05
-0.0019921205481735 -4.94066116679074e-05
-0.00199692345382565 -4.65031186576148e-05
-0.00200141926231197 -4.32922311421934e-05
-0.00200558073139503 -3.98178018763706e-05
-0.00200938387846632 -3.61240419818366e-05
-0.00201280774771399 -3.22553814406444e-05
-0.0020158386010984 -2.82559009641922e-05
-0.00201846433041669 -2.41688781004914e-05
-0.00202067864826343 -2.00366026279894e-05
-0.00202247945823044 -1.58997818790712e-05
-0.00202386745791811 -1.17974788168313e-05
-0.00202484963141841 -7.76656286359794e-06
-0.00202543319570321 -3.84164953736756e-06
-0.00202563049008479 -5.49165630222941e-08
-0.00202545757923806 3.56432331290223e-06
-0.00202493169205632 6.98952918414897e-06
-0.00202407494695429 1.01972149989652e-05
-0.00202290876392787 1.31670396755672e-05
-0.0020214578226732 1.58816583098681e-05
-0.00201974843277906 1.83269336209392e-05
-0.00201780946504811 2.04919325720639e-05
-0.00201566862620154 2.23689019468627e-05
-0.00201335408868844 2.39530074322364e-05
-0.00201089565484302 2.5242383735781e-05
-0.00200832266140343 2.62380265399183e-05
-0.00200566491083031 2.69436368708275e-05
-0.00200295104149114 2.73655376572487e-05
-0.00200020829481773 2.75123705270404e-05
-0.00199746414512458 2.73949786002447e-05
-0.00199474466978389 2.7026190317722e-05
-0.00199207385073225 2.64206851197566e-05
-0.00198947520427696 2.5594664012371e-05
-0.00198696991844808 2.45657373671949e-05
-0.00198457685298863 2.33525776248879e-05
-0.00198231416917043 2.19748062481235e-05
-0.00198019537165735 2.04526331096947e-05
-0.00197823443078342 1.88066337437633e-05
-0.00197644415273604 1.70577752817585e-05
-0.00197483338557642 1.52270914223333e-05
-0.00197340934754432 1.33354317330501e-05
-0.0019721762300666 1.14032630830359e-05
-0.0019711368275677 9.45040669090517e-06
-0.00197029346879819 7.49610785217994e-06
-0.00196964499002454 5.55880368159362e-06
-0.00196918929616493 3.65594146759787e-06
-0.00196892079964691 1.80384875146308e-06
-0.00196883344720431 1.75189726861653e-08
-0.00196892118554495 -1.68922975733081e-06
-0.00196917586586825 -3.30386428601132e-06
-0.00196958701102782 -4.81530330058953e-06
-0.00197014344535224 -6.21396318209932e-06
-0.00197083469162809 -7.49172236727503e-06
-0.00197164678014312 -8.6419357338322e-06
-0.0019725659739766 -9.65964837212809e-06
-0.00197358016599612 -1.05412298335673e-05
-0.0019746763177125 -1.1284429812576e-05
-0.00197583976078842 -1.18883991728925e-05
-0.00197705699100947 -1.23536542439026e-05
-0.00197831380563879 -1.26819908209566e-05
-0.00197959670040658 -1.28764152900352e-05
-0.00198089217101473 -1.29410893368949e-05
-0.00198218787729797 -1.28812024194833e-05
-0.00198347194473338 -1.27028174171737e-05
-0.00198473226594736 -1.24128713338283e-05
-0.00198595836336441 -1.20190741487295e-05
-0.00198714022506015 -1.15297172683395e-05
-0.00198826807192618 -1.09536948934424e-05
-0.00198933445315634 -1.03002732937973e-05
-0.00199033168510655 -9.57903925562524e-06
-0.00199125580942641 -8.79969122082264e-06
-0.00199209960813064 -7.9720219446364e-06
-0.00199285865720144 -7.10594146562495e-06
-0.00199352899828568 -6.21130412263452e-06
-0.00199410876851445 -5.29779315811474e-06
-0.00199459610502158 -4.37488589654506e-06
-0.00199499193892664 -3.4515912685682e-06
-0.00199529464021326 -2.53661099513429e-06
-0.00199550653700224 -1.63822625079456e-06
-0.0019956294917675 -7.64135376480311e-07
-0.0019956665311494 7.85318065793864e-08
-0.00199562301011606 8.83354234918008e-07
-0.0019955010240163 1.64457649769797e-06
-0.00199530499652055 2.35696037409255e-06
-0.00199504028263933 3.01596080501051e-06
-0.00199471247023212 3.61778212374557e-06
-0.00199432738000479 4.15931128490421e-06
-0.00199389129834082 4.63815593239629e-06
-0.00199341051164105 5.05261145320639e-06
-0.00199289130632074 5.40163610885346e-06
-0.00199234020164028 5.68484919939022e-06
-0.0019917641825382 5.90250874777948e-06
-0.00199116976830517 6.05550493271894e-06
-0.00199056301258143 6.145267827125e-06
-0.00198995090034398 6.17377217415919e-06
-0.00198933878676554 6.14353820636892e-06
-0.0019887322598566 6.05740851326083e-06
-0.00198813690763755 5.91867117719948e-06
-0.00198755808530653 5.73096730635894e-06
-0.00198700044957503 5.49824255298512e-06
-0.00198646819149793 5.22469083996191e-06
-0.00198596526930442 4.91471428859958e-06
-0.00198549494273218 4.57283317487501e-06
-0.00198506023869115 4.20367088281711e-06
-0.00198466371843034 3.81191438568722e-06
-0.00198430747753589 3.40226554041692e-06
-0.00198399291310106 2.97936818565098e-06
-0.0019837214222157 2.5477740787077e-06
-0.00198349323781331 2.11193555539699e-06
-0.00198330859282163 1.67612604228462e-06
-0.00198316772016568 1.24444668948235e-06
-0.00198306759312879 8.20679254668472e-07
-0.00198300914311363 4.08320202900138e-07
-0.00198299143887397 1.07521580072593e-08
-0.00198301261783163 -3.68938680040537e-07
-0.00198307081740067 -7.27990157544343e-07
-0.00198316370932703 -1.06395526997156e-06
-0.00198328943101015 -1.37469103466499e-06
-0.00198344472285744 -1.65838025427889e-06
-0.00198362702375941 -1.91358413475021e-06
-0.00198383307410668 -2.13917879412356e-06
-0.00198406054560743 -2.33435768262711e-06
-0.00198430617863691 -2.4986304854261e-06
-0.00198456648073457 -2.63181692132693e-06
-0.00198483865792271 -2.73406411631458e-06
-0.00198511968338918 -2.80577675081627e-06
-0.00198540629748281 -2.84764157768708e-06
-0.00198569500771625 -2.86060982132358e-06
-0.00198598371858106 -2.8459045746344e-06
-0.00198627010173775 -2.80482343063436e-06
-0.00198655113034657 -2.73892424043501e-06
-0.00198682447605687 -2.64992800911527e-06
-0.0019870875776853 -2.5397026684271e-06
-0.00198733880536851 -2.41023387410281e-06
-0.00198757629641082 -2.26356879092122e-06
-0.00198779818811473 -2.1018706359106e-06
-0.00198800308344335 -1.92732977955141e-06
-0.00198819005102252 -1.7421568933966e-06
-0.00198835792664632 -1.54856060974188e-06
-0.00198850647743297 -1.34873168115574e-06
-0.00198863453917884 -1.14481917099386e-06
-0.00198874187900429 -9.38936050016818e-07
-0.00198882849686307 -7.33108525707241e-07
-0.00198889462554225 -5.29265121001522e-07
-0.00198894073066161 -3.2924200172495e-07
-0.00198896657935216 -1.3474135988293e-07
-0.00198897356856295 5.26357629049463e-08
-0.00198896216392337 2.31456914988326e-07
-0.00198893329672886 4.0041782676083e-07
-0.0019888883639387 5.58386537785616e-07
-0.00198882783119365 7.04366691326851e-07
-0.00198875402678388 8.37515692701275e-07
-0.00198866904617788 9.57307467881231e-07
-0.00198857288936394 1.06324777302946e-06
-0.00198846672048956 1.15496848435799e-06
-0.0019883521693669 1.23224267885953e-06
-0.00198823086581106 1.29499565207358e-06
-0.00198810397397948 1.34328838554982e-06
-0.00198797265803206 1.37731416919706e-06
-0.0019878387806239 1.39738022540302e-06
-0.00198770373875123 1.40391335247229e-06
-0.00198756869658267 1.39747980349228e-06
-0.00198743481828697 1.37868219216367e-06
-0.00198730326803672 1.34825695963974e-06
-0.00198717544283609 1.30700403740917e-06
-0.00198705227403004 1.25580660428545e-06
-0.00198693469296344 1.19558788696551e-06
-0.001986823630983 1.12731075381034e-06
-0.00198672001943607 1.05198706205813e-06
-0.00198662409117747 9.70654264027815e-07
-0.00198653468207304 8.84243519536608e-07
-0.00198645365479139 7.93654165639427e-07
-0.00198638194068105 6.99928745598495e-07
-0.00198631953976526 6.04084889823438e-07
-0.00198626668489733 5.07096681131268e-07
-0.00198622384176163 4.09939939825018e-07
-0.00198619077754776 3.13536495862542e-07
-0.00198616702661436 2.18764574927421e-07
-0.00198615258897917 1.26415533682148e-07
-0.00198614746465964 3.72553213968778e-08
-0.00198615095517928 -4.79988247242998e-08
-0.00198616306055153 -1.2872203303e-07
-0.00198618284946566 -2.04356415341861e-07
-0.00198620985627018 -2.74420069655903e-07
-0.00198624361531208 -3.38509014510997e-07
-0.00198628366093751 -3.96280941429572e-07
-0.00198632882899663 -4.47472759406049e-07
-0.00198637888666244 -4.91906931817006e-07
-0.00198643336827565 -5.29458344587959e-07
-0.00198649087685141 -5.60077676166424e-07
-0.00198655117955752 -5.83793712376386e-07
-0.00198661381072995 -6.00689578245973e-07
-0.00198667737337882 -6.10918669897813e-07
-0.00198674256599443 -6.14622551939163e-07
-0.0019868077587534 -6.1204681623241e-07
-0.00198687178749365 -6.034989119383e-07
-0.00198693465220472 -5.89402390571876e-07
-0.00198699565438648 -5.70095760369337e-07
-0.00198705456119746 -5.46018869327682e-07
-0.00198711113979684 -5.1759896271342e-07
-0.00198716445885065 -4.85275773754682e-07
-0.00198721451834687 -4.49543482335113e-07
-0.00198726061978204 -4.10883631495832e-07
-0.0019873027631445 -3.69790473646239e-07
-0.00198734071559145 -3.26778171516953e-07
-0.00198737424428025 -2.82335454761078e-07
-0.00198740334920102 -2.36931468343242e-07
-0.00198742779751171 -1.91029591893252e-07
-0.00198744758920167 -1.45098815840499e-07
-0.0019874627242609 -9.95755204827656e-08
-0.00198747343551115 -5.48653839873257e-08
-0.00198747972294407 -1.1337812547748e-08
-0.00198748158655111 3.06341907834774e-08
-0.00198747949198723 7.07353806422492e-08
-0.00198747343924493 1.08650754983286e-07
-0.00198746366115059 1.44146505798044e-07
-0.00198745062336021 1.76983585420745e-07
-0.00198743432587037 2.06978951969826e-07
-0.00198741500150767 2.33969709133395e-07
-0.00198739334876291 2.57834201423685e-07
-0.00198736960046548 2.78499917078911e-07
-0.00198734398944482 2.95912524279646e-07
-0.00198731628287058 3.10064691322071e-07
-0.0019872881105599 3.20959511164367e-07
-0.00198725784269521 3.28615807006043e-07
-0.00198722757475794 3.33088818666762e-07
-0.00198719730675108 3.34514370937608e-07
-0.00198716703867802 3.33037309374271e-07
-0.00198713677054178 3.28791631244024e-07
-0.00198710650234518 3.21898650267223e-07
-0.00198707809674028 3.12533410281365e-07
-0.00198705015674759 3.00962436933054e-07
-0.00198702384652527 2.87341171471573e-07
-0.00198699846758586 2.71908832121578e-07
-0.00198697518409037 2.54887582452727e-07
-0.001986953763212 2.36511313746364e-07
-0.0019869339721256 2.17013574837707e-07
-0.00198691627649844 1.96620542007152e-07
-0.00198690067633599 1.75574867228735e-07
-0.00198688717164355 1.54106502453163e-07
-0.00198687576242618 1.32436354274238e-07
-0.00198686644868897 1.10768950062259e-07
-0.00198685946326639 8.92945191373687e-08
-0.00198685457333242 6.82122302366264e-08
-0.0019868517788912 4.77013335771319e-08
-0.00198685107994652 2.79338773362392e-08
-0.00198685224367079 9.05840980957445e-09
-0.00198685503723635 -8.77468538454385e-09
-0.00198685969347738 -2.54478863329077e-08
-0.00198686621239499 -4.0874097790005e-08
-0.00198687389549864 -5.49571861361078e-08
-0.00198688320845331 -6.75887561062301e-08
-0.001986893452765 -7.87665673834988e-08
-0.00198690509409906 -8.83895732353007e-08
-0.00198691673546783 -9.64915614458384e-08
-0.00198693023951922 -1.03080376387833e-07
-0.00198694420926989 -1.0806152423706e-07
-0.00198695817905563 -1.11505357468233e-07
-0.00198697214887473 -1.13487928599804e-07
-0.00198698611872582 -1.14067174311096e-07
-0.00198700008860739 -1.13311912075097e-07
-0.00198701405851803 -1.11281889371775e-07
-0.00198702802845659 -1.08027807770375e-07
-0.00198704199842172 -1.03609422902329e-07
-0.00198705596841194 -9.80919226054033e-08
-0.00198706761011404 -9.16012647391926e-08
-0.00198707925183408 -8.43047396493352e-08
-0.00198709089357169 -7.62404709303902e-08
-0.00198710067267602 -6.75255410753639e-08
-0.00198710998612903 -5.83141914162026e-08
-0.00198711860109972 -4.86463721405955e-08
-0.00198712558625867 -3.870623859056e-08
-0.00198713257142255 -2.85506311613337e-08
-0.00198713722827845 -1.82928321630985e-08
-0.00198714188513334 -8.06029501086367e-09
-0.00198714491216967 2.10576359387787e-09
-0.00198714724070727 1.20494539979435e-08
-0.00198714863791514 2.17362829766504e-08
-0.00198714863812738 3.10380338440323e-08
-0.00198714863833021 3.99287553862551e-08
-0.00198714677587426 4.83510958393558e-08
-0.00198714444774227 5.61852187361961e-08
-0.0019871421195974 6.34562071764357e-08
-0.00198713792879069 7.01248254950104e-08
-0.00198713327230443 7.60476724604928e-08
-0.00198712861580222 8.12752149223321e-08
-0.00198712395928471 8.58291492838829e-08
-0.00198711813859702 8.97170929028447e-08
-0.0019871111537354 9.28088315990672e-08
-0.00198710416885572 9.51092783089275e-08
-0.00198709718395878 9.6652837742843e-08
-0.0019870901990453 9.74721038647999e-08
-0.00198708321411604 9.75978515951707e-08
-0.00198707622917163 9.70608723394051e-08
-0.0019870692442128 9.58919492803634e-08
-0.00198706225924023 9.41200464922402e-08
-0.00198705527425445 9.17705231906311e-08
-0.00198704828925606 8.88669110868379e-08
-0.00198704293406384 8.54865534216133e-08
-0.00198703827735852 8.18106988841917e-08
-0.00198703362064707 7.78650390024713e-08
-0.00198702896392961 7.36568250203282e-08
-0.00198702430720644 6.91987324264592e-08
-0.00198701988330881 6.45179227547373e-08
-0.00198701755488891 5.97312024451166e-08
-0.00198701522646873 5.49336260429953e-08
-0.00198701289804841 5.01287983718443e-08
-0.00198701056962781 4.53131142551765e-08
-0.00198700870686898 4.04991511299135e-08
-0.00198700870676264 3.58401353733884e-08
-0.00198700870666094 3.13820992204825e-08
-0.00198700870656368 2.71178077241793e-08
-0.0019870087064709 2.30527095407621e-08
-0.00198700870638228 1.91668616368948e-08
-0.00198701056894696 1.55103808394987e-08
-0.00198701289718291 1.22320677389126e-08
-0.00198701522542738 9.33040386792705e-09
-0.00198701755367986 6.77820307997887e-09
-0.00198701988193999 4.56098735689137e-09
-0.00198702221020736 2.66064893207629e-09
-0.00198702453848164 1.06270159252325e-09
-0.00198702686676254 -2.43711027921034e-10
-0.0019870291950497 -1.27670492884244e-09
-0.00198703152334293 -2.04352327637727e-09
-0.00198703385164189 -2.55864393387817e-09
-0.00198703617994639 -2.83112904647664e-09
-0.00198703850825616 -2.87365402784276e-09
-0.00198704083657099 -2.69345375213462e-09
-0.00198704316489059 -2.30320370111017e-09
-0.00198704549321475 -1.71377659285987e-09
-0.00198704782154344 -9.26983371139778e-10
-0.00198705014987624 4.08873520978126e-11
-0.00198705247821307 1.18439494930372e-09
-0.00198705480655368 2.4944937790719e-09
-0.00198705713489791 3.96394079149251e-09
-0.00198705946324568 5.58729536161845e-09
-0.00198706179159678 7.35732266906805e-09
-0.00198706411995088 9.25953654766845e-09
-0.00198706644830815 1.12993610449155e-08
-0.00198706877666809 1.34550669113331e-08
-0.0019870711050307 1.5730292054171e-08
-0.00198707343339603 1.81232093590146e-08
-0.00198707366628282 2.05457978633833e-08
-0.0019870736663357 2.28635397910189e-08
-0.0019870736663862 2.50780758082568e-08
-0.00198707366643452 2.71948217647235e-08
-0.00198707366648058 2.92137941324856e-08
-0.00198707366652463 3.11458575679401e-08
-0.00198707366656678 3.29928063814468e-08
-0.00198707366660704 3.47564595155718e-08
-0.00198707366664561 3.64495089224051e-08
-0.00198707366668254 3.80683083606517e-08
-0.00198707366671783 3.96146768374961e-08
-0.00198707366675151 4.10886061819569e-08
-0.00198707203696519 4.24363177753233e-08
-0.0019870697086791 4.3516391865818e-08
-0.00198706738038698 4.43321010812694e-08
-0.00198706505208905 4.48924911029824e-08
-0.00198706272378553 4.52084347873916e-08
-0.00198706039547671 4.52907885821821e-08
-0.00198705806716287 4.51540469121117e-08
-0.00198705573884417 4.48036338255436e-08
-0.00198705341052083 4.42522412585217e-08
-0.00198705108219301 4.3501655283204e-08
-0.00198704875386103 4.257000007276e-08
-0.00198704665835559 4.14572674297536e-08
-0.00198704665832935 4.03092688954117e-08
-0.00198704665830451 3.92210181268324e-08
-0.00198704665828074 3.81798475161677e-08
-0.00198704665825804 3.71839380111302e-08
-0.00198704665823633 3.62333061228182e-08
-0.00198704665821564 3.53261245455636e-08
-0.00198704665819578 3.44551585600324e-08
-0.00198704665817674 3.36204079688998e-08
-0.00198704665815852 3.2821872876683e-08
-0.00198704665814113 3.20595532781777e-08
-0.00198704665812447 3.13298276627405e-08
-0.0019870466581086 3.06326877193112e-08
-0.00198704665809338 2.99663391852348e-08
-0.00198704665807882 2.93289630585308e-08
-0.00198704665806501 2.87223618326837e-08
-0.00198704665805172 2.81411196949299e-08
-0.0019870466580391 2.75870309157308e-08
-0.00198704665802701 2.70564822534361e-08
-0.00198704665801541 2.65494818499704e-08
-0.00198704665800439 2.60660132870433e-08
-0.00198704665799386 2.5604274044716e-08
-0.00198704665798379 2.51624533115051e-08
-0.00198704665797416 2.47405510843748e-08
-0.00198704665796495 2.43367566151592e-08
-0.00198704665795615 2.39510698713322e-08
-0.00198704665794772 2.35816801186055e-08
-0.0019870466579397 2.32303981181556e-08
-0.00198704665793201 2.28936022691334e-08
-0.00198704665792465 2.25712926483004e-08
-0.00198704665791766 2.22634610144191e-08
-0.001987046657911 2.19719345599667e-08
-0.00198704665790458 2.1691272729385e-08
-0.00198704665789841 2.14196565844448e-08
-0.00198704665789261 2.1166156377074e-08
-0.00198704665788702 2.09217100423723e-08
-0.00198704665788168 2.06863094188992e-08
-0.00198704665787662 2.04654031230392e-08
-0.00198704665787168 2.02481102145463e-08
-0.00198704665786708 2.00471224481857e-08
-0.00198704665786255 1.98479372828624e-08
-0.00198704665785836 1.96650572618397e-08
-0.00198704665785425 1.94839798336142e-08
-0.00198704665785038 1.93155860316735e-08
-0.00198704665784668 1.91526163427144e-08
-0.00198704665784306 1.89950871559708e-08
-0.00198704665783977 1.88502252292631e-08
-0.00198704665783648 1.87053632921472e-08
-0.00198704665783335 1.85695634103908e-08
-0.00198704665783048 1.84428091873877e-08
-0.00198704735632057 1.83249379654901e-08
-0.00198704945180171 1.83711409214478e-08
-0.001987049451805 1.85160032670911e-08
-0.00198704945180808 1.86499923898395e-08
-0.00198704945181096 1.87767465963627e-08
-0.00198704945181384 1.89035007803345e-08
-0.00198704945181655 1.90211929132836e-08
-0.00198704945181902 1.91298393653616e-08
-0.00198704945182149 1.92384858174396e-08
-0.00198704945182395 1.93471322794923e-08
-0.00198704945182613 1.94412843640586e-08
-0.00198704945182819 1.95318230716661e-08
-0.00198704945183025 1.96223617805746e-08
-0.0019870494518323 1.97129005059631e-08
-0.00198704945183424 1.97961879198211e-08
-0.00198704945183588 1.98686189042084e-08
-0.00198704945183753 1.9941049876019e-08
-0.00198704945183917 2.00134808239771e-08
-0.00198704945184082 2.00859117866804e-08
-0.00198704945184246 2.01583427675983e-08
-0.00198704945184374 2.02126578174519e-08
-0.00198704945184497 2.02669810656086e-08
-0.0019870494518462 2.03213042851424e-08
-0.00198704945184744 2.03756275194214e-08
-0.00198704945184867 2.04299507471951e-08
-0.0019870494518499 2.04842739541522e-08
-0.00198704945185114 2.05385971680482e-08
-0.00198704945185217 2.05820475879595e-08
-0.00198704945185299 2.061826308037e-08
-0.00198704945185381 2.06544785502291e-08
-0.00198704945185463 2.06906940374355e-08
-0.00198704945185546 2.07269095328817e-08
-0.00198704945185628 2.07631250140165e-08
-0.0019870494518571 2.0799340494284e-08
-0.00198704945185792 2.08355559775872e-08
-0.00198704945185875 2.08717714552525e-08
-0.00198704945185957 2.09079869424589e-08
-0.00198704945186039 2.09442024270631e-08
-0.00198704945186101 2.09695450730137e-08
-0.00198704945186142 2.09876528365661e-08
-0.00198704945186183 2.10057605810367e-08
-0.00198704945186224 2.10238683038232e-08
-0.00198704945186265 2.10419760725798e-08
-0.00198704945186306 2.10600837944989e-08
-0.00198704945186347 2.10781915363674e-08
-0.00198704945186389 2.10962992856084e-08
-0.0019870494518643 2.1114407032681e-08
-0.00198704945186471 2.11325147784526e-08
-0.00198704945186512 2.11506225120811e-08
-0.00198704945186553 2.1168730247878e-08
-0.00198704945186594 2.11868380062263e-08
-0.00198704945186635 2.12049457316149e-08
-0.00198704945186676 2.12230534908306e-08
-0.00198704945186718 2.12411612201223e-08
-0.00198704945186759 2.12592689537508e-08
-0.001987049451868 2.12773767086297e-08
-0.00198704945186841 2.12954844444266e-08
-0.00198704945186882 2.13135921988718e-08
-0.00198704945186923 2.13316999359697e-08
-0.00198704945186964 2.13498076513836e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
};
\addplot [very thick, green, mark=diamond*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.131148956024502 0.0251408339982642
0.12697753801571 -0.0389269776754077
0.0958337800877768 -0.08155220449639
0.0497013799085425 -0.0987134584539713
0.00112859510261184 -0.0919732105084418
-0.0392406084376555 -0.0671326915839112
-0.0643732496817204 -0.0325316285619028
-0.0716587168623352 0.00278659300004023
-0.0628000224201014 0.0309209379467193
-0.0427949537901539 0.0468441987971195
-0.0182088076607452 0.0493677412298153
0.00470492455444584 0.0407519781467863
0.0214005756602114 0.0252950676948873
0.0296606870183893 0.00777810665250687
0.0295274617688885 -0.00769246572178202
0.022779268863052 -0.0183505217079844
0.0121865305430108 -0.0230007456206017
0.000742233569227232 -0.0219063907966709
-0.00898782030788926 -0.0164408781169257
-0.0153032605562925 -0.00860646063712395
-0.0175538082423517 -0.000516882705595792
-0.0160756636772411 0.00606262243160363
-0.0119307183526514 0.0100318203150544
-0.00653604584939902 0.0110717283419152
-0.00128694726617611 0.0095599234629908
0.0027385903246951 0.00634270700686301
0.00494385902487263 0.0024515575843572
0.00523878588006754 -0.00115651689090926
0.00395278961932847 -0.00378363214170617
0.00167875197254428 -0.00508080965807065
-0.000904714935681462 -0.00504735125080167
-0.00319205818547836 -0.00395995668247939
-0.00476237851228809 -0.00225986076297363
-0.00543045996440582 -0.000428350683829345
-0.00523842824619986 0.00112212302161417
-0.00440121755127994 0.00212141643034028
-0.00322630040212874 0.0024705780277655
-0.00202988966030194 0.00222829957818128
-0.00106829349960576 0.00156628860869044
-0.000496042174759665 0.000709654537137793
-0.000354162061830499 -0.000121631820070124
-0.000584788261572234 -0.000757964574152674
-0.00106355098979429 -0.00110533553699958
-0.00163926021115995 -0.00114955311449614
-0.00217110442074703 -0.000942956455536594
-0.00255611215231593 -0.000579946925303448
-0.00274311538468592 -0.000168664803117113
-0.00273300390123962 0.000194519830405421
-0.00256798170307848 0.000442919164718265
-0.00231428879892006 0.000547571589113576
-0.00204336071605884 0.000515689781982326
-0.00181572523845253 0.000381776027360933
-0.00167047442471374 0.000194789907848803
-0.00162140489587981 4.88482730881751e-06
-0.00165926487245135 -0.000147390164204409
-0.00175839809106696 -0.000237659761384546
-0.00188547970146019 -0.000259551144852351
-0.00200808415469323 -0.000222368637629608
-0.0021013256633404 -0.000145950483963522
-0.00215155500449561 -5.43556372918372e-05
-0.00215695232598285 3.00544834376843e-05
-0.0021255026630144 9.09775538337977e-05
-0.00207131842158108 0.000120369764043498
-0.00201042839619432 0.000118460442472299
-0.00195700889396966 9.20201960957151e-05
-0.00192078120244159 5.16043326765836e-05
-0.00190587169668238 8.56133723647467e-06
-0.00191107907104776 -2.75169579517171e-05
-0.00193121505892786 -5.04563107412087e-05
-0.00195900408770324 -5.81032963086901e-05
-0.00198704523816327 -5.19598886193203e-05
-0.00200938387846632 -3.61240419818366e-05
-0.00202247945823044 -1.58997818790712e-05
-0.00202545757923806 3.56432331290223e-06
-0.00201974843277906 1.83269336209392e-05
-0.00200832266140343 2.62380265399183e-05
-0.00199474466978389 2.7026190317722e-05
-0.00198231416917043 2.19748062481235e-05
-0.00197340934754432 1.33354317330501e-05
-0.00196918929616493 3.65594146759787e-06
-0.00196958701102782 -4.81530330058953e-06
-0.00197358016599612 -1.05412298335673e-05
-0.00197959670040658 -1.28764152900352e-05
-0.00198595836336441 -1.20190741487295e-05
-0.00199125580942641 -8.79969122082264e-06
-0.00199459610502158 -4.37488589654506e-06
-0.0019956665311494 7.85318065793864e-08
-0.00199471247023212 3.61778212374557e-06
-0.00199234020164028 5.68484919939022e-06
-0.00198933878676554 6.14353820636892e-06
-0.00198646819149793 5.22469083996191e-06
-0.00198430747753589 3.40226554041692e-06
-0.00198316772016568 1.24444668948235e-06
-0.00198307081740067 -7.27990157544343e-07
-0.00198383307410668 -2.13917879412356e-06
-0.00198511968338918 -2.80577675081627e-06
-0.00198655113034657 -2.73892424043501e-06
-0.00198779818811473 -2.1018706359106e-06
-0.00198863453917884 -1.14481917099386e-06
-0.00198896657935216 -1.3474135988293e-07
-0.00198882783119365 7.04366691326851e-07
-0.0019883521693669 1.23224267885953e-06
-0.00198770373875123 1.40391335247229e-06
-0.00198705227403004 1.25580660428545e-06
-0.00198653468207304 8.84243519536608e-07
-0.00198622384176163 4.09939939825018e-07
-0.00198615095517928 -4.79988247242998e-08
-0.00198628366093751 -3.96280941429572e-07
-0.00198655117955752 -5.83793712376386e-07
-0.00198687178749365 -6.034989119383e-07
-0.00198716445885065 -4.85275773754682e-07
-0.00198737424428025 -2.82335454761078e-07
-0.00198747343551115 -5.48653839873257e-08
-0.00198746366115059 1.44146505798044e-07
-0.00198736960046548 2.78499917078911e-07
-0.00198722757475794 3.33088818666762e-07
-0.00198707809674028 3.12533410281365e-07
-0.001986953763212 2.36511313746364e-07
-0.00198687576242618 1.32436354274238e-07
-0.00198685107994652 2.79338773362392e-08
-0.00198687389549864 -5.49571861361078e-08
-0.00198693023951922 -1.03080376387833e-07
-0.00198700008860739 -1.13311912075097e-07
-0.00198706761011404 -9.16012647391926e-08
-0.00198711860109972 -4.86463721405955e-08
-0.00198714491216967 2.10576359387787e-09
-0.00198714677587426 4.83510958393558e-08
-0.00198712861580222 8.12752149223321e-08
-0.00198709718395878 9.6652837742843e-08
-0.00198706225924023 9.41200464922402e-08
-0.00198703362064707 7.78650390024713e-08
-0.00198701522646873 5.49336260429953e-08
-0.00198700870666094 3.13820992204825e-08
-0.00198701289718291 1.22320677389126e-08
-0.00198702453848164 1.06270159252325e-09
-0.00198703617994639 -2.83112904647664e-09
-0.00198704782154344 -9.26983371139778e-10
-0.00198705946324568 5.58729536161845e-09
-0.0019870711050307 1.5730292054171e-08
-0.00198707366643452 2.71948217647235e-08
-0.00198707366664561 3.64495089224051e-08
-0.0019870697086791 4.3516391865818e-08
-0.00198705806716287 4.51540469121117e-08
-0.00198704665835559 4.14572674297536e-08
-0.00198704665823633 3.62333061228182e-08
-0.00198704665814113 3.20595532781777e-08
-0.00198704665806501 2.87223618326837e-08
-0.00198704665800439 2.60660132870433e-08
-0.00198704665795615 2.39510698713322e-08
-0.00198704665791766 2.22634610144191e-08
-0.00198704665788702 2.09217100423723e-08
-0.00198704665786255 1.98479372828624e-08
-0.00198704665784306 1.89950871559708e-08
-0.00198704735632057 1.83249379654901e-08
-0.00198704945181384 1.89035007803345e-08
-0.00198704945182613 1.94412843640586e-08
-0.00198704945183588 1.98686189042084e-08
-0.00198704945184374 2.02126578174519e-08
-0.0019870494518499 2.04842739541522e-08
-0.00198704945185463 2.06906940374355e-08
-0.00198704945185875 2.08717714552525e-08
-0.00198704945186183 2.10057605810367e-08
-0.00198704945186389 2.10962992856084e-08
-0.00198704945186594 2.11868380062263e-08
-0.001987049451868 2.12773767086297e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
-0.00198704945186981 2.13552318294175e-08
};
\addplot [very thick, blue]
table {%
0.1 0.1
0.115594826513299 0.0883254418870514
0.129118663882368 0.0737378658119523
0.138001393166779 0.0565968585640342
0.141510552085688 0.0388115850309954
0.140443113950194 0.0233187297218309
0.136431867375503 0.012239018930571
0.131269706827035 0.00555251715416105
0.126158759892613 0.00193111051776373
0.121583686406387 6.33264929668087e-05
0.117614430338323 -0.000889583316934672
0.11416900889511 -0.00137721112636435
0.111136690284376 -0.00162423385168609
0.108419002533943 -0.00174087212090357
0.105937975448418 -0.00178163896118422
0.103634160768573 -0.00177409403385265
0.101462574293361 -0.00173254800506428
0.0993890112683431 -0.00166459497645244
0.0973872417280823 -0.00157427649363973
0.0954370191765097 -0.00146365862451514
0.0935227169754222 -0.00133365223745341
0.0916324195602201 -0.00118446677601503
0.089757334696662 -0.00101588459258251
0.0878914278940472 -0.000827447989046437
0.0860312046452014 -0.00061860573030259
0.0841755814442351 -0.000388843051740695
0.0823257953686545 -0.000137806694374465
0.0804853074548415 0.000134571441806175
0.0786596600447922 0.00042795436841736
0.0768562552873995 0.000741490958685809
0.0750840328869629 0.00107372858040278
0.0733530406404501 0.00142256012333064
0.0716739102404933 0.00178521756838212
0.0700572703938542 0.00215832072610023
0.068513145401389 0.00253798344891676
0.0670503957959028 0.00291997149293266
0.0656762557382429 0.00329989800395025
0.0643960095782381 0.00367343633213957
0.063212830125047 0.00403652715327252
0.0621277785438323 0.00438555834782162
0.0611399455388968 0.00471750125151216
0.0602466994513815 0.00502999430414142
0.0594440007329755 0.0053213729681274
0.0587267433961509 0.0055906514568842
0.058089090435498 0.00583746630860316
0.0575247792919047 0.00606199388671635
0.0570273828957033 0.00626485379123443
0.0565905200946801 0.0064470085600703
0.0562080155576776 0.00660966763540127
0.055874013396207 0.00675420097280699
0.0555830510206077 0.0068820653011521
0.0553301005836317 0.00699474412610845
0.0551105852264087 0.00709370118286268
0.0549203766305988 0.0071803461523563
0.0547557793991755 0.00725601097546158
0.0546135067409779 0.00732193492642974
0.0544906509453815 0.00737925664225725
0.054384651265881 0.00742901146554242
0.0542932611088531 0.00747213268215918
0.0542145158452447 0.00750945547893256
0.0541467021146005 0.00754172268184461
0.0540883291531902 0.00756959154771142
0.0540381024308996 0.0075936410640447
0.0539948997058266 0.00761437936164344
0.0539577494846775 0.00763225096432296
0.0539258117978001 0.00764764369308923
0.0538983611483781 0.00766089511263046
0.0538747714684877 0.00767229845991557
0.0538545029025519 0.00768210803199132
0.053837090237784 0.00769054403590341
0.0538221328063937 0.00769779692089156
0.0538092856945287 0.00770403122376506
0.0537982521048406 0.00770938896436624
0.0537887767331888 0.0077139926308083
0.0537806400333558 0.00771794779452595
0.053773653257152 0.00772134539410474
0.0537676541696772 0.00772426372467838
0.053762503351277 0.00772677016715928
0.053758081008354 0.00772892268854264
0.053754284224854 0.00773077114153375
0.053751024594912 0.00773235838890596
0.053748226184811 0.0077337212750852
0.053745823779102 0.0077348914649249
0.0537437613719058 0.00773589616723425
0.0537419908694572 0.00773675875845425
0.0537404709746028 0.00773749931994749
0.0537391662279987 0.00773813510059562
0.0537380461841055 0.0077386809149842
0.0537370847031546 0.00773914948591647
0.0537362593428954 0.00773955173905616
0.0537355508360626 0.00773989705621148
0.0537349426415545 0.00774019349310118
0.0537344205589907 0.00774044796649065
0.0537339723976649 0.00774066641500504
0.0537335876922693 0.00774085393728874
0.0537332574588154 0.00774101491070955
0.0537329739850305 0.00774115309329382
0.053732730650399 0.00774127171128902
0.0537325217716589 0.00774137353437898
0.0537323424701341 0.00774146094025374
0.0537321885578921 0.00774153597005411
0.0537320564399133 0.00774160037599225
0.0537319430301846 0.00774165566225293
0.0537318456796498 0.00774170312007216
0.0537317621143201 0.00774174385788551
0.053731690382202 0.00774177882719695
0.0537316288076886 0.00774180884479847
0.0537315759524359 0.00774183461183697
0.0537315305817732 0.0077418567301839
0.0537314916358529 0.00774187571649088
0.0537314582049007 0.00774189201425823
0.0537314295079785 0.00774190600418767
0.0537314048747142 0.00774191801307222
0.0537313837296765 0.00774192832143772
0.0537313655789156 0.00774193717008198
0.0537313499984231 0.00774194476570389
0.0537313366242307 0.00774195128574218
0.0537313251439109 0.00774195688250101
0.05373131528928 0.00774196168672625
0.0537313068301364 0.00774196581064612
0.0537312995688684 0.00774196935058447
0.0537312933358409 0.00774197238924623
0.0537312879854568 0.00774197499761398
0.0537312833927261 0.0077419772366194
0.0537312794503571 0.00774197915856556
0.0537312760662543 0.00774198080835053
0.0537312731613619 0.00774198222451572
0.053731270667825 0.00774198344014065
0.0537312685273905 0.00774198448362684
0.0537312666900585 0.00774198537934567
0.0537312651129049 0.00774198614822352
0.053731263759091 0.00774198680822669
0.0537312625969841 0.00774198737476683
0.0537312615994381 0.00774198786108182
0.0537312607431559 0.00774198827852945
0.0537312600081306 0.00774198863686104
0.0537312593771837 0.00774198894445344
0.0537312588355867 0.00774198920848845
0.0537312583706795 0.00774198943513493
0.0537312579716058 0.00774198962968975
0.053731257629047 0.00774198979669061
0.0537312573349951 0.00774198994004172
0.0537312570825854 0.00774199006309839
0.0537312568659196 0.00774199016872568
0.0537312566799351 0.00774199025939626
0.0537312565202877 0.00774199033722334
0.0537312563832462 0.00774199040403323
0.0537312562656105 0.00774199046138158
0.0537312561646326 0.00774199051061042
0.0537312560779544 0.00774199055286529
0.0537312560035517 0.00774199058914027
0.0537312559396819 0.00774199062027603
0.0537312558848582 0.00774199064700332
0.053731255837798 0.00774199066994474
0.0537312557974001 0.00774199068963877
0.0537312557627256 0.0077419907065448
0.0537312557329619 0.00774199072105386
0.0537312557074099 0.00774199073351278
0.0537312556854825 0.00774199074420268
0.0537312556666532 0.00774199075338045
0.0537312556504927 0.00774199076125903
0.0537312556366256 0.00774199076802007
0.0537312556247169 0.00774199077382409
0.0537312556144967 0.007741990778805
0.0537312556057241 0.00774199078308135
0.0537312555981888 0.00774199078675575
0.0537312555917211 0.00774199078990812
0.0537312555861771 0.00774199079261306
0.0537312555814147 0.00774199079493587
0.0537312555773228 0.0077419907969285
0.053731255573811 0.0077419907986398
0.0537312555708001 0.00774199080010973
0.053731255568211 0.00774199080137383
0.0537312555659941 0.00774199080245408
0.0537312555640863 0.00774199080338245
0.0537312555624494 0.00774199080418181
0.053731255561047 0.00774199080486659
0.053731255559839 0.00774199080545235
0.0537312555588079 0.00774199080595572
0.0537312555579206 0.00774199080638693
0.0537312555571594 0.00774199080675886
0.0537312555564995 0.00774199080707727
0.0537312555559417 0.00774199080735305
0.0537312555554594 0.00774199080758797
0.0537312555550429 0.00774199080778915
0.0537312555546894 0.00774199080796212
0.0537312555543838 0.00774199080810978
0.0537312555541201 0.00774199080824056
0.0537312555538936 0.00774199080834892
0.0537312555536982 0.00774199080844529
0.0537312555535321 0.007741990808527
0.0537312555533918 0.00774199080859761
0.0537312555532692 0.00774199080865579
0.0537312555531635 0.00774199080870885
0.053731255553072 0.00774199080875348
0.0537312555529965 0.00774199080878857
0.0537312555529326 0.00774199080882143
0.0537312555528793 0.00774199080884763
0.0537312555528278 0.0077419908088705
0.0537312555527807 0.00774199080889182
0.0537312555527452 0.00774199080890936
0.0537312555527159 0.00774199080892468
0.0537312555526892 0.00774199080893956
0.0537312555526661 0.00774199080895044
0.0537312555526466 0.00774199080896021
0.0537312555526306 0.00774199080896754
0.0537312555526182 0.00774199080897442
0.0537312555526075 0.0077419908089793
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
};
\addplot [very thick, blue, mark=*, mark size=1.5, mark options={solid}, only marks]
table {%
0.1 0.1
0.140443113950194 0.0233187297218309
0.117614430338323 -0.000889583316934672
0.103634160768573 -0.00177409403385265
0.0935227169754222 -0.00133365223745341
0.0841755814442351 -0.000388843051740695
0.0750840328869629 0.00107372858040278
0.0670503957959028 0.00291997149293266
0.0611399455388968 0.00471750125151216
0.0575247792919047 0.00606199388671635
0.0555830510206077 0.0068820653011521
0.0546135067409779 0.00732193492642974
0.0541467021146005 0.00754172268184461
0.0539258117978001 0.00764764369308923
0.0538221328063937 0.00769779692089156
0.053773653257152 0.00772134539410474
0.053751024594912 0.00773235838890596
0.0537404709746028 0.00773749931994749
0.0537355508360626 0.00773989705621148
0.0537332574588154 0.00774101491070955
0.0537321885578921 0.00774153597005411
0.053731690382202 0.00774177882719695
0.0537314582049007 0.00774189201425823
0.0537313499984231 0.00774194476570389
0.0537312995688684 0.00774196935058447
0.0537312760662543 0.00774198080835053
0.0537312651129049 0.00774198614822352
0.0537312600081306 0.00774198863686104
0.053731257629047 0.00774198979669061
0.0537312565202877 0.00774199033722334
0.0537312560035517 0.00774199058914027
0.0537312557627256 0.0077419907065448
0.0537312556504927 0.00774199076125903
0.0537312555981888 0.00774199078675575
0.053731255573811 0.0077419907986398
0.0537312555624494 0.00774199080418181
0.0537312555571594 0.00774199080675886
0.0537312555546894 0.00774199080796212
0.0537312555535321 0.007741990808527
0.0537312555529965 0.00774199080878857
0.0537312555527452 0.00774199080890936
0.0537312555526306 0.00774199080896754
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
0.0537312555525968 0.00774199080898441
};
